(Random) Trees of Intermediate Uniform Growth

For every sufficiently well-behaved function $g:\mathbb{R}_{\ge 0}\rightarrow\mathbb{R}_{\ge 0}$ that grows at least linearly and at most exponentially we construct a tree $T$ of uniform volume growth $g$, that is, $$C_1\cdot g(r/4)\le |B_{T}(v,r)| \le C_2\cdot g(4r),\quad\text{for all $r\ge 0$ and $v\in V(T)$},$$ where $B_{T}(v,r)$ denotes the ball of radius $r$ centered at a vertex $v$. In particular, this yields examples of trees of uniform intermediate (i.e. super-polynomial and sub-exponential) volume growth. We use this construction to provide first examples of unimodular random rooted trees of uniform intermediate growth, answering a question by Itai Benjamini. We find a peculiar change in structural properties for these trees at growth $r^{\log\log r}$.

==> sec/copy-19.11.22.tex <==
\addtocounter{section}{-1}
\section{Introduction}

Given a finite simple graph $G$, a vertex $v\in V(G)$ and $r\ge 0$, the set 
%
\[\ball Gvr:=\{w\in V(G) \mid d_G(v,w)\leq r\}\]
%
is called the \emph{ball} of radius $r$ around $v$. 
The growth of the cardinality of these~balls as $r$ increases is known as the \emph{growth behavior} or \emph{volume growth} of $G$ around $v$.  
Standard examples usually provided include the regular trees (having exponential volume growth) and the lattice graphs (having polynomial volume growth).
It is an interesting challenge to map the possible growth behaviors in various graph classes, the most famous example potentially being Cayley graphs of finitely generated groups, the central object of study in geometric group theory.
Major results in this regard are the existence of Cayley graphs of \emph{intermediate} growth (\ie\ super-polynomial but sub-exponential \cite{grigorchuck}), and the observation that vertex-transitive graphs can have polynomial growth only for integer exponents \TODO.

Cayley graphs (and more generally vertex-transitive graphs) automatically have the same growth around every vertex. In other graph classes this is not a given, and constitutes an interesting property in its own right. We shall say that a graph $G$ has \emph{uniform} growth if its growth does not vary much between vertices.
Following \cite{babaigrowth}, the precise formulation is as follows: there is a function $g\: \NN\to\NN$ and constants $c_1,C_1,c_2,C_2\in\RR_+$ so that
%
$$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r)\quad\text{for all $r\ge 0$ and $v\in V(G)$}.$$
%
The graph $G$ is then said to be of \emph{uniform growth $g$}.

In this article we construct infinite tree graphs $T$ of uniform volume growth for a wide variety of growth behaviors, including intermediate growth and polynomial growth for non-integer exponents.
%Uniform growth hereby means that the growth of the balls varies not too much from vertex to vertex. A precise definition is given in the next subsection. As an example, vertex-transitive graphs, such as the regular trees, are always of uniform growth.
Trees of uniform polynomial growth (also for non-integer exponents) have previously been constructed in \cite{benjamini2011recurrence}.
%More specifically, we require the existence of functions $\check g,\hat g\:\NN_0\to\RR$ with $\check g=\Theta(\hat g)$ so that
%
%$$\check g(r)\le |\ball Tvr| \le \hat g(r),\quad\text{for all $v\in V(T)$ and all $r\ge 0$}.$$
%
% \cref{ex:non_uniform_growth} shows that this is a stronger requirement than bounding the volume growth between functions of similar growth.

Subsequently we show how our construction gives rise to \emph{unimodular random rooted trees} of the respective growth, answering a question by Benjamini (private communication). 
We investigate the structure of these trees and find qualitative differences between growth below $r^{\log\log r}$ and growth above $r^{\alpha\log\log r}$ when $\alpha>1$. We furthermore construct unimodular random rooted trees of intermediate growth that are supported on a single deterministic tree.

\iffalse % introduction v.2

Given a finite simple graph $G$, a vertex $v\in V(G)$ and $r\ge 0$, the set 
%
\[\ball Gvr:=\{w\in V(G) \mid d_G(v,w)\leq r\}\]
%
is called the \emph{ball} of radius $r$ around $v$. 
The growth of the cardinality of these~balls as $r$ increases is known as the \emph{growth behavior} or \emph{volume growth} of $G$ around $v$.  
Standard examples usually provided include the regular trees (having exponential volume growth) and the lattice graphs (having polynomial volume growth).
It has since been an interesting challenge to map the possible growth behaviors in various graph classes, the most famous example potentially being Cayley graphs of finitely generated groups, the central object of study in geometric group theory.
Major results in this regard are the existence of Cayley graphs of \emph{intermediate} growth (\ie\ super-polynomial but sub-exponential \cite{grigorchuck}), and the observation that vertex-transitive graphs can have polynomial growth only for integer exponents [].

Cayley graphs (and more generally vertex-transitive graphs) automatically have the same growth around every vertex. In other graph classes this has to be put in by hand. For this reason we shall say that a graph has \emph{uniform} growth if its growth varies not too much from vertex to vertex.
For our purpose, the precise formulation is as follows: there is a function $g\: \NN\to\NN$ and constants $c_1,C_1,c_2,C_2\in\RR_+$ so that
%
$$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r)\quad\text{for all $r\ge 0$ and $v\in V(G)$}.$$
%
The graph is said to be of \emph{uniform growth $g$}.

In this article we construct infinite tree graphs $T$ of uniform volume growth for a wide variety of growth behaviors, including intermediate growth and polynomial growth for non-integer exponents.
%Uniform growth hereby means that the growth of the balls varies not too much from vertex to vertex. A precise definition is given in the next subsection. As an example, vertex-transitive graphs, such as the regular trees, are always of uniform growth.
Trees of uniform polynomial growth (also for non-integer exponents) have previously been constructed in \cite{benjamini2011recurrence}.
%More specifically, we require the existence of functions $\check g,\hat g\:\NN_0\to\RR$ with $\check g=\Theta(\hat g)$ so that
%
%$$\check g(r)\le |\ball Tvr| \le \hat g(r),\quad\text{for all $v\in V(T)$ and all $r\ge 0$}.$$
%
% \cref{ex:non_uniform_growth} shows that this is a stronger requirement than bounding the volume growth between functions of similar growth.

Subsequently we show how our construction gives rise to \emph{unimodular random rooted trees} of the respective growth, answering a question by Benjamini (private communication). 
We investigate the structure of these trees and find qualitative differences between growth below $r^{\log\log r}$ and growth above $r^{\alpha\log\log r}$ when $\alpha>1$. We furthermore construct unimodular random rooted trees of intermediate growth that are supported on a single deterministic tree.

\fi

\iffalse % introduction v.1

Given a finite simple graph $G$, a vertex $v\in V(G)$ and $r\ge 0$, the set 
%
\[\ball Gvr:=\{w\in V(G) \mid d_G(v,w)\leq r\}\]
%
is called the \emph{ball} of radius $r$ around $v$. 
The growth of the cardinality of these~balls as $r$ increases is known as the \emph{growth behavior} or \emph{volume growth} of $G$.  
Standard examples include the regular trees (having exponential volume growth) and the lattice graphs (having polynomial volume growth).
It is of great interest to map the possible growth behaviors in various graph classes, the most famous example potentially being the study of the growth of Cayley graphs of finitely generated groups, an important problem in the field of geometric group theory.
Some major results in this regard are the existence of Cayley graphs of \emph{intermediate} growth (\ie\ super-polynomial but sub-exponential \cite{grigorchuck}), and the observation that vertex-transitive graphs can have polynomial growth only for integer exponents [].

In this article we construct infinite tree graphs $T$ of \emph{uniform} volume growth for a wide variety of growth behaviors, including intermediate growth and polynomial growth for non-integer exponents.
Uniform growth hereby means that the growth of the balls varies not too much from vertex to vertex. A precise definition is given in the next subsection. As an example, vertex-transitive graphs, such as the regular trees, are always of uniform growth. Additionally, trees of uniform polynomial growth (also for non-integer exponents) have been constructed in \cite{benjamini2011recurrence}.%More specifically, we require the existence of functions $\check g,\hat g\:\NN_0\to\RR$ with $\check g=\Theta(\hat g)$ so that
%
%$$\check g(r)\le |\ball Tvr| \le \hat g(r),\quad\text{for all $v\in V(T)$ and all $r\ge 0$}.$$
%
% \cref{ex:non_uniform_growth} shows that this is a stronger requirement than bounding the volume growth between functions of similar growth.

Subsequently we show how our construction gives rise to \emph{unimodular random trees} of the respective growth behavior, answering a question of Benjamini (private communication) in the positive. We show that the resulting trees are qualitatively different for growth below $r^{\log\log r}$ and growth above $r^{\alpha\log\log r}$ for $\alpha>1$. We also construct unimodular random rooted trees of intermediate growth that are supported on a single deterministic tree.

Finally, we apply our results to construct planar triangulations of intermediate growth.

\fi




\subsection{Basic definitions and notation}

Let $G$ denote a (not necessarily finite) simple~connected graph with vertex set $V(G)$ and edge set $E(G)$. 
For vertices $v,w\in V(G)$, $d_G(v,w)$ denotes the graph-theoretic distance from $v$ to $w$ in $G$. 
As stated in the beginning, for $v\in V(G)$ and $r\ge 0$, the \emph{ball} of radius $r$ around $v$ in $G$ is
%
$$\ball Gvr := \{w\in V(G) \mid d_G(v,w)\le r\}.$$
%
We reiterate that the terms \emph{(volume) growth}, \emph{growth rate} and \emph{growth behavior} of $G$ around $v\in V(G)$ informally refer to the function $g(r):= |\ball Gvr|$ and its asymptotic behavior.

In general, crafting a graph with a specific growth rate around a particular vertex is simple.
Much less so if we want the graph to have a similar growth rate around each of its vertices -- we say then that $G$ is of \emph{uniform volume growth}. 

\label{ex:non_uniform_growth}
For example, given any graph $G$, it is generally easy to construct a tree of \enquote{similar} volume growth around a vertex in an asymptotic sense: choose a vertex $v\in V(G)$ and let $T$ be a spanning tree that preserves distances to $v$.
\cref{fig:non_uniform_quadratic_growth} shows an example where $G$ is the 2-dimensional lattice graph.

\gsays{Martin, don't you think we need a better example here? Like, a graph that is not vertex-transitive?}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.55\textwidth]{img/non_uniform_quadratic_growth}
    \caption{A tree of quadratic volume growth that is \emph{not} uniform.}
    \label{fig:non_uniform_quadratic_growth}
\end{figure}

%If $w\in V(T)$ has distance $r_0:=d_T(v,w)$ from $w$, it is easy to see that
%
%\begin{equation*}\label{eq:bounds_T_G}
 %|\ball Gv{r-r_0}|\le |\ball Tw{r}|\le |\ball Gv{r+r_0}|, \quad\text{for all $r\ge r_0$}.   
%\end{equation*}
%
%hence $|\ball Twr| = \Theta(|\ball Gv r|)$. 
%However, since these bounds 
%in \eqref{eq:bounds_T_G} 
%depends on $r_0:=d_T(w,v)$, they do not guarantee uniform growth.

In the example of \cref{fig:non_uniform_quadratic_growth} we have $|\ball Tur|=\Theta(r^2)$ for all $u\in V(T)$.
However, there is no $u$-independent quadratic lower bound, as starting in a leaf, the growth is linear for an arbitrarily long initial segment. $T$ is \emph{not} of uniform quadratic growth. 

There has been a decent volume of work on trees of non-uniform intermediate growth (see \cite{amir2022branching} and references therein). In this paper, we construct the first examples of trees of uniform intermediate growth.

There are many in-equivalent ways to formalize \enquote{uniform}. For this article we follow \cite{babaigrowth} and use a comparatively strong form of uniform growth:

\begin{definition}\label{def:uniform_grwoth}
A graph $G$ is of \emph{uniform (volume) growth} $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ if there are constants $c_1,C_1, c_2, C_2\in\RR_{> 0}$ so that%$b_1,c_1,C_1,b_2,c_2,C_2\in\RR_{>0}$ so that
%
%$$C_1\cdot g(c_1 r-b_1) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r+b_2),\quad\text{for all $r\ge 0$},$$
%\end{definition}

%This definition is equivalent to the one given in \cite{...}: there exists an integer $r_0\ge 0$ and constants

%
$$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r)\quad\text{for all $r\ge 0$}.$$.
\end{definition}
%
%We stick with the version given in \cref{def:uniform_grwoth} as it is more natural for proving the main result \cref{thm:main}.

% \begin{definition}\label{def:uniform_grwoth}
% A graph $G$ is of \emph{uniform (volume) growth} $g\:\NN_0\to\NN_0$ if there is an integer $r_0\ge 0$ and constants $c_1,C_1, c_2, C_2\in\RR_{> 0}$ so that
% %
% $$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r),\quad\text{for all $r\ge r_0$}.$$
% \end{definition}

% This definition is equivalent to the existence of constants $b_1,c_1,C_1,b_2,c_2,C_2\in\RR_{>0}$ so that
% %
% $$C_1\cdot g(c_1 r-b_1) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r+b_2),\quad\text{for all $r\ge 0$},$$
% %
% which will be the definition used in \cref{thm:main}.

%We implicitly assume that the argument to $g$ is rounded to the nearest positive integer.
%If $g$ is increasing then this does not change \cref{def:uniform_grwoth} as there are always constants $\bar c_1,\bar c_2\in\RR_0$ so that for sufficiently large $r$
%
%$$
%g(\lceil \bar c_1 r \rceil)\le g(c_1 r)
%\quad\text{and}\quad
%g(\lfloor \bar c_2 r \rfloor)\le g(c_2 r).
%$$
%
%In fact, in the main theorem we show that ...

One generally distinguishes
%
\begin{itemize}
    \item \emph{uniform polynomial growth} if $g(r)=\exp(\mathcal O(\log r))$,
    \item \emph{uniform exponential growth} if $g(r)=\exp(\Omega(r))$,
    \item \emph{uniform intermediate growth} if $g(r)=\exp(o(r))$ and $g(r)=\exp(\omega(\log r))$,
\end{itemize}
%
where we used the Landau symbols $\mathcal O,\Omega, o,\omega$ as usual.


%We should reasonably assume~$g(r)=\Omega(r)$ and $g=e^{\mathcal O(r)}$, but~these and more general conditions will emerge naturally during the analysis of our construction. %As we see in a moment, we will also need to impose restrictions on the~os\-cil\-lation in the growth of $g$.

%\begin{itemize}
 %   \item $\log r=\log_2 r$ is logarithms to base 2. Otherwise write $\ln r = \log_e r$.
%\end{itemize}



\subsection{Overview}

%Starting from a suitable increasing function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$, we achieve the following:
%\begin{enumerate}
    %\item we explicitly construct~a tree $T$ with uniform growth $g(r)$;%in which $|B_v^T(r)|$ grows approximately like $g(r)$, no matter~the~vertex \mbox{$v\in V(T)$}
    %\item we prove the existence of a unimodular tree $\mathcal{T}$ with uniform growth $g(r)$.
%\end{enumerate} 

The main results in the present paper are the following:

\begin{main} \label{main}
   Let $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ be a function that grows at least linearly and at most exponentially, and is in particular super-additive and log-concave. Then there exists a tree $T$ with uniform growth $g(r)$. 
\end{main}

\begin{main} \label{unimain}
     Let $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ be a function that grows at least linearly and at most exponentially, and is in particular super-additive and log-concave. Then there is a unimodular random rooted tree $\mathcal{T}$ with uniform growth $g(r)$.
\end{main}

We also produce a structure theorem (\cref{structure}) that describes the structure of the limit trees obtained in \cref{unimain}. 

We describe the general construction for the tree $T$ in \cref{sec:construction}. In \cref{sec:main}, we show that the volume growth of $T$ is uniform with bounds close to a specified target growth $g\:\RR_{\ge 0}\to\RR_{\ge 0}$. In particular, assuming mild and quite natural conditions on $g$, namely that it be super-additive and log-concave, we prove that $T$ has uniform growth $g(r)$.

In \cref{sec:unimodular} we show how our construction naturally gives rise to a unimodular random tree $\mathcal{T}$ of a prescribed uniform volume growth. We describe the general shape of such trees, and even
give examples for unimodular random rooted trees of intermediate volume growth that are supported on a single tree.

Finally, in \cref{sec:last} we note some further observations as well as directions for this type of inquiry. Most notably, we use our construction in the vein of \cite{benjamini2011recurrence} to obtain planar triangulations of intermediate growth. 


%\noindent
%\hrulefill

%Ideas for literature:
%\begin{itemize}
 %   \item groups of intermediate growth
  %  \item other graphs of intermediate growth
   % \item \cite{benjamini2011recurrence} trees of polynomial growth by Benjamini-Schramm
    %\item \cite{amir2022branching} \enquote{The branching number of intermediate growth trees}
 %by Gideon Amir, Shangjie Yang
%\end{itemize}

\iffalse

\section{The Construction} \label{sec:construction}

%We describe an infinite tree that is not immediately supposed to match a prescribed growth behavior, but depends on countably many parameters that can be used to model a wide range of such behaviors, as we discuss further below.

For each integer sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ with $\delta_n\ge 1$ we describe the construction of a tree $T=T(\delta_1,\delta_2,...)$.

\begin{construction}
\label{constr:tree}

%Fix a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ of integers $\delta_n\ge 1$. 
Consider the following~recursive definition of trees $T_n, n\ge 0$ (see also \cref{fig:construction}):
%
\begin{itemize}
    \item 
    let $T_0:=\{x^*\}$ be the tree consisting of a single vertex called the \emph{global root}.
    For reasons that will become clear shortly, we call $x^*$ also the \emph{root} and an \emph{apocentric vertex} of $T_0$.
    
    \item we build $T_n,n\ge 1$ from $\delta_n$ disjoint copies of $T_{n-1}$ (called \emph{apocentric copies}) that we connect to another copy of $T_{n-1}$ (called the \emph{central copy}) in a way that we make precise below. 
    
    For this we require some further terminology:
    %the \enquote{non-central} copies of $T_{n-1}$ will be called \emph{apocentric copies} of $T_{n-1}$ in $T_n$.
    the root of $T_n$ is the root of the central copy of $T_{n-1}$.
    Likewise, an apocentric vertex of $T_n$~is~an~apocentric vertex of an apo\-centric copy of $T_{n-1}$.
    %Each apocentric vertex of $T_n$ is a leaf, but the converse is not necessarily true.
    
    The connections between the central and the apocentric copies are as follows: each apocentric copy of $T_{n-1}$ is connected to the central copy~by an edge between the root of the apocentric copy and some apocentric vertex of the central copy. There is no preferred choice for the apocentric vertex in the central copy (we~can even attach more than one apocentric copy to the same vertex), but it is~required that the entirety of these connection is distributed maximally uniformly among the apocentric vertices\,%
    \footnote{
    %The meaning of this will become evident when it is applied in the proof of \cref{thm:main}.
    More precisely, every apocentric copy $T_m\subset T_{n-1}, m\le n-1$ (\ie\ a copy of $T_m$ that contains apocentric vertices of $T_{n-1}$) will receive the expected number of connections, rounded up or down (see the proof of \cref{thm:main}).
    }%
    \!.
    %(this will be made precise when we apply it in the proof of \cref{thm:main}, but can be thought of as a uniform distribution).
    %; meaning that every apocentric vertex is attached to approximately the same number of copies.
\end{itemize}
%
\begin{figure}[!h]
    \centering
   % \includegraphics[width=0.7\textwidth]{img/construction.pdf}
   % \includegraphics[width=0.65\textwidth]{img/construction_2.pdf}
    \includegraphics[width=0.83\textwidth]{img/construction_3.pdf}
    \caption{Illustration of the first four steps in the  construction~of $T$ using the sequence $\delta_n:=n+2$. The ringed vertex is the root, and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy of $T_{n-1}$ in $T_n$.}
    \label{fig:construction}
\end{figure}
%

If for each $n\ge 1$ we identify $T_{n-1}$ with its central copy in $T_n$, we obtain an~inclu\-sion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $\smash{T:=\bigcup_{n\ge 0} T_n}$ is a well-defined~tree.
%We shall occasionally denote it by $T(\delta_1,\delta_2,...)$ to emphasize that it is mainly determined by the choice of the integer sequence (the free choice of the connections will play no role as long as it is maximally uniform in a way that will become clear in the proof of \cref{thm:main}).
%
We shall occasionally denote this tree by $T(\delta_1,\delta_2,...)$ even though the tree does also depend on the choice of the connections in each step, but this choice is not relevant in our analysis.
\end{construction}

Our core claim is that for most sequences $\delta_1,\delta_2,\delta_3,...\in\NN$ this tree has a uniform volume growth of some sort, and that with a careful choice of the sequence we can model a wide range of such growth behaviors, including polynomial, intermediate and exponential.

A first feeling for the claimed relation between the sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ and the growth~of $T$ can obtained by two simple observations:
%
\begin{itemize}
    \item the distance from the root of $T_n$ to any of its apocentric vertices is exactly $2^n-1$. In fact, $T_n\subset T$ is the ball of radius $2^n-1$ around the global root $x^*\in V(T)$.
    \item $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ (where the empty product gives $|T_0|=1$).
\end{itemize}
%
In other words, for radii $r=2^n-1$ holds
%
\begin{equation}
\label{eq:ball_volume_in_T}
|\ball T{x^*}r| = |T_n| = (\delta_1+1)\cdots(\delta_n+1).    
\end{equation}
%
Hence, if we aim to model a particular growth function $g\:\NN_0\to\NN$, a plausible first step is to choose a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which $(\delta_1+1)\cdots(\delta_n+1)$~approximates the growth of $f(n):=g(2^n-1)$.
This suggests a choice
%
$$\delta_n + 1\approx \frac{f(n)}{f(n-1)},$$
%
where we necessarily introduce an error when rounding the right side to an integer.

To establish uniform growth with the prescribed rate $g$ it remains to prove
%
\begin{itemize}
    \item the error introduced by rounding $f(n)/f(n-1)$ is manageable.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for radii other than $2^n-1$.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for balls centered at vertices other than the global center $x^*\in V(T)$.
\end{itemize}
%
All these points are addressed in the next section.

We close this section with three examples demonstrating the versatility of the~construction.
For conciseness we use $\bar g(r):=g(r-1)$, then $f(n)=\bar g(2^n)$.

\begin{example}[Polynomial growth]\label{ex:polynomial}
For $\bar g(r)=r^\alpha,\alpha\in\NN$ we have $f(n)=2^{\alpha n}$~and so the sequence $\delta_n=2^\alpha-1$ is \emph{constant}.

In fact, the tree $T(2^\alpha-1,2^\alpha-1,...)$ embeds nicely into the $\alpha$-th power%
\footnote{Recall, the $\alpha$-th power of $G$ is a graph $G^\alpha$ with vertex set $V(G)$ and an edge between any to vertices whose distance in $G$ is at most $\alpha$.}
of~the~$\alpha$-dimensional lattice graph (shown in \cref{fig:2_lattice_construction} for $\alpha=2$), giving independent evidence for polynomial volume growth.
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.92\textwidth]{img/2_lattice_subgraph_3.pdf}
    \caption{
        Embedding of the tree $T(3,3,...)$ into the square of the 2-dimensional lattice graph.
    }
    \label{fig:2_lattice_construction}
\end{figure}

More generally, for constant sequence $\delta_n:=c$, where $c$ is not of the form $2^\alpha-1$ with $\alpha\in\NN$, we expect to find polynomial volume growth with non-integer exponent $\log_2 c$.
\end{example}

\begin{example}[Exponential growth]\label{ex:exponential}
%The $d$-regular tree has growth function $\bar g(r)=d(d-1)^r$. This yield $f(n)=d(d-1)^{2^n}$ and $\delta_n=(d-1)^{2^{n-1}}$.
The sequence $\delta_n:=d^{\kern0.15ex 2^{n-1}}\!,d\in\NN$ yields the $d$-ary tree (see \cref{fig:binary_tree} for the case $d=2$, \ie\ the binary tree).
Replacing $d_1:=d+2$ will result in the $(d+1)$-regular tree.
We have exponential volume growth in both cases.
This is as expected, since for $r=2^n$ holds
%
$$\bar g(r) := (\delta_1+1)\cdots(\delta_n+1)=\prod_{k=1}^n \Big(d^{\kern0.15ex 2^{k-1}}\!\!+1\Big) = \sum_{i=0}^{\mathclap{2^n-1}} d^{\kern0.15ex i} = \frac{d^{\kern0.15ex 2^n}-1}{d-1} = \frac{d^{\kern0.15ex r}-1}{d-1}.$$
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.85\textwidth]{img/binary_tree.pdf}
    \caption{
        The binary tree as constructed from \cref{constr:tree} using sequence $\delta_n=2^{2^{n-1}}$.
    }
    \label{fig:binary_tree}
\end{figure}
\end{example}

Extrapolating from \cref{ex:polynomial} and \cref{ex:exponential} its seems not far-fetched that many unbounded sequences $\delta_1,\delta_2,\delta_3,...$ that grow sufficiently slower than doubly exponentially result in intermediate volume growth.

\begin{example}[Intermediate growth]
Consider $\delta_n:=(n+3)^\alpha -1$, $\alpha\in\NN$~(the~case $\alpha=1$ is shown in \cref{fig:construction}). For $r=2^n$ we estimate
%
\begin{align*}
\bar g(r) := (\delta_1+1)\cdots(\delta_n+1) 
&= (\tfrac16 (n+3)!)^\alpha 
 \sim (n! n^3)^\alpha
 \sim (n^n e^{-n} n^{7/2})^\alpha 
\\ &= r^{\alpha \log\log r} r^{-\alpha/\ln 2}\, (\log r)^{7\alpha/2}
\end{align*}
%
Hence, we expect this choice of the sequence $\delta_1,\delta_2,\delta_3,...$ to lead to a tree of uniform intermediate volume growth.
Trees constructed from $\delta_n\sim n^\alpha$ will
%Trees of growth rate $g(r)\sim r^{\alpha\log\log r}$ will also 
present~an~interes\-ting boundary case in \cref{sec:unimodular} when we discuss unimodular random trees.
% \begin{align*}
% |\ball T{x^*}{r-1}| = |T_n|= \tfrac16 (n+3)! 
% \, &\sim\,
% n! \, n^3  
% \,\sim\,
% % n^n \cdot n^{9/2}e^{-n}
%  n^n e^{-n} \sqrt n \, n^3 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \cdot (\log r)^{7/2}  .
% %\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
% \end{align*}
\end{example}


% \begin{mnote}
% Two further things should be defined rigorously in this section:
% \begin{enumerate}
%     \item \enquote{copy of $T_n$ in $T$}; clarify that this does not refer to just any subgraph isomorphic to $T_n$.
%     \item \enquote{$T_n$ is central/apocentric in $T_m$ for $m\ge n$}.
% \end{enumerate}
% \end{mnote}




% \newpage
% \sepline

% \msays{Find a good place for these remarks.}

% %The following two remarks formalize the notions \enquote{copy of $T_n$ in $T_m$} and \enquote{maximal uniform distribution of adjacencies}. The reader comfortable with an intuitive understanding of these concepts can skip the remarks.

% \begin{remark}\label{rem:copy}
% The notion of \enquote{\emph{copy} of $T_n$ in $T_m$} (where $m\ge n$) will be used~in a formal sense, referring to a special subgraph of $T_m$ isomorphic to $T_n$ that is distinguished by \cref{constr:tree} in a way we explain below.
% %In particular, not every subgraph~isomorphic to $T_n$ is a copy, and we use the notation $T_n\prec T_m$ if it is one.
% In particular, not every subgraph $\tau\subseteq T_m$ iso\-morphic to $T_n$ necessarily is such a copy, and we introduce the notation $\tau\prec_n T_m$ to indicate when it is one.
% We write $\tau\prec T_m$ if $n$ is not~important, and we write \enquote{a copy $T_n\prec T_m$} to refer to an~un\-named copy of $T_n$ in $T_m$.

% A rigorous definition of copy can be given recursively:
% a copy $\tau \prec_n T_n$ is only the full graph itself.
% The copies $\tau\prec_n T_{n+1}$ are exactly the central and apocentric copies as defined in \cref{constr:tree}.
% %central and apocentric copies of $T_n$ in $T_{n+1}$ were defined in \cref{constr:tree}.
% A copy $\tau\prec_n T_{m+1}$ is a copy $\tau\prec_n T_m\prec T_{m+1}$, in words, $\tau$ is a copy of $T_n$ inside a copy of $T_m$ inside of $T_{m+1}$.

% We furthermore say that a copy $\tau \prec T_n$ is central if it contains the root of $T_n$, and
% it is apocentric if it contains apocentric vertices of $T_n$ (one can show that then all apocentric vertices of $\tau$ are also apocentric in $T_n$).
% \end{remark}

% \msays{My worries: at the moment $\prec$ is not a partial order, but more like an abbreviation, \ie\ \enquote{copy $T_n\prec T_m$} is short for \enquote{a copy of $T_n$ inside of $T_m$}, and \enquote{copy $T_n\prec T_m\prec T_k$} is short for \enquote{a copy of $T_n$ inside of a copy of $T_m$ inside $T_k$}.
% If we make $\prec$ into a rigorous partial order then we lose this powerful abbreviation and have to write \enquote{let $\tau\prec T_m$ be a copy of $T_n$} and even worse \enquote{let $\tau\prec \tau'$ be a copy of $T_n$, where $\tau'\prec T_k$ is a copy of $T_m$}. That is, we always have to give names to the copies, don't we? But I am not happy with the current solution either. Hm.}

% \msays{Maybe an idea: write $\tau\prec_n T_m$ for \enquote{copy of $T_n$ in $T_m$}. Then we can write $\tau\prec_n\tau'\prec_m T_k$. Still a bit annoying with the subindex, and we still have to give names.}

% \msays{Check out my updated Remark 2.5 where I used some of these ideas and see whether you think its any better.}

% \gsays{I think that the updated remark resolves the issue perfectly. Copies are now well-defined.}

\newpage

\fi



\section{The construction}
\label{sec:construction}

%\msays{Experimental alternative to the intro of \cref{sec:construction}. Work in progress.}

\par\medskip

% In this section we construct a tree $T$ and explain why we expect it to be 

% We construct a tree $T$ that we later show to be of uniform volume growth.
% More precisely, we construct a tree $T=T(\delta_1,\delta_2,...)$ for each integer sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ with $\delta_n\ge 1$.

For each integer sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ with $\delta_n\ge 1$ we construct a tree~$T=T(\delta_1,\delta_2,...)$.
The choice of sequence will determine the growth rate of $T$.
%
%We shall later see that the tree $T$ can manifest a wide range of growth behaviors depending on the input sequence, and we shall explain this connection in the next section.
%
%The growth behavior of $T$ expectedly depends on the sequence, and we later explain how to choose the $\delta_i$ to model a particular growth.
%
The tree $T$ is constructed as a limit object of the following sequence of trees $T_n$ where $n\ge 0$:

%We first introduce a recursively defined sequence of trees $T_n$ for $n\ge 0$ (see \cref{constr:T_n}) and subsequently define $T$ as a limit object of this sequence (see \cref{constr:T}).


%This tree will be obtained as the limit object of a recursively defined sequence of trees $T_n,n\ge 0$, which itself is built from the sequence $\delta_1,\delta_2,\delta_3,...$.

\begin{construction}\label{constr:T_n}
%We recursively define a sequence of trees $T_n,n\ge 0$ with two types of distinguished vertices, namely, a \emph{root} and a set of \emph{apocentric vertices}:
The trees $T_n$ are defined recursively.
%We recursively define a sequence of trees $T_n$ for $n\ge 0$. 
In each tree we distinguish two special types of vertices: a \emph{centre}, and a set of so-called \emph{apocentric vertices} (or outer\-most or peripheral vertices), both will be defined alongside the trees:
%and in each tree two distinguished types of vertices, a \emph{root} and a set of \emph{apocentric vertices}:
%with two types of distinguished vertices: a \emph{root} and a set of so-called \emph{apocentric vertices}:
%Each $T_n$ has a \emph{root} and a set of so-called \emph{apocentric vertices} which are defined alongside the trees:
%
\begin{myenumerate}
    \item 
    $T_0$ is the tree consisting of a single vertex. This vertex is both the centre of $T_0$ as well as its only apocentric vertex.
    
    \item 
    The tree $T_n$ is built from $\delta_n+1$ disjoint copies $\tau_0, \tau_1,...,\tau_{\delta_n}$ of $T_{n-1}$ that we join into a single tree by adding the following edges:
    %
    %where $\tau_0$ (which we call \emph{central copy}) will be connected to $\tau_1,...,\tau_{\delta_n}$ (which we call \emph{apocentric copies}) in the following way:
    %
    %for each $\tau_i,i\in\{1,...,\delta_n\}$ choose an apocentric vertex of $\tau_0$ and add an edge between this vertex and the root of $\tau_i$.
    for each $i\in\{1,...,\delta_n\}$ add an edge between the centre of $\tau_i$ and some apocentric vertex of $\tau_0$.
    There is a choice in selecting these apocentric vertices of $\tau_0$ (and note that we can choose the same apocentric vertex more than once), but we shall require that these adjacencies are distributed in a maximally uniform way among the apocentric vertices of $\tau_0$ (we postpone a rigorous definition of this until we introduced suitable notation; see \cref{rem:max_uniform}).
    
    It remains to define the distinguished vertices of $T_n$: the root of $T_n$ is~the root of $\tau_0$; the apocentric vertices of $T_n$ are the apocentric vertices~of~$\tau_1,...,$ $\tau_{\delta_n}$.
    
    % \msays{Turns out, in each $T_n$ the root is just the \enquote{center}, and the apocentric vertices are just the \enquote{peripheral vertices}, both are established terms. I don't want to change our terminology, and I don't know what to do with this insight.}
    
    % \gsays{Where did you come upon these established terms?}
    
    % \msays{Wikiepdia, see comment in code}
    % https://en.wikipedia.org/wiki/Distance_(graph_theory)#Related_concepts
    
    %The $\tau_i$ will be called the \enquote{copies of $T_{n-1}$ in $T_n$}, which we also denote by $\tau_i\precdot T_n$.
    
    %One can visualize the $\tau_i,i\in\{1,...,\delta_n\}$ as being arranged around $\tau_0$ in the center, from which the connections to the $\tau_i$ emanate star-like (\cf\ \cref{fig:construction}).
    
    % Intuitively, the copies $\tau_i,i\in\{1,...,\delta_n\}$ are arranged around the copy $\tau_0$ in the center (see \cref{fig:construction}). For this reason $\tau_0$ is called the \emph{central copy} of $T_{n-1}$~in $T_n$, while the others are called \emph{apocentric copies}. We use the notation $\tau_i\precdot T_n$ to refer to these copies of $T_{n-1}$ (a notation we generalize in \cref{rem:copy}).
    
    % Let $\tau_0,\tau_1, ...,\tau_{\delta_n}$ be $\delta_n+1$ disjoint copies of $T_{n-1}$. We add edges to connect these trees to form the next tree $T_n$, but we need some further terminology to describe these connections concisely.
    
    % \begin{itemize}
    %     \item The $\tau_i$ are called \enquote{copies of $T_{n-1}$ in $T_n$}, which distinguishes them among other subgraphs of $T_n$ isomorphic to $T_{n-1}$. We denote this by $\tau_i\precdot T_n$.
    %     \item $\tau_0$ will be called \emph{central copy}, whereas the $\tau_1,...,\tau_{d_n}$ are the \emph{apocentric copies}.
    %     \item the root of $T_n$ is the root of the central copy $\tau_0$, whereas a vertex~of $T_n$~is apocentric if it is apocentric in any of the  $\tau_i,i\in\{1,...,\delta_n\}$.
    % \end{itemize}
    
    % The adjacencies between the copies $\tau_i$ are as follows: to each apocentric copy $\tau_i,i\in\{1,...,\delta_n\}$ we choose an apocentric vertex in $\tau_0$ and add an edge between this vertex and the root of $\tau_i$.
    
    % ...
    
    % The connections between the central and the apocentric copies are as follows: each apocentric copy of $T_{n-1}$ is connected to the central copy~by an edge between the root of the apocentric copy and some apocentric vertex of the central copy. There is no preferred choice for the apocentric vertex in the central copy (we~can even attach more than one apocentric copy to the same vertex), but it is~required that the entirety of these connection is distributed maximally uniformly among the apocentric vertices (see \cref{rem:max_uniform} for a rigorous explanation)
\end{myenumerate}
%
% We write $\tau\precdot T_n$ to denote that $\tau$ is such a copy. 
% This defines a relation on trees isomorphic to the $T_n$.
% Let $\prec$ be the transitive closure of $\precdot$, then we can write $\tau\prec T_n$ to denote the canonical copies of $T_m$ in $T_n$ for general $m< n$.
% We write $\tau\prec_m T_n$ to emphasize that $\tau$ is a copy of $T_m$.
%
See \cref{fig:construction} for an illustration of this recursive definition.
    
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.85\textwidth]{img/construction_4.pdf}
    \caption{Illustration of the first four trees $T_0,...,T_3$ defined using the sequence $\delta_n:=n+2$. The ringed vertex is the root, and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy $\tau_0$ in $T_n$. The dashed lines are the new edges added to connect the copies to form a single tree.}
    \label{fig:construction}
\end{figure}
\end{construction}

The following three properties follow immediately from the recursive definition:

\begin{observation}\label{res:T_n_properties} \quad
\begin{myenumerate}
    \item $T_n$ has exactly $(\delta_1+1)\cdots(\delta_n+1)$ vertices.
    \item $T_n$ has exactly $\delta_1\cdots\delta_n$ apocentric vertices, all of which are leaves of the tree (but not all leaves are necessarily apocentric).
    \item the distance from the centre of $T_n$ to any of its apocentric vertices is $2^n-1$.
\end{myenumerate}
\end{observation}

One way to construct a \enquote{limit} of the $T_n$ is the following:

%The definition of $T:=T(\delta_1,\delta_2,...)$ as a limit object is straightforward.

\begin{construction}\label{constr:T}
For each $n\ge 1$ identify $T_n$ with one of its copies $\tau_0,\tau_1,...,\tau_{\delta_{n+1}}$ in $T_{n+1}$.
In this way we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the~union $T:=\bigcup_{n\ge 0} T_n$ is an infinite tree.
\end{construction}

%\msays{either remove $T(d_1,d_2,...)$ everywhere, or define it.}

In the following we shall write $T(\delta_1,\delta_2,...)$ to denote a limit tree obtained~from the sequence $\delta_1,\delta_2,\delta_3,...\in\NN$.
%
\iftrue % types of limit trees vs types of inclusion chains
%
For later use we also distinguish three natural~types of limit trees:
%One natural way is to identify $T_n$ with its \enquote{central copy} $\tau_0\subset T_{n+1}$. The resulting inclusion chain will be called \emph{completely central}.
%Other conventions are conceivable, such as
%For later use we give names to the following other ways to define inclusion:
%
\begin{itemize}
    \item \emph{centric limits} always identify $T_n$ with the \enquote{central copy} $\tau_0$ in $T_{n+1}$.
    \item \emph{apocentric limit}s always identify $T_n$ with an \enquote{apocentric copy} $\tau_i$ in $T_{n+1}$.
    \item \emph{balanced limits} make both central and apocentric identifications infinitely often.
\end{itemize}
%
In \cref{sec:unimodular} we discuss a different and arguably more canonical way (via Benjamini-Schramm limits) that circumvents any arbitrary identification.

\else

For later use we distinguish three natural types of inclusion chains:
%One natural way is to identify $T_n$ with its \enquote{central copy} $\tau_0\subset T_{n+1}$. The resulting inclusion chain will be called \emph{completely central}.
%Other conventions are conceivable, such as
%For later use we give names to the following other ways to define inclusion:
%
\begin{itemize}
    \item \emph{centric} inclusion chains identify $T_n$ with the \enquote{central copy} $\tau_0$ in $T_{n+1}$.
    \item \emph{apocentric} inclusion chains identify $T_n$ with an \enquote{apocentric copy} $\tau_i$ in $T_{n+1}$.
    \item \emph{balanced} inclusion chains make both central and apocentric identifications infinitely often.
\end{itemize}
%
In \cref{sec:unimodular} we discuss a different and arguably more canonical way to make these identification via Benjamini-Schramm limits.

\fi

\iffalse % old construction of T

\begin{construction}\label{constr:T}
For each $n\ge 1$ identify $T_{n-1}$ with its \enquote{central copy} $\tau_0$ in $T_n$.
This yields an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $\smash{T:=\bigcup_{n\ge 0} T_n}$~is a~well-defined tree\footnote{Note that \cref{constr:T_n} \itm2 involves freedom in choosing the edges between $\tau_0$ and~$\tau_1,...,$ $\tau_{\delta_n}$. Therefore the notation $T(\delta_1,\delta_2,...)$ is strictly speaking not well-defined. However,\nlspace the exact choice is not relevant to our analysis and we tacitly fix some instance of the construction.}\!.

The tree $T$ has a canonical notion of root, namely the unique vertex of $T_0\subset T$, which we shall call the \emph{global root} of $T$.
\end{construction}

\begin{remark}
Based on the choice of identification, the inclusion chain $T_0\subset T_1\subset T_2\subset \cdots$ in \cref{constr:T} could be called \emph{completely centric}.
Other identification are conceivable and lead to other limit trees: \emph{completely apocentric} inclusion chains (always identifying $T_n$ with an \enquote{apocentric copy} $\tau_i \prec_n T_{n+1}$) or \emph{mixed} inclusion chains (making both, a central and apocentric choice infinitely often).

%The centric chain will be most useful to our discussion of grwoth
We shall see that choosing a different chain comes with no significant change to our analysis of growth.
Still, different chains will be relevant to \cref{sec:unimodular} when we discuss a less biased approach using Benjamini-Schramm limits.
%
%
%
%
%In an alternative to \cref{constr:T} one could identify each $T_{n-1}$ with an \emph{apocentric copy} in $T_n$ rather than the central copy (or even make a different choice in each step). This would then result in a different limit tree.
%In \cref{sec:unimodular} we explore such a \enquote{less biased} approach using Benjamini-Schramm limits.
%Our analysis of the growth of $T$ will carry over to this more general setting (see \cref{rem:general_limit_growth}).
%
%
%
% The given construction of $T$ is however more suitable for our immediate~analysis, which also carries over to the general case
%
% Alternative limit procedures are conceivable, \eg\ where we always (or just for some $n$) identify $T_{n-1}$ with one of its apocentric copies in $T_n$ (rather than the central one).
% \cref{sec:unimodular} follows a \enquote{less biased} approach via distributional limits.
% The given construction of $T$ is however more suitable for our immediate~analysis, which also carries over to the general case (see \cref{rem:general_limit_growth}).
\end{remark}

\fi

Our core claim is now that for \enquote{most} sequences $\delta_1,\delta_2,\delta_3,...\in\NN$ and independent of the type of the limit, the tree $T$ has a uniform volume growth of some sort, and that with a careful choice of the sequence we can model a wide range~of~growth~behaviors, including polynomial, intermediate and exponential.

%\msays{remove reference to global center.}

The following example computation gives us
%is meant to provide a first idea
a first idea of
%of 
the connection 
%that we should expect to find 
between the sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ and the growth rate of $T$.
For this, let $T$ be the centric limit and $x^*\in V(T_0)\subset V(T)$ its \enquote{global center}.
By \cref{res:T_n_properties}~\itm3 the ball of radius $r=2^n-1$ in $T$, centered at $x^*$, is exactly $T_n\subset T$.
By \cref{res:T_n_properties} \itm1 it follows
%
%This computation is based on three properties of the $T_n$ that follow immediately from the recursive definition:
%
%For later use we mention the following properties of $T_n$, all of which follow directly from the recursive definition:
%
%
% \begin{itemize}
%     \item the distance from the root of $T_n$ to any of its apocentric vertices is exactly $2^n-1$. In fact, $T_n\subset T$ is the ball of radius $2^n-1$ around the global root $x^*\in V(T)$.
%     \item $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ (where the empty product gives $|T_0|=1$).
% \end{itemize}
%
%In other words, for radii $r=2^n-1$ holds
%
\begin{equation}
\label{eq:ball_volume_in_T}
|\ball T{x^*\!}r| = |T_n| = (\delta_1+1)\cdots(\delta_n+1).    
\end{equation}
%
Thus, if we aim for, say, $\ball T{x^*\!}r\approx g(r)$ with a given growth function $g\:\NN_0\to\NN_0$, then \eqref{eq:ball_volume_in_T} suggests to use a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which 
%
% Thus, looking for 
% %Therefore, if we start from an increasing function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ and we want~to find 
% a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which $|\ball T{x^*\!}r| \approx g(r)$, where $g\:\NN\to\NN$ is some given growth function, \eqref{eq:ball_volume_in_T} suggests to use a sequence for which
$(\delta_1+1)\cdots(\delta_n+1)$ approximates $g(2^n-1)$.
In practice it turns out more convenient to approximate $g(2^n)$ (the computations are nicer and we still can prove uniform growth), and so we are lead to
%Thus, we are lead to
% Therefore, if we want $T$ to model a particular volume growth 
% %prescribed by a function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$, that is, 
% $|\ball T{x^*}r| \approx g(r)$, then we should choose a sequence $\delta_1,\delta_2,\delta_3,...$ for which $(\delta_1+1)\cdots(\delta_n+1)$ approximates $f(n):=g(2^n-1)$.
%
\begin{equation} \label{eq:suggestions}
    \delta_n + 1\approx \frac{g(2^n)}{g(2^{n-1})},
\end{equation}
%
where we necessarily introduce an error when rounding the right side to an integer.
%
%In actuality we shall work with $g(2^n)$ instead of $g(2^n-1)$ because the~computations turn out nicer and we still can prove uniform growth.
%
%Our definition of \enquote{uniform growth} is flexible enough to allow for~this as any deviations can be absorbed into the constants.
%
%The We will still be able to prove uniform growth.
%
To establish uniform growth with a prescribed growth rate $g$ it remains to prove
%
\begin{itemize}
    %\item the error introduced by rounding $f(n)/f(n-1)$ is manageable.
    \item the error introduced by rounding the right side of \eqref{eq:suggestions} is manageable.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for radii $r$ that are not of the form $2^n-1$.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for general limit trees and around vertices other than a designated \enquote{global center}.
\end{itemize}
%
These points are addressed in the next section.

The remainder of this section is used to introduce helpful notation, clarify the phrase \enquote{maximally uniform distribution of adjacencies} used in \cref{constr:T_n} and provide examples.

%In the remainder of this section we address the \enquote{maximal uniform distribution of adjacencies} left undefined in \cref{constr:T_n} \itm2, and give examples that demonstrate the versatility of out construction.




\begin{notation}
By \cref{constr:T_n} \itm2 for every $n\in \mathbb{N}$, $T_n$ (and each tree isomorphic to $T_n$) comes with a canonical decomposition into copies of $T_{n-1}$.
Recursively we obtain a canonical decomposition of $T_n$ into copies of $T_m$ for each $m\le n$ (see \cref{fig:copies_of_T1}). We shall use the notation $\tau\prec_m T_n$ to indicate that $\tau$ is such a canonical copy of $T_m$, or $\tau \prec T_n$ if $m$ is not relevant.
%Lastly, by a slight abuse of notation, we may write \enquote{a copy $T_m\prec T_n$} to refer to an unnamed copy of $T_m$ inside of $T_n$.

A copy $\tau\prec T_n$ is called \emph{central} if it contains the center of $T_n$; it is called \emph{apocentric} if it shares apocentric vertices with $T_n$ (and one can show that then \emph{all} apocentric vertices of $\tau$ are apocentric in $T_n$).
\end{notation}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{img/copies_of_T1.pdf}
    \caption{All canonical copies $\tau\prec_1 T_3$ are highlighted. The central~and apocentric copies are highlighted in white, the others in gray. %Observe that $T_3$ contains further subgraphs isomorphic to $T_1$ that are not copies.
    }
    \label{fig:copies_of_T1}
\end{figure}

% \begin{remark}\label{rem:copy}
% The symbol $\precdot$ defines a relation between (graphs isomorphic to) the $T_n,n\ge0$.
% Let $\prec$ be its transitive closure.
% If $\tau\prec T_n$ we say \,\enquote{$\tau$ is a copy in $T_n$}, and we write $\tau\prec_m T_n$ to emphasize that $\tau$ is a copy of $T_m$.
% We call $\tau\prec T_n$ a \emph{central copy} if it contains the root of $T_n$, we call it an \emph{apocentric copy} if it shares apocentric vertices with $T_n$ (and it is not hard to see that then all apocentric vertices of $\tau$ are also apocentric in $T_n$).
% \end{remark}

% The \enquote{maximally uniform distribution of adjacencies} between the apocentric vertices of $\tau_0$ and the roots of $\tau_1,...,\tau_{\delta_n}$ in \cref{constr:T_n} \itm2 will later be crucial for establishing uniform growth of $T$ (see \cref{thm:main}).
% A formal definition is given below.

With this notation in place we can clarify our mention of \enquote{maximal uniform distribution of adjacencies} in \cref{constr:T_n} \itm2.

\begin{remark}\label{rem:max_uniform}
%\enquote{Maximal uniform distribution of adjacencies} roughly means that certain \enquote{important} subsets of apocentric vertices of $\tau_0$ are involved in the expected number of \enquote{outwards adjacencies} to the apocentric copies $\tau_1,...,\tau_{\delta_n}$.

%To understand what is the \enquote{expected number}, note that $T_n$ has exactly $\delta_1\cdots\delta_n$ apocentric vertices.
%We make this precise.

Let $\tau_0\prec_{n-1} T_{n}$ be the central copy.
%An \emph{outwards edge} is an edge connecting $\tau$ with an apocentric copy $T_n\prec T_{n+1}$. Roughly, \enquote{maximal uniform distribution of adjacencies} means that the end vertices of these edges that lie in $\tau$ are distributed \enquote{as if they were chosen at random}.
Then there are exactly $\delta_n$ \enquote{outwards edges} connecting $\tau_0$ to the apocentric copies $\tau_1,...,\tau_{\delta_n}\prec_{n-1} T_n$.
%
%More formally, let $\mathcal E$ be the set of outwards edges as defined above.
%For each apocentric copy $\tau'\prec_m \tau$ with $m\le n$ let $\mathcal E'\subseteq\mathcal E$ be the subset of outwards edges that end in $\tau'$.
%Then maximally uniform means that $\mathcal E'$ contains very close to the number of edges that one would expect, namely
\enquote{Maximal uniform distribution} means that every apocentric copy $\tau\prec_m \tau_0$ (where $m\le n-1$) intersects the expected number of these edges (up to rounding). More precisely, if $E_\tau$ is the number of the \enquote{outwards edges} that have an end in $\tau$, then
%
\begin{equation}\label{eq:max_uniform}
\Big\lfloor \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot \delta_n \Big\rfloor
\le
E_\tau
\le 
\Big\lceil \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot \delta_n \Big\rceil,
\end{equation}
%
where $(\delta_1\cdots\delta_m)/(\delta\cdots\delta_{n-1})$ is exactly the fraction of apocentric vertices of $\tau_0$ that are also in $\tau$ (\cf\ \cref{res:T_n_properties} \itm2).

% More formally, given the central copy $\tau_0\prec_{n-1} T_{n}$, % of $T_n$ in $T_{n+1}$. 
% %An \emph{outwards edge} is an edge connecting $\tau$ with an apocentric copy $T_n\prec T_{n+1}$. Roughly, \enquote{maximal uniform distribution of adjacencies} means that the end vertices of these edges that lie in $\tau$ are distributed \enquote{as if they were chosen at random}.
% let $\mathcal E_0\subseteq E(T_{n})$ be its set of \enquote{outwards edges}, % emanating from $\tau$,
% \ie\ edges connecting $\tau_0$ with the apocentric copies $\tau_1,...,\tau_{\delta_n}\prec_{n-1} T_n$.
% %
% %More formally, let $\mathcal E$ be the set of outwards edges as defined above.
% %For each apocentric copy $\tau'\prec_m \tau$ with $m\le n$ let $\mathcal E'\subseteq\mathcal E$ be the subset of outwards edges that end in $\tau'$.
% %Then maximally uniform means that $\mathcal E'$ contains very close to the number of edges that one would expect, namely
% Then, every apocentric copy $\tau\prec_m \tau_0$ (where $m\le n-1$) intersects the expected number of these outwards edges, up to rounding. More precisely, if $\mathcal E\subseteq\mathcal E_0$ is the subset of edges that have one end in $\tau$, then
% %
% \begin{equation}\label{eq:max_uniform}
% \Big\lfloor \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot |\mathcal E_0|\, \Big\rfloor
% \le
% |\mathcal E| 
% \le 
% \Big\lceil \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot |\mathcal E_0|\, \Big\rceil    
% \end{equation}
% %
% Note that $(\delta_1\cdots\delta_m)/(\delta\cdots\delta_{n-1})$ is exactly the fraction of apocentric vertices of $\tau_0$ that are in $\tau$ (see \cref{res:T_n_properties} \itm2).

It is not hard to see that in each step of \cref{constr:T_n} this distribution can be achieved by adding the \enquote{outwards edges} one by one. % (\eg\ choose the next apocentric vertex of $\tau_0$ maximally distant from all previously chosen apocentric vertices).
The reader can verify that the steps shown in \cref{fig:construction} are in accordance with~a~max\-imally uniform distribution.

%Maximal uniform distribution of the connections from the apocentric vertices of $\tau$ to the apocentric copies of $T_{n}\prec T_{n+1}$ means, roughly, that the 

% We give a rigorous definition of what we mean by \enquote{maximally uniform distribution of adjacencies}.

% Let $\tau\prec_n T_{n+1}$ be the central copy of $T_n$.
% Let $a(\tau)\in\NN$ be its number of apocentric vertices and $a_+(\tau)\le a(\tau)$ the number of \emph{outwards vertices} among them, that is, apocentric vertices that are adjacent to apocentric copies $T_n\prec T_{n+1}$. 
% \enquote{Maximally uniform distribution of connections} means that for each apocentric copy $\tau' \prec_m \tau$, where $m\le n$, the number $a_+(\tau')$ of outwards vertices in $\tau'$ is maximally close to what we would expect if the adjacencies were distributed at random:
% %
% $$
% \Big\lfloor\, \frac{a_+(\tau)}{a(\tau)}\cdot a(\tau')\, \Big\rfloor
% \le a_+(\tau')
% \le \Big\lceil\, \frac{a_+(\tau)}{a(\tau)} \cdot a(\tau') \, \Big\rceil.
% $$
\end{remark}

We close with three examples demonstrating the versatility~of~\cref{constr:T}.
%For conciseness we use $\bar g(r):=g(r-1)$, then $f(n)=\bar g(2^n)$.

\begin{example}[Polynomial growth]\label{ex:polynomial}
If we aim for polynomial growth $g(r)=r^\alpha,\alpha\in\NN$ then the heuristics \eqref{eq:suggestions} suggests to use a constant sequence $\delta_n:=2^\alpha-1$.

In fact, the tree $T(2^\alpha-1,2^\alpha-1,...)$ embeds nicely into the $\alpha$-th power%
\footnote{Recall, the $\alpha$-th power of $G$ is a graph $G^\alpha$ with vertex set $V(G)$ and an edge between any to vertices whose distance in $G$ is at most $\alpha$.}
of~the~$\alpha$-dimensional lattice graph (shown in \cref{fig:2_lattice_construction} for $\alpha=2$), giving further evidence for polynomial volume growth.
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.92\textwidth]{img/2_lattice_subgraph_3.pdf}
    \caption{
        Embedding of the tree $T(3,3,...)$ into the square of the 2-dimensional lattice graph.
    }
    \label{fig:2_lattice_construction}
\end{figure}

More generally, for any constant sequence $\delta_n:=c$ we expect to find polynomial volume growth, potentially with a non-integer exponent $\log(c+1)$.
\end{example}

\begin{example}[Exponential growth]\label{ex:exponential}
%The $d$-regular tree has growth function $\bar g(r)=d(d-1)^r$. This yield $f(n)=d(d-1)^{2^n}$ and $\delta_n=(d-1)^{2^{n-1}}$.
The sequence $\delta_n:=d^{\kern0.15ex 2^{n-1}}\!,d\in\NN$ yields the~$d$-ary tree,
%Replacing $d_1:=d+2$ will result in the $(d+1)$-regular tree.
in particular, exponential volume growth (see \cref{fig:binary_tree} for the case $d=2$, \ie\ the binary tree).
This is compatible with \eqref{eq:ball_volume_in_T}: for $r=2^n$ we compute
%
 $$|\ball T{x^*}{r-1}| = (\delta_1+1)\cdots(\delta_n+1)=\prod_{k=1}^n \Big(d^{\kern0.15ex 2^{k-1}}\!\!+1\Big) = \sum_{i=0}^{\mathclap{2^n-1}} d^{\kern0.15ex i} = \frac{d^{\kern0.15ex 2^n}-1}{d-1} = \frac{d^{\kern0.15ex r}-1}{d-1}.$$
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.85\textwidth]{img/binary_tree.pdf}
    \caption{
        The binary tree as constructed from \cref{constr:T_n} using the doubly exponential sequence $\delta_n=2^{2^{n-1}}$.
    }
    \label{fig:binary_tree}
\end{figure}
\end{example}

Extrapolating from \cref{ex:polynomial} and \cref{ex:exponential}, it seems not far-fetched that unbounded sequences $\delta_1,\delta_2,\delta_3,...$ with a growth sufficiently below doubly exponential result in intermediate volume growth.

\begin{example}[Intermediate growth]\label{ex:loglogr}
For $\delta_n:=(n+3)^\alpha -1$, $\alpha\in\NN$ we can compute this explicitly (see \cref{fig:construction} for the case $\alpha=1$): $r=2^n$ yields
%
\begin{align*}
%\bar g(r) 
|\ball T{x^*}{r-1}|
= (\delta_1+1)\cdots(\delta_n+1) 
&= (\tfrac16 (n+3)!)^\alpha 
 \sim (n! n^3)^\alpha
 \sim (n^n e^{-n} n^{7/2})^\alpha 
\\ &= r^{\alpha \log\log r} r^{-\alpha/\ln 2}\, (\log r)^{7\alpha/2}
%  \sim \tfrac16(n! n^3)^\alpha
%  \sim \tfrac16(n^n e^{-n} n^{7/2})^\alpha 
% \\ &= \tfrac16r^{\alpha \log\log r} r^{-\alpha/\ln 2}\, (\log r)^{7\alpha/2}
\end{align*}
%
We therefore expect this choice of sequence to lead to a tree of uniform intermediate volume growth.
Trees constructed with $\delta_n\sim n^\alpha$ will furthermore
%Trees of growth rate $g(r)\sim r^{\alpha\log\log r}$ will also 
present an interes\-ting boundary case in \cref{sec:unimodular} when we discuss unimodular random trees.
% \begin{align*}
% |\ball T{x^*}{r-1}| = |T_n|= \tfrac16 (n+3)! 
% \, &\sim\,
% n! \, n^3  
% \,\sim\,
% % n^n \cdot n^{9/2}e^{-n}
%  n^n e^{-n} \sqrt n \, n^3 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \cdot (\log r)^{7/2}  .
% %\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
% \end{align*}
\end{example}

%\newpage

\section{Uniform volume growth}
\label{sec:main}


We fix an increasing function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ that shall serve as our target growth rate. %; we also set $\bar g(r)$ $:=g(r-1)$.
The goal of this section is to construct an appro\-priate sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which we can show that $T:=T(\delta_1,\delta_2,...)$ is of uniform volume growth $g(r)$. 
%\textcolor{lightgray}{
We shall show in particular that this is feasible if $g$ is super-additive and log-concave, thus proving \cref{main}.
%}

Recall that the uniform growth rate of a graph must be at least linear (like in~a path graph) and at most exponential (like in a regular tree).
It would therefore~be reasonable to impose these constraints on the target growth rate $g$ right away.\nlspace
%As $g$ is supposed to be the uniform growth rate of a locally finite graph, intuitively we should require that $g$ grows at least linearly and at most exponentially.
However, we shall not do this: these constraints will also emerge naturally during our journey towards the main theorem of this section.
In fact, we shall uncover even more precise constraints expressed in terms of the sequence $\delta_1,\delta_2,\delta_3,...$ (see \cref{rem:c,rem:dbar}) and we discuss how they relate to the natural constraints of $g$ growing at least linear and at most exponential.
% (see \cref{rem:c} and \cref{rem:dbar}, as well as \cref{thm:main})
%These can often be expressed more directly in terms of the sequence of $\delta_n$, but we make an effort to provide versions in terms of $g$ as well.

Following our motivation from the last section we first try to approximate $g(2^n)$ by $(\delta_1+1)\cdots(\delta_n+1)$.

\begin{lemma}\label{res:d_i}
There exists a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ so that
%
\begin{equation}\label{eq:d_bounds}
(1-c)\cdot g(2^n)  \;<\; (\delta_1+1)\cdots(\delta_n+1) \;<\; (1+c)\cdot g(2^n),
\end{equation}
%
for all $n\ge 0$, where $c:=\sup_n g(2^n)/g(2^{n+1}) \le 1$.
%
\begin{proof}
For this proof we abbreviate $\bar\delta_n:=\delta_n+1$. 
We set $\bar\delta_1 := g(2)$ and recursively %\msays{$f(1)$ might not be an integer}
%
$$\bar\delta_{n+1}:=\begin{cases}
\lceil g(2^{n+1})/g(2^n)\rceil & \text{if $\bar\delta_1\cdots\bar\delta_{n}\le g(2^n)$}\\
\lfloor g(2^{n+1})/g(2^n)\rfloor & \text{if $\bar\delta_1\cdots\bar\delta_{n}> g(2^n)$}
\end{cases}.
$$

This sequence satisfies \eqref{eq:d_bounds} as we show by induction on $n$: the induction base is clear from the definition of $\bar\delta_1$. Next, if \eqref{eq:d_bounds} holds for $n$, and $\bar\delta_1\cdots\bar\delta_{n}\le g(2^n)$, then
%
\begin{align*}
\bar\delta_1\cdots \bar\delta_n \cdot\bar\delta_{n+1} &\le g(2^n) \cdot\Big\lceil \frac{g(2^{n+1})}{g(2^n)} \Big\rceil 
< g(2^n)\cdot \Big( \frac{g(2^{n+1})}{g(2^n)} + 1\Big)
\\&= \Big( 1+ \frac{g(2^n)}{g(2^{n+1})} \Big) \cdot g(2^{n+1}) \le ( 1+ c )\cdot  g(2^{n+1}), \\[1ex]
\bar\delta_1\cdots \bar\delta_n \cdot\bar\delta_{n+1} 
&> (1-c)\cdot g(2^n)\cdot \Big\lceil \frac{g(2^{n+1}}{g(2^n)} \Big\rceil 
\ge (1-c)\cdot g(2^n)\cdot \frac{g(2^{n+1})}{g(2^n)}
\\&=(1-c)\cdot g(2^{n+1}).
\end{align*}
%
An analogous argument applies in the case $\bar\delta_1\cdots\bar\delta_{n}> g(2^n)$.
\end{proof}
\end{lemma}

%In the following let $\delta_1,\delta_2,\delta_3,...\in\NN$ be the sequence constructed in the proof of \cref{res:d_i}.

\begin{remark}\label{rem:c}
Recall that \cref{constr:T_n} requires $\delta_n \ge1$ for all $n\ge 1$ in order for $T(\delta_1,\delta_2,...)$ to be well-defined.
The sequence provided by the proof of \cref{res:d_i} does not generally have this property unless further requirements on $g$ are met.
%
One such is \emph{super-additivity}, which turns out to also formalize the idea of \enquote{$g$ growing at least linear}.

Super-additivity means $g(r_1+r_2)\ge g(r_1)+ g(r_2)$ and indeed implies $g(2^{n+1}) = g(2^n+2^n)\ge 2g(2^n)$, and hence
%
%More precisely, the following is sufficient: $g(1)\ge 2$ and $\bar g$ is \emph{super-additive}, \ie\ $\bar g(r_1+r_2)\ge \bar g(r_1)+\bar g(r_2)$.
%Then $\bar g(2r)\ge 2\bar g(r)\implies f(n+1)\ge 2f(n)$, from which follows
%
$$\delta_{n+1}+1\ge \Big\lfloor\frac{g(2^{n+1})}{g(2^n)}\Big\rfloor \ge 2.$$
%
%In the following we shall therefore assume that $g$ is super-additive.
%This formalizes \enquote{$g$ should grow at least linearly}, and also yields
%This implies 
This moreover implies $c:=\sup_n g(2^n)/g(2^{n+1}) \le 1/2 <1$ and guarantees that the lower bound in \cref{res:d_i} is not vacuous.
%
%Together with $g(0)=1$, these are the only requirements on the growth of $g$ from below.
%This also captures the intuition that $g$ should grow \enquote{at least linearly}.
\end{remark}

%In the following we assume that $g$ is super-additive to ensure that $T$ exists.

\begin{remark}\label{rem:dbar}
%\Cref{constr:tree} provide a reason to put upper bounds on the growth of $g$:
%An upper bound on the growth of $g$ emerges as necessary~if~we~investigate the vertex degrees in $T$.
Recall that graphs of uniform growth are necessarily of bounded~degree.
But again, the sequence constructed in the proof of \cref{res:d_i} does not~necessarily produce such a tree unless further requirements on $g$ are met.
We elaborate how these requirements can be interpreted as \enquote{$g$ growing at most exponentially}.
%
%Making sure that \cref{constr:T} yields such a graph leads us to a more precise formulation of \enquote{$g$ should grow at most exponentially}.
% by the fact that graphs of uniform growth are necessarily of finite maximum degree.

The tree $T_{n-1}$ has exactly $\delta_1\cdots\delta_{n-1}$ apocentric vertices. That is, each apocentric vertex of the central copy $\tau_0\prec_{n-1}T_n$ is adjacent, on average,\nlspace to
%
\begin{equation}\label{eq:Delta}
\Delta(n):= \frac{\delta_n}{\delta_1\cdots\delta_{n-1}}
\end{equation}
%
apocentric copies $\prec_{n-1} T_n$.
By the maximal uniform distribution of adjacencies (\cf\ \cref{rem:max_uniform}) the maximum degree among the apocentric vertices of $\tau_0$ is exactly $\lceil \Delta(n) \rceil + 1$.
Thus, since $T$ contains $T_n$ for each $n\ge 0$, $T$ is of bounded degree~only if $\bar \Delta:=\sup_n \lceil\Delta(n)\rceil + 1<\infty$.
We can use this to put an upper bound on the growth of the sequence $\delta_1,\delta_2,\delta_3,...$: for $n\ge 2$ holds
%Expanding \eqref{eq:Delta} under the constraint $\Delta(n)\le\bar \Delta-1$ yields
%One can expand \eqref{eq:Delta} under this bound  to obtain % that this bound together with \eqref{eq:Delta} yields
%
$$
\frac{\delta_n}{\delta_1\cdots\delta_{n-1}}\le\bar\Delta - 1
\;\implies \;
\delta_n\le \big((\bar \Delta-1)\delta_1\big)^{2^{n-2}}.
$$
%
Comparing with \cref{ex:exponential} suggests that $g$ grows at most exponentially. 

%Besides bounding the growth of $g$, putting an upper bound on $\Delta(n)$ has further more subtle effects, such as preventing strong oscillations in the growth of $g$ (see~\eg\ \cref{res:conditions_in_g}).

% More precisely, the maximum degree among apocentric vertices of $T_{n-1}$ (when viewed as vertices in $T$) is $\lceil\Delta(n)\rceil+1$.
% Since a graph of uniform volume growth must be locally finite, we found that $\Delta$ must be bounded.
% This imposes a first necessary upper bound on the growth of $g$: roughly, this corresponds to $g$ growing at most exponentially; but it is more subtle in that it also prevents strong oscillations in the growth of $g$.

% However, $\Delta$ being bounded is not quite sufficient for uniform volume growth.
% In the following main theorem we show that a comparatively simple sufficient criterion can be nicely stated in terms of $\Delta$ as well.
\end{remark}

It remains to prove the main result of this section: establishing the exact growth rate of $T:=T(\delta_1,\delta_2,...)$ in terms of $g$.
As we shall see, bounded degree (as discussed in \cref{rem:dbar}) is not sufficient to prove uniform volume growth. Instead we require an additional criterion that too can be concisely expressed in terms of the function $\Delta$.
In terms of $g$ this can be interpreted as preventing too strong oscillations in the growth of $g$ (\cf\ \cref{res:conditions_in_g}).

In order to state the main result we recollect that $g\:\NN_0 \to\NN$ is a strictly~increas\-ing super-additive function.
The sequence $\delta_1$,\nlspace $\delta_2$, $\delta_3,...$ $\in\NN$ is chosen to satisfy
%
$$
(1-c)\cdot g(2^n)  \;<\; (\delta_1+1)\cdots(\delta_n+1) \;<\; (1+c)\cdot g(2^n),
$$
for some $c\le 1/2$ (according to \cref{res:d_i}) and satisfies $\delta_n\ge 1$ by \cref{rem:c}. In particular, $T:=T(\delta_1,\delta_2,...)$ exists.
Finally, $\Delta(n)$ is defined as in \eqref{eq:Delta}. The main result then reads as follows:


\iffalse 

% The choice of the sequence allows us to model a wide variety of trees. An~erratically looking example is shown in \cref{fig:construction} using the sequence $\delta_n=n+2$.
% This tree turns out to be of uniform intermediate volume growth.
% With $\delta_1=d+1$ and $\delta_n=d^{2^{n-1}},n\ge 2$ we obtain the $d$-regular tree which is clearly of uniform exponential volume growth.
% For constant sequence $\delta:=2^\alpha$ we find a sub-tree of the $(\alpha$-th power of the) $\alpha$-dimensional lattice graph, and we shall see that it is of uniform polynomial volume grwoth.

\noindent\hrulefill

We demonstrate the general idea of the construction with the following example aiming for intermediate growth in the vicinity of $r^{\log\log(r)}$.

% \begin{example}\label{ex:loglogr}
% Let $T_0$ be the 3-star, that is, the tree consisting of a vertex $x^*$~(which we call the \emph{root} of $T_0$) adjacent to three leaves (that we call the \emph{apocentric~vertices} of $T_0$).
% We then define trees $T_n,n\ge 1$ recursively as follows (\cf\ \cref{fig:construction}):
% %
% \begin{itemize}
%     \item let $T_1$ consist of \emph{four} copies of $T_0$ attached to another central copy of~$T_0$~(in a way that we make precise below).
%     \item let $T_2$ consist of \emph{five} copies of $T_1$ attached to another central copy of $T_1$.
%     \item let $T_3$ consist of \emph{six} copies of $T_2$ attached to another central copy of $T_2$.
%     \item ...
% \end{itemize}
% %
% In each step we have $n+3$ non-central copies of $T_{n-1}$ that we will call the \emph{\mbox{apocentric} co\-pies}. The root of the central copy of $T_{n-1}$ will continue to be called the root~of~$T_n$, and the apocentric vertices of the apocentric copies of $T_{n-1}$ will be called apocentric vertices of $T_n$. % (all of which are leaves, but not all leaves are apocentric; see also \cref{fig:construction}).

% %
% % \begin{itemize}
% %     \item let $T_1$ be a copy of $T_0$ (the \emph{central copy}) and \emph{four} further copies of $T_0$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy (it is permitted to identify more than one root to an apocentric vertex).
% %     \item let $T_2$ be a copy of $T_1$ (the \emph{central copy}) and \emph{five} further copies of $T_1$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy.
% %     \item let $T_3$ be a copy of $T_2$ (the \emph{central copy}) and \emph{six} further copies of $T_2$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy.
% %     \item ...
% %     \item let $T_n$ be a copy of $T_{n-1}$ (the \emph{central copy}) and $n-3$ further copies of $T_{n-1}$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy (it is permitted to identify more than one root to an apocentric vertex, though in this example this is only necessary to define $T_1$).
% % \end{itemize}

% It remains to give a precise meaning to the \enquote{attachment of the apocentric copies}:
% in each step, each apocentric copy of $T_{n-1}$ is \enquote{attached to the central copy of $T_{n-1}$} by identifying its root with some apocentric vertex of the central copy. 
% The choice of the apocentric vertex is more or less free (we can even attach more than one copy to the same vertex).
% However, it will be important for the analysis of the growth behavior that we do this in a maximally uniform manner, attaching approximately the same number of copies to each apocentric vertex.

% If we now identify $T_{n-1}$ with its central copy in $T_n$ we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $T:=\bigcup_{n\ge 0} T_n$ is well-defined.
% We claim that $T$ is a tree of intermediate volume growth.

% To see that this is plausible, make the following two observations:
% %We want to make this at least plausible. Observe the following:
% %
% \begin{itemize}
%     \item the distance from the root of $T_n$ to any apocentric vertex is exactly $2^n$. In fact, $T_n\subset T$ is the ball of radius $2^n$ centered at the \emph{global root} $x^*$ in $T$.
%     \item it holds $|T_n|=4\cdot5\cdots (n+4)=\frac16(n+4)!$. %\,\sim\, n^4n!\,\sim\, n^4 \cdot n^n \sqrt n \,e^{-n}$ 
%     %\sim n^4n! $.
% \end{itemize}
% %
% Thus, for $r=2^n$ we can estimate
% %
% \begin{align*}
% |\ball T{x^*}r| = |T_n| = \tfrac16 (n+4)! 
% \,&\sim\,
% n! \, n^4  
% \,\sim\,
% % n^n \cdot n^{9/2}e^{-n}
%  n^n e^{-n} \sqrt n \, n^4 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \, (\log r)^{9/2}  .
% %\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
% \end{align*}
% %
% Recall that we are using $\log r := \log_2 r$.

% While this suggests intermediate growth for balls around the global root $x^*$, we still need to establish
% %
% \begin{itemize}
%     \item a similar volume growth around other vertices of $T$, in particular, we need~to establish that the growth is \emph{uniform}, and
%     \item that a similar estimation is valid for balls of radii that are not of the form~$2^n$.
% \end{itemize}
% %
% Both points will be addressed in the discussion of the general construction.
% \end{example}

\begin{example}\label{ex:loglogr}
Let $T_0:=\{x^*\}$ be the tree consisting of a single vertex (called \emph{global root}).
We proceed by recursively defining trees $T_n,n\ge 1$ as follows (\cf\ \cref{fig:construction}): 
%
\begin{itemize}
    \item let $T_1$ consist of \emph{three} copies of $T_0$ connected to another central copy of~$T_0$.
    \item let $T_2$ consist of \emph{four} copies of $T_1$ connected to another central copy of $T_1$.
    \item let $T_3$ consist of \emph{five} copies of $T_2$ connected to another central copy of $T_2$.
    \item ...
\end{itemize}
%
In each step we add $n+2$ \enquote{non-central} copies of $T_{n-1}$ that we shall call the~\emph{apocentric co\-pies} of $T_{n-1}$. 
In order to describe the connection between the central and the apocentric copies we need to introduce the notion of \emph{root} and \emph{apocentric vertex} of $T_n$:
%
\begin{itemize}
    \item the unique vertex $x^*$ of $T_0$ is both the root and an apocentric vertex of $T_0$.
    \item the root of $T_n$ is the root of its central copy of $T_{n-1}$.
    \item an apocentric vertex of $T_n$ is an apocentric vertex in an apocentric copy of $T_{n-1}$ (all of them are leave of $T_n$, but not all leaves are apocentric).
\end{itemize}
%
% \begin{figure}[!h]
%     \centering
%   % \includegraphics[width=0.7\textwidth]{img/construction.pdf}
%   % \includegraphics[width=0.65\textwidth]{img/construction_2.pdf}
%     \includegraphics[width=0.83\textwidth]{img/construction_3.pdf}
%     \caption{Illustration of the first four steps in the  construction~of~\cref{ex:loglogr}. The ringed vertex is the root and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy of $T_{n-1}$ in $T_n$.}
%     \label{fig:construction}
% \end{figure}
%
We can now finalize the definition of $T_n$: each apocentric copy of $T_{n-1}$ is connected to the central copy of $T_{n-1}$ by adding an edge between the root of the apocentric copy and some apocentric vertex of the central copy.
The choice of the apocentric vertex in the central copy is more or less free (we can even connect more than one apocentric copy to the same vertex).
However, it will be important for the analysis of the growth behavior that we do this in a maximally uniform manner, attaching approximately the same number of copies to each apocentric vertex.

If we now identify $T_{n-1}$ with its central copy in $T_n$ we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $T:=\bigcup_{n\ge 0} T_n$ is well-defined.
We claim that $T$ is a tree of intermediate volume growth.

To see that this is plausible, make the following two observations:
%We want to make this at least plausible. Observe the following:
%
\begin{itemize}
    \item the distance from the root of $T_n$ to any apocentric vertex is exactly $2^n-1$. In fact, $T_n\subset T$ is the ball of radius $2^n-1$ centered at the global root~$x^*$.
    \item for $n\ge 1$ holds $|T_n|=4\cdot5\cdots (n+3)=\frac16(n+3)!$. %\,\sim\, n^4n!\,\sim\, n^4 \cdot n^n \sqrt n \,e^{-n}$ 
    %\sim n^4n! $.
\end{itemize}
%
Thus, for $r=2^n$ we can estimate
%
\begin{align*}
|\ball T{x^*}{r-1}| = |T_n|= \tfrac16 (n+3)! 
\, &\sim\,
n! \, n^3  
\,\sim\,
% n^n \cdot n^{9/2}e^{-n}
 n^n e^{-n} \sqrt n \, n^3 
\\ &= \,
r^{\log\log r}\cdot
r^{-1/\ln 2} \cdot (\log r)^{7/2}  .
%\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
\end{align*}
%
Recall the convention $\log r := \log_2 r$.

While this suggests intermediate growth for balls around the global root $x^*$, we still need to establish
%
\begin{itemize}
    \item a similar volume growth around other vertices of $T$, in particular, we need~to establish that the growth is \emph{uniform}, and
    \item that a similar estimation is valid for balls of radii other than $2^n-1$.
\end{itemize}
%
Both points will be addressed in the discussion of the general construction.



% We make two simple observations:
% %
% \begin{itemize}
%     \item the distance from the central vertex of $T_n$ to an apocentric vertex of $T_n$ is exactly $2^n-1$, and
%     \item for $n\ge 1$ holds $|T_n|=4\cdot5\,\cdots\, (n+3)=\frac16 (n+3)!$\,.
% \end{itemize}
% %
% If we identify $T_{n-1}$ with its central copy in $T_{n}$, we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset \cdots$ and the limit tree $T:=\bigcup_n T_n$ is well-defined. Technically, we can interpret $(T,x^*)$ as the distributional limit of the sequence $(T_n,o_n)$ of biased random rooted trees, where $o_n$ is the global center of $T_n$ with probability $1$. 

% Setting $r=2^n-1$, a straight-forward estimation shows
% %
% \begin{align*}
% |\ball T{x^*}r| = |T_n| = \tfrac16 (n+4)! 
% \,&\sim\,
% n! \, n^4  
% \,\sim\,
%  n^n e^{-n} \sqrt n \, n^4 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \, (\log r)^{9/2}.
% \end{align*}

% %Thus, we expect intermediate volume growth around the global center~$x^*$ and it remains to establish suitable behavior for the other vertices.

% Thus, we found intermediate volume growth, at least around the global root~$x^*$ for radii of the form $r=2^n,n\in\NN$.
% It would then remain to establish that
% %
% \begin{myenumerate}
%     \item a similar estimation holds for balls centered at other vertices, and
%     \item the estimation does not deviate too much from the intended growth for radii that are not of the form $2^n$.
% \end{myenumerate}
% %
% We postpone the discussion of these details until the discussion of the general case in \cref{res:g_growth_trees}.
\end{example}

The strength of the construction in \cref{ex:loglogr} lies in the many free parameters that we can use to model a wide range of growth behaviors.
More precisely,\nlspace after choosing a sequence $\delta_0,\delta_1,\delta_2,...\in\NN$ we can consider the following analogous~construction for the $T_n$:
%
\begin{itemize}
    \item let $T_0$ be the $\delta_0$-star, that is, the tree consisting of a vertex $x^*$ adjacent to $\delta_0$ further vertices.
    \item let $T_n,n\ge 1$ consist of $\delta_n$ copies of $T_{n-1}$ attached to a further central copy.
\end{itemize}
%
In \cref{ex:loglogr} we used $\delta_n:=n+3$.

If we set $T:=\bigcup_{n\ge 0} T_n$ as before, then we again find that $T_n\subset T$ is~the~ball~in $T$ of radius $2^n$ centered at the global root $x^*$.
But now these balls have volume~$|T_n|=(\delta_0+1)\cdots(\delta_n+1)$, and so to achieve a specific volume growth $g\:\NN_0\to\RR$~it is plausible to choose integers $\delta_0,\delta_1,\delta_2,...\in\NN$ for which $(\delta_1+1)\cdots(\delta_n+1)$ approximates the growth of $f(n):=g(2^n)$.

% This construction has many free parameters (the number of copies of $T_{n-1}$ that make up $T_n$) that allow us to model a wide range of growth behaviors. 
% If the~total number of copies in step $n$ (central and apocentric) is $\delta_n$, then $|T_n|=\delta_1\cdots \delta_n$, and so a first step towards the general construction is to choose the $\delta_i$ so that $\delta_1\cdots\delta_n$ approximates the desired growth, more precisely, $f(n):=g(2^n)$.


% \textcolor{lightgray}{
% As we shall see, we can most often not guarantee $|\ball Gvr|=\theta(g(r))$. For that reason, the function $g$ shall be called \emph{target growth} of our construction, in the sense that we aim for achieving this growth, but the actually provable lower and upper bounds on $|\ball Gvr|$ will be not quite $g$, but slight modifications thereof (see \cref{res:g_growth_trees}).
% }

% In order to construct this tree, we need to approximate the desired growth function $g(r)$, or more precisely $f(n):=g(2^n-1)$, by a product of integers~$\delta_1,\delta_2,\delta_3,...\in\NN$, that is, we want
% %
% $$\delta_1\cdots\delta_n\in \theta(f(n)).$$
% %
% %We call this sequence of $\delta_i$ the \emph{decomposition sequence} of $f$ (\resp\ $g$).

\begin{lemma}\label{res:d_i}
Given an increasing function $f\:\NN_0\to\RR$, there is a sequence of integers $\delta_1,\delta_2,\delta_3,...\in\NN$ so that
%
\begin{equation}\label{eq:d_bounds}
(1-c)\cdot f(n)  \;<\; \delta_1\cdots\delta_n \;<\; (1+c)\cdot f(n),\qquad\text{for all $n\ge 0$}
\end{equation}
%
%
where $c:=\sup_n (f(n)/f(n+1)) \le 1$.
%
\begin{proof}
Set $\delta_1 := f(1)$.
Then define iteratively
%
$$\delta_{n+1}:=\begin{cases}
\lceil f(n+1)/f(n)\rceil & \text{if $\delta_1\cdots\delta_{n}\le f(n)$}\\
\lfloor f(n+1)/f(n)\rfloor & \text{if $\delta_1\cdots\delta_{n}> f(n)$}
\end{cases}.
$$

That this definition satisfies \eqref{eq:d_bounds} is shown by induction. It is clearly satisfied for $n=1$. If it is satisfied for $n$ and $\delta_1\cdots\delta_{n}\le f(n)$, then
%
\begin{align*}
\delta_1\cdots \delta_n \cdot\delta_{n+1} &\le f(n) \cdot\Big\lceil \frac{f(n+1)}{f(n)} \Big\rceil 
< f(n)\cdot \Big( \frac{f(n+1)}{f(n)} + 1\Big)
\\&= \Big( 1+ \frac{f(n)}{f(n+1)} \Big) \cdot f(n+1) \le ( 1+ c )\cdot  f(n+1), \\[1ex]
\delta_1\cdots \delta_n \cdot\delta_{n+1} 
&> (1-c)\cdot f(n)\cdot \Big\lceil \frac{f(n+1)}{f(n)} \Big\rceil 
\ge (1-c)\cdot f(n)\cdot \frac{f(n+1)}{f(n)}
\\&=(1-c)\cdot f(n+1).
\end{align*}
%
Equivalently for the case $\delta_1\cdots\delta_{n}> f(n)$.
\end{proof}
\end{lemma}

Note that the lower bound is useful only for $c<1$, which requires $f(n)=g(2^n-1)$ to grow at least exponentially, or equivalently, $g(r)=\Omega(r)$.

Most properties of the constructed tree can be concisely expressed in terms of the sequence $\delta_n$.
Ultimately we are interested in expressing these properties in~terms of $g$, and so we shall spend some time understanding the relation between $g$ and its sequence.
The following list contains some first examples of this:
%
\begin{itemize}
    \item 
    A polynomial function $g(r)=r^\alpha$ will have a constant sequence $\delta_n=2^\alpha$.\nlspace If $\delta_n$ is not a power of two then this models polynomial growth with non-integer exponent $\log_2\alpha$.
    
    \item As soon as the target growth is super-polynomial, that is $g(r)=r^{\omega(1)}$, the sequence $\delta_n$ is unbounded and $\delta_n/s_n\to 1$.
    
    \item 
    If $g$ is exponential, say $g(r)=b^r$, we obtain a sequence $\delta_n=b^{2^n}$.

    \item A special role will be played by target growth $g$ with sequence $\delta_n\sim n^\alpha$ for a fixed $\alpha>0$. Roughly, those correspond to growth behaviors of the order $r^{\alpha \log\log r}$. \cref{ex:loglogr} demonstrates this for $\alpha=1$.
    Later we shall find that for $\alpha>1$ our construction exhibits additional nice properties.
\end{itemize}

A necessary criterion for uniform volume growth is a finite maximum degree, and we need to check this for $T$.
Note that in each step of the construction, we add $\delta_n-1$ new apocentric copies of $T_{n-1}$ that need to be connected to the $(\delta_1-1)\cdots(\delta_{n-1}-1)$ apocentric vertices of the central copy of $T_{n-1}$ (all of which are leaves). If for each $n\ge 1$ we distribute the connections maximally uniformly, we can achieve maximum degree
%
$$\Delta:= \Big\lceil \sup_n \frac{\delta_{n}-1}{(\delta_1-1)\cdots(\delta_{n-1}-1)} \Big\rceil +1.$$
%
In particular, this value must be finite. So, when is this the case? Roughly speaking, when $g(r)=e^{\mathcal O(r)}$ and when $g$ changes its growth behavior not~too suddenly.\nlspace We~believe that $g$ being log-concave is sufficient.


% The maximum degree of the tree that we are going to construct can be expressed in terms of the $\delta_i$ as follows
% %
% $$\Delta:= \Big\lceil \sup_n \frac{\delta_{n}-1}{(\delta_1-1)\cdots(\delta_{n-1}-1)} \Big\rceil +1.$$
% % As long as $g$ is at most exponential, this yields a finite maximum degree $\Delta=\Delta(T)$.
% We require this expression to yield a finite value. 
% This happens, roughly speaking, if $g$ grows at most exponentially.
% But this condition also captures the more technical aspect that the growth behavior of $g$ should not change too rapidly.

% \begin{lemma}\label{res:Delta_def}
% If $g=e^{\mathcal O(r)}$ with decomposition sequence $\delta_1,\delta_2,\delta_3,...\in\NN$, then
% %
% $$\Delta:=\Big\lceil \sup_n\frac{\delta_n-1}{(\delta_1-1)\cdots(\delta_{n-1}-1)}\Big\rceil+1$$
% %
% is finite.
% \end{lemma}
% %
% \begin{proof}
% We have $f(n):=g(2^n)=e^{h(n)}$ with $h\in\mathcal O(2^n)$ strictly increasing, that is, $h(n)\le C2^n$ for all $n\ge N$. Following the construction of $\delta_n$ in the proof of \cref{res:d_i} this yields
% %
% $$\delta_n\le \Big\lceil\frac{f(n)}{f(n-1)}\Big\rceil \le \frac{f(n)}{f(n-1)} + 1 
% = e^{h(n)-h(n-1)}+1 \le e^{C2^n}+1.
% $$
% $$\delta_n\ge \Big\lfloor\frac{f(n)}{f(n-1)}\Big\rfloor \le \frac{f(n)}{f(n-1)} - 1 
% = e^{h(n)-h(n-1)}-1 \ge ...
% $$
% \end{proof}

% \begin{theorem}
% Given a strictly increasing function $g\in \mathcal O(e^r)$ with $g(r)\ge r$, there is a tree $T$ all whose vertices $v\in V(T)$ satisfy
% %
% $$A \cdot g(r/4) \le |B_v^T(r)|\le B \cdot g(2r)^2,\quad\text{for all $r\ge 0$},$$
% %
% with $A>0$ and $B<8\Delta$, where $\Delta:= \lceil \sup_n g(2^{n+1})/g(2^n) \rceil + 1$ is the maximum~degree of $T$.
% \end{theorem}

We can now prove that $T$ has the desired volume growth around \emph{every} vertex.

% \begin{theorem}
% Let $\delta_1,\delta_2,\delta_3,...\in\NN$ be a sequence of integers with
% %
% $$\delta_{n+1}\le(\Delta-1)\delta_1\cdots\delta_n$$
% %
% for some $\Delta\in\NN$. Set $f(n):=\delta_1\cdots\delta_n$.

% Then there exists a tree $T$ of maximum degree $\Delta$, all whose vertices $v\in V(T)$~satisfy
% %
% $$f(n-1) \;\le\; |B_v^T(2^n)| \;\le\; 2\Delta f(n)^2,\quad\text{for all $n\ge 0$},$$
% \end{theorem}

% \hrulefill

% \begin{theorem}
% Let $g\:\NN_0\to\NN$ be strictly increasing and let $\delta_1,\delta_2,\delta_3,...\in \NN$ be its decomposition sequence, so that (by \cref{res:d_i})
% %
% $$(1-c)\cdot g(2^n) \;\le\; \delta_1\cdots\delta_n \;\le\; (1+c)\cdot  g(2^n),\quad\text{for all $n\ge 1$}.$$
% %
% with $c<1$. If the $\delta_i$ satisfy
% $$\Delta:=\Big\lceil\sup_n\frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_n-1)}\Big\rceil + 1<\infty,$$
% %
% then there exists a tree $T$ of maximum degree $\Delta$, all whose vertices $v\in V(T)$~satisfy
% %
% $$(1-c) \cdot g(r/4) \;\le\; |B_v^T(r)| \;\le\; 2\Delta(1+c) \cdot g(2r)^2,\quad\text{for all $r\ge 0$},$$
% \end{theorem}

% \hrulefill

% \begin{theorem}\label{res:g_growth_trees}
% Given an increasing function $g\:\NN_0\to\NN$ and a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ of integers satisfying (see \cref{res:d_i})
% %
% $$ %\begin{equation}\label{eq:d_bounds}
% (1-c)\cdot g(2^n-1)  \;<\; \delta_1\cdots\delta_n \;<\; (1+c)\cdot g(2^n-1),\quad\text{for all $n\ge 0$}
% $$ %\end{equation}
% %
% Suppose that $\delta_i\ge 2$ (which implies $c\le 1/2$) and
% %
% \begin{equation}\label{eq:conditions_g}
% \Delta:= \Big\lceil \sup_n \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_n-1)} \Big\rceil +1 < \infty.
% \end{equation}
% %
% Then the tree $T$ is of maximum degree $\Delta$ and all its vertices \mbox{$v\in V(T)$} satisfy
% %
% $$\textstyle\frac12 \cdot g(\frac14r-\frac34) \;\le\; |B_v^T\!(r)| \;\le\; {\textstyle\frac92\Delta} \cdot g(2r+1)^2,\quad\text{for all $r\ge 0$}.$$
% % $$(1-c) \cdot g(r/4) \;\le\; |B_v^T(r)| \;\le\; 2\Delta(1+c)^2 \cdot g(2r)^2,\quad\text{for all $r\ge 0$}.$$
% \end{theorem}

% % \begin{theorem}\label{res:g_growth_trees}
% % Let $g\:\NN_0\to\NN$ be strictly increasing so that
% % %
% % \begin{equation}\label{eq:conditions_g}
% % c:=\sup_n \frac{g(r)}{g(2r)} < 1
% % \quad\text{and}\quad
% % \Delta:= \Big\lceil\frac{c+1}{(c-1)^2}\cdot \sup_r \frac{r\cdot g(2r)}{g(r)^2} \,\Big\rceil + 1 < \infty.
% % \end{equation}
% % %
% % Then there exists a tree $T$ of maximum degree at most $\Delta$, all whose vertices \mbox{$v\in V(T)$} satisfy
% % %
% % $$(1-c) \cdot g(r/4) \;\le\; |B_v^T(r)| \;\le\; 2\Delta(1+c)^2 \cdot g(2r + 1)^2,\quad\text{for all $r\ge 0$}.$$
% % \end{theorem}

% % Conditions \eqref{eq:conditions_g} is satisfied, roughly speaking, for all functions $g$ between (and~including) linear and exponential growth, but it also ensures that $g$ does not vary too strongly in its growth behaviour.
% % In particular, \cref{res:g_growth_trees} can be used to construct trees of \emph{uniform intermediate growth}.

% \begin{proof}
% % % By \cref{res:d_i} we can choose a sequence of integers $\delta_1,\delta_2,\delta_3,...\ge 1$ so that
% % % %
% % % $$(1-c)\cdot g(2^n) \;\le\; \delta_1\cdots\delta_n \;\le\; (1+c)\cdot  g(2^n),\quad\text{for all $n\ge 1$}.$$
% % % %
% % % where $c<1$ by the first condition in \eqref{eq:conditions_g}. 
% % % %A consequence from the other part of \eqref{eq:conditions_g} for later use is

% % We recursively define trees $T_n,n\in\NN_0$ as follows: let $T_0=\{\bullet\}$ be the tree~on a single vertex called the \emph{global center}.
% % For $n\ge 1$, let $T_n$ consist of $\delta_n$ disjoint copies of $T_{n-1}$; $\delta_n - 1$ so-called \emph{apocentric} copies, and one \emph{central} copy.
% % In order to~describe how to connect these sub-trees to form the tree $T_n$, we still need to define \emph{central} and \emph{apocentric} vertices:
% % %
% % \begin{myenumerate}
% %     \item the single vertex of the tree $T_0$ is both central and apocentric.
% %     \item a vertex of a tree $T_n$ is central (\resp\ apocentric) if it is contained in~a~cen\-tral (\resp\ apocentric) copy of $T_{n-1}$, and is central (\resp\ apocentric) in this copy.
% % \end{myenumerate}
% % %
% % Each tree $T_n$ has a unique central vertex and $(\delta_1-1)\cdots(\delta_n-1)$ apocentric vertices.

% % To finalize the definition of $T_n$ we add edges as follows: for each apocentric copy of $T_{n-1}$ add an edge between the central vertex of this copy and some apocentric vertex of the central copy of $T_{n-1}$. Do this in a way to keep the maximum degree of $T_n$ at or below $\Delta$, which is possible by condition \eqref{eq:conditions_g}:
% % %
% % % \begin{align*}
% % %     \frac{\#\{\text{new apocentric copies of $T_{n-1}$}\}}{\#\{\text{apocentric vertices in the central $T_{n-1}$}\}}
% % %     &=\frac{\delta_{n}-1}{(\delta_1-1)\cdots (\delta_{n-1}-1)}
% % %     \\&\le 2^{n-1}\cdot\frac{\delta_{n}}{\delta_1\cdots \delta_{n-1}}
% % %     \\&= 2^{n-1}\cdot\frac{\delta_1\cdots \delta_{n}}{(\delta_1\cdots \delta_{n-1})^2}
% % %     \\&\le \frac{c+1}{(c-1)^2} \cdot \frac{2^{n-1}\cdot g(2^{n})}{g(2^{n-1})^2} \le \Delta - 1.
% % % \end{align*}
% % \begin{align*}
% %     \frac{\#\{\text{new apocentric copies of $T_{n-1}$}\}}{\#\{\text{apocentric vertices in the central $T_{n-1}$}\}}
% %     &=\frac{\delta_{n}-1}{(\delta_1-1)\cdots (\delta_{n-1}-1)}
% %      \le \Delta - 1.
% % \end{align*}
% % %
% % We can now see that the the distance from the central vertex of $T_n$ to every apocentric vertex of $T_n$ is exactly $2^n - 1$. We also have $|T_n|=\delta_1\cdots \delta_n$, hence
% % %
% % $$(c-1)\cdot g(2^n - 1) \;\le\; |T_n| \;\le\; (1+c)\cdot g(2^n - 1).$$
% % %

% % % Note that this ensures that all apocentric vertices of $T_n$ are leaves, and that since $\delta_i\le (\Delta-1)\kern0.7pt\delta_1\cdots\delta_{i-1}=\text{\#apocentric vertices of $T_{i-1}$}$, the edges can be chosen to keep the maximal degree of $T_i$ at at most $\Delta$.

% % By identifying $T_{n-1}$ with its central copy in $T_n$, we can write down a chain~of graphs $T_0\subset T_1\subset T_2\subset \cdots$ with limit graph $T:=\bigcup_i T_i$. Clearly, $T$ is a tree. %We show that $T$ has the appropriate growth behavior.

% % % To show this, let $x^*$ be the \emph{global center}, \ie\ the central vertex of each of the canonical subgraphs $T_i\subset T$.
% % % Next, note the following properties of $T_i$:
% % % %
% % % \begin{myenumerate}
% % %     \item The vertices farthest away from the central vertex in $T_i$ are exactly the apocentric vertices at distance $2^i$. In particular, $B_{2^i}^T(x^*)=T_i$.
% % %     \item for $i\ge 1$ we have $|T_i| = (\delta_1+1)\cdots(\delta_i+1)=g(2^i)$.
% % % \end{myenumerate}

% %It remains to prove the lower and upper bounds on the size of balls in $T$. In the following, f
% Fix a vertex $v\in V(T)$ and a number $r\ge 0$. Let $T_n(v)$ denote the copy~of~$T_n$ (from the recursive construction of $T$) that contains $v$.

% To prove the lower bound, choose $n\in\NN$ so that $2^{n+1}-1\le r\le 2^{n+2}-1$. Let~$x$ be the central vertex of $T_n(v)$. Each vertex of $T_n(v)$ can be reached from $v$ in at most $2(2^n-1)\le r$ steps: at most $2^n-1$ steps from $v$ to $x$, and at most $2^n-1$ steps from $x$ to any other vertex of $T_n(v)$. Thus
% %
% $$|B_v^T\!(r)|\ge |B_v^T\!(2(2^n-1))|\ge |T_n| \ge (1-c)\cdot g(2^n-1) \ge {\textstyle\frac12}\cdot g(\textstyle\frac14r-\frac34).$$

% To establish the upper bound, choose $n\in\NN$ so that $2^{n-1} - 1\le r\le 2^n - 1$. Let $T_n(v)$ be the copy of $T_n$ that contains $v$. Let $m\in\NN$ be the largest integers so that the apocentric vertices of $T_n(v)$ are also apocentric in $T_m\subset T$. Necessarily $m\ge n$.

% We estimate the number of copies of $T_n$ that are connected to apocentric vertices of $T_n(v)$.
% Note that there are $\delta_1\cdots\delta_m$ apocentric vertices in $T_m\subset T$ and $\delta_1\cdots\delta_n$ apocentric vertices in $T_n(v)$. Assuming that the $\delta_{m+1}$ copies of $T_m$ that are attached to the apocentric vertices of $T_m\subset T$ are distributed maximally uniformly, we can expect that there are no more than
% %
% $$
% \Big\lceil \delta_{m+1} \cdot \frac{\delta_1\cdots\delta_n}{\delta_1\cdots\delta_m}\Big\rceil
% =
% \Big\lceil \frac{\delta_{m+1}}{\delta_1\cdots\delta_m} \cdot \Big( \frac{\delta_{n+1}}{\delta_1\cdots\delta_n}\Big)^{-1} \cdot \delta_{n+1} \Big\rceil
% $$
% %
% copies of $T_m$ attached to the apocentric vertices of $T_n(v)\subseteq T_m\subset $T$.

% \noindent\hrulefill

% To establish the upper bound, choose $n\in\NN$ so that $2^{n-1} - 1\le r\le 2^n - 1$ and enumerate the copies of $T_n$ that can be reached from $v$ in at most $2^n-1$ steps.
% Note that the only way \enquote{out of $T_n(v)$} is either through one of its apocentric vertices, or through its central vertex $x$:
% %
% \begin{itemize}
%     \item through an apocentric vertex: having reached an apocentric vertex of $T_n(v)$, up to $\Delta-1$ central vertices of other copies of $T_n$ can be reached. From these no further copies can be reached, as in the remaining $<2^n-1$ steps we cannot reach any apocentric vertex in the same copy. How many apocentric vertices of $T_n(v)$ can be reached in $\le 2^n-1$ steps? Hard to say, but at most $|T_n|$ many.
%     \item through the central vertex $x$: having reached $x$ (and assuming that $x$~is not the global center), we can reach an apocentric vertex $w$ of some \enquote{earlier} copy of $T_n$. Starting in $w$ we can reach other apocentric vertices of $T_n(w)$, certainly less than $|T_n|$ many. As before, from each apocentric vertex of $T_n(w)$ we can reach up to $\Delta-1$ central vertices of other copies of $T_n$, from which no further copies can be reached. Like-wise, in the remaining $<2^n-1$ steps we cannot reach from $w$ to the central vertex of $T_n(w)$, and so we enumerated all reachable copies of $T_n$.
% \end{itemize}
% %
% To summarize, we can reach at most $2\Delta\cdot|T_n|$ copies of $T_n$ (that is, $T_n(v)$, $T_n(w)$, and from each at most $(\Delta-1)|T_n|$ other copies via apocentric vertices). In each of those we can reach at most $|T_n|$ vertices. This yields
% %
% $$|B_v^T\!(r)| \le |B_v^T\!(2^n-1)| \le 2\Delta\cdot|T_n|^2 \le 2\Delta(1+c)^2\cdot g(2^n-1)^2 \le {\textstyle\frac92}\Delta\cdot g(2r+1)^2.$$
% \end{proof}


Let $\bar g\:\NN\to\RR^d$ be super-additive, \ie\ $\bar g(a+b)\ge \bar g(a)+\bar g(b)$.

\fi

%\newpage

%The following theorem proves the essential result, that under some mild technical conditions the tree $T$ is of uniform volume growth $g$.

%\msays{We need to emphasize more that $g$ is increasing.}

\begin{theorem}\label{thm:main}
Fix $v\in V(T)$ and $r\ge 0$. Then holds
%
\begin{myenumerate}
\setlength\itemsep{1ex}
\item \, \\ \,
\vspace{-2.325\baselineskip}
\begin{align*}
\mathrlap{
    |\ball Tvr| \,\ge\, (1-c) \cdot g(r/4) 
                \,\ge\, \tfrac12\, g(r/4),
} \hspace{16em}
\end{align*}
%
where $r/4$ in the argument of $g$ is rounded down to the largest integer.
 
\item If $\bar\Delta:=\smash{\displaystyle\sup_n}\lceil\Delta(n)\rceil +1<\infty$, then $T$ is of maximum degree $\bar\Delta$ and
%
\begin{align*}
\mathrlap{
    |\ball Tvr| \,\le\,  2\bar\Delta \cdot (1+c)^2 \cdot g(2r)^2 
                \,\le\, \tfrac92\bar\Delta\cdot g(2r)^2.
} \hspace{16em}
\end{align*}

\item
If $\Gamma:= \smash{\displaystyle\sup_{m\ge n}}  \lceil\Delta(m)/\Delta(n) \rceil < \infty$, then $\bar\Delta<\infty$ and
%
\begin{align*}
\mathrlap{
     |\ball Tvr| \,\le\, 2(1+c) \cdot \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
} \hspace{16em}
\\ 
\mathrlap{
 \phantom{|\ball Tvr| } 
 \,\le\, 3 \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
} \hspace{16em}
\\ 
\mathrlap{
 \phantom{|\ball Tvr| } 
 %\,\le\, 3\max\{1,\Gamma\} \cdot g(4r).
 \,\le\, 3\Gamma \cdot g(4r).
} \hspace{16em}
\end{align*}
   % 
In particular, if $\Gamma<\infty$ then $T$ is of uniform volume growth $g$.
\end{myenumerate}
\end{theorem}

% \begin{theorem}\label{thm:main}
% For each $v\in V(T)$ and $r\ge 0$ holds
% %

% \begin{align*}
% \mathrlap{
%     |\ball Tvr| \,\ge\, (1-c) \cdot g(r/4) 
%                 \,\ge\, \tfrac12\, g(r/4)
% } \hspace{16em}
% \end{align*}
% %
% where $r/4$ in the argument of $g$ is rounded down to the largest integer.
 
% If $\bar\Delta:=\smash{\displaystyle\sup_n}\lceil\Delta(n)\rceil +1<\infty$, then $T$ is of maximum degree $\bar\Delta$ and
% %
% \begin{align*}
% \mathrlap{
%     |\ball Tvr| \,\le\,  2\bar\Delta \cdot (1+c)^2 \cdot g(2r)^2 
%                 \,\le\, \tfrac92\bar\Delta\cdot g(2r)^2.
% } \hspace{16em}
% \end{align*}

% If $\Gamma:= \smash{\displaystyle\sup_{m\ge n}}  \lceil\Delta(m)/\Delta(n) \rceil < \infty$, then $\bar\Delta<\infty$ and
% %
% \begin{align*}
% \mathrlap{
%      |\ball Tvr| \,\le\, 2(1+c) \cdot \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
% } \hspace{16em}
% \\ 
% \mathrlap{
%  \phantom{|\ball Tvr| } 
%  \,\le\, 3 \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
% } \hspace{16em}
% \\ 
% \mathrlap{
%  \phantom{|\ball Tvr| } 
%  \,\le\, 3\min\{1,\Gamma\} \cdot g(4r).
% } \hspace{16em}
% \end{align*}
%   % 
% In particular, if $\Gamma<\infty$ then $T$ is of uniform volume growth $g$.
% \end{theorem}

Note that the lower bound holds unconditionally. % (only subject to $\bar g$ being super-additive to ensure that $T$ exists, \cf\ \cref{rem:c}). %(only assuming $g$ is super-additive as discussed in \cref{rem:c}.
The conditions $\bar\Delta<\infty$~and~$\Gamma<\infty$ for the upper bounds are technical, but there are natural~criteria in terms of $g$ that imply both, such as being \emph{log-concave} (see \cref{res:conditions_in_g} below).

% \begin{theorem}\label{thm:main}
% Let $g\:\NN_0\to\RR$ be an increasing function and set $f(n):=g(2^n-1)$. 
% Let $\delta_1,\delta_2,\delta_3,...\in\NN$ be a sequence of integers with
% %
% $$ %\begin{equation}\label{eq:d_bounds}
% (1-c)\cdot f(n)  \;<\; (\delta_1+1)\cdots(\delta_n+1) \;<\; (1+c)\cdot f(n)
% $$ %\end{equation}
% for all $n\ge 0$, where $c:=\sup_n f(n)/f(n+1)\le 1$. 
% Set $T:=T(\delta_1,\delta_2,...)$ and
% %
% $$\Delta(n):=\frac{\delta_n}{\delta_1\cdots\delta_{n-1}}\;\;\text{where}\;\;\Delta(1):=\delta_1.$$
% %
% For each $v\in V(T)$ and $r\ge 0$ then holds
% \begin{myenumerate}
%     \item \quad
%     \vspace{-1\baselineskip}
%     $$|\ball Tvr| \,\ge\, (1-c) \cdot g(r/4).$$
%     \item 
%     if $\bar\Delta:=\smash{\displaystyle\sup_n}\lceil\Delta(n)\rceil +1<\infty$ then $T$ is of maximum degree $\bar\Delta$ and
%     %
%     $$|\ball Tvr| \,\le\,  2\bar\Delta \cdot (1+c)^2 \cdot g(2r + 1)^2.$$
%     \item 
%     if $\Gamma:= \smash{\displaystyle\sup_{m\ge n}}  \lceil\Delta(m)/\Delta(n) \rceil < \infty$ \nf(which implies $\bar\Delta<\infty$\nf) then
%     %
%     $$|\ball Tvr| \,\le\,  (\Gamma+1)\cdot (1+c) \cdot g(2r + 1).$$
% \end{myenumerate}
% %
% In particular, if $c<1$ and \itm3 applies, then $T$ is of uniform volume growth $g$.
% \end{theorem}

% The preconditions of \itm2 and \itm3 in \cref{thm:main} are technical in nature but are usually easy to check and are also satisfied for most naturally defined functions in the feasible growth range. %; and it~is usually easy to check this for any particular function.
% In \cref{res:conditions_in_d} we give some very accessible criteria in terms of the sequence of $\delta_n$.
% Investing more effort, one can show that it suffices to have $g$ being log-concave (as we show in \cref{res:conditions_in_g}).
% %A concrete criterion is given in \cref{res:conditions_in_g}, where it is shown that any log-concave function $g$ is natural in this sense.

% We remark that for most naturally defined functions $g$ of an appropriate growth holds $c<1$ as well as that the conditions of \itm2 and \itm3 are satisfied, and thus that $T$ is of uniform volume growth $g$. See \cref{res:...} for a more precise statement about which functions satisfy these conditions.
% Roughly, if $g$ is sub-exponential, then \itm2 applies; if $g$ is even log-concave, then also \itm3 applies.

\begin{proof}[Proof of \cref{thm:main}]
%Fix $v\in V(T)$ and $r\ge 4$.
For a vertex $w\in V(T)$ we use the notation $\tau_n(w)$ to denote the unique copy $\prec_n T$ that contains $w$.
%
%Moreover, let us agree that whenever we write $T_n\subset T$, we refer to the canonical sub-graph $T_n$ in $T$ from the defining inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ in \cref{constr:tree}.

To prove \itm1 choose $n\in\NN_0$ with $2^{n+1}\le r\le 2^{n+2}$. 
%Let $x$ be the root of $T_n(v)$. 
Each vertex of $\tau_n(v)$ can be reached from $v$ in at most $2(2^n-1)$ steps: 
at most $2^n-1$ steps from $v$ to the root of $\tau_n(v)$, and at most $2^n-1$ steps from this root to any other vertex of $\tau_n(v)$. 
This yields
%
\begin{align*}
|\ball Tvr|
%|B_v^T\!(r)|
\ge |\ball Tv{2^{n+1}}|
%|B_v^T\!(2^{n+1})|
> |\ball Tv{2(2^n-1)}|
%|B_v^T\!(2(2^n-1))|
\ge |T_n| 
&
\ge (1-c)\cdot g(2^n) 
\\ &
\ge (1-c)\cdot g(r/4).
\end{align*}
%
Here and in the following the final form of the bound is obtained by using $c\le 1/2$.

% For \itm2 observe first that $T_{n-1}$ has $\delta_1\cdots\delta_{n-1}$ apocentric vertices, each of which is a leaf. 
% Hence, when forming $T_n$ by attaching $\delta_n$ new copies of $T_{n-1}$ to these,\nlspace and assuming a maximally uniform distribution of the attachment among them, we find that none of the formerly apocentric vertices will attain a degree above $\lceil\Delta(n)\rceil+1$ (but some will in fact attain this degree).
% Thus, if $\lceil\Delta(n)\rceil+1$ is bounded, then this gives the maximum degree of $T$.

To prove \itm2 choose $n\in\NN$ with $2^{n-1}\le r\le 2^n$.
Let $x$ be the root of $\tau_n(v)$, and, if it exists,
%(if $x$ is not the global root)
let $w$ be the unique neighbor of $x$ outside of $\tau_n(v)$.
%the parent of $x$ (\ie\ the unique neighbor of $x$ that lies closer to the global root).
%be the apocentric vertex of the central copy of $T_n$ in $T_{n+1}(v)$ to which $x$ is adjacent.
Which other copies $\prec_n T$ are reachable from $v$ within $2^n$ steps? The following list is exhaustive:
%The following list contains all copies $\tau\prec_n T$ that might be reached from $v$ in at most $2^n$ steps (some of them might actually not be reachable, but we are not missing any):
%
\begin{itemize}
    \item $\tau_n(v)$ and $\tau_n(w)$, % itself,
    \item a copy $\tau \prec_n T$ adjacent to an apocentric vertex of $\tau_n(v)$ \resp\ $\tau_n(w)$.
    %There are less than $|T_n|$ apocentric vertices and each one is attached to at most $\bar\Delta-1$ further copies of $T_n$.
    %\item $\tau_n(w)$,
    %\item a copy $\tau\prec_n T$ adjacent to an apocentric vertex of $\tau_n(w)$.
\end{itemize}
%
Both $\tau_n(v)$ and $\tau_n(w)$ have not more than $|T_n|$ apocentric vertices, each of which~is adjacent to at most $\smash{\bar\Delta-1}$ copies $\tau\prec_n T$.
In conclusion, 
%Thus, including $\tau_n(v)$ and~$\tau_n(w)$, we count that 
at most $2\bar\Delta\cdot|T_n|$ copies of $T_n$ are reachable from $v$ in $2^n$ steps, containing a total of at most $2\bar\Delta\cdot |T_n|^2$ vertices.
We therefore find
%
% To prove the upper bound, choose $n\in\NN$ so that $2^{n-1} - 1\le r\le 2^n - 1$ and enumerate the copies of $T_n$ that can be reached from $v$ in at most $2^n-1$ steps.
% Note that the only way \enquote{out of $T_n(v)$} is either through one of its apocentric vertices, or through its root $x\in T_n(v)$:
% %
% \begin{itemize}
%     \item 
%     through an apocentric vertex: having reached an apocentric vertex of $T_n(v)$, up to $\bar\Delta-1$ roots of other copies of $T_n$ can be reached. From these, no~further copies can be reached, as the remaining $<2^n-1$ steps are insufficient to reach an apocentric vertex in the same copy. How many apocentric vertices of $T_n(v)$ can be reached from $v$ in $\le 2^n-1$ steps? This is hard to say; but at most $|T_n|$ many.
%     \item 
%     through the root $x$: having reached $x$ (and assuming that $x$~is not the global root), we can step into some \enquote{earlier} copy of $T_n$ via one of its apocentric vertices, say $w$. Starting in $w$ we can reach other apocentric vertices of $T_n(w)$, certainly less than $|T_n|$ many. As before, from each apocentric vertex of $T_n(w)$ we can reach up to $\Delta-1$ central vertices of other copies of $T_n$, from which no further copies can be reached. Like-wise, in the remaining $<2^n-1$ steps we cannot reach from $w$ to the central vertex of $T_n(w)$, and so we enumerated all reachable copies of $T_n$.
% \end{itemize}
% %
% To summarize, we can reach at most $2\bar\Delta\cdot|T_n|$ copies of $T_n$ (that is, $T_n(v)$, $T_n(w)$, and from each at most $(\bar\Delta-1)|T_n|$ other copies via apocentric vertices). In each of those we can reach at most $|T_n|$ vertices. This yields
%
\begin{align*}
%|B_v^T\!(r)| 
|\ball Tvr|
\le |\ball Tv{2^n}|
%|B_v^T\!(2^n)| 
\le 2\bar\Delta\cdot|T_n|^2 
&\le 2\bar\Delta\cdot(1+c)^2\cdot g(2^n)^2 
\\&\le 2\bar\Delta \cdot (1+c)^2 \cdot g(2r)^2.    
\end{align*}

One might suggest a much better estimation for the number of copies $\tau\prec_n T$ reachable through apocentric vertices of $\tau_n(v)$ \resp\ $\tau_n(w)$: namely $\delta_{n+1}$.
However, this is only true if $\tau_n(v)$ is a central copy in $\tau_{n+1}(v)$.
In general, $\tau_n(v)$ can as well be apocentric in $\tau_{n+1}(v)$, or can even be apocentric in $\tau_m(v)$ for some very large $m > n$.
If so, then the number of copies $\prec_n T$ reachable through apocentric vertices of $\tau_n(v)$ is more plausibly related to $\delta_{m+1}$ than $\delta_{n+1}$, which is the reason for the very crude estimation above. %We make this precise below.
With a more~careful analysis we can prove the second upper bound.

To show \itm3 let $m \ge n$ be maximal so that $\tau_n(v)$ is apocentric in $\tau_m(v)$.
Such an $m$ might not exist (\eg\ when defining $T$ from a completely apocentric inclusion chain), in which case the apocentric vertices of $\tau_n(v)$ are leaves in $T$ and no other copies $\prec_n T$ are reachable through them.
If $m$ exists however, then $\tau_m(v)$~is necessarily central in $\tau_{m+1}(v)$. 
In particular, the $\delta_1\cdots \delta_m$ apocentric vertices of $\tau_m(v)$ are adja\-cent to $\delta_{m+1}$ apocentric copies $\prec_{m} \tau_{m+1}(v)$.
By the maximally uniformly distribution of adjacencies we can estimate how many of these copies are reachable through the $\delta_1\cdots\delta_n$ apocentric vertices of $\tau_n(v)$.
Following \cref{rem:max_uniform} this number is at most
%
%
%is apocentric in $T_m(v)$ 
% Note~that such an $m$ exists and satisfies $m\ge n$. 
% Note further that $\tau_m(v)$ is then a central copy in $\tau_{m+1}(v)$: otherwise $\tau_n(v)$ and $\tau_{m+1}(v)$ share apocentric vertices, contradicting the choice of $m$.
% The $\delta_1\cdots \delta_m$ apocentric vertices of $\tau_m(v)$ are therefore adjacent to $\delta_{m+1}$ apocentric copies $\tau \prec_{m} \tau_{m+1}(v)$.
% Recall that these adjacencies are distributed maximally uniformly, so that we can estimate how many of them involve the $\delta_1\cdots\delta_n$ apocentric vertices of $\tau_n(v)\prec_n\tau_m(v)$.
% Following \cref{rem:max_uniform} this number is at most
%
%
%
% The careful reader may have realized that there is a much tighter (and somewhat obvious) estimation for the number of copies of $T_n$ attached to apocentric vertices of $T_n(a)$, namely, $\delta_{n+1}$.
% Unfortunately, this estimation does not necessarily apply to the number of copies of $T_n$ attached to $T_n(v)$.
%
%Recall now that $T_m(v)$ has $\delta_1\cdots\delta_m$ apocentric vertices and $T_n(v)$ has  $\delta_1\cdots\delta_n$ apocentric vertices. 
%Recall also that the adjacencies between the $\delta_1\cdots\delta_m$ apocentric vertices of $T_m(v)$ and the $\delta_{m+1}$ apocentric copies of $T_m$ in $T_{m+1}(v)$ distributed maximally uniformly among the apocentric vertices.
%There are then no more than 
%\msays{Why does such an $m$ exist?} \gsays{$m$ obviously exists, since everything is only a finite distance from $x^*$...} \msays{There are copies of $T_n$ that are not apocentric in any $T_m$.} \gsays{Oh, you don't mean that the set of m's may be unbounded, you mean that it may be empty. Yeah, that's fair. But doesn't the same upper bound apply then as well? In which case, we can simply distinguish cases.} \msays{I think I fixed it; we don't want a maximally large $T_m\subset T$ but a maximally large $T_m(v)$, such one always exists so that $T_n(v)$ is apocentric in it ($m=n$ works), and $m$ is, as you say, obviously bounded.}
%
\begin{align*}
\Big\lceil \frac{\delta_1\cdots\delta_n}{\delta_1\cdots\delta_m} \cdot \delta_{m+1}  \Big\rceil
&=
\Big\lceil \frac{\delta_{m+1}}{\delta_1\cdots\delta_m} \cdot \Big( \frac{\delta_{n+1}}{\delta_1\cdots\delta_n}\Big)^{-1} \cdot \delta_{n+1} \Big\rceil
\\&=\Big\lceil\frac{\Delta(m+1)}{\Delta(n+1)}\cdot\delta_{n+1}\Big\rceil
\le  \Gamma \cdot\delta_{n+1}.
\end{align*}
%
%copies of $T_n$ (inside of copies of $T_m$) adjacent to the apocentric vertices of $T_n(v)$.
This yields an improved upper bound on the number of copies $\tau\prec_n T$ adjacent to apo\-centric vertices of $\tau_n(v)$.
The same argument applies to $\tau_n(w)$.
Including $\tau_n(v)$ and $\tau_n(w)$ there are then at most $2\Gamma \cdot\delta_{n+1} + 2$ copies $\prec_n T$ reachable from $v$ in $2^n$ steps, and thus:
%
\begin{align*}
|\ball Tvr|
%|B_v^T\!(r)| 
\le |\ball Tv{2^n}|
%|B_v^T\!(2^n)| 
&\le (2\Gamma\cdot\delta_{n+1}+2)|T_n|
%\\ &\le 2\Gamma\cdot\delta_{n+1}\cdot|T_n| + 2|T_n|
\\ &\le 2\big(\Gamma\cdot (\delta_{n+1}+1)|T_n| - (\Gamma-1)\cdot|T_n|\big)
\\ &\le 2\big(\Gamma\cdot |T_{n+1}| - (\Gamma-1)\cdot|T_n|\big)
\\ &\le 2(c+1)\cdot\big(\Gamma\cdot g(2^{n+1}) - (\Gamma-1)\cdot g(2^n)\big).
\\ &\le 2(c+1)\cdot\big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big).
\end{align*}
%
%This establishes the improved upper bound.
\end{proof}

%One might wonder for which $g$ the technical condition $\Gamma<\infty$ in \cref{thm:main}~is satisfied.
%For the remainder of this section we make an effort to derive various~sufficient conditions.

It appears non-trivial to actually provide a target growth rate $g$ for which $\Gamma$~diverges, and so it seems we can feel confident that \cref{thm:main} applies quite generally.
Yet, for the remainder of this section we discuss criteria that are sufficient to imply  $\Gamma<\infty$.

\begin{proposition}\label{res:conditions_in_d}
$\Gamma<\infty$ holds in any of the following cases:
%
\begin{myenumerate}
    \item
    $\delta_{n+1}\le \delta_n^2$ eventually.
    % \item
    % $\delta_{n+1}\ge \delta_n^2$ and $\delta_{n+1}\le C\delta_n^2$ for some $C>1$ eventually.
    \item 
    the sequence of $\delta_n$ is bounded.
\end{myenumerate}
%
\begin{proof}
Note that $\Delta(n+1)=\delta_{n+1}/\delta_n^2 \cdot\Delta(n)$.
Assuming \itm1, $\Delta(n)$ will eventually~be non-increasing and so either $\Gamma\le1$ or the value $\Gamma$ is attained only on a finite initial segment, thus, is finite.

For part \itm2 observe $\Delta(m)/\Delta(n)=\delta_m / (\delta_n^2\cdot\delta_{n+1}\cdots\delta_{m-1})\le \displaystyle\smash{\max_i \delta_i}$.
\end{proof}
\end{proposition}

Condition \itm2 of \cref{res:conditions_in_d} holds, for example, when $g$ is a polynomial as discussed in \cref{ex:polynomial}.
%Note that this is not quite the same as being of polynomial growth $g(r)\in\theta(r^\alpha)$, which is not sufficient.

% Part \itm1 of \cref{res:conditions_in_d} holds for all $g$ that are not growing to fast.
% Part \itm2 includes in particular all $g$ of polynomial growth (\cf\ \cref{ex:lattice_tight_upper_bound}.

% One natural condition that \emph{almost} makes the preconditions of \itm2 and \itm3~satisfied is requiring $g$ to be \emph{log-concave}.
% The relevant instance of this is
% %
% $$
% \tfrac13 \log g(2r) + \tfrac23 \log g(r/2) \le \log 
% g(r)
% %g\big(\overbrace{\tfrac13 (2r) + \tfrac23 (r/2)}^{=\, r}\big).
% $$
% %
% (note that indeed $\frac13(2r)+\frac23(r/2)=r$).
% Unfortunately, this is not quite sufficient, and we instead need an $\eps>1$ for which the following stronger equation holds
% %
% $$
% \tfrac13 \log g(2r) + \tfrac23 \log g(r/2) \le \eps \log 
% g(r),
% $$
% %
% at least eventually.

% \begin{proposition}
% If for some $\eps>1$ holds
% %
% $$
% \tfrac13 \log g(2r) + \tfrac23 \log g(r/2) \le \eps \log 
% $$
% %
% eventually (\ie\ for all sufficiently large $r\ge1$), then the conditions of \itm2 and \itm3 in \cref{thm:main} are satisfied.
% %
% \begin{proof}
% \TODO
% \end{proof}
% \end{proposition}

% In general, $g$ being log-concave is already a pretty good indicator that the bounds of \cref{thm:main} apply. Constructing counterexamples in a reasonable growth range is possible but needs some work.

% \begin{example}
% \TODO
% \end{example}

It remains to provide a criterion for $\Gamma<\infty$ in terms of $g$.
Below we show that~$g$ being \emph{log-concave} is sufficient, where log-concave means
%
$$\alpha\log g(x) + \beta \log g(y) \le \log g(\alpha x + \beta y)$$
%
for all $\alpha,\beta\in[0,1]$ with $\alpha+\beta=1$.
Intuitively, being log-concave works because~it prevents both super-exponential growth and strong oscillations in the growth rate. 

\begin{theorem}\label{res:conditions_in_g}
If $g$ is log-concave, then $\Gamma<\infty$.
%
\begin{proof}
%The presented proof consists of a rather intuitive, and a more technical~part.
We start from a well-chosen instance of log-concavity:
%
$$\alpha=1/3,\quad \beta=2/3, \quad x=2^{n+1},\quad y=2^{n-1}.$$
%
One can verify $\alpha x+\beta y = 2^n$.
Since $g$ is log-concave, we have
%
$$\tfrac13\log g(2^{n+1}) + \tfrac23 \log g(2^{n-1}) \le \log g(2^n).$$
%
This further rearranges to
%
$$\log g(2^{n+1}) + 2\log g(2^{n-1}) \le 3\log g(2^n) \;\implies\; \frac{g(2^{n+1})}{g(2^n)} \le \Big(\frac{g(2^n)}{g(2^{n-1})}\Big)^2\!.$$
%
Recall that roughly $\delta_n\approx g(2^n)/g(2^{n-1})$, and so the right-most inequality resembles $\delta_{n+1}\le \delta_n^2$.
If this were exact then $\Gamma<\infty$ would already follow from \cref{res:conditions_in_d} \itm1.
%
However, the actual definition of $\delta_n$ from the proof of \cref{res:d_i} only yields
%The reality however is less nice: from the actual definition of the $\delta_n$
%\cref{res:d_i}
%follows %, and using the actual definition of $\delta_n$ from \cref{res:d_i} yields:
%
\begin{equation}\label{eq:d_d_2}
\delta_{n+1}
\le \Big\lfloor\frac{g(2^{n+1})}{g(2^n)}\Big\rfloor
\le \frac{g(2^{n+1})}{g(2^n)}
\le \Big(\frac{g(2^n)}{g(2^{n-1})}\Big)^2
\le \Big\lceil\frac{g(2^n)}{g(2^{n-1})}\Big\rceil^2
\le (\delta_n+2)^2.
\end{equation}
%
% which we can rearrange to
% %
% \begin{equation}\label{eq:nu}
% \nu(n)
% :=\frac{\delta_{n+1}}{\delta_n^2}
% \le \Big(1+\frac2{\delta_n}\Big)^2
% %\le 1+\frac4{\delta_n}+\frac4{\delta_n^2}
% . %\le 1 + \frac{2}{\delta_n-2}.
% \end{equation}
% %
% Recall that $\Delta(n+1)=\nu(n)\Delta(n)$.
% By \eqref{eq:nu} it is possible that $\Delta$ is increasing and so we can not put a bound on $\Delta(m)/\Delta(n)$ right away.

This turns out to be sufficient for proving $\Gamma<\infty$, though the argument becomes more technical.
Define $\gamma\:\NN\to\RR$ with
%
$$
\gamma(1):=25,\qquad \gamma(\delta):=\prod_{k=0}^{\infty} %\Big(1+\frac4{\delta^{2^k}}+\frac4{\delta^{2^{k+1}}}\Big)
\Big(1+\frac2{\delta^{2^k}}\Big)^{\!2}\!
,\;\;\,\text{whenever $\delta\ge 2$.}
$$
%
To keep this proof focused, most technicalities surrounding this function have been moved to \cref{sec:gamma_properties}.
This includes a proof of convergence of the infinite product (\cref{res:estimate_gamma}) as well as a proof of the following crucial property $(*)$ of $\gamma$: for~any two integers $\delta_1,\delta_2\ge 1$ with $\delta_1\le(\delta_2+2)^2$ holds $\delta_1\gamma(\delta_1)\le\delta_2^2\gamma(\delta_2)$ (\cref{res:gamma_property_d_d2}).

Lastly, we define $\pot(n):=\gamma(\delta_n)\Delta(n)$, intended to represent the \emph{potential} for $\Delta$ to increase, as we shall see that it is an upper bound on $\Delta(m)$ for \emph{all} $m\ge n$.
This follows from two observations.
First, $\Delta(m)< \pot(m)$ since $\gamma(\delta)>1$. Second, $\pot(n)$ is decreasing in $n$: since $\delta_{n+1}\le(\delta_n+2)^2$ by \eqref{eq:d_d_2}, we can apply property $(*)$ to find
%
$$\pot(n+1) = \gamma(\delta_{n+1})\Delta(n+1) = \gamma(\delta_{n+1})\frac{\delta_{n+1}}{\delta_n^2}\Delta(n) \overset{\smash{(*)}}\le \gamma(\delta_n)\Delta(n)=\pot(n).$$
%
To summarize, for all $m\ge n$ holds
%
\begin{equation*}\label{eq:goal}
\Delta(m)<\pot(m)
%\overset{\mathclap{(*)}}
\le\pot(n)=\Delta(n)\gamma(\delta_n) \,\implies\, \frac{\Delta(m)}{\Delta(n)}\le\gamma(\delta_n)\le 25,
\end{equation*}
%
where we used that $\gamma(\delta)$ is decreasing in $\delta$ (\cref{res:gamma_decreasing}) and so attains its maximum at $\gamma(1)=25$. This proves $\Gamma\le25$.
\end{proof}
\end{theorem}

Combining \cref{thm:main} and \cref{res:conditions_in_g} yields \cref{main}, achieving the main purpose of this section.



\iftrue % remark for non-central inclusion chains

%\begin{remark}\label{rem:general_limit_growth}
%Let $T'$ be the limit tree obtained from a different inclusion chain compared to \cref{constr:T} (\eg\ always identifying $T_{n-1}$ with an apocentric copy in $T_n$). 
%For each $v\in V(T')$ and $r\ge 0$ the ball~$\ball {T'}vr$ appears as a subgraph of $T$. Additionally, $\ball {T'}vr$ contains a subtree isomorphic to a ball of radius $r/2$ in $T$. \msays{how so?}
%Therefore, using the growth estimations for $T$ proven in \cref{thm:main}, we see that $T'$ has uniform volume growth $g$ as well. In particular, for any arbitrary tree $T'$ obtained from our construction with appropriate identifications, we have
%\[\tfrac12 g(r/8)\leq \ball {T'}vr\leq 3\max\{1,\Gamma\}\cdot g(4r).\]
%\[\tfrac12 g(r/8)\leq \ball {T'}vr\leq 3\Gamma\cdot g(4r).\]

%Finally, note that every ball of radius $\leq 2^n-1$ in $T_n$ is isomorphic to a ball of such a limit tree $T'$, and therefore admits the same bounds. This observation will be of use in the next section.
%\msays{Not entirely true, \eg\ if $T'$ is completely apocentric and $v$ is completely apocentric the ball cannot necessarily be found in $T$.} \gsays{Of course it can, it just won't be a ball.}
%\end{remark}

% \sepline

% This infinite product converges, and the function $\gamma$ has the following essential properties (see \cref{sec:gamma_properties} for proofs of these facts):
% %
% \begin{myenumerate}
%     \item $\gamma(\delta)$ is decreasing in $\delta$, \ie\ if $\delta_1 < \delta_2$ then $\gamma(\delta_1) > \gamma(\delta_2)$. This is clear from the definition if $\delta_1,\delta_2\ge 2$, but it requires estimating $\gamma(2)$ when $\delta_1=1$ (see \cref{res:gamma_bounds}).
%     \item if $\delta_1\le \delta_2$ then $\delta_1\gamma(\delta_1)\le\delta_2^2\gamma(\delta_2)$ (see \cref{res:gamma_property_d_d2}).
% \end{myenumerate}

% The second function is the \emph{potential} $\pot(n):=\gamma(\delta_n)\Delta(n)$.
% Intuitively, it measures how much $\Delta$ can still increase for $m\ge n$, or formally, it is an upper bound on $\Delta(m)$ for any $m\ge n$; a fact that we are going to prove.
% This suffices to prove $\Gamma<\infty$:
% %
% \begin{equation}\label{eq:goal}
% \Delta(m)<\pot(m)
% %\overset{\mathclap{(*)}}
% \le\pot(n)=\Delta(n)\gamma(\delta_n) \,\implies\, \frac{\Delta(m)}{\Delta(n)}\le\gamma(\delta_n)\le 25,
% \end{equation}
% %
% hence $\Gamma\le 25$.
% In the remaining proof we show that $\pot(n)$ is non-increasing.

% Fix a pair $m > n$ for which we aim to show $\Delta(m)/\Delta(n)\le 25$ (the case $m=n$ being trivial). 
% We can assume that $n$ is a local minimum, \ie\ $\Delta(n) < \Delta(n+1)$, and that $m$ is a local maximum, \ie\ $\Delta(m) > \Delta(m-1)$; as otherwise we can move $n$ and $m$ closer together, making the quotient $\Delta(m)/\Delta(n)$ at most bigger.
% %W.l.o.g.\ assume $\Delta(n)<\Delta(n+1)$ and $\Delta(m)>\Delta(m-1)$, as otherwise the pair $m-1\ge n$ or $m\ge n+1$ yields an even bigger quotient.

% Let then $[n_1,m_1],...,[n_s,m_s]\subset[n,m]$ be an enumeration of maximal intervals on which $\Delta$ is strictly increasing, where the indexing is chosen to satisfy $n=n_1<m_1<n_2<m_2<\cdots<n_s<m_s=m$ (see \cref{fig:Delta_n}). 
% %In particular, $\Delta(n_i)<\Delta(n_i+1)$ for all $i\in\{1,...,s\}$. 
% %\msays{Why do we emphasize this?} \gsays{So that the reader understands where the decreasing interval ends and the increasing interval begins when we have many consecutive numbers with the same $\Delta$}
% %
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.65\textwidth]{img/Delta_n_2.pdf}
%     \caption{Visualization of $\Delta(n)$ and the parition of $[n,m]$ into increasing and non-increasing intervals.}
%     \label{fig:Delta_n}
% \end{figure}

% Our plan is to show $\pot(m)\le \pot(n)$ and to invoke the reasoning of \eqref{eq:goal}.
% More precisely, we show $\pot(n_1)\ge \pot(n_2)\ge \cdots\ge\pot(n_s)\ge\pot(m_s)$.
% This is achieved in two separate steps: showing $\pot(n_i)\ge\pot(n_{i+1})$ and $\pot(n_i)\ge \pot(m_i)$.

% \emph{Step 1}: we show $\pot(n_i)\ge \pot(m_i)$.
% By the definition of the intervals, for any $k\in[n_i,m_i-1]$ holds $\Delta(k)<\Delta(k+1)=\nu(k)\Delta(k)\implies\nu(k)>1\implies\delta_{k+1}>\delta_k^2\implies\gamma(\delta_{k+1})<\gamma(\delta_k^2)$, and therefore
% %
% \begin{align*}
% \pot(k+1)
% &=\Delta(k+1) \gamma(\delta_{k+1})
% <\Delta(k+1) \gamma(\delta_k^2)
% =\Delta(k) \nu(k)\cdot \gamma(\delta_k^2)
% \\&\le \Delta(k) \cdot \Big(1+\frac2{\delta_k}\Big)^2  \cdot  \prod_{k = 0}^\infty \Big(1+\frac2{(\delta_k^2)^{2^k}}\Big)^2  
% = \Delta(k) \cdot \prod_{k = 0}^\infty \Big(1+\frac2{\delta_k^{2^k}}\Big)^2  
% \\&= \Delta(k) \gamma(\delta_k) = \pot(k).
% \end{align*}
% %
% We conclude that $\pot(\free)$ is increasing on $[n_i,m_i]$, from which the claim of step 1 follows.
% Note also $\Delta(m_i)\le \pot(m_i)\le\pot(n_i)$.

% Next we show that $\pot(\free)$ is non-increasing on the intervals $[m_i,n_{i+1}]$. 
% As before, we pick a $k\in[m_i,n_{i+1}-1]$ and show $\pot(k+1)\le\pot(k)$. 
% Note that $\Delta(k+1)\le\Delta(k)$. 
% If $\delta_{k+1}\ge\delta_k$ then immediately follows
% %
% \begin{align*}
% \pot(k+1) 
% &= \Delta(k+1)\gamma(\delta_{k+1})
% \le \Delta(k)\gamma(\delta_k)
% =\pot(k).
% \end{align*}
% %
% If however $\delta_{k+1}<\delta_k$, then we proceed via
% %
% $$\pot(k+1)=\Delta(k+1)\gamma(\delta_{k+1}) = \nu(k)\Delta(k)\gamma(\delta_{k+1}) \overset{\smash{(*)}}\le \Delta(k)\gamma(\delta_k)=\pot(k),$$
% %
% where in $(*)$ we used $\delta_{k+1}\gamma(\delta_{k+1})\le\delta_k^2\gamma(\delta_k)$ (property \itm3 of $\gamma$, \cf\ \cref{res:estimate_gamma}).





% If however $\delta_{k+1}<\delta_k$, then we have to distinguish several cases:
% %
% \begin{enumerate}[label=(\arabic*),topsep=1em,itemsep=1em]
%     \item if $\delta_k\ge5$, then we show
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1})
%     = \nu(k) \Delta(k) \gamma(\delta_{k+1}) \overset{\smash{(*)}}\le \Delta(k)\le\pot(k).
%     \end{align*}
%     %
%     where in $(*)$ we use $\nu(k)\gamma(\delta_{k+1})\le \gamma(\delta_k)$.
    
%     \item if $\delta_{k+1}<\delta_k\le 4$, we are left with the finitely many cases
%     %
%     $$(\delta_{k+1},\delta_k)\in\{\;(2,1),(3,1),(3,2),(4,1),(4,2),(4,3) \;\}$$
%     %
%     and one can verify (see \cref{res:estimate_gamma} for the approximate value of $\gamma(\delta)$ for small $\delta$) that $\nu(k)\gamma(\delta_{k+1})\le\gamma(\delta_k)$ for all of them.
%     It follows
%     %
%     $$\pot(k+1)=\gamma(\delta_{k+1})\Delta(k+1) = \gamma(\delta_{k+1})\nu(k)\Delta(k) \le \gamma(\delta_k)\Delta(k)=\pot(k).$$
% \end{enumerate}
% \hrulefill
% %
% \begin{enumerate}[label=(\arabic*),topsep=1em,itemsep=1em]
%     \item 
%     if $\delta_{k}\geq 5$ and $\delta_{k+1}\geq 3$, then \mbox{$\Delta(k+1)/\Delta(k)\le \delta_{k+1}/\delta_{k}^2< \frac{1}{5}$} and it follows 
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1}) <  \tfrac15 \Delta(k)\gamma(\delta_{k+1}) 
%     %\\&
%     \overset{\smash{(*)}}< \Delta(k)\le\pot(k),
%     \end{align*}
%     %
%     where in $(*)$ we used $\gamma(\delta_{k+1})\le\gamma(3)<4$.
    
%     \item if $\delta_{k}\geq 5$ and $\delta_{k+1}=2$, then \mbox{$\Delta(k+1)/\Delta(k)\le\delta_{k+1}/\delta_{k}^2 \le \frac{2}{25}$} and it follows
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1}) \le  \tfrac2{25} \Delta(k)\gamma(2) 
%     %\\& 
%     \overset{\smash{(**)}}< \Delta(k)\le\pot(k),
%     \end{align*}
%     %
%     where in $(**)$ we used $\gamma(2)<12.5$.
    
%     \item if $\delta_{k}\geq 5$ and $\delta_{k+1}=1$, then analogously \mbox{$\Delta(k+1)/\Delta(k) \le \frac{1}{25}$} and 
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1}) \le  \tfrac1{25} \Delta(k)\gamma(1) 
%     %\\& 
%     \overset{\smash{(***)}}= \Delta(k)\le\pot(k),
%     \end{align*}
%     %
%     where in $(*\!*\!*)$ we used $\gamma(1)=25$.
    
%   % \TODO
    
%     \item it remains $\delta_{m_i}\le 4$. 
%     Recall $\delta_k^2 < \delta_{k+1}$ for all $k\in[n_i,m_i-1]$.
%     \mbox{In particular}, $\delta_{m_i-1}^2<\delta_{m_i}\le 4$ and therefore $\delta_{m_i-1}=1$.
%     It furthermore follows~$(\x)\;\nu(m_i-1)$ $=$ $\delta_{m_i}/\delta_{m_i-1}^2 = \delta_{m_i}$.
%     Moreover, $n_i=m_i-1$, because if $n_i<m_i-1$ then $1\le \delta_{n_i}^2<\delta_{m_i-1}=1$.
%     Taken together we obtain
%     %
%     \begin{align*}
%     \Delta(n_{i+1}) 
%       &= \nu(m_i+1)\cdots\nu(n_{i+1}) \cdot \Delta(m_i)
%       =\frac{\delta_{n_i+1}}{\delta_{m_i}} \cdots \frac{1}{\delta_{m_i}\cdots\delta_{n_{i+1}-1}}\cdot \Delta(m_i)
%     \\&\le \frac{\Delta(m_i)}{\delta_{m_i}}
%       = \frac{\nu(m_i-1)\Delta(m_i-1)}{\delta_{m_i}} 
%       %= \frac{\Delta(n_i)}{\delta_{m_i-1}^2} 
%       \overset{(\x\x)}= \Delta(m_i-1) \overset{(\x)}=\Delta(n_i).
%     \end{align*}
%     %
%     %From this and $\delta_{n_i}=1\le\delta_{n_i+1}$ follows
%     From this and $\gamma(\delta_{n_{i+1}})\le \gamma(1) = \gamma(\delta_{n_i})$ follows
%     %
%     $$\pot(n_{i+1})=\gamma(\delta_{n_{i+1}}) \Delta(n_{i+1}) \le \gamma(\delta_{n_i})\Delta(n_i) \le \pot(n_i).$$
    
% \end{enumerate}
% %
% This concludes the proof.


% \hrulefill

% \emph{Step 2}: we show $\pot(n_{i+1})\le\pot(n_i)$ via case analysis.
% Note that~$\Delta$ is non-increasing on $[m_i,n_{i+1}]$, in particular, $\Delta(n_{i+1})\le \Delta(m_i)$.
% %
% \begin{enumerate}[label=(\arabic*)]
%     \item if $\delta_{m_i}\le\delta_{n_{i+1}}$ then
%     %
%     \begin{align*}
%     \pot(n_{i+1}) 
%     &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}})
%     < \Delta(m_i)\gamma(\delta_{m_i})
%     \\&=\pot(m_i)\le\pot(n_i).
%     \end{align*}
    
%     \item otherwise $\delta_{m_i}>\delta_{n_{i+1}}$and we distinguish the following sub-cases:
%     % In the following we repeatedly use
%     % %
%     % $$m\ge n \implies \frac{\Delta(m)}{\Delta(n)} = \frac{\delta_{m}/\delta_n}{\delta_n\cdots\delta_{m-1}}.$$
%     % %
%     % for various estimations of the quotient.
    
%     \vspace{1ex}
%     \begin{enumerate}[label=(\alph*)]
%         \item 
%         if $\delta_{m_i}\geq 5$ and $\delta_{n_{i+1}}\geq 3$, then \mbox{$\Delta(n_{i+1})/\Delta(m_i)\le \delta_{n_{i+1}}/\delta_{m_i}^2< \frac{1}{5}$} and 
%         %
%         \begin{align*}
%         \pot(n_{i+1}) &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}}) <  \tfrac15 \Delta(m_i)\gamma(\delta_{n_{i+1}}) \\
%         & \overset{\smash{\mathclap{(*)}}}< \Delta(m_i)\le\pot(n_i),
%         \end{align*}
%         %
%         where in $(*)$ we used $\gamma(\delta_{n_{i+1}})\le\gamma(3)<4$.
        
%         \item if $\delta_{m_i}\geq 5$ and $\delta_{n_{i+1}}=2$, then \mbox{$\Delta(n_{i+1})/\Delta(m_i)\le\delta_{n_{i+1}}/\delta_{m_i}^2 \le \frac{2}{25}$} and 
%         %
%         \begin{align*}
%         \pot(n_{i+1}) &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}}) \le  \tfrac2{25} \Delta(m_i)\gamma(2) \\
%         & \overset{\smash{\mathclap{(**)}}}< \Delta(m_i)\le\pot(n_i),
%         \end{align*}
%         %
%         where in $(**)$ we used $\gamma(2)<12.5$.
        
%         \item if $\delta_{m_i}\geq 5$ and $\delta_{n_{i+1}}=1$, then analogously \mbox{$\Delta(n_{i+1})/\Delta(m_i) \le \frac{1}{25}$} and 
%         %
%         \begin{align*}
%         \pot(n_{i+1}) &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}}) \le  \tfrac1{25} \Delta(m_i)\gamma(1) \\
%         & \overset{\smash{\mathclap{(***)}}}= \Delta(m_i)\le\pot(n_i),
%         \end{align*}
%         %
%         where in $(*\!*\!*)$ we used $\gamma(1)=25$.
        
%       % \TODO
        
%         \item it remains to discuss $\delta_{m_i}\le 4$. 
%         Recall from step 1 that $\delta_k^2 < \delta_{k+1}$ for all $k\in[n_i,m_i-1]$.
%         So we can conclude $\delta_{m_i-1}^2<\delta_{m_i}\le 4\implies \delta_{m_i-1}=1$.
%         Moreover, $n_i<m_i-1$ yields the contradiction $1\le \delta_{n_i}^2<\delta_{m_i-1}=1$, thus $n_i = m_i-1$.
%         Note that $\nu(m_i-1) = \delta_{m_i}/\delta_{m_i-1}^2 = \delta_{m_i}$. Then
%         %
%         \begin{align*}
%         \Delta(n_{i+1}) 
%           &= \nu(n_{i+1}-1)\cdots\nu(m_i) \cdot \Delta(m_i)
%         \\&=\frac{\delta_{n_i+1}}{\delta_{m_i}} \cdots \frac{1}{\delta_{m_i}\cdots\delta_{n_{i+1}-1}}\cdot \Delta(m_i)
%         \\&\le \frac{\Delta(m_i)}{\delta_{m_i}}
%           = \frac{\nu(m_i-1)\Delta(m_i-1)}{\delta_{m_i}} 
%           %= \frac{\Delta(n_i)}{\delta_{m_i-1}^2} 
%           = \Delta(n_i).
%         \end{align*}
%         %
%         and finally
%         %
%         $$\pot(n_{i+1})=\gamma(\delta_{n_{i+1}}) \Delta(n_{i+1}) \le \gamma(\delta_{n_i})\Delta(n_i) \le \pot(n_i).$$
        
%     \end{enumerate}
% \end{enumerate}
% %
% This finishes the proof.




% \sepline

% If $\delta_{n+1} \ge \delta_n^2$ then
% %
% $$\delta_{n+1}\gamma(\delta_{n+1}) \le \delta_{n+1}\gamma(\delta_n^2) = \frac{\delta_{n+1}}{\delta_n^2} \delta_n^2 \gamma(\delta_n^2) \le \Big(1+\frac2{\delta_n}\Big)^2 \delta_n^2 \gamma(\delta_n^2) = \delta_n^2 \gamma(\delta_n).$$

% If $\delta_n\le\delta_{n+1}\le\delta_n^2$ then
% %
% $$\delta_{n+1}\gamma(\delta_{n+1}) \le \delta_n^2 \gamma(\delta_n).$$

% If $\delta_{n+1}\le\delta_n$ then by \cref{res:gamma_property_d_d2}
% %
% $$\delta_{n+1}\gamma(\delta_{n+1})\le\delta_n^2\gamma(\delta_n).$$

% \begin{lemma}
% If $a\le (b+2)^2$, then $a\gamma(a)\le b^2\gamma(b)$.
% \end{lemma}

% $$\gamma(\delta_{n+1})\Delta(n+1) = \frac{\delta_{n+1}\gamma(\delta_{n+1})}{\delta_n^2}\Delta(n) \le \gamma(\delta_n)\Delta(n).$$





\iffalse

\newpage

\msays{I believe we have a working proof of \cref{res:conditions_in_g} now, but it is quite a bit different than anticipated. I was able to shorten the proof significantly by outsourcing the case analysis to a discussion of properties of $\gamma$ in the Appendix (I like to have it in an Appendix because these technicalities distract from our main message). The key insight was that the previous case analysis came down to repeatedly using one special property of $\gamma$. It is even a bit stronger now, as it proves that $\pot(\free)$ is always decreasing, not only on the $\Delta$-increasing segments}

\msays{For cleanup, I removed (that is, made into a comment) most of the previous proof attempts, but I left what you wrote in case we need to rewind. }

We aim to show that $\frac{\Delta(m)}{\Delta(n)}$, $m\geq n$ is bounded. It is sufficient to prove this if $\Delta$ assumes a local minimum in $n$ (we may also assume that $\Delta(n)<\Delta(n+1)$, without loss of generality). To achieve this, we will prove that $pot(n')<pot(n)$ for every $n'>n$ at which $\Delta$ assumes a local minimum, where $pot(i):=\Delta(i)\gamma(\delta_i)$ if $\delta_i\geq 2$ and $pot(i):=24.66\Delta(i)$ otherwise. From this the desired result immediately follows. Indeed, observe that $[n,m]$ is partitioned in $\Delta$-monotone intervals $[n_0:=n,m_0]$, $[m_0,n_1]$, $[n_1,m_1]$,...$[n_l,m_l:=m]$. Then $\Delta(m)\leq pot(n_l)\leq pot(n)<24.66\Delta(n)$.

The proof will be by induction over the number of maximal monotone intervals partitioning $[n,n']$. The inductive basis is trivial.

For the inductive step, let $[n_j,m_j]$, $[m_j,n']$ be the last two maximal $\Delta$-monotone intervals of $[n,n']$, the former increasing and the latter decreasing, and suppose that we know that $pot(n_j)\leq pot(n)$. We shall show that $pot(n')\leq pot(n)$. 

We distinguish cases:

\begin{enumerate}
    \item If $\delta_{m_j}\leq ...\leq \delta_{n'}$, then we have $\gamma(\delta_{n'})\leq \gamma(\delta_{m_j})\Rightarrow pot(n')<pot(m_j)\leq pot(n_j)\leq pot(n)$.
    \item If there exists some index $i$ in $[m_j+1,n']$ with $\delta_i<\delta_{i-1}$, then:
    \begin{enumerate}
        \item If $\delta_{m_j}\geq 5$ and $\delta_{n'}\geq 3$, we observe that $\frac{\Delta(n')}{\Delta(m_j)}\leq \frac{1}{5}$. Therefore, \[pot(n')\leq \frac{\Delta(m_j)}{5}\gamma(\delta_{n'})<\Delta(m_j)\leq pot(n_j)\leq pot(n).\]
        \item If $\delta_{m_j}\geq 5$ and $\delta_{n'}=2$, we observe that $\frac{\Delta(n')}{\Delta(m_j)}\leq \frac{2}{25}$. Therefore, \[pot(n')\leq \frac{2\Delta(m_j)}{25}\gamma(2)<\Delta(m_j)\leq pot(n_j)\leq pot(n).\] 
        \item If $\delta_{m_j}\geq 5$ and $\delta_{n'}=1$, we observe that $\frac{\Delta(n')}{\Delta(m_j)}\leq \frac{1}{25}$. Therefore, \[pot(n')<\Delta(m_j)\leq pot(n_j)\leq pot(n).\] 
        \item If $\delta_{m_j}<5$, then $\delta_{n_j}=1$ and 
        \begin{enumerate}
            \item either $n_j=m_j-1$ and $\delta_{m_j}\in\{2,3,4\}$, in which case $\Delta(m_j)=\delta_{m_j}\Delta(n_j)$ and $\Delta(n')\leq \frac{\Delta(m_j)}{\delta_{m_j}}=\Delta(n_j)$;
            \item or $n_j=m_j-2$, $\delta_{m_j-1}=2$ and $\delta_{m_j}=4$, in which case $\Delta(m_j)=2\Delta(n_j)$ and $\Delta(n')\leq \frac{\Delta(m_j)}{\delta_{m_j}}=\frac{\Delta(n_j)}{2}$.
        \end{enumerate}
        In either case $\Delta(n')\leq \Delta(n_j)$, so \[pot(n')\leq pot(n_j)\leq pot(n).\]
    \end{enumerate}
\end{enumerate}

The proof is complete.




\noindent\hrulefill

To put an upper bound on $\Delta(m)/\Delta(n)$ note that it suffices to consider $m,n\in\NN$ so that for all $k\in[n,m]$ holds $\Delta(n)<\Delta(k)<\Delta(m)$, as otherwise the quotient can be further increased.
For such $m$ and $n$ we are going to prove $\Delta(m)/\Delta(n)\le \gamma(\delta_n)$, where
%
$$
\gamma(\delta):=\prod_{k=0}^{\infty} %\Big(1+\frac4{\delta^{2^k}}+\frac4{\delta^{2^{k+1}}}\Big)
\Big(1+\frac2{\delta^{2^k}}\Big)^2
,\quad\text{if $\delta\ge 2$, \quad and $\gamma(1):=24$.}
$$
%
%and $\gamma(1) := 24$ otherwise.
This will be sufficient as the infinite product converges whenever $\delta\ge 2$ (see Appendix A), and in fact, $\gamma(\delta)\le 100$ for all $\delta$. Note also that~$\gamma$ is decreasing in its argument.

Proving this upper bound will proceed differently depending on whether we consider a decreasing or increasing segment of $\Delta$.
For that reason let $[n_1,m_1],...,[n_s,m_s]$ $\subseteq[n,m]$ be an enumeration of the maximal intervals on which $\Delta$ is non-decreasing.
Then $n=n_1<m_1<n_2<\cdots<n_s<m_s=m$.
We then are going to show that $\Delta(m_i)/\Delta(n)\ge\gamma(\delta_n)$ for all $i\in\{1,...,s\}$ by induction on $i$. 

In the next step we prove $\Delta(m_i)/\Delta(n_i)\ge\gamma(\delta_{n_i})$ which contains the induction base as the special case for $i=1$.
Since $\Delta$ is non-decreasing on $[n_i,m_i]$, we have $\delta_{n_i+k+1}\ge\delta_{n_i+k}^2$ for all $k\in\{0,...,m_i-n_i-1\}$, which expands to $\delta_{n_i+k}\ge \smash{\delta_{n_i}^{2^k}}$.
For $\delta_{n_i}\ge 2$ follows
%
\begin{align*}
\frac{\Delta(m_i)}{\Delta(n_i)}
\;&=\; \prod_{k=0}^{\mathclap{m_i-n_i-1}} \nu(n_i+k) 
\;\le\; \prod_{k=0}^{\mathclap{m_i-n_i-1}}\; \Big(1+\frac2{\delta_{n_i+k}}+\frac4{\delta_{n_i+k}^2}\Big)
\\\;&\le\; \prod_{k=0}^{\mathclap{m_i-n_i-1}}\; \Big(1+\frac2{\delta_{n_i}^{2^k}}+\frac4{\delta_{n_i}^{2^{k+1}}}\Big)
< \gamma(\delta_{n_i}).
\end{align*}
%
If $\delta_{n_i}=1$, by \eqref{eq:nu} holds $\delta_{n_i+1}\le 7$.

\fi

% $$
% \Delta(m_{i+1})\gamma(\delta_{m_{i+1}}) 
% \,\overset{\mathclap{(*)}}\le\, \Delta(n_{i+1})\gamma(\delta_{n_{i+1}})
% \,\overset{\mathclap{(**)}}\le\, \Delta(m_i)\gamma(\delta_{m_i})
% \,\overset{\mathclap{(***)}}\le\, \Delta(n)\gamma(\delta_{n})
% $$

% \newpage

% Define the \emph{potential} $\pot(k):=\Delta(k)\gamma(\delta_k)$ at index $k$.
% We are going to show
% %
% \begin{equation}
%     \tag{$*$} \pot(n_1)\ge\pot(m_1)\ge\pot(n_2)\ge\cdots\ge\pot(n_s)\ge\pot(m_s).
% \end{equation}
% %
% This would suffice to conclude the proof as $\Delta(m)\le \pot(m)\le\pot(n)=\Delta(n)\gamma(n)\le 36\Delta(n)$.
% The chain $(*)$ is composed of two types of inequalities: $\pot(n_i)\ge\pot(m_i)$ and $\pot(m_i)\ge\pot(n_{i+1})$.

% For the first inequality, recall that $\Delta$ is non-decreasing on $[n_i,m_i]$, and so $\delta_{k+1}\ge\delta_k^2$ for all $k\in[n_i,m_i-1]$. The first inequality then follows from
% %
% \begin{align*}
% \pot(k+1)
% &=\Delta(k+1) \cdot \gamma(\delta_{k+1})
% \le\Delta(k+1) \cdot \gamma(\delta_k^2)
% \\&=\Delta(k) \cdot \nu(k+1)\cdot \gamma(\delta_k^2)
% \\&\le \Delta(k) \cdot \Big(1+\frac4{\delta_k}+\frac4{\delta_k^2}\Big)  \cdot  \prod_{k = 0}^\infty \Big(1+\frac4{(\delta_k^2)^{2^{k}}}+\frac4{(\delta_k^2)^{2^{k+1}}}\Big) 
% \\&= \Delta(k) \cdot \prod_{k = 0}^\infty \Big(1+\frac4{\delta_k^{2^k}}+\frac4{\delta_k^{2^{k+1}}}\Big) 
% \\&= \Delta(k) \cdot \gamma(\delta_k) = \pot(k).
% \end{align*}

% For the second inequality we first show $\delta_{n_{i+1}}\ge \delta_{m_i}$. Otherwise there would be a $k\in[m_i,n_{i+1}-1]$ for which $\delta_{k+1}<\delta_k\implies \nu(k+1)<1/\delta_k$, and therefore
% %
% $$
% \Delta(k+1)
% =\nu(k+1)\Delta(k)
% <\frac1{\delta_k}\Delta(k)
% \le \frac1{\delta_k}\Delta(m_i)
% \le\frac{\gamma(\delta_{n_i})}{\delta_k}\Delta(n_i)
% \le\Delta(n_i).
% $$
% %
% This is a contradiction to the choice of the interval $[n,m]$.
% The second~inequality is now a simple consequence of combining $\Delta(m_i)>\Delta(n_{i+1})$ and $\delta_{n_{i+1}}\ge \delta_{m_i}$:
% %
% $$
% \pot(n_{i+1}) 
%   = \Delta(n_{i+1})\gamma(\delta_{n_{i+1}})
%   < \Delta(m_i) \gamma(\delta_{m_i})
%   = \pot(m_i).
% $$

% \noindent
% \hrulefill

% %We now decompose the interval $[n,m]$ into segments of increasing and decreasing $\Delta$.
% Let $[n_i,m_i]\subseteq[n,m],i\in\{1,...,s\}$ be an enumeration of the maximal intervals on which $\Delta$ is non-decreasing.
% Then $n=n_1<m_1<n_2<\cdots<n_s<m_s=m$.

% For that purpose, let $n=n_1<n_2<\cdots<n_s$ be an enumeration of the start indices of increasing segments of $\Delta$, and likewise, let $m_1<m_2<\cdots<m_s=m$ be an enumeration of the end indices of increasing segments of $\Delta$. In particular, $n_1<m_1<n_2<\cdots<n_s<m_s$ (see \cref{fig:Delta_n}).


% %

% Fix $m,n\in\NN$ with $m\ge n$.
% Our goal is to derive an upper bound for $\Delta(m)/\Delta(n)$. 
% Our argument is strongest when the fraction is largest, and so w.l.o.g.\ we can assume that for all $k\in[n,m]$ holds $\Delta(n)\le\Delta(k)\le\Delta(m)$.

% % \noindent
% % \hrulefill

% % From log-concave follows
% % %
% % $$
% % \delta_{n+1}-1
% % \le\Big\lfloor\frac{f(n+1)}{f(n)}\Big\rfloor 
% % \le \frac{f(n+1)}{f(n)} 
% % \le \Big(\frac{f(n)}{f(n-1)}\Big)^2
% % \le \Big\lceil\frac{f(n)}{f(n-1)}\Big\rceil^2
% % \le (\delta_n+1)^2.
% % $$
% % %
% % which rearranges to
% % %
% % $$
% % \nu(n+1):=\frac{\delta_{n+1}}{\delta_n^2}\le 1+\frac2{\delta_n}+\frac2{\delta_n^2} 
% % %\le 1+\frac1{\sqrt{\delta_n}}+\frac1{\delta_n}.
% % %\le 1+\frac1{\delta_n-1}.
% % \le 1+ \frac1{\delta_n^{1/2}},
% % $$
% % %
% % where the last inequality holds at least for $\delta_n\ge 6$.

% % Suppose that $\nu(n+k)\ge 1$ for all $k\in\{1,...,m-n\}$.
% % First, it follows $\delta_{n+k}\ge \delta_n^{2^k}$ which yields
% % %
% % \begin{align*}
% % \frac{\Delta(m)}{\Delta(n)} = \prod_{k=1}^{\mathclap{m-n}} \nu(n+k) 
% % &\le \prod_{k=1}^\infty \Big(1+\frac{1}{(\delta_n^{2^k})^{1/2}}\Big) =: G(\delta_n). \\ 
% % G(\delta_n)&\le \prod_{k=0}^\infty \Big(1+\frac{1}{\delta_n^{2^k}}\Big) = \sum_{s=0}^\infty \delta_n^{-s} = \frac{1}{1-1/\delta_n} = \frac{\delta_n}{\delta_n-1}\le \delta_n.
% % \end{align*}
% % %
% % Note that $G(\delta)$ is decreasing in $\delta$.
% % Thus, in order for $\Delta(\free)$ to grow beyond $G(\delta_n)\cdot\Delta(n
% % )$.

% % \hrulefill

% % Choose $m,n\in\NN$ with $m\ge n$.
% % Since our goal is to derive an upper bound for $\Delta(m)/\Delta(n)$ we can assume w.l.o.g.\ that for all $k\in(n,m)$ holds $\Delta(n)<\Delta(k)<\Delta(m)$.

% Let $n=n_1<n_2<\cdots<n_s$ be an enumeration of the start indices of increasing segments of $\Delta$, and likewise, let $m_1<m_2<\cdots<m_s=m$ be an enumeration of the end indices of increasing segments of $\Delta$. In particular, $n_1<m_1<n_2<\cdots<n_s<m_s$ (see \cref{fig:Delta_n}).

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.65\textwidth]{img/Delta_n.pdf}
%     \caption{...}
%     \label{fig:Delta_n}
% \end{figure}

% Consider the infinite product
% %
% $$G(\delta):=\prod_{k = 1}^\infty \Big(1+\frac2{\delta^{2^k}}+\frac4{\delta^{2^{k+1}}}\Big).$$
% %
% One can show (see Appendix 1.1) that $G(\delta)<36$ for all $\delta\ge 2$ and that $G$ is decreasing in $\delta$.
% Our goal is now to show that $\Delta(m)/\Delta(n)\le G(\delta_n)$.
% More precisely, we show that $\Delta(m_i)/\Delta(n)\le G(\delta_n)$ for all $i\in\{1,...,s\}$. We show this by induction.

% For the induction base, note that since $\Delta$ is increasing on $[n_i,m_i]$, it holds $\nu(n_i+k)=\Delta(n_i+k)/\Delta(n_i+k-1)\ge 1$ for all $k\in[1,...,m_i-n_i]$, which rearranges to $\delta_{n_i+k}\ge \delta_{n_i+k-1}^2$. Expanding this recursive inequality yields $\delta_{n_i+k}\ge \delta_{n_i}^{2^k}$.
% Thus
% %
% \begin{align*}
% \frac{\Delta(m_i)}{\Delta(n_i)}
% &= \prod_{k=1}^{\mathclap{m_i-n_i}} \nu(n_i+k) 
% \le \prod_{k=1}^{\mathclap{m_i-n_i}} \Big(1+\frac2{\delta_{n_i+k}}+\frac2{\delta_{n_i+k}^2}\Big)
% \\&\le \prod_{k=1}^{\mathclap{m_i-n_i}} \Big(1+\frac2{\delta_{n_i}^{2^k}}+\frac2{\delta_{n_i}^{2^{k+1}}}\Big)
% < G(\delta_{n_i}).
% \end{align*}
% %
% With $i=1$ this gives the induction base $\Delta(m_1)/\Delta(n)<G(\delta_n)$.
% In fact, this can be strengthened: for $k\in[n_i,m_i-1]$ holds
% %
% \begin{align*}
% \Delta(k+1) \cdot G(\delta_{k+1})
% &\le\Delta(k+1)\cdot G(\delta_k^2)
% =\Delta(k) \cdot \nu(k+1)\cdot G(\delta_k^2)
% \\&\le \Delta(k) \cdot \Big(1+\frac2{\delta_k}+\frac2{\delta_k^2}\Big)  \cdot  \prod_{k = 0}^\infty \Big(1+\frac2{(\delta_k^2)^{2^{k}}}+\frac2{(\delta_k^2)^{2^{k+1}}}\Big) 
% \\&= \Delta(k) \cdot \prod_{k = 0}^\infty \Big(1+\frac2{\delta_k^{2^k}}+\frac2{\delta_k^{2^{k+1}}}\Big) 
% = \Delta(k)\cdot G(\delta_k).
% \end{align*}
% %
% Applied iteratively, this yields $\Delta(m_i)G(\delta_{m_i})\le\Delta(n_i)G(\delta_{n_i})$.

% For the induction step we first need to prove that $\delta_{n_{i+1}}\ge \delta_{m_i}$. If this were not the case, then there would be a $k\in[m_i,n_{i+1}-1]$ so that $\delta_{k+1}<\delta_k$ which implies $\nu(k+1)=\delta_{k+1}/\delta_k^2 <1/\delta_k$ and further
% %
% $$
% \Delta(k+1)
% =\nu(k+1)\Delta(k)
% <\frac1{\delta_k}\Delta(k)
% \le \frac1{\delta_k}\Delta(m_i)
% \le\frac1{\delta_n}G(\delta_n)\Delta(n)
% \le\Delta(n).
% $$
% %
% This would be a contradiction to the choice of $n$.

% With this in place, we can finish the induction step by
% %
% $$
% \Delta(m_{i+1})
% \le G(\delta_{n_{i+1}})\Delta(n_{i+1})
% \le G(\delta_{m_i})\Delta(m_i) 
% \le G(\delta_n)\Delta(n).
% $$



% \noindent\hrulefill


% Note that the upper bound in \cref{res:g_growth_trees} is quadratic in $g$, hence does capture the desired growth behavior even worse than, say, an upper bound of $g(2r+1)$. This is not a problem for establishing the existence of trees of intermediate growth.
% But it prevents us from concluding that there are trees of any particular polynomial growth.

% In the next section we show that for a target growth rate of at least $g(r)\sim r^{\alpha\log\log r}$ for $\alpha>1$, together with some further natural condition, the upper bound can be improved to be linear in $g(2r+1)$.

% This still fails to rescue the case for polynomial growth.
% However, if $\bar g(r)=r^\alpha$ has integer exponents and $\delta_n=2^\alpha-1$, then we can embed $T$ into the $\alpha$-th power of the $\alpha$-dimensional integer lattice as shown in \cref{fig:2_lattice_construction} (recall that the $\alpha$-th power $G^\alpha$ of a graph $G$ is obtained by adding edges to $G$ between any pair of vertices at distance at most $\alpha$).
% This established a $r^\alpha$ upper bound on the volume growth of $T$.

%\begin{example}\label{ex:lattice_tight_upper_bound}

% Consider the following slightly modified construction of the tree $T_n$: instead of identifying the root of each apocentric copy of $T_{n-1}$ with an apocentric vertex of the central copy of $T_{n-1}$, we now let the central and apocentric copies of $T_{n-1}$ be disjoint, and we add edges between their apocentric vertices (see \cref{fig:compare_constructions}).

% \begin{figure}[h!]
%     \centering
%     %\includegraphics[width=0.5\textwidth]{img/compare_constructions.pdf}
%     \includegraphics[width=0.55\textwidth]{img/compare_constructions_2.pdf}
%     \caption{Comparison of $T_1$ from \cref{ex:loglogr} for the old construction (left) and the new construction (right). The dashed lines on the~right~indicate the new edges added to $T_1$ that connect the disjoint copies of $T_0$.}
%     \label{fig:compare_constructions}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     %\includegraphics[width=0.95\textwidth]{img/2_lattice_subgraph_2.pdf}
%     \includegraphics[width=0.95\textwidth]{img/2_lattice_subgraph_3.pdf}
%     %\caption{Illustration of the first four steps in the  construction~of~\cref{ex:lattice_tight_upper_bound}. %The ringed vertex is the root, and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy of $T_{n-1}$ in $T_n$.
%     %}
%     \caption{
%         Embedding of the tree $T$ with constant sequence $\delta_n=3$ into the square of the 2-dimensional lattice graph.
%     }
%     \label{fig:2_lattice_construction}
% \end{figure}

% There are two things to note about this modified construction: first, the proof of \cref{res:g_growth_trees} applies with only minor modifications (one of which is that the distance from the central vertex to an apocentric vertex in $T_n$ is no longer $2^n$, but $(3^n-1)/2$).
% Second, if we use a constant sequence $\delta_n=3^\alpha-1$ for $\alpha\ge 1$we find that the resulting tree is a spanning tree of $L^2$, where $L$ is the $\alpha$-dimensional lattice graph, and $L^2$ means that we add additional edges between vertices that are at distance two in $L$.
% In particular, since the volume growth of $L^2$ is still of on the order of $r^\alpha$, this provides an equivalent upper bound on the volume growth of the resulting limit tree $T$.

%\end{example}




% \section{A linear upper bound}
% \label{sec:linear_bound}

% In this section we assume that $g$ has the following three properties:
% %
% \begin{enumerate}
%     \item $g$ is log-concave.
%     \item $f(n):=g(2^n)$ is log-convex.
%     \item $g\in\Omega(r^{\alpha\log\log r})$ for some $\alpha>1$.
% \end{enumerate}
% %
% The first two conditions just make sure that $g$ grows nicely enough, that is, does not change its growth behavior too rapidly. Most naturally occurring functions satisfy these conditions anyway.
% The last condition turns out to be a \enquote{magic} barrier to our techniques analysing this specific construction.

% \begin{proposition} \label{res:d_i_loglog_r}
% If $g(r)=r^{\omega(1)}$ grows super-polynomially then $s_n:=f(n)/f(n-1)$ is increasing, and $(\delta_n-1)/s_n\to 1$. 

% If we furthermore have $g\in\Omega(r^{\alpha\log\log r})$ for some $\alpha>1$, then there are $0<A_n \le B_n<1$ with
% %
% $$A_n s_n \le \delta_n-1 \le B_n s_n,\quad\text{for all $n\ge 1$},$$
% %
% and so that $A_n,B_n\to 1$, and
% %
% $$\prod_{i=1}^\infty \frac{B_i}{A_i^2}<\infty$$
% %
% converges \emph{(\emph{note that the terms $B_i/A_i^2\ge 1$, so the partial products never decrease})}.
% \end{proposition}

% \begin{proof}
% For brevity, define $s_n:=g(2^n)/g(2^{n-1})$. By definition of the $\delta_n$, we have
% %
% $$\frac{\delta_n-1}{s_n} \ge \frac{\lfloor s_n\rfloor -1}{s_n} =: A_n, \qquad \frac{\delta_n-1}{s_n} \le \frac{\lceil s_n\rceil -1}{s_n} =: B_n.$$
% % 
% Since $s_n\ge 2$ we indeed have $0<A_n\le B_n<1$.
% Since $g$ is super-polynomial, the $s_n$ are unbounded, and so $A_n,B_n\to1$.
% If $s_n=2$, then $B_n/A_n^2=1$. If $s_n>2$ we have the following estimation:
% %
% $$1<\frac{B_n}{A_n^2} = \frac{s_n(\lceil s_n\rceil-1)}{(\lfloor s_n\rfloor-1)^2} \ge \frac{s_n^2}{(s_n-2)^2} = \Big(1-\frac2{s_n}\Big)^{-2}<\infty$$
% %
% As established previously, the conditions on $g$ guarantee that the infinite product~of these terms converges.
% \end{proof}

% \begin{proposition}\label{res:average_degree_estimation}
% There exists a constant $C>1$ so that for all $m\ge n$ holds
% %
% $$\frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)} \le C\cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)}.$$
% %
% In particular, the maximum degree 
% %
% \begin{equation*}%\label{eq:conditions_g}
% \Delta:= \Big\lceil \sup_m \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_m-1)} \Big\rceil +1 \;\le\; \lceil C(\delta_1-1)\rceil + 1.
% \end{equation*}
% %
% is finite.
% \end{proposition}
% %
% \begin{proof}
% Since $g$ is log-concave, we have
% %
% \begin{align*}
%     \textstyle \frac13\log g(2^{m+1}) + \frac23 \log g(2^{m-1}) &\le \log g\big(\overbrace{\textstyle\frac23(2^{m-1})+\overset{\phantom .}{\frac13}(2^{m+1})}^{2^m}\big)
%     \\
%     g(2^{m+1})[g(2^{m-1})]^2 &\le [g(2^m)]^3
%     \\
%     \frac1{B_n}(\delta_{m+1} - 1)\le \frac{g(2^{m+1})}{g(2^m)} &\le \Big[\frac{g(2^{m})}{g(2^{m-1})}\Big]^2 \le \frac1{A_m^2}(\delta_m-1)^2
%     \\
%     \delta_{m+1}-1 &\le \frac{B_m}{A_m^2} \cdot (\delta_m-1)^2
%     \\
%     \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)} &\le \frac{B_m}{A_m^2} \cdot \frac{\delta_{m}-1}{(\delta_1-1)\cdots(\delta_{m-1}-1)}
%     \\
%     &\le \cdots \le 
%     \Big(\prod_{i=n+1}^{m}\frac{B_i}{A_i^2}\Big) \cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)}
%     \\
%     &\le C \cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)},
% \end{align*}
% %
% where we set $C:=\prod_{i=1}^\infty B_i/A_i^2$, which exists by \cref{res:d_i_loglog_r}.
% \end{proof}

% \begin{theorem}
% There is a constant $D>1$ so that
% %
% $$|B_v^T\!(r)|\le D\cdot g(2r-1).$$
% %
% %In particular, $|B_v^T\!(r)| = \theta(g)$.
% \end{theorem}
% %
% \begin{proof}
% Fix a vertex $v\in V(T)$ and $r\ge 0$. Choose $n$ so that $2^{n-1}-1 \le r \le 2^n-1$ and let $T_n(v)$ be the copy of $T_n$ that contains $v$. Let $m$ be the biggest number so that $T_n(v)$ is an apocentric copy of $T_n$ in $T_m\subset T$, or $n$ if $T_n(v)=T_n\subset T$. Then $m\ge n$ and by  \cref{res:average_degree_estimation} holds
% %
% $$
% \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)} 
% \le C \cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)}
% $$
% %
% for some $C>1$ that only depends on $g$.
% This rearranges to
% %
% \begin{align*}
% \delta_{n+1}-1 
% &\ge \frac1C \cdot (\delta_1-1)\cdots(\delta_{n}-1) \cdot \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)}.
% % \\
% % &\le \frac1C \cdot \Big\lceil(\delta_1-1)\cdots(\delta_{n}-1) \cdot \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)}\Big\rceil.
% \end{align*}
% %
% Since $\delta_{n+1}-1$ is an integer, we actually have
% %
% \begin{align*}
% \delta_{n+1}-1 
% &\ge \frac1C \cdot \Big\lceil(\delta_1-1)\cdots(\delta_{n}-1) \cdot \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)}\Big\rceil.
% \end{align*}
% %
% The left side of this inequality is the number of edges leaving $T_n\subset T$ via apocentric vertices, while the right side is $1/C$ times an upper bound for the number of edges leaving $T_m(v)$ via apocentric vertices.

% % As in the proof of the upper bound in \cref{res:g_growth_trees}, $T_n(v)$ can be left in only two ways, via an apocentric vertex of $T_n(v)$, or via the center of $T_n(v)$.
% % %
% % \begin{itemize}
% %     \item How many copies ...
% % \end{itemize}
% \end{proof}

\section{Unimodular random trees}
\label{sec:unimodular}

%\begin{mnote}
%Notes:
%\begin{enumerate}
    %\item We need to define a ton of terminology surrounding (unimodular) random graphs/trees, and in my opinion the right place for this would be over the course of this section. Note that this does not mean that everything has to be define in the first paragraph: random graph should be define at the start, but \eg\ transport functions, BS-convergence and unimodularity can be defined only when we explain how to obtain unimodular graphs later on (before Theorem 4.1).
    %\item What are \enquote{nice functions}?
    %\item In Theorem 4.1, better use the sequence $(T_n,x^*)$, and maybe subsequence $(T_{n_i},x^*)$? \gsays{I would advise against it; even if these graphs are conceptualised as an inclusion chain, I still need their roots to be chosen \emph{independently} u.r., so I cannot use the same variable for all of their roots. That said, we can still discuss changes in style.}
    %\item I would say for defining \enquote{generalized canopy tree} we can combine intuition and formal definition: start from the modified inclusion chain $T_1\subset T_2\subset \dots$ where we identify $T_{n-1}$ with an \emph{apocentric} copy in $T_{n}$ instead of the central copy. Then all $T_n$ can still be chosen rooted at $o_n=x^*$, because this \enquote{global root} (a bad name now) stays apocentric forever. \gsays{I think we've already written this.}
    %\item Perhaps we should explain what the usual canopy tree is in a footnote.
    %\item We need a new graphics for the generalized canopy tree (I am working on that).
    %\item I am not a fan of abbreviations, I would write \enquote{almost surely} instead of a.s. (or at least mention once what it stands for). \gsays{But this is very standard!}
    %\item Is the sequence $(T_n,o_n)$ in the definition of  \enquote{complete central/apocentric} and \enquote{eventually apocentric} \emph{the} sequence from Construction 2.1? If yes, say so.
    %\item You define \enquote{undecided} for a sequence of vertices instead of rooted trees. \gsays{I mean, those vertices are the roots of rooted trees. Yes I would rather say that the root of a tree is undecided rather than that a rooted tree is undecided. Does it make a difference? I mean, apart from the fact that using these words for roots is more intuitive.}
    %\item On that note, maybe we can/should define these notions (completely central/apocentric and undecided) also for random trees. For example, a random tree $(T,x)$ is completely apocentric if $x$ is apocentric in every $T_n(x)$ with probability one (see my note on Proposition 4.2 below for why I think so).\gsays{...but we have done this. This is exactly what I mean when I write "these adjectives also apply to...". The only difference between what you are proposing and what is written is that you say that a rooted tree is, say, completely apocentric, and I say that its root is completely apocentric. And might I add, we already have a word for what you would call an "eventually apocentric tree": it is the generalised canopy tree.} \gsays{Hm, all right, we never explained that if the root of a limit tree is eventually central or eventually apocentric or undecided, then so is every vertex of the tree, and therefore that these are properties of both the tree and the root. I should say that.}
    %\item I consider proofs black boxes. If you use something outside of a proof, then it should be defined outside of a proof. I am specifically referring to $\mathcal T$. \gsays{But this is the underlying graph of the limit of a subsequence of $(T_n,o_n)$ that is only important in the context of the proof!}
    %\item You need to explain what Kolmogorov's law is, or avoid using it (we don't necessarily need to invoke big theorems if it can be done elementary :D).
    %\item Proposition 4.2 is supposed to be a general structure theorem on the limit tree. Maybe it is better to formulate it as follows: if the $\delta_n$ grow like this, then the limit is completely apocentric, if it grows like that, then it is completely central, otherwise undecided.
    %\item Proposition 4.3 is not used anywhere, is it? It should also be proven properly. \gsays{Apart from one minor thing that I fixed, it looks correct.}
    %\item We should use consistent terminology: always Benjamini-Schramm limit, or always distributional limit (idea: let's stick to BS limit). \gsays{Hm, but there is a slight difference here...}
    %\item Should we make Example 4.4 more rigorous? (especially the last two sentences).
    %\item Should we say a word about why the limit trees that result from inclusion chains $T_0\subset T_1\subset T_2\subset\cdots$ other than the standard one (where $T_{n-1}$ is central in $T_n$) still satisfy the conclusion of Theorem 3.4 (that is, the uniform volume growth)?
    %\item Meta thought: there are clearly two styles of writing and two styles of formatting in this paper. I wonder whether we should make this more uniform. And how?
%\end{enumerate}
%\end{mnote}

%\begin{mnote}
%Notes (08/07/2022):
%\begin{enumerate}
 %   \item can we show that $T_1,T_2,T_3,...$ actually BS-converge, not just that it has a convergent sub-sequence?
    %\item Is a generalized canopy tree the same as a 1-ended tree?
%\end{enumerate}
%\end{mnote}

In this paper, we have been working with rooted graphs, \ie\ pairs of the form $(G,o)$, $o\in V(G)$. It is now useful to define the notion of a \emph{random rooted graph} as introduced in \cite{benjamini2011recurrence}. For this, we must firstly note that there is a natural topology over the set of rooted graphs, the \emph{local topology}, induced by the metric 
%
\begin{align*}
\dist\!\big((G,o),(G',o')\big):=2^{-R} \quad &\text{if } \ball Gor\cong \ball{G'}{o'}r \text{ for all } 0\leq r\leq R
\\
&\text{and } \ball Go{R+1}\ncong \ball{G'}{o'}{R+1}.
\end{align*}
%
% \[d((G,o),(G',o'))=2^{-k} \hspace{1mm}\text{if}\hspace{1mm} \ball Gor\cong \bal{G'}{o'}r \hspace{1mm} \text{for}\hspace{1mm} 0\leq r\leq k\]
% %
% \[\text{and}\hspace{1mm} \ball Go{k+1}\ncong \ball{G'}{o'}{k+1}.\]

A random rooted graph $(G,o)$ is a Borel probability measure (for the local topology) over the set of locally finite, connected rooted graphs. We call $(G,o)$ \emph{finite} if the set of infinite rooted graphs has $(G,o)$-measure $0$. If the conditional distribution of the root of a finite random rooted graph $(G,o)$ over each of the underlying graphs in its support is uniform, then $(G,o)$ is called \emph{unbiased}. 

Given a sequence $(G_n,o_n)$ of unbiased random rooted graphs together with a random rooted graph $(G,o)$, we say that $(G,o)$ is the \emph{Benjamini-Schramm limit} of $(G_n,o_n)$ if for every finite rooted graph $H$ and natural number $r$ we have 
%
\[\lim_{\mathclap{n\to \infty}}P\big(\ball{G_n\!}{o_n}r\cong H\big)=P\big(\ball{G}{o}r\cong H\big).\] 
%
If a random rooted graph $(G,o)$ is the Benjamini-Schramm limit of some sequence, we say that it is \emph{sofic}. By a standard result \cite{benjamini2011recurrence} the bounded degree graphs form a compact subset in the local topology, from which it follows that a sequence $(G_n,o_n)$ of bounded degree graphs always has a convergent subsequence.

The notion of uniform growth is well-defined in random rooted graphs. We say that a random rooted graph $(G,o)$ has uniform growth $g(r)$ if there exists a function $g:\RR_{\ge 0}\rightarrow \RR_{\ge 0}$ and positive constants $c_1, C_1, c_2, C_2$ such that for every $r\ge 0$ a.s. $C_1\cdot g(c_1r)\leq |B_G(o,r)|\leq C_2\cdot g(c_2r)$. Although this definition focuses on the growth around the root, this attention to the root is not undue; this is indeed the natural way to define uniform growth in random rooted graphs, as the root ``may be any vertex''. That is to say, for each underlying graph $G$, $o$ is a representative of each orbit of $\Aut(G)$ with positive probability \TODO.

The precise statement of Benjamini's question requests a \emph{unimodular} tree of intermediate growth. A random rooted graph $(G,o)$ is unimodular if it obeys the mass transport principle, \ie
%
\[\mathbb E\Big[\sum_{\mathclap{x\in V(G)}}f(G,o,x)\Big]=\mathbb E\Big[\sum_{\mathclap{x\in V(G)}}f(G,x,o)\Big]\]
%
for every transport function $f$. For an exact definition of transport functions we direct the reader to \cite{aldouslyons}. For the purpose of this paper, it suffices to say that transport functions are Borel functions over doubly-pointed graphs that output non-negative values and simulate mass transport between vertices. The mass transport principle simply states that the root $o$ on average sends as much mass to other vertices as it receives from them. Unimodular graphs are quite significant in the theory of random graphs and encompass some interesting classes. The most basic non-trivial example is that all sofic graphs are unimodular. The famous Aldous-Lyons conjecture asks for the converse \cite{aldouslyons}. 

In the preceding sections, given a super-additive, log-concave growth function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$, we constructed a deterministic rooted tree $(T,x^*)$ which exhibits uniform growth $g(r)$. However, $(T,x^*)$ is not necessarily unimodular. Indeed, suppose that we construct $(T,x^*)$ as a centric limit, and that $|\frac{\delta_n}{\delta_1...\delta_{n-1}}-(\delta_1-1)|\geq 1$ for every $n\geq 2$. Then $x^*$ is the only vertex with degree $\delta_1$. Consider the transport function $f(G,x,y)$ which equals $1$ if $G=T$, $x\sim y$ and $d_T(x,x^*)<d_T(y,x^*)$, and $0$ otherwise. Then $\mathbb{E}[\Sigma_{x\in V(T)}f(T,x^*,x)]=\delta_1\neq 0=\mathbb{E}[\Sigma_{x\in V(T)}f(T,x,x^*)]$.

That said, a unimodular tree with uniform growth $g(r)$ necessarily exists: 

\begin{proposition}\label{converge?}
    Let $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ be super-additive and log-concave. Then there exists a unimodular random rooted tree with uniform growth $g(r)$. In particular, there exists a unimodular tree with intermediate uniform growth.
\end{proposition}

\begin{proof}
Assume the full setting of \autoref{thm:main}. Consider a sequence $(T_n,o_n)$ of unbiased random rooted trees, where each $T_n$ is a.s. as in \cref{constr:T_n}. Since the space of bounded-degree graphs with the local topology is compact, there exists a subsequence of $(T_n,o_n)$, say $(\mathcal{T}_n,\mathcal{o}_n)$, converging to a random rooted tree $(\mathcal{T},\mathcal{o})$. By the definition of the Benjamini-Schramm limit, every ball of $(\mathcal{T},\mathcal{o})$ centered at $\mathcal{o}$ is \as\ isomorphic to a ball of $\mathcal{T}_n$ for $n$ large enough. However, every ball of radius $\leq 2^n-1$ in $T_n$ is isomorphic to a ball of a limit tree $T$ as in \cref{constr:T}, and therefore admits the respective bounds. %Every ball of $(\mathcal{T},\mathcal{o})$ is contained in a ball rooted at  $\mathcal{o}$, and is thus \as\ a ball of $\mathcal{T}_n$. 
Hence, $\mathcal{T}$ exhibits uniform growth of order $g(r)$. Additionally, since $(\mathcal{T},\mathcal{o})$ is sofic, it is also unimodular.
\end{proof}

In fact, we may even eschew focusing on a subsequence:

\begin{proposition}\label{converge}
    The sequence $T_n,n\ge 0$ is BS-convergent.
\end{proposition}

\begin{proof}
    Fix $r\ge 1$ and a graph $H$.
    Call a vertex $v\in V(T_n)$ \emph{good} if $\ball{T_n} v r\cong H$.
    Let $P_n$ be the probability that a uniformly chosen vertex of $T_n$ is good.
    %We show $|P_{n+k}-P_n|\le C_r 2^{-n}$ for all $k\ge 0$ and a constant $C_r\ge 1$ that only depends on $r$.
    %In other words, $P_n$ is a Cauchy sequence, hence convergent, and $T_n$ is BS-convergent.
    We show that $P_n$ is a Cauchy sequence, hence convergent.

    Let $s_n$ be the number of good vertices in $T_n$.
    Since $T_n$ consists of $\delta_n+1$ copies of $T_{n-1}$, one might expect $s_n\approx (\delta_n+1)s_{n-1}$.
    However, besides the copies, $T_n$ also contains $\delta_n$ new edges, and so if $\tau\prec_{n-1} T_n$ and $v\in V(\tau)$, the $r$-ball around $v$ in $\tau\cong T_{n-1}$ might look different from the $r$-ball around $v$ in $T_n$.
    Still, this can only happen if $v$ is $r$-close to one of the $2\delta_n$ ends of the new edges.
    Let $C_r$ be an upper bound on the size of an $r$-ball in $T$ (which exists since $T$ is of bounded degree). We can then conclude
    %
    $$|s_n-(\delta_n+1)s_{n-1}|\le 2C_r\delta_n.$$
    %
    Since $P_n=s_n/|T_n|$, division by $|T_n|=(\delta_n+1)|T_{n-1}|$ yields
    %
    \begin{align*}
        &|P_n-P_{n-1}|\le \frac{\delta_n}{\delta_n+1}\frac{2C_r}{|T_{n-1}|}\le \frac{2C_r}{|T_{n-1}|}.
    \end{align*}
    %
    It follows for all $k\ge 1$
    %    
    \begin{align*}
    |P_{n+k}-P_n| 
    &\le |P_{n+k}-P_{n+k-1}|+\cdots+|P_{n+1}-P_n|
    \\ &\le 2C_r\Big(\frac1{|T_{n+k-1}|}+\cdots+\frac1{|T_{n}|}\Big)
    \le 2C_r\sum_{i=n}^{\infty} \frac1{|T_i|}.
    \end{align*}
    %
    Since $\delta_n\ge 1$ and $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ we have $|T_n|\ge 2^n$. It therefore follows
    %
    \begin{align*}
    |P_{n+k}-P_n| \le \frac{4C_r}{2^n},
    \end{align*}
    %
    and $P_n$ is indeed a Cauchy sequence.
\end{proof}


\cref{converge?} and \cref{converge} prove \cref{unimain}. However, since their proofs are not constructive, one might still wonder about the exact structure of $\mathcal{T}$. To answer this question, we require certain definitions and observations. We allow the notations $(T_n,o_n)$, and $(\mathcal{T},\mathcal{o})$ to retain their meaning for the rest of this section.  

Let $p_n:=\frac{\delta_n}{\delta_n+1}$. We say that the sequence $(T_n,o_n)$ is \emph{apocentric} if $\prod_{n=1}^{\infty}p_n>0$. Otherwise, we say that it is \emph{balanced}. Note that a sequence is apocentric if and only if the same is true for each of its subsequences. %For brevity, these adjectives will be called the \emph{type} of the subsequence.  

A \emph{generalized canopy tree}\footnote{Recall that the \emph{canopy tree} is the Benjamini-Schramm limit of a sequence of full binary trees of increasing depths. The canopy tree is the single most famous example of a generalized canopy tree.} is the Benjamini-Schramm limit of an apocentric sequence. On the other hand, a \emph{balanced tree} is the Benjamini-Schramm limit of a balanced sequence.

Let us continue our analysis by establishing conditions on $\delta_n$ (and, by extension, $g$) under which $(\mathcal{T}, \mathcal{o})$ is a generalised canopy tree or a balanced tree.

\begin{proposition}\label{res:types_of_limits}
If $\delta_n>n^{\alpha}$ for some $\alpha>1$ and all sufficiently large $n$, then $(\mathcal{T}, \mathcal{o})$ is \as\ a generalized canopy tree. 
If $\delta_n$ grows at most linearly, then $(\mathcal{T},\mathcal{o}$) is \as\ a balanced tree.
\end{proposition}

\begin{proof}
The limit tree $(\mathcal{T},\mathcal{o})$ is a.s. a generalised canopy tree if and only if $(T_n,o_n)$ is an apocentric sequence, equivalently if $\Sigma_{n=1}^{\infty}\ln\frac{\delta_n+1}{\delta_n}<\infty$, which is true for $\delta_n>n^{\alpha}$. Indeed,
%
%\begin{align*}
%\ln\frac{\delta_n+1}{\delta_n}&<\frac{1}{n^{\alpha}}\Leftrightarrow
%\\
%\frac{\delta_n+1}{\delta_n}&<e^{\frac{1}{n^{\alpha}}}\Leftrightarrow
%\\
%1-\frac{1}{\delta_n+1}&>e^{-\frac{1}{n^{\alpha}}}\Leftrightarrow
%\\
%\delta_n>\frac{1}{1-e^{-\frac{1}{n^{\alpha}}}}-1&=\frac{e^{-\frac{1}{n^{\alpha}}}}{1-e^{-\frac{1}{n^{\alpha}}}}=\frac{1}{e^{\frac{1}{n^{\alpha}}}-1}\Leftarrow
%\\
%\delta_n&>n^{\alpha}.
%\end{align*}
%
\begin{align*}
\delta_n>n^\alpha \ge \frac{1}{\exp(1/n^\alpha)-1}
%=\frac1{1-\exp(-1/n^\alpha)}-1 
\;\implies\; \ln\Big(\frac{\delta_n+1}{\delta_n}\Big)<\frac1{n^\alpha}
\;\implies\; \sum_{n=0}^\infty \ln\Big(\frac{\delta_n+1}{\delta_n}\Big) <\infty.
\end{align*}

Therefore, if we eventually have $\delta_n>n^{\alpha}$, $\alpha>1$, $(\mathcal{T},\mathcal{o})$ is a.s. a generalized canopy tree with an apocentric vertex for a root. 

%Subsequently, we may ask for the probability that  $(\mathcal{T}_n,\mathcal{o}_n)$ is eventually apocentric. But this event contains the event that $\mathcal{o}_n$ is a sequence of apocentric vertices, and for $\delta_n>n^{\alpha}$ the latter has positive probability. By Kolmogorov's Law, every tail event has probability either $0$ or $1$. Therefore, for $\delta_n>n^{\alpha}$, $(\mathcal{T},\mathcal{o})$ is a.s. a generalized canopy tree. 

On the other hand, if $\delta_n<kn$, and since $kn(e^{\frac{1}{kn}}-1)\rightarrow 1$, we obtain
%
%\[\delta_n+1<\frac{1}{1-e^{-\frac{1}{kn}}}\Leftrightarrow\]\[1-\frac{1}{\delta_n+1}<e^{-\frac{1}{kn}}\Leftrightarrow\]\[\ln \frac{\delta_n+1}{\delta_n}>\frac{1}{kn},\] 
%
%\msays{My attempt:}
\begin{align*}
\delta_n<kn \le \frac{1}{\exp(1/kn)-1}
%=\frac1{1-\exp(-1/n^\alpha)}-1 
\;\implies\; \ln\Big(\frac{\delta_n+1}{\delta_n}\Big)>\frac1{kn}
\;\implies\; \sum_{n=0}^\infty \ln\Big(\frac{\delta_n+1}{\delta_n}\Big) =\infty,
\end{align*}
%
implying that $(T_n,o_n)$ is balanced. %As mentioned previously, the probability that $(\mathcal{T}_n,\mathcal{o}_n)$ is eventually central is also 0. 
So, for linear or sublinear $\delta_n$, $(\mathcal{T},\mathcal{o})$ is a.s. balanced.
\end{proof}

\begin{proposition}
If $g\in\Omega(r^{\alpha\log\log r})$ for some $\alpha >0$ and $f(n):=g(2^n-1)$ is log-con\-vex, then $\delta_n=\Omega(n^\alpha)$. For $\alpha>1$ it follows that $(\mathcal{T},\mathcal{o})$ is \as\ a generalized canopy tree. As a consequence, every nice growth ($g$ super-additive, log-concave; $g(2^n-1)$ log-convex) is exhibited by a generalized canopy tree.
%
$$
%\lim_{n\to\infty} \frac{(\delta_1)\cdots (\delta_n)}{(\delta_1-1)\cdots(\delta_n-1)} = \prod_{n=1}^\infty \Big(1-\frac1{\delta_n+1}\Big) > 0.
$$
\end{proposition}
\begin{proof}
Let $C>0$ so that $g(r)\ge C r^{\alpha\log\log r}$ for all sufficiently large $r$. 
In terms of $\log f(n)$ this reads
%
$$(*)\quad \log f(n)
\ge \log(C) + \alpha \log(2^n-1) \log\log(2^n-1) 
\geq \log(C) + \alpha n \log(n).
$$
%
for all sufficiently large $n$.

We show that $s_n:=f(n)/f(n-1)\ge n^\alpha$ for all sufficiently large $n$. The statement for $\delta_n$ then follows from $\delta_n/s_n \to 1$ for super-polynomial $g$.

Assume the contrary, that $s_n< n^\alpha$ for infinitely many $n$, or equivalently, that $(**)\;\log f(n) - \log f(n-1) < \alpha \log(n)$. By log-convexity $(\times)$ of $f$ follows
%
\begin{align*}
    \frac{1}{n-1} \log f(1) + \Big(1-\frac{1}{n-1}\Big)\log f(n) \,& \overset{\mathclap{(\times)}}\ge\, \log f(n-1)
    %\\&
    \,\overset{\mathclap{(**)}}>\,  \log f(n) - \alpha\log(n)
    \\
    \implies\quad \log f(1)  &> \log f(n) - \alpha(n-1)\log(n)
    \\[-1ex]
    & \overset{\mathclap{(*)}}\ge \log(C) + \alpha n \log(n) - \alpha(n-1)\log(n)
    \\[0.7ex]
    &= \alpha\log(n) + \log(C),
\end{align*}
%
which cannot be true for arbitrary large $n$.
\end{proof}

We are now equipped to prove our structure theorem:

\begin{main}[Structure Theorem]\label{structure}\quad
\begin{myenumerate}
    \item
    If $(\mathcal{T},\mathcal{o})$ is a generalised canopy tree, then it is \as\ an apocentric limit. In particular, it is 1-ended.
    \item
    If $(\mathcal{T},\mathcal{o})$ is a balanced tree, then it is \as\ a balanced limit, it is supported on uncountably many trees, and it is \as\ 1-ended or 2-ended, with the former holding \as\ if $\delta_n\neq 1$ eventually.    
\end{myenumerate}
\end{main}
\begin{proof}\quad 
    \begin{myenumerate}
        \item For an apocentric sequence, any tail product $p^{(k)}:=\prod_{n=k+1}^{\infty}p_n$ is positive. Additionally, $p^{(k)}$ is the limit of the probability that $o_n$ lies in an apocentric $\tau\prec_k T_n$ as $n\to\infty$. So, consider the event $A_{k,r}$ that the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball centered at a vertex of an apocentric $\tau\prec_k T_n$, $n>\log(2r+2^k)$, and note that, for every $r\geq 0$, $P(A_{k,r})\geq p^{(k)}$. Let $A_k:=\bigcap_{r\geq 0}A_{k,r}$. That is, $A_k$ is the event that for every $r\geq 0$ the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball centered at an apocentric $\tau\prec_k T_n$, $n>\log(2r+2^k)$. Since $A_{k,r}$ is decreasing in $r$, we have $P(A_k)=\lim_{r\rightarrow \infty}P(A_{k,r})\geq p^{(k)}$. Since $A_k$ is increasing in $k$, $P(\bigcup_{i=1}^{\infty}A_k)=\lim_{k\rightarrow \infty}P(A_k)\geq \lim_{k\rightarrow \infty}p^{(k)}=1$. Therefore, there exists \as\ $k\in \NN_0$ such that the event $A_k$ occurs, implying that $(\mathcal{T},\mathcal{o})$ is an apocentric limit. 

        Let $v\in V(\mathcal{T})$ and let $k$ be such that a copy $\tau\prec_k\mathcal{T}$ contains both $\mathcal{o}$ and $v$. Take $r$ large enough so that $\tau\subset B_{\mathcal{T}}(\mathcal{o},r)$ \TODO. Then all but one of the connected components of $\mathcal{T}\setminus v$ are subtrees of $\tau$, therefore finite. Hence, $\mathcal{T}$ is 1-ended.

        \item For a balanced sequence, let $p_{(k)}:=\prod_{n=1}^kp_n$ and note that $p_{(k)}$ is the probability that a uniformly chosen vertex of a tree $T_n$, $n\geq k$ is apocentric in a copy $\tau\prec_k T_n$. Let $B_{k,r}$ be the event that the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball centered at an apocentric vertex of a copy $\tau\prec_k T_n$ that is a leaf of $T_n$, $n>\log(2r+2^k)$. Note that, for $r\geq 2^{k+1}-1$, the only vertices that are the centers of balls isomorphic to \textcolor{red}{such} balls are indeed apocentric vertices of \textcolor{red}{such} copies, hence $P(B_{k,r})\leq p_{(k)}$. Also, observe that $B_{k,r}$ is a decreasing sequence in $r$. Let $B_k:=\bigcap_{r\geq 0}B_{k,r}$. That is, $B_k$ is the event that for every $r\geq 0$ the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball centered at an apocentric vertex of a copy $\tau\prec_k T_n$ that is a leaf of $T_n$. We deduce that $P(B_k)=\lim_{r\rightarrow \infty}P(B_{k,r})\leq \lim_{r\rightarrow \infty}p_{(k)}=p_{(k)}$. Since $B_k$ is also a decreasing sequence in $k$, $P(\bigcap_{k\geq 0}B_k)=\lim_{k\rightarrow \infty}P(B_k)\leq \lim_{k\rightarrow \infty}p_{(k)}=0$. Therefore, there exists a.s. some $k\in \NN_0$ such that $\mathcal{o}\in \tau\prec_{k}\tau'\prec_{k+1} \mathcal{T}$ with $\tau$ being central in $\tau'$. We may repeat this argument for the sequence $(T_n,o_n)$ with copies of $T_k$ contracted \TODO, etc. Thus we deduce that $\mathcal{o}$ lies \as\ in a sequence of copies $\tau\prec_{k_n}\tau'\prec_{k_n+1}\mathcal{T}$ with $\tau$ central in $\tau'$. It is also straightforward \TODO\ to see that $\mathcal{o}$ lies \as\ in a sequence of copies that are apocentric in some copy. We have shown that $(\mathcal{T},\mathcal{o})$ is \as\ a balanced limit. 
        
        Note that each rooted tree in the support of a balanced tree is sampled with probability 0, so the support of a balanced tree is uncountable. 

        The final piece of this proof is to deduce the number of ends of a balanced random rooted tree. It is well-known result \cite{...} that every unimodular random rooted tree with average root degree 2 has \as\ either one or two ends. As we show below, this set happens to include the Benjamini-Schramm limits of balanced sequences.

        \msays{use short version}

        Let us direct our attention to the neighbourhood of the root $\mathcal{o}$ and calculate its mean degree. 
    
    With probability $1-p_1=\frac{1}{\delta_1+1}$, $\mathcal{o}$ is the centre of a copy of $T_1$, which has degree $\delta_1+1$, yielding a summant of 1. 
    
    With probability $p_1=\frac{\delta_1}{\delta_1+1}$, $\mathcal{o}$ is a leaf of a copy of $T_1$. Therefore, its average degree depends on the minimum $k\in\NN$ such that $v\in \tau\prec_k\tau'\prec_{k+1} \mathcal{T}$ with $\tau$ being apocentric in $\tau'$. Specifically, it equals $\frac{\delta_{k+1}}{\prod_{n=1}^k\delta_n}+1$. The probability that a specific number $k$ has this property if $\mathcal{o}$ is a leaf of a copy of $T_1$ is $(1-p_{k+1})\prod_{n=1}^kp_k=\frac{\prod_{n=1}^k\delta_k}{\prod_{n=1}^{k+1}(\delta_n+1)}$. Thus, the second summant is $\sum_{k=1}^{\infty}\frac{\delta_{k+1}}{\prod_{n=1}^{k+1}(\delta_n+1)}+p_1=(1-p_1)+p_1=1$ and we have $\mathbf{E}(deg(\mathcal{o}))=1+1=2$.

We have shown that balanced trees have \as\ one or two ends. One ray $R_1$ of $\mathcal{T}$ is obtained by starting at the root $\mathcal{o}$ and moving to the center of $\tau'$ for each instance of $\mathcal{o}\in\tau\prec_n\tau'\prec_{n+1}\mathcal{T}$ where $\tau$ is apocentric in $\tau'$.  Let $k_n$ be the sequence for the terms of which we have $\mathcal{o}\in \tau\prec_{k_n}\tau'\prec_{k_n+1} \mathcal{T}$ and $\tau$ is central in $\tau'$. 
Then $\mathcal{o}$ emits another ray $R_2$ disjoint from $R_1$ if and only if for each $k_n$ there exists a copy $\tau_n\prec_{k_{n+1}}\mathcal{T}$ that is attached to an apocentric leaf of a copy centered at $\mathcal{o}$ \TODO. 
This implies that the average number of such rays is  $\mathcal{R}:=\prod_{n=1}^{\infty}\frac{\delta_{k_n}}{\prod_{m=k_{n-1}}^{k_n-1}\delta_m}$. Suppose that $\delta_n>1$ for every $n>~c$. 
Using \cref{res:types_of_limits}, we have $\delta_n=o(n^2)$ and we observe that $\frac{k_n^2}{2^{k_n-n-c}}$ is eventually an upper bound for the partial products of $\mathcal{R}$. Additionally, define $t(n):=\max\{t\in \NN_0|k_t\leq n\}$ and note that the sequence $X_n:=t(n)-\frac{n}{2}$ is a supermartingale. Since $X_{k_n}=n-\frac{k_n}{2}$, by Azuma's inequality, $P(n-\frac{k_n}{2}>\frac{k_n}{2}-3\log k_n-c)\leq e^{-\frac{2(\frac{k_n}{2}-3\log k_n-c)^2}{\frac{k_n}{4}}}\leq e^{-\frac{k_n}{2}}$. Since $\sum_{n=1}^{\infty}e^{-\frac{k_n}{8}}<\infty$, by the Borel-Cantelli Lemma it \as\ eventually holds that $n\leq k_n-3\log k_n-c$ for every $n$, implying that $\mathcal{R}\leq\lim_{n\rightarrow \infty}\frac1{k_n}=0$. Therefore, \as\ no such rays exist, and we have that $\mathcal{T}$ is 1-ended. 

    \end{myenumerate}

\end{proof}

%This observation reveals the structure of $\mathcal{T}$: it is a tree that we obtain by modifying \cref{constr:T_n} so that, for each $n\in \NN$, $T_n$ is identified with an apocentric copy of $T_{n+1}$. For instance, the generalised canopy tree for \cref{ex:loglogr} would look as follows: 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.43\textwidth]{img/canopy_3.pdf}
    %\includegraphics[width=0.8\textwidth]{img/canopy_2.pdf}
    %\includegraphics[width=0.6\textwidth]{img/canopy.pdf}
    \caption{A figure that perhaps needs work.}
\end{figure}

%Types can also apply to the vertices of the limit $(\mathcal{T}, \mathcal{o})$ of a converging subsequence $(T_{n_k},o_{n_k})$ in the obvious manner. It is an easy exercise to prove that the root $\mathcal{o}$ will be of the same type as $o_{n_k}$. Since every vertex of $\mathcal{T}$ lies at a finite distance from $\mathcal{o}$, all of $V(\mathcal{T})$ agrees in type with $\mathcal{o}$. Therefore, the type of the underlying tree $\mathcal{T}$ is well-defined. 

%Note that the tree of \cref{constr:T_n} is completely central, whereas the eventually apocentric trees are exactly the generalized canopy trees.    

%Finally, on the antipode from generalised canopy trees sits the limit tree of \cref{constr:T_n}, which can be similarly obtained as the limit of an eventually central sequence. However, due to the fact that any ball of fixed radius around the centre of a tree $T_n$ must be finite, whereas the trees $T_n$ grow arbitrarily large, we deduce that almost no unbiased sequences $(\mathcal{T}_n, \mathcal{o}_n)$ are eventually central.   

%We are now sufficiently equipped to explore the structure of the limit tree $(\mathcal{T},\mathcal{o})$. The following structure theorem describes the structure of $(\mathcal{T},\mathcal{o})$ depending on the sequence $\delta_1,\delta_2,\delta_3...\in\NN$ that generates it.

%We have demonstrated that every fast-growing nice function is the growth function of a random rooted generalized canopy tree, given as a limit of a subsequence of $(T_n,o_n)$. In fact, even the following is true:

%\begin{theorem}
    %If $\delta_{n+1}\geq e^{\frac{\alpha}{n}}\delta_n-1$ eventually for some $\alpha>1$ (which again implies a minimum growth of at least around $r^{\alpha \log\log r}$), then the very sequence $T_n$ converges to $\mathcal{T}$ (rather than merely a subsequence). 
%\end{theorem}

%\begin{proof}
 %Indeed, for $\mathcal{B}$ an isomorphism class of rooted balls of radius $r$, take $m\gg\log r$ and let $c$ be the density of $\mathcal{B}$ in $T_m$. Then in $T_{m+1}$, only the vertices that are $r$-close to the apocentric leaves of the central copy of $T_m$ may see changes in their respective $r$-balls. Suppose that there exist $\kappa$ such vertices and let $\lambda:=\frac{\kappa}{\prod_{k=1}^{m+1}(\delta_k+1)}$. Then the density of $\mathcal{B}$ in $T_{m+1}$ lies between $c-\lambda$ and $c+\lambda$. In general, the density of $\mathcal{B}$ in $T_n$, $n>m$ is between $c-\lambda(\sum_{k=m+1}^{n-1}\prod_{j=m+1}^k\frac{\delta_j}{\delta_{j+1}+1})$ and $c-\lambda(\sum_{k=m+1}^{n-1}\prod_{j=m+1}^k\frac{\delta_j}{\delta_{j+1}+1})$. Under the assumption, it is straightforward to show that the sequence $\sum_{k=m+1}^{n-1}\prod_{j=m+1}^k\frac{\delta_j}{\delta_{j+1}+1}$ converges, so that the density of $\mathcal{B}$ converges absolutely.  
%\end{proof}

 Depending on the circumstances, our knowledge about the structure of $(\mathcal{T},\mathcal{o})$ can be even more precise; in fact, as seen in the following example, there exists a particular choice of the sequence $\delta_n$ for which the Benjamini-Schramm limit of $(\mathcal{T}_n,\mathcal{o}_n)$ is supported on a single deterministic tree. Note that, once again, this felicitous situation requires fast growth; since the support of a balanced tree is uncountable, and it only contains rooted trees on countable vertices, it cannot, in particular, only contain rooted trees all of which have the same underlying tree.  

%\msays{I tried to make the example below rigorous, and while I succeeded in proving that the $T_n$ are very symmetric, as you can see, the argument exploded. I am experimenting with the proof in the sandbox \cref{res:symmetric_tree}.}

%\msays{To show that the symmetry of the $T_n$ leads to a deterministic unimodular tree it would be better to first finish the definition parts of this section, so that we know what we are working with.}

%\begin{example}\label{ex:deterministic}
%Define the sequence $\delta_0,\delta_1,\delta_2,...$ with initial terms $\delta_0\ge 1,\delta_1\geq 2$ and recurrence $\delta_{n+1}:=\delta_n\delta_{n-1}$.
%In explicit form this yields
%
%$$\delta_n=\delta_0^{\smash{F_{n-1}}}\delta_1^{\smash{F_{n}}},\quad\text{for $n\ge 2$},$$
%
%where $F_n$ is the $n$-th Fibonacci number starting with $F_0=F_1=1$. 

%Let $T_n, n\in \NN_0$ be the trees constructed from this sequence as in \cref{constr:tree}.
%Since $\delta_{n+1} =\delta_n\delta_{n-1}\le \delta_n^2$ for $n\ge 2$, the sequence satisfies \cref{res:conditions_in_d} \itm1 and \cref{thm:main} yields uniform volume growth for the limit tree $T:=\bigcup_n T_n$.

%For $\bar g(2^n)=(\delta_0+1)\cdots(\delta_n+1)$, one can verify that 
%
%\msays{I don't remember how I came to these estimates. Should be checked.}
%
%\[b^{r^\alpha-\frac{\log r}{2}} \leq \bar g(r)\leq (\delta_0+1)rb^{(r^\alpha+\frac{1}{2})\log r}\!\!,\] \[\quad\text{with $b=(\delta_0^{1/\varphi}\delta_1)^{1/\sqrt{5}}\gtrsim 1.363$ and $\alpha=\log\varphi \approx 0.694$},\]
%
%where $\varphi\approx 1.618$ is the golden ratio. In particular, $T$ is of intermediate growth.

%It remains to verify that the Benjamini-Schramm limit of the sequence of $T_n$ is supported on a single tree.
%The key  observation is that the $T_n$ are very symmetric, in that they are transitive on their apocentric copies of $T_k$, for any $k\le n$. 
%More precisely, for any two apocentric copies $\tau_1,\tau_2\subset T_n$ of $T_k$, there is an automorphism $\phi\in\Aut(T_n)$ that fixes the root of $T_n$ and sends $\phi(\tau_1)=\tau_2$.
%This is clear for $T_0$ and $T_1$.
%Suppose that it is proven for $T_0,...,T_n$, then we can prove it for $T_{n+1}$:
%observe first that $\delta_{n+1}=\delta_n\delta_{n-1}$ is exactly the number of apocentric copies of $T_{n-2}$ in $T_n$.
%That is, by maximal uniform distribution of adjacencies, each apocentric copy of $T_{n-2}$ in the central $T_n\subset T_{n+1}$ is adjacent to \emph{exactly one} apocentric copy of $T_n$ in $T_{n+1}$. The unique vertex of each $T_{n-2}$ participating in this \enquote{outwards adjacency} will be called the \emph{outwards vertex}.
%Let now $\tau_1,\tau_2\subset T_{n+1}$ be two apocentric copies of $T_k,k\le n+1$ in $T_{n+1}$.
%The existence of an appropriate symmetry is clear when $k=n+1$, so let us assume $k<n+1$.
%Let $T_n(\tau_i)$ be the apocentric copy of $T_n$ that contains $\tau_i$, let $v_i$ be the outwards vertex in the central copy $T_n\subset T_{n+1}$ adjacent to $T_n(\tau_i)$, and let $T_{n-2}(v_i)$ be its containing copy of $T_{n-2}$, which is apocentric in the central $T_n\subset T_{n+1}$.
%By induction assumption there exists a symmetry $\phi_1\in\Aut(T_n)$ of the central $T_n\subset T_{n+1}$ that sends $T_{n-2}(v_1)$ onto $T_{n-2}(v_2)$. 
%Also by induction assumption, any apocentric copy of $T_{n-2}$ in $T_n$ is transitive on its apocentric vertices, and so we can modify $\phi_1$ into a symmetry $\phi_2\in\Aut(T_n)$ that sends outwards vertices to outwards vertices. 
%This then allows us to extend $\phi_2$ to a symmetry $\phi_3\in\Aut(T_{n+1})$.
%This symmetry necessarily sends $T_n(\tau_1)$ to $T_n(\tau_2)$. By induction assumption $T_n(\tau_2)$ is transitive on its apocentric copies of $T_k$, and so we can modify $\phi_3$ into a symmetry $\phi_4\in\Aut(T_{n+1})$ that sends $\tau_1$ onto $\tau_2$. All involved symmetries clearly fix the root of $T_{n+1}$.

%The upshot of this is: up to isomorphism of rooted graphs there exists a unique rooted tree $(T_n,r)$ with root $r$ at an apocentric vertex.

%If we identify $T_n$ with an apocentric copy of $T_n$ in $T_{n+1}$ we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset \cdots$ whose limit tree $T:=\bigcup_n T_n$ is a generalized canopy tree. Note that because of symmetry, the identification of $T_n$ with a sub-tree of $T_{n+1}$ involved no choice, and so $T$ is the unique limit tree obtainable by this procedure.

\begin{comment}
From this construct trees $T_n$ according to \cref{constr:T_n}, but as before, identify $T_{n-1}$ with an \emph{apocentric copy} in $T_n$. The sequence $(T_n,x^*)$ is then completely apocentric and the limit tree $T:=\bigcup_n T_n$ is a generalized canopy tree.

To see this for $T_{n+1}$, note that $\delta_{n+1}=\delta_n\delta_{n-1}$ is exactly the number of apocentric copies of $T_{n-2}$ in $T_n$. By maximal uniform distribution of adjacencies, we find that each apocentric copy of $T_{n-2}$ in the central copy $T_n$ in $T_{n+1}$ is adjacent to exactly one apocentric copy of $T_n$ in $T_{n+1}$.
That is, up to isomorphism of rooted graphs, there is a unique rooted tree $(T_n,x^*)$, where $x^*$ is apocentric.

Note that the sequence $\delta_0,\delta_1,\delta_2,...$ satisfies \cref{res:conditions_in_d} \itm1 and $T$ is thus of uniform growth (by \cref{thm:main}).
According to \cref{res:types_of_limits} the Benjamini-Schramm limit of (some sub-sequence of) the sequence $(T_n,x^*)$ is a generalized canopy tree, and we claim that this is exactly $T$.

Let $(T_n,x^*)$ be the completely apocentric sequence, where the trees $T_n$ are constructed from the sequence $\delta_0,\delta_1,\delta_2,...$ according to \cref{constr:tree}.


Construct trees $T_n$ according to \cref{constr:tree}, but as before, consider $T_{n-1}$ as an apocentric copy in $T_n$. The limit $T:=\bigcup_n T_n$ is then a generalize canopy tree.
We show that also the Benjamini-Schramm limit of $(T_n,x^*)$ (where $x^*$ is 

By \cref{res:conditions_in_d} and \cref{thm:main}, the tree $T$ constructed according to the sequence $\delta_n$ has uniform growth. In particular, for the growth $g(r)$ of $T$ we have $g(r)\sim A^{r^\alpha}$ with~$A=(\delta_0^{1/\phi}\delta_1)^{1/\sqrt{5}}\ge 1.6513...$ and $\alpha=\log\phi = 0.6942...$\,, therefore the growth of $T$ is intermediate. 

In particular, $g(r)=\Omega(r^{a\log \log r})$, so that the Benjamini-Schramm limit of the sequence $T_i$ is a random rooted generalised canopy tree with an a.s. eventually apocentric root. Since \cref{constr:tree} dictates that at step $n$ we distribute the apocentric copies of $T_{n-1}$ over the apocentric vertices of the central copy as uniformly as possible, and the function $\delta_n$ has been chosen so that exactly one apocentric copy of $T_{n-1}$ can be glued to each apocentric copy of $T_{n-2}$ in the central copy of $T_{n-1}$, all of the apocentric vertices in each step have identical neighbourhoods of each order. Thus, the Benjamini-Schramm limit of the $T_i$ is indeed supported on a single tree.   
\end{comment}
%\end{example}

\begin{example}\label{ex:deterministic}
Define recursively $\delta_1:=1,\delta_2:=2$ and $\delta_{n+1}:=\delta_n\delta_{n-1}$.
In explicit form this reads
%
$$\delta_n=2^{F_n}, \quad\text{for all $n\ge 0$},$$
%
where $F_n$ denotes the $n$-th Fibonacci number starting with $F_1=0, F_2=1$. 

%Let $T=T(\delta_1,\delta_2,\delta_3,...)$ be the tree according to \cref{constr:T}.
%Let $T_n$ for $n\ge 0$ be the trees according to \cref{constr:T_n}.
%The sequence~is~BS-convergent to a unimodular tree $\mathcal T$.
Since $\delta_{n+1} =\delta_n\delta_{n-1}\le \delta_n^2$ for $n\ge 2$, the~sequence satisfies \cref{res:conditions_in_d} \itm1, and \cref{unimain} yields that $(T_n,o_n)$ converges in the Benjamini-Schramm sense to a random rooted tree $(\mathcal T,\mathcal{o})$ that is \as\ of uni\-form volume growth.
%
%Since $\delta_n$ is unbounded, the volume of $T$ grows super-polynomially.
%One can~furthermore verify that $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ approximates $g(2^n)$ where
From $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ one can estimate
%
$$\tfrac12 D^{r^\alpha}\!\! \le |T_n|\le \tfrac 12r\cdot D^{r^\alpha}\!\!\!,\;\;\text{with $D:=2^{\varphi^2/\sqrt 5}\approx 2.251$ and $\alpha:=\log\varphi\approx 0.6942$}.$$
%
Here $\varphi\approx 1.618$ denotes the golden ratio.
The growth is therefore \emph{intermediate}.
\end{example}

We claim that $(\mathcal T, \mathcal{o})$ is supported on a single underlying tree: by \cref{res:types_of_limits} $(\mathcal T,\mathcal{o})$ is a generalized canopy tree, \ie\ supported on apocentric limits.
But as we show below (\cref{res:highly_symmetric}), the $T_n$ are highly symmetric in~that any two apocentric copies $\tau,\tau'\prec_{n-1} T_n$ are in fact indistinguishable by symmetry. 
In consequence, there exists (up to symmetry) only one apocentric inclusion chain, and $\mathcal T$ is supported on the unique tree obtained as its limit.

In the following we establish the symmetry of $T_n$ in an even stronger form:

%As we shall see, this is because the $T_n$ are~highly symmetric, and the BS-limit therefore \enquote{has no choice} but to converge to one single tree.
%We characterize the symmetry of $T_n$:

\begin{lemma}\label{res:highly_symmetric}
%If $\delta_{n+1}=\delta_{n-1}\delta_n$ for $n\ge 1$, then 
With the sequence of \cref{ex:deterministic} the trees $T_n$ are transitive on~apocentric copies $\tau\prec_m T_n$ for each $m\le n$, \ie\ for any two apocentric copies $\tau_1,\tau_2\prec_m T_n$ there is a symmetry $\phi\in\Aut(T_n)$ sending $\phi(\tau_1)=\tau_2$.
\end{lemma}

\begin{proof}
The proof is by induction on $n$. The cases $n\in\{0,1\}$ are trivially verified~and form the induction basis. Suppose that the statement is proven up to some $n\ge 1$; we prove the statement for $T_{n+1}$.

Let $\tau_0\prec_n T_{n+1}$ denote the central copy, and let $\tau_1,...,\tau_{\delta_{n+1}} \prec_n T_{n+1}$ denote the apocentric copies.
%
From our specific choice of sequence follows that the apocentric copies $\prec_n T_{n+1}$ are in one-to-one relation with the apocentric copies $\prec_{n-2} \tau_0$: by the \enquote{maximally uniform distribution of adjacencies} (\cf\ \cref{rem:max_uniform}, especially~equation \eqref{eq:max_uniform}) the expected number of \enquote{outwards adjacencies} of an apocentric copy $\hat\tau\prec_{n-2}\tau_0$ is exactly
$$
\frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
= \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
$$
%
In other words, there are exactly $\delta_{n+1}$ apocentric copies $\hat\tau_1,...,\hat\tau_{\delta_{n+1}}\prec_{n-2} \tau_0$ and they are in one-to-one relation with the $\tau_i$.
We can assume an enumeration so that $\hat\tau_i$ and $\tau_i$ are connected by an edge, its end in $\hat\tau_i$ we call $x_i$. %and that $x_i\in\hat\tau_i$ is the \enquote{outwards vertex} adjacent to $\tau_i$.

Fix two apocentric copies $\rho_1,\rho_2\prec_m T_{n+1}$ for some $m\le n+1$.
The goal is to construct a symmetry of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$. 

Let $i_k\in\NN$ be indices so that $\rho_k\prec_m \tau_{i_k}$.
%
By induction hypothesis there is a symmetry $\phi_0\in\Aut(\tau_0)$ that maps $\hat\tau_{i_1}$ onto $\hat\tau_{i_2}$. More generally, $\phi_0$ permutes the trees $\hat\tau_1,...,\hat\tau_n$, that is, $\phi_0$ sends $\hat\tau_i$ onto $\hat\tau_{\sigma(i)}$ for some permutation $\sigma\in\Sym(n)$.
It holds $\sigma(i_1)=i_2$.
Note however that $\phi_0$~does not necessarily map $x_i$ onto $x_{\sigma(i)}$. %\enquote{outwards vertices} onto \enquote{outwards vertices}.
We can fix this: invoking the induction hypothesis again, for each $i\in\{1,...,n\}$ exists a symmetry $\phi_1^i\in\Aut(\hat\tau_i)$ that sends $\phi_0(x_i)$ onto $x_{\sigma(i)}$. The map
%
$$
\phi_2(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
is then a symmetry of $\tau_0$ that sends the pair $(\hat\tau_i,x_i)$ onto $(\hat\tau_{\sigma(i)},x_{\sigma(i)})$.
Having this, $\phi_2$ extends to a symmetry $\phi_3\in\Aut(T_{n+1})$ that necessarily sends $\tau_i$ onto $\tau_{\sigma(i)}$.
In particular, it sends $\tau_{i_1}$ (which contains $\rho_1$) onto $\tau_{i_2}$ (which contains $\rho_2$).
As before, $\phi_3$ does not necessarily send $\rho_1$ onto $\rho_2$ right away; but also as before, this can be fixed: by induction hypothesis there is a symmetry $\phi_4\in\Aut(\tau_{i_2})$ that sends $\phi_3(\rho_1)$ onto $\rho_2$. The map
%
$$
\phi_5(x):=\begin{cases}
(\phi_4\circ\phi_3)(x) & \text{if $x\in \tau_{i_1}$} \\
\phi_3(x) & \text{otherwise}
\end{cases}.
$$
is a symmetry of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$.
\end{proof}

% \begin{theorem}
%     $\mathcal T$ is deterministic.
% \end{theorem}

% \begin{proof}
%     Since $\delta_n=\Omega(n)$, $\mathcal T$ is a generalized canopy tree, \ie\ $\mathcal T$ is supported exactly on the limits of completely apocentric inclusion chains (\cf\ \cref{rem:general_limit_growth}).
%     Note however that up to symmetry there is only one such chain: since $T_{n+1}$ is transitive on its apocentric copies $\prec_{n} T_{n+1}$, there is (up to symmetry) no choice for the apocentric identification $T_n\subset T_{n+1}$. 
%     Since there is no choice involved, $\mathcal T$ is supported on a single tree.
% \end{proof}

Unimodular random rooted trees with a deterministic underlying tree of even smaller uniform growth can be construct\-ed by choosing $\delta_{n+1}:=\delta_n\delta_{n-1}$ only for some $n$, and $\delta_{n+1}:=\delta_n$ otherwise.
However, since the support of BS-limits from slow growing sequences is necessarily~uncountable, there is a limit to this approach and one might wonder:

\begin{question}
    Can a deterministic tree of uniform growth, say, $g\in O(r^{\log\log r})$ be unimodular?
\end{question}

%A slight modification of the above example in which we define $\delta_{n+1}:=\delta_n\delta_{n-1}$ for some $n$, and $\delta_{n+1}:=\delta_n$ for others, yields deterministic unimodular random trees of a wide range of uniform volume growth above $r^{\log\log r}$.

\newpage


\section{Conclusions and open questions}
\label{sec:last}

\subsection{Planar triangulations}

Planar triangulations of an unexpected uniform volume growth $\sim r^4$ have previously been observed in physical context \cite{angel2003growth,ambj1997quantum}.
This was generalized to $\sim r^\alpha$ for any $\alpha\ge 1$ in \cite{benjamini2011recurrence} by observing that any tree $T$ of maximum degree $\bar \Delta$ can be turned into a planar triangulation with the same grwoth behavior: fix a triangulated sphere with at least $\bar\Delta$ pairwise disjoint triangles. Take a copy of this sphere for each vertex of $T$ and glue two spheres along a triangle when the associated vertices are adjacent. 

Having established the existence of trees for a variety of growth rates, we can likewise conclude the existence of planar triangulations with the same wide range of growth behaviors.

But we can say even more: previously known triangulations of polynomial growth are planar, but not necessarily triangulations of the plane, \ie\ they are not necessarily homeomorphic to $\RR^2$. For this to be true, one needs the tree $T$ to be \emph{one-ended}.
Going back to \cref{constr:T} and instead associating $T_n$ with some \emph{apocentric copy} $\prec T_{n+1}$ instead of the central copy, we obtain a one-ended limit tree $T'$. 
From this we obtain triangulations of the plane for a wider range of growth behaviors.
%The same analysis \cref{thm:main} of the growth behavior applies to this tree and so we obtain triangulations of the plane with arbitrary uniform growth.

\subsection{Future research}

Having shown that trees of intermediate growth exist and that their growth can be determined at high granularity, the next natural step is to identify such trees in other objects. As discussed in Section 2, the trees of \cref{constr:tree} occasionally span graphs which are ``typical'' for their growth. It would be interesting to determine whether this is by necessity:

\begin{question} \label{quest1}
Let $G$ be a graph of uniform growth $g(r)$. Is there a tree embedded in $G$ with the same uniform growth? In particular, is there a spanning tree of $G$ with the same uniform growth? 
\end{question}

This is more general than requesting a tree quasi-isometric to $G$. Indeed, although quasi-isometry implies agreement of growth (up to a multiplicative constant), one can construct a counterexample to the converse by taking a set of cycles of unbounded length and connecting them serially with edges. Then $G$ is a homeomorphic image of the double ray with fibers of size at most $2$ and therefore has linear growth, but $G$ has infinite perimeter, hence no quasi-isometric spanning trees. 

\begin{center}
    \includegraphics[width=0.65\textwidth]{img/chain_of_cycles}
\end{center}

%\msays{The subsequent paragraph is not true. An affirmative answer to Question 6.1 shows the existence of intermediate growth trees, but does not prove Theorem 3.4.}

Observe that \cref{quest1}, if proven true, would immediately imply the existence of trees of intermediate volume growth by considering, for instance, an appropriate spanning tree of the Grigorchuck Cayley graph.

Weaker versions of \cref{quest1} may also be interesting:

\begin{question}
Let $G$ be a graph of uniform growth $g(r)$. Does every graph $G$ have a planar subgraph with the same uniform growth? What about subgraphs from other minor-closed families?
\end{question}

Or even:

\begin{question}
Let $G$ be a graph with uniform growth $g(r)$. Is there some $k\in\mathbb{N}$, perhaps dependent on $g(r)$, such that $G$ has a subgraph which is not $k$-connected and has the same uniform growth?  
\end{question}

%\msays{Potential open question: is there a unimodular deterministic tree of intermediate volume growth below, say, $\exp(\sqrt n)$ or even $\exp(n^{o(1)})$?}

%\msays{We can probably find all kind of feasible growth behaviors: just define the sequence of $\delta_i$ to sometimes satisfy $\delta_{n+1}=\delta_n\delta_{n-1}$, and sometimes just $\delta_{n+1}=\delta_n$, see also \cref{res:symmetric_tree}.}





\begin{comment}
\msays{This section is just a bunch of experiments. Can be ignored}

%\section{Some interesting properties of $T(\delta_0,\delta_1,...)$}
\section{Some experiments}

The following function will play a central role in our investigation of $T$:

$$\Delta(n):=\frac{\delta_{n}}{\delta_0\cdots\delta_{n-1}}.$$

\begin{proposition}
Among the apocentric vertices of $T_n\subset T$, the average \resp\ maximum degree is $\Delta(n+1)+1$ \resp $\lceil\Delta(n+1)\rceil + 1$.

In particular, the maximum degree of $T$ is $\displaystyle\sup_n\lceil\Delta(n)\rceil + 1$.
\begin{proof}
\TODO
\end{proof}
\end{proposition}

\begin{proposition}
If $\delta_{n+1}\le \delta_0\cdots\delta_{n}$, then all vertices of $T$ have degree $1$, $2$, $\delta_0$ or $\delta_0+1$, where if $\delta_0\not=1$, then the only vertex with degree $\delta_0$ s the global root. %If we smooth vertices of degree $2$, then the resulting tree has only two possible vertex degrees, while the growth behavior changes at most by a factor of 2.
%
\begin{proof}
\TODO
\end{proof}
\end{proposition}

The next theorem shows that the rule of maximally uniform distribution~of~ad\-ja\-cen\-cies can lead to highly symmetric trees if the sequence of $\delta_i$ is chosen appropriately. 

% \begin{theorem}
% Fix $N\ge 0$. If $\delta_0\ge1$, $\delta_1 = \kappa\delta_0$ $($for some $\kappa\ge 1)$ and for all $n\in\{1,...,N\}$ holds either
% %
% $$\delta_{n+1}=\delta_n\delta_{n-1}\cdots\delta_{s(n)},$$
% %
% then $T_N$ is transitive on apocentric copies of $T_k$ for each $k\le N$. That means that for any two apocentric copies $\tau_1,\tau_2\subset T_N$ of $T_k$ exists a symmetry $\phi\in\Aut(T_N)$ that sends $\phi(\tau_1)=\tau_2$.
% \end{theorem}

\begin{theorem}\label{res:symmetric_tree}
Fix $N\ge 0$. If for each $n\in\{0,...,N-1\}$ holds either
\begin{myenumerate}
    \item $\delta_{n+1}=\delta_n\delta_{n-1}\cdots\delta_{s(n)}$ for some $s(n)\ge 0$, or
    %for some $K(n)\ge 1$ and $s(n)\le n$, or
    \item $\delta_{n+1}=K(n)\cdot \delta_n\delta_{n-1}\cdots\delta_0$ for some $K(n)\ge 1$,
    %
    %for some $K(n)\ge 1$, 
\end{myenumerate}
%
then $T_N$ is transitive on apocentric copies of $T_k\subset T_N$ for each $k\le N$.
That means that for any two apocentric copies $\tau_1,\tau_2\subset T_N$ of $T_k$ there is an automorphism~$\phi\in\Aut(T_N)$ that sends $\phi(\tau_1)=\tau_2$.
\end{theorem}

Some of the previously discussed examples are instances of \cref{res:symmetric_tree}. This includes constant sequences $\delta_n=c$, which lead to polynomial growth; and $\delta_0:=2$, $\delta_{n+1}:=\delta_0\cdots\delta_n=2^{2^n}$\!, which leads to exponential growth. 
The simplest instance resulting in intermediate growth is perhaps $\delta_0:=1, \delta_1:=2$, $\delta_{n+1}:=\delta_n\delta_{n-1}$, which expands to
%
$$\delta_n=2^{F_n},$$
%
where $F_n$ is the $n$-th Fibonacci number, starting with $F_0=0, F_1=1$.

\begin{proof}[Proof of \cref{res:symmetric_tree}]
We prove the statement by induction in $N$. The statement is clearly true for $N=0$.

Assume that the statement is proven up to some $N-1$ and that \itm1 \resp\ \itm2 holds for each $n\in\{1,...,N\}$.
Fix some $k\le N-1$ (the statement is trivial for $k=N$) and choose apocentric copies $\tau_1,\tau_2\subset T_N$ of $T_k$.
We construct the symmetry $\phi\in\Aut(T_N)$ that sends $\phi(\tau_1)=\tau_2$.
We consider two cases depending on whether $\delta_N$ falls in case \itm1 or \itm2.

\emph{Case \itm1}:
note that $\delta_n\cdots\delta_{s(n)}$ is exactly the number of apocentric copies of $T_{s(n)-1}$ in $T_N$. 
By the maximal uniform distribution of the adjacencies we find that in case \itm1 each of these copies of $T_{s(n)-1}$ in the central $T_N\subset T_{N+1}$ has therefore \emph{exactly one} \enquote{outwards adjacencies} to an apocentric $T_N\subset T_{N+1}$.

\TODO
\end{proof}


\newpage

Consider the recursively defined sequence of integers $\delta_0:=1$, $\delta_1:=2$ and~$\delta_{n+1}:=\delta_{n-1}\delta_n$.
Let $T_n,n\ge 0$ be the corresponding sequence of trees from \cref{constr:T_n}. 

\begin{lemma}
%If $\delta_{n+1}=\delta_{n-1}\delta_n$ for $n\ge 1$, then 
Each $T_n$ is transitive on apocentric copies $\tau\prec_m T_n$ for each $m\le n$, \ie\ for any two apocentric copies $\tau_1,\tau_2\prec_m T_n$ there is a symmetry $\phi\in\Aut(T_n)$ sending $\phi(\tau_1)=\tau_2$.
%
\begin{proof}
The proof is by induction on $n$. The cases $n\in\{0,1\}$ are trivially verified~and form the induction basis. Suppose that the statement is proven up to some $n\ge 1$; we prove the statement for $T_{n+1}$.

Let $\tau_0\prec_n T_{n+1}$ denote the central copy, and let $\tau_1,...,\tau_{\delta_{n+1}} \prec_n T_{n+1}$ denote the apocentric copies.
%
By our specific choice of sequence we find that the apocentric copies $\prec_n T_{n+1}$ are in one-to-one relation with the apocentric copies $\prec_{n-2} \tau_0$.\nlspace
In fact, by the \enquote{maximally uniform distribution of adjacencies} (see \cref{rem:max_uniform}, especially equation \eqref{eq:max_uniform}) we find that the expected number of \enquote{outwards adjacencies} of an apocentric copy $\hat\tau\prec_{n-2}\tau_0$ is exactly
$$
\frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
= \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
$$
%
Thus, there are exactly $\delta_{n+1}$ apocentric copies $\hat\tau_1,...,\hat\tau_{\delta_{n+1}}\prec_{n-2} \tau_0$ with $\hat\tau_i$ being adjacent to $\tau_i$. Let $x_i\in\hat\tau_i$ be the \enquote{outwards vertex} adjacent to $\tau_i$.

Fix two apocentric copies $\rho_1,\rho_2\prec_m T_{n+1}$ for some $m\le n+1$.
The goal is to find a sequence of symmetries of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$. Let $i_k\in\NN$ be so that $\tau_{i_k}$ contains $\rho_k$.

By induction hypothesis there is a symmetry $\phi_0\in\Aut(\tau_0)$ that maps $\hat\tau_{i_1}$ onto $\hat\tau_{i_2}$. More generally, $\phi_0$ permutes the trees $\hat\tau_1,...,\hat\tau_n$, that is, $\phi_0$ sends $\hat\tau_i$ onto $\hat\tau_{\sigma(i)}$ for some permutation $\sigma\in\Sym(n)$.
It holds $\sigma(i_1)=i_2$.
Note however that $\phi_0$~does not necessarily map \enquote{outwards vertices} onto \enquote{outwards vertices}.
We can fix this: invoking the induction hypothesis again, for each $i\in\{1,...,n\}$ exists a symmetry $\phi_1^i\in\Aut(\hat\tau_i)$ that sends $\phi_0(x_i)$ onto $x_{\sigma(i)}$. The map
%
$$
\phi_2(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
is then a symmetry of $\tau_0$ that sends the pair $(\hat\tau_i,x_i)$ onto $(\hat\tau_{\sigma(i)},x_{\sigma(i)})$.
Because of this, $\phi_2$ actually extends to a symmetry $\phi_3\in\Aut(T_{n+1})$ that necessarily sends $\tau_i$ onto $\tau_{\sigma(i)}$.
In particular, it sends $\tau_{i_1}$ (which contains $\rho_1$) onto $\tau_{i_2}$ (which contains $\rho_2$).
As before, $\phi_3$ does not necessarily send $\rho_1$ onto $\rho_2$ right away; but also as before, this can be fixed: by induction hypothesis there is a symmetry $\phi_4\in\Aut(\tau_{i_2})$ that sends $\phi_3(\rho_1)$ onto $\rho_2$. The map
%
$$
\phi_5(x):=\begin{cases}
(\phi_4\circ\phi_3)(x) & \text{if $x\in \tau_{i_1}$} \\
\phi_3(x) & \text{otherwise}
\end{cases}.
$$
is a symmetry of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$.
%
%
% Given an apocentric copy $\hat\tau\prec_{n-2}\tau_0$, how many edges emanate from $\hat \tau$ \enquote{outwards} to the apocentric copies $\tau_1,...,\tau_{\delta_{n+1}}$?
% %
% As it turns out, by our specific choice of sequence and by \enquote{maximally uniform distribution of adjacencies} there is always \emph{exactly one} such edge (\cf\ \cref{rem:max_uniform}, especially \eqref{eq:max_uniform}):
% %
% $$
% \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
% = \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
% $$
% %
% Each apocentric copy of $T_{n-1}$ in $\tau_0$ can therefore be denoted by $\hat\tau_i$, where the subscript 
%
% The apocentric copies $\hat\tau\prec_{n-2}\tau_0$ are therefore in one-to-one correspondence with the apocentric copies $\tau_i\prec_n T_{n+1}$.
% Let then $\hat\tau_i\prec_{n-2}\tau_0$ be the unique apocentric copy adjacent to $\tau_i$, and let $x_i\in\hat\tau_i$ be its \enquote{outwards vertex}.
%
%
% Let us fix an enumeration $\tau_1,...,\tau_{\delta_{n+1}}\prec_n T_{n+1}$ of the apocentric copies. We furthermore define
% %
% \begin{itemize}
%     \item $x_i\in\tau_0$, the \enquote{outwards vertex} adjacent to $\tau_i$, and
%     \item $\hat\tau_i\prec_{n-2} \tau_0$, the apocentric copy containing $x_i$.
% \end{itemize}
%
% For some $m \le n$ choose $\tau_i^m \prec_m \tau_i$.
% \Wlog\ the goal is to find a symmetry $\phi\in\Aut(T_{n+1})$ mapping $\phi(\tau_1^m)=\tau_2^m$.
%
%
%
%
% Note that $\delta_{n-1}\delta_n$ is exactly the number of apocentric copies of $T_{n-2}$ in $\tau_0$. By $\delta_{n+1}=\delta_{n-1}\delta_n$, this matches the number of apocentric copies of $T_n$ in $T_{n+1}$, and by maximally uniform distribution of adjacencies (\cf\ \cref{rem:max_uniform}) every apocentric copy $\tau\prec_{n-2}\tau_0$ contains a unique \enquote{outwards vertex}, that is, a vertex adjacent to an apocentric copy $\tau'\prec_n T_{n+1}$.
%
\iffalse

Fix two apocentric copies $\tau_1,\tau_2\prec_m T_{n+1}$ for some $m\le n+1$.
The goal is to find a sequence of symmetries of $T_{n+1}$ that send $\tau_1$ onto $\tau_2$.
%
We need to give names to some sub-structures of $T_{n+1}$:
%
\begin{itemize}
    \item let $\tau_0\prec_n T_{n+1}$ be the central copy of $T_n$
    in $T_{n+1}$.
    \item let $\tau_i^n \prec_n T_{n+1}$ be the unique apocentric copy of $T_n$ that contains $\tau_i$.
    \item let $x_i\in\tau_0$ be the apocentric vertex of $\tau_0$ that is adjacent to $\tau_i^n$.
    \item let $\hat \tau_i \!\prec_{n-2} \tau_0$ be the unique apocentric copy of $T_{n-2}$ in $\tau_0$ that contains $x_i$.
\end{itemize}

By induction hypothesis there is a symmetry $\phi_0\in\Aut(\tau_0)$ that maps $\hat\tau_1$ onto $\hat\tau_2$.
Note that $\phi_0$ not necessarily sends $x_1$ onto $x_2$.
We can fix this: by induction hypothesis there is also a symmetry $\phi_1\in\Aut(\hat\tau_2)$ that maps $\phi_0(x_1)$ onto $x_2$.
Then
%
$$
\phi_2(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
is a symmetry of $\tau_0$ and sends the pair $(\hat\tau_1,x_1)$ onto $(\hat\tau_2,x_2)$.


\par\medskip
Let $\tau_0\prec_n T_{n+1}$ denote the central copy.
We first note that each apocentric copy $\prec_{n-2}\tau_0$ has \emph{exactly one} \enquote{outwards adjacency} to an apocentric copy $\prec_n T_{n+1}$.
This follows from our special choice of sequence $\delta_{n+1}=\delta_{n-1}\delta_n$ and \enquote{maximally uniform distribution of adjacencies} (\cf\ \cref{rem:max_uniform} \eqref{eq:max_uniform}):
$$
\frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
= \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
$$

\sepline

Fix two apocentric copies $\tau_1,\tau_2\prec_m T_{n+1}$ for some $m\le n+1$, the goal is to find a symmetry $\phi\in\Aut(T_{n+1})$ sending $\phi(\tau_1)=\tau_2$. The statement is clear for $m=n+1$; so we assume $m\le n$. 
We give names to the following substructures:
%
\begin{itemize}
    %\item let $\tau_0\prec_n T_{n+1}$ be the central copy of $T_n$.
    \item let $\tau_i^n \prec_n T_{n+1}$ be the unique apocentric copy of $T_n$ that contains $\tau_i$.
    \item let $\hat x_i\in\tau_0$ be the apocentric vertex of $\tau_0$ that is adjacent to $\tau_i^n$.
    \item let $\hat \tau_i \!\prec_{n-2} \tau_0$ the unique apocentric copy of $T_{n-2}$ in $\tau_0$ that contains $\hat x_i$.
\end{itemize}

W.l.o.g.\ fix apocentric copies $\tau_1^m,\tau_2^m\prec_m T_{n+1}$, where 

The symmetry $\phi$ is build in multiple steps.
%
\begin{enumerate}
    \item 
By induction hypothesis there exists a symmetry $\phi_0\in\Aut(\tau_0)$ sending $\phi_0(\hat\tau_1)=\hat\tau_2$.
More generally, there is a permutation $\sigma\in\Sym(n)$ with $\phi_0(\hat \tau_i)=\hat \tau_{\sigma(i)}$. Note that $\phi_0$ not necessarily sends $x_i$ onto $x_{\sigma(i)}$, but onto $y_i:=\phi_0(x_i)\in\hat \tau_{\sigma(i)}$. 

    \item 
Invoking the induction hypothesis again, for each $i\in\{1,...,\delta_n\}$ there is a symmetry $\phi_1^i\in\Aut(\hat\tau_{\sigma(i)})$ sending $y_i$ onto $x_{\sigma(i)}$. From this we can build a symmetry $\phi_1\in\Aut(\tau_0)$:
%
$$
\phi_1(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
This symmetry now maps $\phi_1(x_i)=x_{\sigma(i)}$.
In particular, this symmetry now extends to a symmetry $\phi_2\in\Aut(T_{n+1})$ that maps $\phi_2(\tau_1)=\tau_2$.
However, it not necessarily sends $\tau_1^m$ to $\tau_2^m$, but only to $\tau_2^m':=\phi_2(\tau_2^m)$. Again, this can be fixed.

    \item
As before, we invoke the induction hypothesis to obtain a symmetry $\phi_3\in\Aut(\tau_2)$ that maps $\phi_3(\tau_2^m')=\tau_2^m$. 
This can be combined in the final symmetry $\phi\in\Aut(T_{n+1})$:
%
$$\phi(x):=\begin{cases}
(\phi_3\circ\phi_2)(x) & \text{if $x\in\tau_1$} \\
\phi_2(x) & \text{otherwise}
\end{cases}.$$
%
This symmetry maps $\phi(\tau_1^m)=\tau_2^m$.   

\end{enumerate}
%
This concludes the proof.
%
\fi
\iffalse
\sepline

% Let furthermore $\tau_0\prec_n T_{n+1}$ be the central copy.
% Let now $\tau_i^n \prec_n T_{n+1}$ be the unique apocentric copy that contains $\tau_i$, $x_i\in\tau_0$ the apocentric vertex of $\tau_0$ adjacent to $\tau_i^n$, and $\tau_i^m \prec_m \tau_0$ the unique apocentric copy that contains $x_i$.

By induction hypothesis we know that the following symmetries exist:
%
\begin{itemize}
    \item a symmetry $\phi_0\in\Aut(\tau_0)$ sending $\phi_0(\tau_1^{n-2}) = \tau_2^{n-2}$. Then $x_1':=\phi_0(x_1)$ is an apocentric vertex of $\tau_2^{n-2}$.
    \item a symmetry $\phi_1\in\Aut(\tau_2^{n-2})$ sending $\phi_1(x_1')=x_2$.
\end{itemize}
%
The following is then also a symmetry of $\tau_0$:
%
$$\phi_2(x):=\begin{cases}
\phi_0(x) & \text{if $x\not\in\tau_1^{n-2}$} \\
\phi_1\circ \phi_0(x) & \text{if $x\in\tau_1^{n-2}$}
\end{cases}.
$$
%
This symmetry sends the pair $(\tau_1^{n-2}\!,x_1)$ onto $(\tau_2^{n-2}\!, x_2)$.
%$\phi_2(\tau_1^m)=\tau_2^m$ and $\phi_2(x_1)=x_2$.

We now use that $\delta_{n+1}=\delta_{n-1}\delta_n$ is exactly the number of apocentric copies of $T_{n-2}$ in $\tau_0$. By the maximally uniform distribution of adjacencies, every apocentric copy $\tau\prec_{n-2} \tau_0$ therefore contains a unique \enquote{outwards vertex}, that is, a vertex adjacent to an apocentric copy of $T_n$ in $T_{n+1}$. Since $\phi_2$ sends an outwards


This now guarantees that $\phi_2$ extends to a symmetry $\phi_3\in\Aut(T_{n+1})$ sending $\phi_3(\tau_1^n)=\tau_2^n$. Then $\tau_1':=\phi_3(\tau_1)\prec_m \tau_2^n$ is an apocentric copy of $T_m$. Again, by induction hypothesis there exists 
%
\begin{itemize}
    \item a symmetry $\phi_4\in\Aut(\tau_2^n)$ sending $\phi_4(\tau_1')=\tau_2$.
\end{itemize}
%
As before, the following is then also a symmetry of $T_{n+1}$:
%
$$\phi(x):=\begin{cases}
\phi_3(x) & \text{if $x\not\in\tau_1$} \\
\phi_4\circ \phi_3(x) & \text{if $x\in\tau_1$}
\end{cases}.
$$
%
The symmetry $\phi\in\Aut(T_{n+1})$ sends $\tau_1$ onto $\tau_2$, which concludes the proof.
\fi
\end{proof}
\end{lemma}

\begin{theorem}
The distributional limit of the sequence $T_n$ is supported on a single tree.
%
\begin{proof}
\TODO
\end{proof}
\end{theorem}



\newpage







\newpage

\subsection{Unimodular trees supported on a single tree}

%A random rooted graph $\mathcal G$ is \emph{deterministic} if it is supported on a single tree.
%In other words, it is a usual (non-random) graph with merely a random choice of root.
%One might wonder whether a determi\-nistic tree of intermediate growth can be unimodular.
%The answer is affirmative as we demonstrated below.








\newpage

We say that a sequence $\delta_n$ is \emph{growing fast} if
%
$$\sum_{n=0}^\infty \frac1{\delta_n}<\infty,$$
%$$\prod_{n=0}^\infty \frac{\delta_n}{\delta_n+1}>0,$$
%$$\prod_{n=0}^\infty \frac{1}{1+1/\delta_n}>0,$$
%
otherwise we say it is \emph{growing slow}.
It turns out that this distinction is a crucial~deciding factor for the structure of the limit $$T_n\xrightarrow{\mathrm{BS}} \mathcal T.$$

\begin{remark}
    \msays{$\delta_n>n^\alpha$ with $\alpha>1$ grows fast, $\delta_n\in O(n)$ grows slow}
\end{remark}

\begin{remark}
    \msays{What does this mean in terms of $g$?}
\end{remark}

\newpage 
\end{comment}




\newpage

\appendix

\section{Existence and properties of $\gamma$}
\label{sec:gamma_properties}

Recall the function $\gamma\:\NN\to\RR$ introduced in the proof of \cref{res:conditions_in_g}, defined by $\gamma(1):=25$ and
%
\begin{equation}\label{eq:gamma}
 \gamma(\delta):=\prod_{k=0}^\infty \Big(1+\frac2{\delta^{2^k}}\Big)^{\!2},\quad\text{whenever $\delta\ge 2$}.   
\end{equation}
%
It is evident from the definition that $\gamma(\delta)> 1$. % and $\gamma$ is decreasing in its argument (except $\gamma(1)>\gamma(2)$, which is shown in \cref{res:gamma_bounds})
We show that it is well-defined:

\begin{lemma}\label{res:estimate_gamma}
$\gamma(\delta)$ is well-define, \ie\ the infinite product \eqref{eq:gamma} converges. % for $\delta\ge 2$.
%For $\delta\geq 2$, $\gamma(\delta):=\!\prod_{k\ge 0} \!\big(1+2 / \delta^{\kern0.1ex2^k} \big)^2\!$ converges.
%In particular, we have the following upper bounds: $\gamma(2)<12.33$, $\gamma(3)<5$, $\gamma(5)<4$, $\gamma(7)<3$, and $\gamma(9)<2$. %\nlspace
%
%$$
    %\gamma(2) \le 11.33 
    %\quad
    %\text{ and } 
    %\quad
    %\gamma(3) \le 5.
%$$
\end{lemma}

\begin{proof}
$\gamma(\delta)$ is the square of
 %
 \[
 \prod_{k=0}^\infty\Big(1+\frac{2}{\delta^{2^k}}\Big)
 =\sum_{i=0}^\infty\frac{2^{b(i)}}{\delta^i},
 \] 
 %
 where $b(i)$ denotes the number of 1's in the binary representation of $i$. Since $b(i)\leq \lfloor\log_2(i)\rfloor+1\leq \frac{i}{2}$ for $i\geq 10$, a geometric series estimation yields 
 %
 \begin{equation}\label{eq:gamma_upper_bound}
 \prod_{k=0}^\infty\Big(1+\frac{2}{\delta^{2^k}}\Big)
 \,\leq\, \sum_{i=0}^9\frac{2^{b(i)}}{\delta^i}
    +\sum_{\mathclap{i=10}}^\infty\frac{\sqrt 2^{\kern0.1ex i}}{\delta^i}
 \,\leq\, \sum_{i=0}^9\frac{2^{b(i)}}{\delta^i}
    +
    %\underbrace{
    %\frac{1}{32}\frac{\sqrt{2}}{\sqrt{2}-1}
    \frac{2+\sqrt 2}{32}
    %}_{\approx\, 0.106694...}
    ,
 \end{equation}
%
which is finite. 
%
%The given upper bounds can be easily verified.
\end{proof}

% \begin{align*}
% \begin{array}{rcl}
%     11 <& \!\! \gamma(2) \!\! &< 12 \\
%     4 <& \!\! \gamma(3) \!\! &< 5 \\
%     2 <& \!\! \gamma(4) \!\! &< 3
% \end{array}
% \end{align*}


\begin{corollary}\label{res:gamma_bounds}
The following bounds apply:
\begin{align*}
\arraycolsep=0.5ex
\begin{array}{rcccl}
9&<&\gamma(2)&<&25/2 \\
25/9&<&\gamma(3)&<&5.
\end{array}
\end{align*}
%
\begin{proof}
The upper bounds can be verified from the proof of \eqref{eq:gamma_upper_bound}.
%
The lower bounds follow via
\begin{align*}
\gamma(2) &> \Big(1+\frac2{2}\Big)^2\Big(1+\frac24\Big)^2 = 9, \\
\gamma(3) &> \Big(1+\frac23\Big)^2 = \frac{25}9.
\end{align*}
\end{proof}
\end{corollary}

\begin{corollary}\label{res:gamma_decreasing}
$\gamma(\delta)$ is strictly decreasing in $\delta$.
%
\begin{proof}
For $2\le \delta_1<\delta_2$ follows $\gamma(\delta_1)<\gamma(\delta_2)$ straight from the definition.
For~$\delta_1=1$ we use the bounds in \cref{res:gamma_bounds} and find
%
$\gamma(1) = 25 > 25/2 > \gamma(2).$
\end{proof}
\end{corollary}

\begin{proposition}\label{res:d_gamma_monotone}
$\delta^2\gamma(\delta)$ is strictly increasing for $\delta\ge 3$.
%
\begin{proof}
The function in question is the square of
%
$$f(\delta):=\delta \prod_{k=0}^\infty \Big(1+\frac2{\delta^{2^k}}\Big).$$
%
If we consider $\delta$ as a continuous parameter, we can compute the derivative of $\log f(\delta)$ \wrt\ $\delta$, which yields
%
$$(\log f(\delta))'=\frac1\delta - \frac2\delta\sum_{k=0}^\infty \frac{2^k}{\delta^{2^k}+2}.$$
%
For $\delta^2 \gamma(\delta)$ to be increasing, we require this expression to be positive, which, after some rearranging, is equivalent to
%
$$\sum_{k=0}^\infty\frac{2^k}{\delta^{2^k}+2}<\frac12.$$
%
The sum is clearly decreasing in $\delta$ and so it suffices to verify the case $\delta=3$:
%
\begin{align*}
\sum_{k=0}^\infty \frac{2^k}{3^{2^k}+2} 
&=\frac15+\frac29 + \sum_{k=2}^\infty \frac{2^k}{3^{2^k}+2}
\\&<\frac{21}{55} + \sum_{k=2}^\infty \frac{2^k}{3^{2^k}}
<\frac{21}{55} + \sum_{\ell=4}^\infty \frac{\ell}{3^{\ell}} = \frac{21}{55}+\frac1{12}<\frac12.
\end{align*}
\end{proof}
\end{proposition}

% \begin{lemma}\label{res:gamma_property_d_d2}
% For $\delta_1\le\delta_2$ holds $\delta_1\gamma(\delta_1)\le \delta_2^2\gamma(\delta_2)$.
% %
% \begin{proof}
% The statement is clear for $\delta_1=\delta_2$, so we assume $\delta_1<\delta_2$.
% We proceed by case analysis.
% We repeatedly invoke the bounds from \cref{res:gamma_bounds} as well as the monotonicity result \cref{res:d_gamma_monotone}, the latter we indicate by $(*)$.
% %
% \begin{enumerate}[label=(\arabic*),topsep=0.7em]
%     \item if $\delta_1\ge 3$, then
%     %
%     $$\delta_1\gamma(\delta_1)<\delta_1^2\gamma(\delta_1) \overset{\smash{(*)}}\le \delta_2^2\gamma(\delta_2).$$
    
%     \item if $\delta_1 = 2$, then $\delta_2\ge 3$ and 
%     %
%     $$\delta_1\gamma(\delta_1)=2\gamma(2) < 25 < 3^2\gamma(3) \overset{\smash{(*)}}\le \delta_2^2\gamma(\delta_2).$$
    
%     \item if $\delta_1 = 1$ and $\delta_2\ge 3$ then 
%     %
%     $$\delta_1\gamma(\delta_1)=1\gamma(1)= 25 < 3^2\gamma(3) \overset{\smash{(*)}}\le \delta_2^2\gamma(\delta_2).$$
    
%     \item if $\delta_1 = 1$ and $\delta_2 = 2$ then 
%     %
%     $$\delta_1\gamma(\delta_1)=1\gamma(1)= 25 < 36 < 2^2\gamma(2).$$
% \end{enumerate}
% \end{proof}
% \end{lemma}

The following property of $\gamma$ is used in the proof of \cref{res:conditions_in_g}.

\begin{lemma}\label{res:gamma_property_d_d2}
If $\delta_1\le(\delta_2+2)^2$ then $\delta_1\gamma(\delta_1)\le \delta_2^2\gamma(\delta_2)$.
%
\begin{proof}
We proceed by case analysis. A use of \cref{res:gamma_decreasing} (\ie\ $\gamma$ is decreasing) is indi\-cated by $(*)$, a use of \cref{res:d_gamma_monotone} (\ie\ $\delta^2\gamma(\delta)$ is increasing) by $(**)$. We also use the bounds proven in \cref{res:gamma_bounds}. 
%
\begin{enumerate}[topsep=0.7em,itemsep=0.7em]
\item
If $\delta_1\ge \delta_2^2$ then
%
\begin{align*}
    \delta_1\gamma(\delta_1) 
      &\overset{\mathclap{\smash{(*)}}}\le (\delta_2+2)^2 \gamma(\delta_2^2)
       = \delta_2^2 \Big(1+\frac2{\delta_2}\Big)^2 \prod_{k=0}^\infty \Big(1+\frac2{(\delta_2^2)^{2^k}}\Big)^2 
    \\[-1.5ex]&\!= \delta_2^2 \prod_{k=0}^\infty \Big(1+\frac2{\delta_2^{2^k}}\Big)^2
       \!= \delta_2^2 \gamma(\delta_2).
\end{align*}

\item
If $\delta_2 \le \delta_1< \delta_2^2$ then $\delta_1\gamma(\delta_1) \overset{\mathclap{\smash{(*)}}}< \delta_2^2\gamma(\delta_2)$ follows by factor-wise comparison

\item If $3\le\delta_1\le\delta_2$ then
%
$$\delta_1\gamma(\delta_1)<\delta_1^2\gamma(\delta_1) \overset{\smash{(**)}}\le \delta_2^2\gamma(\delta_2).$$

\item If $\delta_1 = 2$ and $\delta_2\ge 3$ then
%
$$\delta_1\gamma(\delta_1)=2\gamma(2) < 25 < 3^2\gamma(3) \overset{\smash{(**)}}\le \delta_2^2\gamma(\delta_2).$$

\item If $\delta_1 = 1$ and $\delta_2\ge 3$ then
%
$$\delta_1\gamma(\delta_1)=1\gamma(1)= 25 < 3^2\gamma(3) \overset{\smash{(**)}}\le \delta_2^2\gamma(\delta_2).$$

\item if $\delta_1 = 1$ and $\delta_2=2$ then
%
$$\delta_1\gamma(\delta_1)=1\gamma(1)= 25 < 36 < 2^2\gamma(2).$$
\end{enumerate}
\end{proof}
\end{lemma}

==> sec/copy-29.11.2022.tex <==
\addtocounter{section}{-1}
\section{Introduction}

Given a finite simple graph $G$, a vertex $v\in V(G)$ and $r\ge 0$, the set 
%
\[\ball Gvr:=\{w\in V(G) \mid d_G(v,w)\leq r\}\]
%
is called the \emph{ball} of radius $r$ around $v$. 
The growth of the cardinality of these~balls as $r$ increases is known as the \emph{growth behavior} or \emph{volume growth} of $G$ around $v$.  
Standard examples usually provided include the regular trees (having exponential volume growth) and the lattice graphs (having polynomial volume growth).
It is an interesting challenge to map the possible growth behaviors in various graph classes, the most famous example potentially being Cayley graphs of finitely generated groups, the central object of study in geometric group theory.
Major results in this regard are the existence of Cayley graphs of \emph{intermediate} growth (\ie\ super-polynomial but sub-exponential \cite{grigorchuck}), and the observation that vertex-transitive graphs can have polynomial growth only for integer exponents.

Cayley graphs (and more generally vertex-transitive graphs) automatically have the same growth around every vertex. In other graph classes this is not a given, and constitutes an interesting property in its own right. We shall say that a graph $G$ has \emph{uniform} growth if its growth does not vary much between vertices.
Following \cite{babaigrowth}, the precise formulation is as follows: there is a function $g\: \NN\to\NN$ and constants $c_1,C_1,c_2,C_2\in\RR_+$ so that
%
$$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r)\quad\text{for all $r\ge 0$ and $v\in V(G)$}.$$
%
The graph $G$ is then said to be of \emph{uniform growth $g$}.

In this article we construct infinite tree graphs $T$ of uniform volume growth for a wide variety of growth behaviors, including intermediate growth and polynomial growth for non-integer exponents.
%Uniform growth hereby means that the growth of the balls varies not too much from vertex to vertex. A precise definition is given in the next subsection. As an example, vertex-transitive graphs, such as the regular trees, are always of uniform growth.
Trees of uniform polynomial growth (also for non-integer exponents) have previously been constructed in \cite{benjamini2011recurrence}.
%More specifically, we require the existence of functions $\check g,\hat g\:\NN_0\to\RR$ with $\check g=\Theta(\hat g)$ so that
%
%$$\check g(r)\le |\ball Tvr| \le \hat g(r),\quad\text{for all $v\in V(T)$ and all $r\ge 0$}.$$
%
% \cref{ex:non_uniform_growth} shows that this is a stronger requirement than bounding the volume growth between functions of similar growth.

Subsequently we show how our construction gives rise to \emph{unimodular random rooted trees} of the respective growth, answering a question by Benjamini (private communication). 
We investigate the structure of these trees and find qualitative differences between growth below $r^{\log\log r}$ and growth above $r^{\alpha\log\log r}$ when $\alpha>1$. We furthermore construct unimodular random rooted trees of intermediate growth that have a single deterministic underlying tree.

\iffalse % introduction v.2

Given a finite simple graph $G$, a vertex $v\in V(G)$ and $r\ge 0$, the set 
%
\[\ball Gvr:=\{w\in V(G) \mid d_G(v,w)\leq r\}\]
%
is called the \emph{ball} of radius $r$ around $v$. 
The growth of the cardinality of these~balls as $r$ increases is known as the \emph{growth behavior} or \emph{volume growth} of $G$ around $v$.  
Standard examples usually provided include the regular trees (having exponential volume growth) and the lattice graphs (having polynomial volume growth).
It has since been an interesting challenge to map the possible growth behaviors in various graph classes, the most famous example potentially being Cayley graphs of finitely generated groups, the central object of study in geometric group theory.
Major results in this regard are the existence of Cayley graphs of \emph{intermediate} growth (\ie\ super-polynomial but sub-exponential \cite{grigorchuck}), and the observation that vertex-transitive graphs can have polynomial growth only for integer exponents [].

Cayley graphs (and more generally vertex-transitive graphs) automatically have the same growth around every vertex. In other graph classes this has to be put in by hand. For this reason we shall say that a graph has \emph{uniform} growth if its growth varies not too much from vertex to vertex.
For our purpose, the precise formulation is as follows: there is a function $g\: \NN\to\NN$ and constants $c_1,C_1,c_2,C_2\in\RR_+$ so that
%
$$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r)\quad\text{for all $r\ge 0$ and $v\in V(G)$}.$$
%
The graph is said to be of \emph{uniform growth $g$}.

In this article we construct infinite tree graphs $T$ of uniform volume growth for a wide variety of growth behaviors, including intermediate growth and polynomial growth for non-integer exponents.
%Uniform growth hereby means that the growth of the balls varies not too much from vertex to vertex. A precise definition is given in the next subsection. As an example, vertex-transitive graphs, such as the regular trees, are always of uniform growth.
Trees of uniform polynomial growth (also for non-integer exponents) have previously been constructed in \cite{benjamini2011recurrence}.
%More specifically, we require the existence of functions $\check g,\hat g\:\NN_0\to\RR$ with $\check g=\Theta(\hat g)$ so that
%
%$$\check g(r)\le |\ball Tvr| \le \hat g(r),\quad\text{for all $v\in V(T)$ and all $r\ge 0$}.$$
%
% \cref{ex:non_uniform_growth} shows that this is a stronger requirement than bounding the volume growth between functions of similar growth.

Subsequently we show how our construction gives rise to \emph{unimodular random rooted trees} of the respective growth, answering a question by Benjamini (private communication). 
We investigate the structure of these trees and find qualitative differences between growth below $r^{\log\log r}$ and growth above $r^{\alpha\log\log r}$ when $\alpha>1$. We furthermore construct unimodular random rooted trees of intermediate growth that are supported on a single deterministic tree.

\fi

\iffalse % introduction v.1

Given a finite simple graph $G$, a vertex $v\in V(G)$ and $r\ge 0$, the set 
%
\[\ball Gvr:=\{w\in V(G) \mid d_G(v,w)\leq r\}\]
%
is called the \emph{ball} of radius $r$ around $v$. 
The growth of the cardinality of these~balls as $r$ increases is known as the \emph{growth behavior} or \emph{volume growth} of $G$.  
Standard examples include the regular trees (having exponential volume growth) and the lattice graphs (having polynomial volume growth).
It is of great interest to map the possible growth behaviors in various graph classes, the most famous example potentially being the study of the growth of Cayley graphs of finitely generated groups, an important problem in the field of geometric group theory.
Some major results in this regard are the existence of Cayley graphs of \emph{intermediate} growth (\ie\ super-polynomial but sub-exponential \cite{grigorchuck}), and the observation that vertex-transitive graphs can have polynomial growth only for integer exponents [].

In this article we construct infinite tree graphs $T$ of \emph{uniform} volume growth for a wide variety of growth behaviors, including intermediate growth and polynomial growth for non-integer exponents.
Uniform growth hereby means that the growth of the balls varies not too much from vertex to vertex. A precise definition is given in the next subsection. As an example, vertex-transitive graphs, such as the regular trees, are always of uniform growth. Additionally, trees of uniform polynomial growth (also for non-integer exponents) have been constructed in \cite{benjamini2011recurrence}.%More specifically, we require the existence of functions $\check g,\hat g\:\NN_0\to\RR$ with $\check g=\Theta(\hat g)$ so that
%
%$$\check g(r)\le |\ball Tvr| \le \hat g(r),\quad\text{for all $v\in V(T)$ and all $r\ge 0$}.$$
%
% \cref{ex:non_uniform_growth} shows that this is a stronger requirement than bounding the volume growth between functions of similar growth.

Subsequently we show how our construction gives rise to \emph{unimodular random trees} of the respective growth behavior, answering a question of Benjamini (private communication) in the positive. We show that the resulting trees are qualitatively different for growth below $r^{\log\log r}$ and growth above $r^{\alpha\log\log r}$ for $\alpha>1$. We also construct unimodular random rooted trees of intermediate growth that are supported on a single deterministic tree.

Finally, we apply our results to construct planar triangulations of intermediate growth.

\fi




\subsection{Basic definitions and notation}
Let $G$ denote a (not necessarily finite) simple~connected graph with vertex set $V(G)$ and edge set $E(G)$. 
For vertices $v,w\in V(G)$, $d_G(v,w)$ denotes the graph-theoretic distance from $v$ to $w$ in $G$. 
As stated in the beginning, for $v\in V(G)$ and $r\ge 0$, the \emph{ball} of radius $r$ around $v$ in $G$ is
%
$$\ball Gvr := \{w\in V(G) \mid d_G(v,w)\le r\}.$$
%
We reiterate that the terms \emph{(volume) growth}, \emph{growth rate} and \emph{growth behavior} of $G$ around $v\in V(G)$ informally refer to the function $g(r):= |\ball Gvr|$ and its asymptotic behavior.

In general, crafting a graph with a specific growth rate around a particular vertex is simple.
Much less so if we want the graph to have a similar growth rate around each of its vertices -- we say then that $G$ is of \emph{uniform volume growth}. 

\label{ex:non_uniform_growth}
For example, given any graph $G$, it is generally easy to construct a tree of \enquote{similar} volume growth around a vertex in an asymptotic sense: choose a vertex $v\in V(G)$ and let $T$ be a spanning tree that preserves distances to $v$.
\cref{fig:non_uniform_quadratic_growth} shows an example where $G$ is the 2-dimensional lattice graph.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.55\textwidth]{img/non_uniform_quadratic_growth}
    \caption{A tree of quadratic volume growth that is \emph{not} uniform.}
    \label{fig:non_uniform_quadratic_growth}
\end{figure}

%If $w\in V(T)$ has distance $r_0:=d_T(v,w)$ from $w$, it is easy to see that
%
%\begin{equation*}\label{eq:bounds_T_G}
 %|\ball Gv{r-r_0}|\le |\ball Tw{r}|\le |\ball Gv{r+r_0}|, \quad\text{for all $r\ge r_0$}.   
%\end{equation*}
%
%hence $|\ball Twr| = \Theta(|\ball Gv r|)$. 
%However, since these bounds 
%in \eqref{eq:bounds_T_G} 
%depends on $r_0:=d_T(w,v)$, they do not guarantee uniform growth.

In the example of \cref{fig:non_uniform_quadratic_growth} we have $|\ball Tur|=\Theta(r^2)$ for all $u\in V(T)$.
However, there is no $u$-independent quadratic lower bound, as starting in a leaf, the growth is linear for an arbitrarily long initial segment. $T$ is \emph{not} of uniform quadratic growth. 

There has been a decent volume of work on trees of non-uniform intermediate growth (see \cite{amir2022branching} and references therein). In this paper, we construct the first examples of trees of uniform intermediate growth.

There are many inequivalent ways to formalize \enquote{uniform}. For this article we follow \cite{babaigrowth} and use a comparatively strong form of uniform growth:

\begin{definition}\label{def:uniform_grwoth}
A graph $G$ is of \emph{uniform (volume) growth} $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ if there are constants $c_1,C_1, c_2, C_2\in\RR_{> 0}$ so that%$b_1,c_1,C_1,b_2,c_2,C_2\in\RR_{>0}$ so that
%
%$$C_1\cdot g(c_1 r-b_1) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r+b_2),\quad\text{for all $r\ge 0$},$$
%\end{definition}

%This definition is equivalent to the one given in \cite{...}: there exists an integer $r_0\ge 0$ and constants

%
$$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r)\quad\text{for all $r\ge 0$}.$$.
\end{definition}
%
%We stick with the version given in \cref{def:uniform_grwoth} as it is more natural for proving the main result \cref{thm:main}.

% \begin{definition}\label{def:uniform_grwoth}
% A graph $G$ is of \emph{uniform (volume) growth} $g\:\NN_0\to\NN_0$ if there is an integer $r_0\ge 0$ and constants $c_1,C_1, c_2, C_2\in\RR_{> 0}$ so that
% %
% $$C_1\cdot g( c_1 r) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r),\quad\text{for all $r\ge r_0$}.$$
% \end{definition}

% This definition is equivalent to the existence of constants $b_1,c_1,C_1,b_2,c_2,C_2\in\RR_{>0}$ so that
% %
% $$C_1\cdot g(c_1 r-b_1) \;\le\; |\ball Gvr| \;\le\;  C_2\cdot g( c_2 r+b_2),\quad\text{for all $r\ge 0$},$$
% %
% which will be the definition used in \cref{thm:main}.

%We implicitly assume that the argument to $g$ is rounded to the nearest positive integer.
%If $g$ is increasing then this does not change \cref{def:uniform_grwoth} as there are always constants $\bar c_1,\bar c_2\in\RR_0$ so that for sufficiently large $r$
%
%$$
%g(\lceil \bar c_1 r \rceil)\le g(c_1 r)
%\quad\text{and}\quad
%g(\lfloor \bar c_2 r \rfloor)\le g(c_2 r).
%$$
%
%In fact, in the main theorem we show that ...

One generally distinguishes
%
\begin{itemize}
    \item \emph{uniform polynomial growth} if $g(r)=\exp(\mathcal O(\log r))$,
    \item \emph{uniform exponential growth} if $g(r)=\exp(\Omega(r))$,
    \item \emph{uniform intermediate growth} if $g(r)=\exp(o(r))$ and $g(r)=\exp(\omega(\log r))$,
\end{itemize}
%
where we used the Landau symbols $\mathcal O,\Omega, o,\omega$ as usual.


%We should reasonably assume~$g(r)=\Omega(r)$ and $g=e^{\mathcal O(r)}$, but~these and more general conditions will emerge naturally during the analysis of our construction. %As we see in a moment, we will also need to impose restrictions on the~os\-cil\-lation in the growth of $g$.

%\begin{itemize}
 %   \item $\log r=\log_2 r$ is logarithms to base 2. Otherwise write $\ln r = \log_e r$.
%\end{itemize}



\subsection{Overview}

%Starting from a suitable increasing function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$, we achieve the following:
%\begin{enumerate}
    %\item we explicitly construct~a tree $T$ with uniform growth $g(r)$;%in which $|B_v^T(r)|$ grows approximately like $g(r)$, no matter~the~vertex \mbox{$v\in V(T)$}
    %\item we prove the existence of a unimodular tree $\mathcal{T}$ with uniform growth $g(r)$.
%\end{enumerate} 

The main results in the present paper are the following:

\begin{main} \label{main}
   If $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ is (eventually) super-additive and log-concave, then there exists a tree $T$ of uniform growth $g$. 
%   Let $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ be a function that grows at least linearly and at most exponentially, and is in particular super-additive and log-concave. Then there exists a tree $T$ with uniform growth $g(r)$. 
\end{main}

\begin{main} \label{unimain}
     Let $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ be a function that grows at least linearly and at most exponentially, and is in particular super-additive and log-concave. Then there is a unimodular random rooted tree $\mathcal{T}$ with uniform growth $g(r)$.
\end{main}

We also produce a structure theorem (\cref{structure}) that describes the structure of the trees obtained in \cref{unimain}. 

We describe the general construction for the tree $T$ in \cref{sec:construction}. In \cref{sec:main}, we show that the volume growth of $T$ is uniform with bounds close to a specified target growth $g\:\RR_{\ge 0}\to\RR_{\ge 0}$. In particular, assuming mild and quite natural conditions on $g$, namely that it be super-additive and log-concave, we prove that $T$ has uniform growth $g(r)$.

In \cref{sec:unimodular} we show how our construction naturally gives rise to a unimodular random tree $\mathcal{T}$ of a prescribed uniform volume growth. We describe the general shape of such trees, and even
give examples for unimodular random rooted trees of intermediate volume growth that have a single underlying tree.

Finally, in \cref{sec:last} we note some further observations as well as directions for this type of inquiry. Most notably, we use our construction in the vein of \cite{benjamini2011recurrence} to obtain planar triangulations of intermediate growth. 


%\noindent
%\hrulefill

%Ideas for literature:
%\begin{itemize}
 %   \item groups of intermediate growth
  %  \item other graphs of intermediate growth
   % \item \cite{benjamini2011recurrence} trees of polynomial growth by Benjamini-Schramm
    %\item \cite{amir2022branching} \enquote{The branching number of intermediate growth trees}
 %by Gideon Amir, Shangjie Yang
%\end{itemize}

\iffalse

\section{The Construction} \label{sec:construction}

%We describe an infinite tree that is not immediately supposed to match a prescribed growth behavior, but depends on countably many parameters that can be used to model a wide range of such behaviors, as we discuss further below.

For each integer sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ with $\delta_n\ge 1$ we describe the construction of a tree $T=T(\delta_1,\delta_2,...)$.

\begin{construction}
\label{constr:tree}

%Fix a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ of integers $\delta_n\ge 1$. 
Consider the following~recursive definition of trees $T_n, n\ge 0$ (see also \cref{fig:construction}):
%
\begin{itemize}
    \item 
    let $T_0:=\{x^*\}$ be the tree consisting of a single vertex called the \emph{global root}.
    For reasons that will become clear shortly, we call $x^*$ also the \emph{root} and an \emph{apocentric vertex} of $T_0$.
    
    \item we build $T_n,n\ge 1$ from $\delta_n$ disjoint copies of $T_{n-1}$ (called \emph{apocentric copies}) that we connect to another copy of $T_{n-1}$ (called the \emph{central copy}) in a way that we make precise below. 
    
    For this we require some further terminology:
    %the \enquote{non-central} copies of $T_{n-1}$ will be called \emph{apocentric copies} of $T_{n-1}$ in $T_n$.
    the root of $T_n$ is the root of the central copy of $T_{n-1}$.
    Likewise, an apocentric vertex of $T_n$~is~an~apocentric vertex of an apo\-centric copy of $T_{n-1}$.
    %Each apocentric vertex of $T_n$ is a leaf, but the converse is not necessarily true.
    
    The connections between the central and the apocentric copies are as follows: each apocentric copy of $T_{n-1}$ is connected to the central copy~by an edge between the root of the apocentric copy and some apocentric vertex of the central copy. There is no preferred choice for the apocentric vertex in the central copy (we~can even attach more than one apocentric copy to the same vertex), but it is~required that the entirety of these connection is distributed maximally uniformly among the apocentric vertices\,%
    \footnote{
    %The meaning of this will become evident when it is applied in the proof of \cref{thm:main}.
    More precisely, every apocentric copy $T_m\subset T_{n-1}, m\le n-1$ (\ie\ a copy of $T_m$ that contains apocentric vertices of $T_{n-1}$) will receive the expected number of connections, rounded up or down (see the proof of \cref{thm:main}).
    }%
    \!.
    %(this will be made precise when we apply it in the proof of \cref{thm:main}, but can be thought of as a uniform distribution).
    %; meaning that every apocentric vertex is attached to approximately the same number of copies.
\end{itemize}
%
\begin{figure}[!h]
    \centering
   % \includegraphics[width=0.7\textwidth]{img/construction.pdf}
   % \includegraphics[width=0.65\textwidth]{img/construction_2.pdf}
    \includegraphics[width=0.83\textwidth]{img/construction_3.pdf}
    \caption{Illustration of the first four steps in the  construction~of $T$ using the sequence $\delta_n:=n+2$. The ringed vertex is the root, and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy of $T_{n-1}$ in $T_n$.}
    \label{fig:construction}
\end{figure}
%

If for each $n\ge 1$ we identify $T_{n-1}$ with its central copy in $T_n$, we obtain an~inclu\-sion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $\smash{T:=\bigcup_{n\ge 0} T_n}$ is a well-defined~tree.
%We shall occasionally denote it by $T(\delta_1,\delta_2,...)$ to emphasize that it is mainly determined by the choice of the integer sequence (the free choice of the connections will play no role as long as it is maximally uniform in a way that will become clear in the proof of \cref{thm:main}).
%
We shall occasionally denote this tree by $T(\delta_1,\delta_2,...)$ even though the tree does also depend on the choice of the connections in each step, but this choice is not relevant in our analysis.
\end{construction}

Our core claim is that for most sequences $\delta_1,\delta_2,\delta_3,...\in\NN$ this tree has a uniform volume growth of some sort, and that with a careful choice of the sequence we can model a wide range of such growth behaviors, including polynomial, intermediate and exponential.

A first feeling for the claimed relation between the sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ and the growth~of $T$ can obtained by two simple observations:
%
\begin{itemize}
    \item the distance from the root of $T_n$ to any of its apocentric vertices is exactly $2^n-1$. In fact, $T_n\subset T$ is the ball of radius $2^n-1$ around the global root $x^*\in V(T)$.
    \item $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ (where the empty product gives $|T_0|=1$).
\end{itemize}
%
In other words, for radii $r=2^n-1$ holds
%
\begin{equation}
\label{eq:ball_volume_in_T}
|\ball T{x^*}r| = |T_n| = (\delta_1+1)\cdots(\delta_n+1).    
\end{equation}
%
Hence, if we aim to model a particular growth function $g\:\NN_0\to\NN$, a plausible first step is to choose a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which $(\delta_1+1)\cdots(\delta_n+1)$~approximates the growth of $f(n):=g(2^n-1)$.
This suggests a choice
%
$$\delta_n + 1\approx \frac{f(n)}{f(n-1)},$$
%
where we necessarily introduce an error when rounding the right side to an integer.

To establish uniform growth with the prescribed rate $g$ it remains to prove
%
\begin{itemize}
    \item the error introduced by rounding $f(n)/f(n-1)$ is manageable.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for radii other than $2^n-1$.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for balls centered at vertices other than the global center $x^*\in V(T)$.
\end{itemize}
%
All these points are addressed in the next section.

We close this section with three examples demonstrating the versatility of the~construction.
For conciseness we use $\bar g(r):=g(r-1)$, then $f(n)=\bar g(2^n)$.

\begin{example}[Polynomial growth]\label{ex:polynomial}
For $\bar g(r)=r^\alpha,\alpha\in\NN$ we have $f(n)=2^{\alpha n}$~and so the sequence $\delta_n=2^\alpha-1$ is \emph{constant}.

In fact, the tree $T(2^\alpha-1,2^\alpha-1,...)$ embeds nicely into the $\alpha$-th power%
\footnote{Recall, the $\alpha$-th power of $G$ is a graph $G^\alpha$ with vertex set $V(G)$ and an edge between any to vertices whose distance in $G$ is at most $\alpha$.}
of~the~$\alpha$-dimensional lattice graph (shown in \cref{fig:2_lattice_construction} for $\alpha=2$), giving independent evidence for polynomial volume growth.
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.92\textwidth]{img/2_lattice_subgraph_3.pdf}
    \caption{
        Embedding of the tree $T(3,3,...)$ into the square of the 2-dimensional lattice graph.
    }
    \label{fig:2_lattice_construction}
\end{figure}

More generally, for constant sequence $\delta_n:=c$, where $c$ is not of the form $2^\alpha-1$ with $\alpha\in\NN$, we expect to find polynomial volume growth with non-integer exponent $\log_2 c$.
\end{example}

\begin{example}[Exponential growth]\label{ex:exponential}
%The $d$-regular tree has growth function $\bar g(r)=d(d-1)^r$. This yield $f(n)=d(d-1)^{2^n}$ and $\delta_n=(d-1)^{2^{n-1}}$.
The sequence $\delta_n:=d^{\kern0.15ex 2^{n-1}}\!,d\in\NN$ yields the $d$-ary tree (see \cref{fig:binary_tree} for the case $d=2$, \ie\ the binary tree).
Replacing $d_1:=d+2$ will result in the $(d+1)$-regular tree.
We have exponential volume growth in both cases.
This is as expected, since for $r=2^n$ holds
%
$$\bar g(r) := (\delta_1+1)\cdots(\delta_n+1)=\prod_{k=1}^n \Big(d^{\kern0.15ex 2^{k-1}}\!\!+1\Big) = \sum_{i=0}^{\mathclap{2^n-1}} d^{\kern0.15ex i} = \frac{d^{\kern0.15ex 2^n}-1}{d-1} = \frac{d^{\kern0.15ex r}-1}{d-1}.$$
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.85\textwidth]{img/binary_tree.pdf}
    \caption{
        The binary tree as constructed from \cref{constr:tree} using sequence $\delta_n=2^{2^{n-1}}$.
    }
    \label{fig:binary_tree}
\end{figure}
\end{example}

Extrapolating from \cref{ex:polynomial} and \cref{ex:exponential} its seems not far-fetched that many unbounded sequences $\delta_1,\delta_2,\delta_3,...$ that grow sufficiently slower than doubly exponentially result in intermediate volume growth.

\begin{example}[Intermediate growth]
Consider $\delta_n:=(n+3)^\alpha -1$, $\alpha\in\NN$~(the~case $\alpha=1$ is shown in \cref{fig:construction}). For $r=2^n$ we estimate
%
\begin{align*}
\bar g(r) := (\delta_1+1)\cdots(\delta_n+1) 
&= (\tfrac16 (n+3)!)^\alpha 
 \sim (n! n^3)^\alpha
 \sim (n^n e^{-n} n^{7/2})^\alpha 
\\ &= r^{\alpha \log\log r} r^{-\alpha/\ln 2}\, (\log r)^{7\alpha/2}
\end{align*}
%
Hence, we expect this choice of the sequence $\delta_1,\delta_2,\delta_3,...$ to lead to a tree of uniform intermediate volume growth.
Trees constructed from $\delta_n\sim n^\alpha$ will
%Trees of growth rate $g(r)\sim r^{\alpha\log\log r}$ will also 
present~an~interes\-ting boundary case in \cref{sec:unimodular} when we discuss unimodular random trees.
% \begin{align*}
% |\ball T{x^*}{r-1}| = |T_n|= \tfrac16 (n+3)! 
% \, &\sim\,
% n! \, n^3  
% \,\sim\,
% % n^n \cdot n^{9/2}e^{-n}
%  n^n e^{-n} \sqrt n \, n^3 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \cdot (\log r)^{7/2}  .
% %\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
% \end{align*}
\end{example}


% \begin{mnote}
% Two further things should be defined rigorously in this section:
% \begin{enumerate}
%     \item \enquote{copy of $T_n$ in $T$}; clarify that this does not refer to just any subgraph isomorphic to $T_n$.
%     \item \enquote{$T_n$ is central/apocentric in $T_m$ for $m\ge n$}.
% \end{enumerate}
% \end{mnote}




% \newpage
% \sepline

% \msays{Find a good place for these remarks.}

% %The following two remarks formalize the notions \enquote{copy of $T_n$ in $T_m$} and \enquote{maximal uniform distribution of adjacencies}. The reader comfortable with an intuitive understanding of these concepts can skip the remarks.

% \begin{remark}\label{rem:copy}
% The notion of \enquote{\emph{copy} of $T_n$ in $T_m$} (where $m\ge n$) will be used~in a formal sense, referring to a special subgraph of $T_m$ isomorphic to $T_n$ that is distinguished by \cref{constr:tree} in a way we explain below.
% %In particular, not every subgraph~isomorphic to $T_n$ is a copy, and we use the notation $T_n\prec T_m$ if it is one.
% In particular, not every subgraph $\tau\subseteq T_m$ iso\-morphic to $T_n$ necessarily is such a copy, and we introduce the notation $\tau\prec_n T_m$ to indicate when it is one.
% We write $\tau\prec T_m$ if $n$ is not~important, and we write \enquote{a copy $T_n\prec T_m$} to refer to an~un\-named copy of $T_n$ in $T_m$.

% A rigorous definition of copy can be given recursively:
% a copy $\tau \prec_n T_n$ is only the full graph itself.
% The copies $\tau\prec_n T_{n+1}$ are exactly the central and apocentric copies as defined in \cref{constr:tree}.
% %central and apocentric copies of $T_n$ in $T_{n+1}$ were defined in \cref{constr:tree}.
% A copy $\tau\prec_n T_{m+1}$ is a copy $\tau\prec_n T_m\prec T_{m+1}$, in words, $\tau$ is a copy of $T_n$ inside a copy of $T_m$ inside of $T_{m+1}$.

% We furthermore say that a copy $\tau \prec T_n$ is central if it contains the root of $T_n$, and
% it is apocentric if it contains apocentric vertices of $T_n$ (one can show that then all apocentric vertices of $\tau$ are also apocentric in $T_n$).
% \end{remark}

% \msays{My worries: at the moment $\prec$ is not a partial order, but more like an abbreviation, \ie\ \enquote{copy $T_n\prec T_m$} is short for \enquote{a copy of $T_n$ inside of $T_m$}, and \enquote{copy $T_n\prec T_m\prec T_k$} is short for \enquote{a copy of $T_n$ inside of a copy of $T_m$ inside $T_k$}.
% If we make $\prec$ into a rigorous partial order then we lose this powerful abbreviation and have to write \enquote{let $\tau\prec T_m$ be a copy of $T_n$} and even worse \enquote{let $\tau\prec \tau'$ be a copy of $T_n$, where $\tau'\prec T_k$ is a copy of $T_m$}. That is, we always have to give names to the copies, don't we? But I am not happy with the current solution either. Hm.}

% \msays{Maybe an idea: write $\tau\prec_n T_m$ for \enquote{copy of $T_n$ in $T_m$}. Then we can write $\tau\prec_n\tau'\prec_m T_k$. Still a bit annoying with the subindex, and we still have to give names.}

% \msays{Check out my updated Remark 2.5 where I used some of these ideas and see whether you think its any better.}

% \gsays{I think that the updated remark resolves the issue perfectly. Copies are now well-defined.}

\newpage

\fi



\section{The construction}
\label{sec:construction}

%\msays{Experimental alternative to the intro of \cref{sec:construction}. Work in progress.}

\par\medskip

% In this section we construct a tree $T$ and explain why we expect it to be 

% We construct a tree $T$ that we later show to be of uniform volume growth.
% More precisely, we construct a tree $T=T(\delta_1,\delta_2,...)$ for each integer sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ with $\delta_n\ge 1$.

For each integer sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ with $\delta_n\ge 1$ we construct a tree~$T=T(\delta_1,\delta_2,...)$.
The choice of sequence will determine the growth rate of $T$.
%
%We shall later see that the tree $T$ can manifest a wide range of growth behaviors depending on the input sequence, and we shall explain this connection in the next section.
%
%The growth behavior of $T$ expectedly depends on the sequence, and we later explain how to choose the $\delta_i$ to model a particular growth.
%
The tree $T$ is constructed as a limit object of the following sequence of trees $T_n$ where $n\ge 0$:

%We first introduce a recursively defined sequence of trees $T_n$ for $n\ge 0$ (see \cref{constr:T_n}) and subsequently define $T$ as a limit object of this sequence (see \cref{constr:T}).


%This tree will be obtained as the limit object of a recursively defined sequence of trees $T_n,n\ge 0$, which itself is built from the sequence $\delta_1,\delta_2,\delta_3,...$.

\begin{construction}\label{constr:T_n}
%We recursively define a sequence of trees $T_n,n\ge 0$ with two types of distinguished vertices, namely, a \emph{root} and a set of \emph{apocentric vertices}:
The trees $T_n$ are defined recursively.
%We recursively define a sequence of trees $T_n$ for $n\ge 0$. 
In each tree we distinguish two special types of vertices: a \emph{center}, and a set of so-called \emph{apocentric vertices} (or outer\-most or peripheral vertices), both will be defined alongside the trees:
%and in each tree two distinguished types of vertices, a \emph{root} and a set of \emph{apocentric vertices}:
%with two types of distinguished vertices: a \emph{root} and a set of so-called \emph{apocentric vertices}:
%Each $T_n$ has a \emph{root} and a set of so-called \emph{apocentric vertices} which are defined alongside the trees:
%
\begin{myenumerate}
    \item 
    $T_0$ is the tree consisting of a single vertex. This vertex is both the center of $T_0$ as well as its only apocentric vertex.
    
    \item 
    The tree $T_n$ is built from $\delta_n+1$ disjoint copies $\tau_0, \tau_1,...,\tau_{\delta_n}$ of $T_{n-1}$ that we join into a single tree by adding the following edges:
    %
    %where $\tau_0$ (which we call \emph{central copy}) will be connected to $\tau_1,...,\tau_{\delta_n}$ (which we call \emph{apocentric copies}) in the following way:
    %
    %for each $\tau_i,i\in\{1,...,\delta_n\}$ choose an apocentric vertex of $\tau_0$ and add an edge between this vertex and the root of $\tau_i$.
    for each $i\in\{1,...,\delta_n\}$ add an edge between the center of $\tau_i$ and some apocentric vertex of $\tau_0$.
    There is a choice in selecting these apocentric vertices of $\tau_0$ (and note that we can choose the same apocentric vertex more than once), but we shall require that these adjacencies are distributed in a maximally uniform way among the apocentric vertices of $\tau_0$ (we postpone a rigorous definition of this until we introduced suitable notation; see \cref{rem:max_uniform}).
    
    It remains to define the distinguished vertices of $T_n$: the center of~$T_n$~is the center of $\tau_0$; the apocentric vertices of $T_n$ are the apocentric vertices~of $\tau_1,...,$ $\tau_{\delta_n}$.
    
    % \msays{Turns out, in each $T_n$ the root is just the \enquote{center}, and the apocentric vertices are just the \enquote{peripheral vertices}, both are established terms. I don't want to change our terminology, and I don't know what to do with this insight.}
    
    % \gsays{Where did you come upon these established terms?}
    
    % \msays{Wikiepdia, see comment in code}
    % https://en.wikipedia.org/wiki/Distance_(graph_theory)#Related_concepts
    
    %The $\tau_i$ will be called the \enquote{copies of $T_{n-1}$ in $T_n$}, which we also denote by $\tau_i\precdot T_n$.
    
    %One can visualize the $\tau_i,i\in\{1,...,\delta_n\}$ as being arranged around $\tau_0$ in the center, from which the connections to the $\tau_i$ emanate star-like (\cf\ \cref{fig:construction}).
    
    % Intuitively, the copies $\tau_i,i\in\{1,...,\delta_n\}$ are arranged around the copy $\tau_0$ in the center (see \cref{fig:construction}). For this reason $\tau_0$ is called the \emph{central copy} of $T_{n-1}$~in $T_n$, while the others are called \emph{apocentric copies}. We use the notation $\tau_i\precdot T_n$ to refer to these copies of $T_{n-1}$ (a notation we generalize in \cref{rem:copy}).
    
    % Let $\tau_0,\tau_1, ...,\tau_{\delta_n}$ be $\delta_n+1$ disjoint copies of $T_{n-1}$. We add edges to connect these trees to form the next tree $T_n$, but we need some further terminology to describe these connections concisely.
    
    % \begin{itemize}
    %     \item The $\tau_i$ are called \enquote{copies of $T_{n-1}$ in $T_n$}, which distinguishes them among other subgraphs of $T_n$ isomorphic to $T_{n-1}$. We denote this by $\tau_i\precdot T_n$.
    %     \item $\tau_0$ will be called \emph{central copy}, whereas the $\tau_1,...,\tau_{d_n}$ are the \emph{apocentric copies}.
    %     \item the root of $T_n$ is the root of the central copy $\tau_0$, whereas a vertex~of $T_n$~is apocentric if it is apocentric in any of the  $\tau_i,i\in\{1,...,\delta_n\}$.
    % \end{itemize}
    
    % The adjacencies between the copies $\tau_i$ are as follows: to each apocentric copy $\tau_i,i\in\{1,...,\delta_n\}$ we choose an apocentric vertex in $\tau_0$ and add an edge between this vertex and the root of $\tau_i$.
    
    % ...
    
    % The connections between the central and the apocentric copies are as follows: each apocentric copy of $T_{n-1}$ is connected to the central copy~by an edge between the root of the apocentric copy and some apocentric vertex of the central copy. There is no preferred choice for the apocentric vertex in the central copy (we~can even attach more than one apocentric copy to the same vertex), but it is~required that the entirety of these connection is distributed maximally uniformly among the apocentric vertices (see \cref{rem:max_uniform} for a rigorous explanation)
\end{myenumerate}
%
% We write $\tau\precdot T_n$ to denote that $\tau$ is such a copy. 
% This defines a relation on trees isomorphic to the $T_n$.
% Let $\prec$ be the transitive closure of $\precdot$, then we can write $\tau\prec T_n$ to denote the canonical copies of $T_m$ in $T_n$ for general $m< n$.
% We write $\tau\prec_m T_n$ to emphasize that $\tau$ is a copy of $T_m$.
%
See \cref{fig:construction} for an illustration of this recursive definition.
    
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.85\textwidth]{img/construction_4.pdf}
    \caption{Illustration of the first four trees $T_0,...,T_3$ defined using the sequence $\delta_n:=n+2$. The ringed vertex is the center, and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy $\tau_0$ in $T_n$. The dashed lines are the new edges added to connect the copies to form a single tree.}
    \label{fig:construction}
\end{figure}
\end{construction}

The following three properties follow immediately from the recursive definition:

\begin{observation}\label{res:T_n_properties} \quad
\begin{myenumerate}
    \item $T_n$ has exactly $(\delta_1+1)\cdots(\delta_n+1)$ vertices.
    \item $T_n$ has exactly $\delta_1\cdots\delta_n$ apocentric vertices, all of which are leaves of the tree (but not all leaves are necessarily apocentric).
    \item the distance from the center of $T_n$ to any of its apocentric vertices is $2^n-1$.
\end{myenumerate}
\end{observation}

One way to construct a \enquote{limit} of the $T_n$ is the following:

%The definition of $T:=T(\delta_1,\delta_2,...)$ as a limit object is straightforward.

\begin{construction}\label{constr:T}
For each $n\ge 1$ identify $T_n$ with one of its copies $\tau_0,\tau_1,...,\tau_{\delta_{n+1}}$ in $T_{n+1}$.
In this way we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the~union $T=T(\delta_1,\delta_2,...):=\bigcup_{n\ge 0} T_n$ is an infinite tree.
\end{construction}

%\msays{either remove $T(d_1,d_2,...)$ everywhere, or define it.}

% In the following we shall write $T(\delta_1,\delta_2,...)$ to denote a limit tree obtained~from the sequence $\delta_1,\delta_2,\delta_3,...\in\NN$.
%
\iftrue % types of limit trees vs types of inclusion chains
%
For later use we distinguish three natural~types of limits:
%One natural way is to identify $T_n$ with its \enquote{central copy} $\tau_0\subset T_{n+1}$. The resulting inclusion chain will be called \emph{completely central}.
%Other conventions are conceivable, such as
%For later use we give names to the following other ways to define inclusion:
%
\begin{itemize}
    \item the \emph{centric limit} always identifies $T_n$ with the \enquote{central copy} $\tau_0$ in $T_{n+1}$. It comes with a designated vertex $x^*\in V(T_0)\subset V(T)$, the \emph{global center}.
    \item \emph{apocentric limit}s always identify $T_n$ with an \enquote{apocentric copy} $\tau_i$ in $T_{n+1}$.
    \item \emph{balanced limits} make both central and apocentric identifications infinitely often.
\end{itemize}
%
In \cref{sec:unimodular} we discuss a different and arguably more canonical way to take a limit (the Benjamini-Schramm limit) that avoids arbitrary identifications.

\else

For later use we distinguish three natural types of inclusion chains:
%One natural way is to identify $T_n$ with its \enquote{central copy} $\tau_0\subset T_{n+1}$. The resulting inclusion chain will be called \emph{completely central}.
%Other conventions are conceivable, such as
%For later use we give names to the following other ways to define inclusion:
%
\begin{itemize}
    \item \emph{centric} inclusion chains identify $T_n$ with the \enquote{central copy} $\tau_0$ in $T_{n+1}$.
    \item \emph{apocentric} inclusion chains identify $T_n$ with an \enquote{apocentric copy} $\tau_i$ in $T_{n+1}$.
    \item \emph{balanced} inclusion chains make both central and apocentric identifications infinitely often.
\end{itemize}
%
In \cref{sec:unimodular} we discuss a different and arguably more canonical way to make these identification via Benjamini-Schramm limits.

\fi

\iffalse % old construction of T

\begin{construction}\label{constr:T}
For each $n\ge 1$ identify $T_{n-1}$ with its \enquote{central copy} $\tau_0$ in $T_n$.
This yields an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $\smash{T:=\bigcup_{n\ge 0} T_n}$~is a~well-defined tree\footnote{Note that \cref{constr:T_n} \itm2 involves freedom in choosing the edges between $\tau_0$ and~$\tau_1,...,$ $\tau_{\delta_n}$. Therefore the notation $T(\delta_1,\delta_2,...)$ is strictly speaking not well-defined. However,\nlspace the exact choice is not relevant to our analysis and we tacitly fix some instance of the construction.}\!.

The tree $T$ has a canonical notion of root, namely the unique vertex of $T_0\subset T$, which we shall call the \emph{global root} of $T$.
\end{construction}

\begin{remark}
Based on the choice of identification, the inclusion chain $T_0\subset T_1\subset T_2\subset \cdots$ in \cref{constr:T} could be called \emph{completely centric}.
Other identification are conceivable and lead to other limit trees: \emph{completely apocentric} inclusion chains (always identifying $T_n$ with an \enquote{apocentric copy} $\tau_i \prec_n T_{n+1}$) or \emph{mixed} inclusion chains (making both, a central and apocentric choice infinitely often).

%The centric chain will be most useful to our discussion of grwoth
We shall see that choosing a different chain comes with no significant change to our analysis of growth.
Still, different chains will be relevant to \cref{sec:unimodular} when we discuss a less biased approach using Benjamini-Schramm limits.
%
%
%
%
%In an alternative to \cref{constr:T} one could identify each $T_{n-1}$ with an \emph{apocentric copy} in $T_n$ rather than the central copy (or even make a different choice in each step). This would then result in a different limit tree.
%In \cref{sec:unimodular} we explore such a \enquote{less biased} approach using Benjamini-Schramm limits.
%Our analysis of the growth of $T$ will carry over to this more general setting (see \cref{rem:general_limit_growth}).
%
%
%
% The given construction of $T$ is however more suitable for our immediate~analysis, which also carries over to the general case
%
% Alternative limit procedures are conceivable, \eg\ where we always (or just for some $n$) identify $T_{n-1}$ with one of its apocentric copies in $T_n$ (rather than the central one).
% \cref{sec:unimodular} follows a \enquote{less biased} approach via distributional limits.
% The given construction of $T$ is however more suitable for our immediate~analysis, which also carries over to the general case (see \cref{rem:general_limit_growth}).
\end{remark}

\fi

Our core claim is now that for \enquote{most} sequences $\delta_1,\delta_2,\delta_3,...\in\NN$ and independent of the type of the limit, the tree $T$ has a uniform volume growth of some sort, and that with a careful choice of the sequence we can model a wide range~of~growth~behaviors, including polynomial, intermediate and exponential.

%\msays{remove reference to global center.}

The following example computation gives us
%is meant to provide a first idea
a first idea of
%of 
the connection 
%that we should expect to find 
between the sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ and the growth rate of $T$.
For this, let $T$ be the centric limit with global center $x^*\in V(T)$.
By \cref{res:T_n_properties}~\itm3 the ball of radius $r=2^n-1$ in $T$, centered at $x^*$, is exactly $T_n\subset T$.
By \cref{res:T_n_properties} \itm1 it follows
%
%This computation is based on three properties of the $T_n$ that follow immediately from the recursive definition:
%
%For later use we mention the following properties of $T_n$, all of which follow directly from the recursive definition:
%
%
% \begin{itemize}
%     \item the distance from the root of $T_n$ to any of its apocentric vertices is exactly $2^n-1$. In fact, $T_n\subset T$ is the ball of radius $2^n-1$ around the global root $x^*\in V(T)$.
%     \item $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ (where the empty product gives $|T_0|=1$).
% \end{itemize}
%
%In other words, for radii $r=2^n-1$ holds
%
\begin{equation}
\label{eq:ball_volume_in_T}
|\ball T{x^*\!}r| = |T_n| = (\delta_1+1)\cdots(\delta_n+1).    
\end{equation}
%
Thus, if we aim for, say, $\ball T{x^*\!}r\approx g(r)$ with a given growth function $g\:\NN_0\to\NN_0$, then \eqref{eq:ball_volume_in_T} suggests to use a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which 
%
% Thus, looking for 
% %Therefore, if we start from an increasing function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ and we want~to find 
% a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which $|\ball T{x^*\!}r| \approx g(r)$, where $g\:\NN\to\NN$ is some given growth function, \eqref{eq:ball_volume_in_T} suggests to use a sequence for which
$(\delta_1+1)\cdots(\delta_n+1)$ approximates $g(2^n-1)$.
In practice it turns out more convenient to approximate $g(2^n)$ (the computations are nicer and we still can prove uniform growth), and so we are lead to
%Thus, we are lead to
% Therefore, if we want $T$ to model a particular volume growth 
% %prescribed by a function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$, that is, 
% $|\ball T{x^*}r| \approx g(r)$, then we should choose a sequence $\delta_1,\delta_2,\delta_3,...$ for which $(\delta_1+1)\cdots(\delta_n+1)$ approximates $f(n):=g(2^n-1)$.
%
\begin{equation} \label{eq:suggestions}
    \delta_n + 1\approx \frac{g(2^n)}{g(2^{n-1})},
\end{equation}
%
where we necessarily introduce an error when rounding the right side to an integer.
%
%In actuality we shall work with $g(2^n)$ instead of $g(2^n-1)$ because the~computations turn out nicer and we still can prove uniform growth.
%
%Our definition of \enquote{uniform growth} is flexible enough to allow for~this as any deviations can be absorbed into the constants.
%
%The We will still be able to prove uniform growth.
%
To establish uniform growth with a prescribed growth rate $g$ it remains to prove
%
\begin{itemize}
    %\item the error introduced by rounding $f(n)/f(n-1)$ is manageable.
    \item the error introduced by rounding the right side of \eqref{eq:suggestions} is manageable.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for radii $r$ that are not of the form $2^n-1$.
    \item an estimation close to \eqref{eq:ball_volume_in_T} holds for general limit trees and around vertices other than a designated \enquote{global center}.
\end{itemize}
%
These points are addressed in the next section.

The remainder of this section is used to introduce helpful notation, clarify the phrase \enquote{maximally uniform distribution of adjacencies} used in \cref{constr:T_n} and provide examples.

%In the remainder of this section we address the \enquote{maximal uniform distribution of adjacencies} left undefined in \cref{constr:T_n} \itm2, and give examples that demonstrate the versatility of out construction.




\begin{notation}
By \cref{constr:T_n} \itm2 for every $n\in \mathbb{N}$, $T_n$ (and each tree isomorphic to $T_n$) comes with a canonical decomposition into copies of $T_{n-1}$.
Recursively we obtain a canonical decomposition of $T_n$ into copies of $T_m$ for each $m\le n$ (see \cref{fig:copies_of_T1}). We shall use the notation $\tau\prec_m T_n$ to indicate that $\tau$ is such a canonical copy of $T_m$, or $\tau \prec T_n$ if $m$ is not relevant.
%Lastly, by a slight abuse of notation, we may write \enquote{a copy $T_m\prec T_n$} to refer to an unnamed copy of $T_m$ inside of $T_n$.

A copy $\tau\prec T_n$ is called \emph{central} if it contains the center of $T_n$; it is called~\emph{apocentric} if it shares apocentric vertices with $T_n$ (and one can easily show that then \emph{all}~apocentric vertices of $\tau$ are apocentric in $T_n$).
\end{notation}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{img/copies_of_T1.pdf}
    \caption{All canonical copies $\tau\prec_1 T_3$ are highlighted. The central~and apocentric copies are highlighted in white, the others in gray. %Observe that $T_3$ contains further subgraphs isomorphic to $T_1$ that are not copies.
    }
    \label{fig:copies_of_T1}
\end{figure}

% \begin{remark}\label{rem:copy}
% The symbol $\precdot$ defines a relation between (graphs isomorphic to) the $T_n,n\ge0$.
% Let $\prec$ be its transitive closure.
% If $\tau\prec T_n$ we say \,\enquote{$\tau$ is a copy in $T_n$}, and we write $\tau\prec_m T_n$ to emphasize that $\tau$ is a copy of $T_m$.
% We call $\tau\prec T_n$ a \emph{central copy} if it contains the root of $T_n$, we call it an \emph{apocentric copy} if it shares apocentric vertices with $T_n$ (and it is not hard to see that then all apocentric vertices of $\tau$ are also apocentric in $T_n$).
% \end{remark}

% The \enquote{maximally uniform distribution of adjacencies} between the apocentric vertices of $\tau_0$ and the roots of $\tau_1,...,\tau_{\delta_n}$ in \cref{constr:T_n} \itm2 will later be crucial for establishing uniform growth of $T$ (see \cref{thm:main}).
% A formal definition is given below.

With this notation in place we can clarify our use of \enquote{maximal uniform~distribution of adjacencies} in \cref{constr:T_n} \itm2.

\begin{remark}\label{rem:max_uniform}
%\enquote{Maximal uniform distribution of adjacencies} roughly means that certain \enquote{important} subsets of apocentric vertices of $\tau_0$ are involved in the expected number of \enquote{outwards adjacencies} to the apocentric copies $\tau_1,...,\tau_{\delta_n}$.

%To understand what is the \enquote{expected number}, note that $T_n$ has exactly $\delta_1\cdots\delta_n$ apocentric vertices.
%We make this precise.

Let $\tau_0\prec_{n-1} T_{n}$ be the central copy.
%An \emph{outwards edge} is an edge connecting $\tau$ with an apocentric copy $T_n\prec T_{n+1}$. Roughly, \enquote{maximal uniform distribution of adjacencies} means that the end vertices of these edges that lie in $\tau$ are distributed \enquote{as if they were chosen at random}.
Then there are exactly $\delta_n$ \enquote{outwards edges} connecting $\tau_0$ to the apocentric copies $\tau_1,...,\tau_{\delta_n}\prec_{n-1} T_n$.
%
%More formally, let $\mathcal E$ be the set of outwards edges as defined above.
%For each apocentric copy $\tau'\prec_m \tau$ with $m\le n$ let $\mathcal E'\subseteq\mathcal E$ be the subset of outwards edges that end in $\tau'$.
%Then maximally uniform means that $\mathcal E'$ contains very close to the number of edges that one would expect, namely
\enquote{Maximal uniform distribution} means that every apocentric copy $\tau\prec_m \tau_0$ (where $m\le n-1$) intersects the expected number of these edges (up to rounding). More precisely, if $E_\tau$ is the number of the \enquote{outwards edges} that have an end in $\tau$, then
%
\begin{equation}\label{eq:max_uniform}
\Big\lfloor \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot \delta_n \Big\rfloor
\le
E_\tau
\le 
\Big\lceil \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot \delta_n \Big\rceil,
\end{equation}
%
where $(\delta_1\cdots\delta_m)/(\delta\cdots\delta_{n-1})$ is exactly the fraction of apocentric vertices of $\tau_0$ that are also in $\tau$ (\cf\ \cref{res:T_n_properties} \itm2).

% More formally, given the central copy $\tau_0\prec_{n-1} T_{n}$, % of $T_n$ in $T_{n+1}$. 
% %An \emph{outwards edge} is an edge connecting $\tau$ with an apocentric copy $T_n\prec T_{n+1}$. Roughly, \enquote{maximal uniform distribution of adjacencies} means that the end vertices of these edges that lie in $\tau$ are distributed \enquote{as if they were chosen at random}.
% let $\mathcal E_0\subseteq E(T_{n})$ be its set of \enquote{outwards edges}, % emanating from $\tau$,
% \ie\ edges connecting $\tau_0$ with the apocentric copies $\tau_1,...,\tau_{\delta_n}\prec_{n-1} T_n$.
% %
% %More formally, let $\mathcal E$ be the set of outwards edges as defined above.
% %For each apocentric copy $\tau'\prec_m \tau$ with $m\le n$ let $\mathcal E'\subseteq\mathcal E$ be the subset of outwards edges that end in $\tau'$.
% %Then maximally uniform means that $\mathcal E'$ contains very close to the number of edges that one would expect, namely
% Then, every apocentric copy $\tau\prec_m \tau_0$ (where $m\le n-1$) intersects the expected number of these outwards edges, up to rounding. More precisely, if $\mathcal E\subseteq\mathcal E_0$ is the subset of edges that have one end in $\tau$, then
% %
% \begin{equation}\label{eq:max_uniform}
% \Big\lfloor \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot |\mathcal E_0|\, \Big\rfloor
% \le
% |\mathcal E| 
% \le 
% \Big\lceil \, \frac{\delta_1\cdots\delta_m}{\delta_1\cdots\delta_{n-1}} \cdot |\mathcal E_0|\, \Big\rceil    
% \end{equation}
% %
% Note that $(\delta_1\cdots\delta_m)/(\delta\cdots\delta_{n-1})$ is exactly the fraction of apocentric vertices of $\tau_0$ that are in $\tau$ (see \cref{res:T_n_properties} \itm2).

It is not hard to see that in each step of \cref{constr:T_n} this distribution can be achieved by adding the \enquote{outwards edges} one by one. % (\eg\ choose the next apocentric vertex of $\tau_0$ maximally distant from all previously chosen apocentric vertices).
The reader can verify that the steps shown in \cref{fig:construction} are in accordance with~a~max\-imally uniform distribution.

%Maximal uniform distribution of the connections from the apocentric vertices of $\tau$ to the apocentric copies of $T_{n}\prec T_{n+1}$ means, roughly, that the 

% We give a rigorous definition of what we mean by \enquote{maximally uniform distribution of adjacencies}.

% Let $\tau\prec_n T_{n+1}$ be the central copy of $T_n$.
% Let $a(\tau)\in\NN$ be its number of apocentric vertices and $a_+(\tau)\le a(\tau)$ the number of \emph{outwards vertices} among them, that is, apocentric vertices that are adjacent to apocentric copies $T_n\prec T_{n+1}$. 
% \enquote{Maximally uniform distribution of connections} means that for each apocentric copy $\tau' \prec_m \tau$, where $m\le n$, the number $a_+(\tau')$ of outwards vertices in $\tau'$ is maximally close to what we would expect if the adjacencies were distributed at random:
% %
% $$
% \Big\lfloor\, \frac{a_+(\tau)}{a(\tau)}\cdot a(\tau')\, \Big\rfloor
% \le a_+(\tau')
% \le \Big\lceil\, \frac{a_+(\tau)}{a(\tau)} \cdot a(\tau') \, \Big\rceil.
% $$
\end{remark}

We close with three examples demonstrating the versatility~of~\cref{constr:T}.
%For conciseness we use $\bar g(r):=g(r-1)$, then $f(n)=\bar g(2^n)$.

\begin{example}[Polynomial growth]\label{ex:polynomial}
If we aim for polynomial growth $g(r)=r^\alpha,\alpha\in\NN$ then the heuristics \eqref{eq:suggestions} suggests to use a constant sequence $\delta_n:=2^\alpha-1$.

In fact, the corresponding trees $T_n$ embed nicely into the $\alpha$-th power%
\footnote{Recall, the $\alpha$-th power of $G$ is a graph $G^\alpha$ with vertex set $V(G)$ and an edge between any to vertices whose distance in $G$ is at most $\alpha$.}
of~the~$\alpha$-dimensional lattice graph (shown in \cref{fig:2_lattice_construction} for $\alpha=2$). %, giving further evidence for polynomial volume growth.
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.92\textwidth]{img/2_lattice_subgraph_3.pdf}
    \caption{
        Embedding of the tree $T(3,3,...)$ into the square of the 2-dimensional lattice graph.
    }
    \label{fig:2_lattice_construction}
\end{figure}

More generally, for any constant sequence $\delta_n:=c$ we expect to find polynomial volume growth, potentially with a non-integer exponent $\log(c+1)$.
\end{example}

\begin{example}[Exponential growth]\label{ex:exponential}
%The $d$-regular tree has growth function $\bar g(r)=d(d-1)^r$. This yield $f(n)=d(d-1)^{2^n}$ and $\delta_n=(d-1)^{2^{n-1}}$.
For the sequence $\delta_n:=d^{\kern0.15ex 2^{n-1}}\!,d\in\NN$ the~centric limit $T$ is the $d$-ary tree,
%Replacing $d_1:=d+2$ will result in the $(d+1)$-regular tree.
in particular, of exponential volume growth (see~\cref{fig:binary_tree} for the case $d=2$, \ie\ the binary tree).
In fact, using \eqref{eq:ball_volume_in_T} for $r=2^n$ (where $x^*\in V(T)$ is the global center) we find
%
 $$|\ball T{x^*\!}{r-1}| = (\delta_1+1)\cdots(\delta_n+1)=\prod_{k=1}^n \Big(d^{\kern0.15ex 2^{k-1}}\!\!+1\Big) = \sum_{i=0}^{\mathclap{2^n-1}} d^{\kern0.15ex i} = \frac{d^{\kern0.15ex 2^n}-1}{d-1} = \frac{d^{\kern0.15ex r}-1}{d-1}.$$
%
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.85\textwidth]{img/binary_tree.pdf}
    \caption{
        The binary tree as constructed from \cref{constr:T_n} using the doubly exponential sequence $\delta_n=2^{2^{n-1}}$.
    }
    \label{fig:binary_tree}
\end{figure}
\end{example}

Extrapolating from \cref{ex:polynomial} and \cref{ex:exponential}, it seems reasonable that unbounded sequences $\delta_1,\delta_2,\delta_3,...$ with a growth sufficiently below doubly exponential result in intermediate volume growth.

\begin{example}[Intermediate growth]\label{ex:loglogr}
For $\delta_n:=(n+3)^\alpha -1$, $\alpha\in\NN$ we can compute this explicitly (see \cref{fig:construction} for the case $\alpha=1$).
If $T$ is the centric limit with global center $x^*\in V(T)$ and $r=2^n$, then:
%
\begin{align*}
%\bar g(r) 
|\ball T{x^*\!}{r-1}|
= (\delta_1+1)\cdots(\delta_n+1) 
&= (\tfrac16 (n+3)!)^\alpha 
 \sim (n! n^3)^\alpha
 \sim (n^n e^{-n} n^{7/2})^\alpha 
\\ &= r^{\alpha \log\log r} r^{-\alpha/\ln 2}\, (\log r)^{7\alpha/2}
%  \sim \tfrac16(n! n^3)^\alpha
%  \sim \tfrac16(n^n e^{-n} n^{7/2})^\alpha 
% \\ &= \tfrac16r^{\alpha \log\log r} r^{-\alpha/\ln 2}\, (\log r)^{7\alpha/2}
\end{align*}
%
We therefore expect this choice of sequence to lead to a tree of uniform intermediate volume growth.
Trees constructed from $\delta_n\sim n^\alpha$ present an interes\-ting~boundary case in \cref{sec:unimodular} when we discuss unimodular random trees (see~\cref{res:types_of_limits}).
% \begin{align*}
% |\ball T{x^*}{r-1}| = |T_n|= \tfrac16 (n+3)! 
% \, &\sim\,
% n! \, n^3  
% \,\sim\,
% % n^n \cdot n^{9/2}e^{-n}
%  n^n e^{-n} \sqrt n \, n^3 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \cdot (\log r)^{7/2}  .
% %\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
% \end{align*}
\end{example}

%\newpage

\section{Uniform volume growth}
\label{sec:main}


We fix an increasing function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ that shall serve as our target growth rate. %; we also set $\bar g(r)$ $:=g(r-1)$.
The goal of this section is to construct an appro\-priate sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ for which we can show that $T:=T(\delta_1,\delta_2,...)$ is of uniform volume growth $g(r)$. 
%\textcolor{lightgray}{
We shall show in particular that this is feasible if $g$ is super-additive and log-concave, thus proving \cref{main}.
%}

Recall that the uniform growth rate of a graph must be at least linear (like in~a path graph) and at most exponential (like in a regular tree).
It would therefore~be reasonable to impose these constraints on the target growth rate $g$ right away.\nlspace
%As $g$ is supposed to be the uniform growth rate of a locally finite graph, intuitively we should require that $g$ grows at least linearly and at most exponentially.
However, we shall not do this: these constraints will also emerge naturally during our journey towards the main theorem of this section.
In fact, we shall uncover even more precise constraints expressed in terms of the sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ (see \cref{rem:c,rem:dbar}) and we discuss how they relate to the natural constraints of $g$ growing at least linear and at most exponential.
% (see \cref{rem:c} and \cref{rem:dbar}, as well as \cref{thm:main})
%These can often be expressed more directly in terms of the sequence of $\delta_n$, but we make an effort to provide versions in terms of $g$ as well.

Following our motivation from the last section we first try to approximate $g(2^n)$ by $(\delta_1+1)\cdots(\delta_n+1)$.

\begin{lemma}\label{res:d_i}
There exists a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ so that
%
\begin{equation}\label{eq:d_bounds}
(1-c)\cdot g(2^n)  \;<\; (\delta_1+1)\cdots(\delta_n+1) \;<\; (1+c)\cdot g(2^n),
\end{equation}
%
for all $n\ge 0$, where $c:=\sup_n g(2^n)/g(2^{n+1}) \le 1$.
%
\begin{proof}
For this proof we abbreviate $\bar\delta_n:=\delta_n+1$. 
We set $\bar\delta_1 := g(2)$ and recursively %\msays{$f(1)$ might not be an integer}
%
$$\bar\delta_{n+1}:=\begin{cases}
\lceil g(2^{n+1})/g(2^n)\rceil & \text{if $\bar\delta_1\cdots\bar\delta_{n}\le g(2^n)$}\\
\lfloor g(2^{n+1})/g(2^n)\rfloor & \text{if $\bar\delta_1\cdots\bar\delta_{n}> g(2^n)$}
\end{cases}.
$$

This sequence satisfies \eqref{eq:d_bounds} as we show by induction on $n$: the induction base is clear from the definition of $\bar\delta_1$. Next, if \eqref{eq:d_bounds} holds for $n$, and $\bar\delta_1\cdots\bar\delta_{n}\le g(2^n)$, then
%
\begin{align*}
\bar\delta_1\cdots \bar\delta_n \cdot\bar\delta_{n+1} &\le g(2^n) \cdot\Big\lceil \frac{g(2^{n+1})}{g(2^n)} \Big\rceil 
< g(2^n)\cdot \Big( \frac{g(2^{n+1})}{g(2^n)} + 1\Big)
\\&= \Big( 1+ \frac{g(2^n)}{g(2^{n+1})} \Big) \cdot g(2^{n+1}) \le ( 1+ c )\cdot  g(2^{n+1}), \\[1ex]
\bar\delta_1\cdots \bar\delta_n \cdot\bar\delta_{n+1} 
&> (1-c)\cdot g(2^n)\cdot \Big\lceil \frac{g(2^{n+1}}{g(2^n)} \Big\rceil 
\ge (1-c)\cdot g(2^n)\cdot \frac{g(2^{n+1})}{g(2^n)}
\\&=(1-c)\cdot g(2^{n+1}).
\end{align*}
%
An analogous argument applies in the case $\bar\delta_1\cdots\bar\delta_{n}> g(2^n)$.
\end{proof}
\end{lemma}

%In the following let $\delta_1,\delta_2,\delta_3,...\in\NN$ be the sequence constructed in the proof of \cref{res:d_i}.

\begin{remark}\label{rem:c}
Recall that \cref{constr:T_n} requires $\delta_n \ge1$ for all $n\ge 1$ in order for $T(\delta_1,\delta_2,...)$ to be well-defined.
The sequence provided by the proof of \cref{res:d_i} does not generally have this property unless further requirements on $g$ are met.
%
One such is \emph{super-additivity}, which turns out to also formalize the idea of \enquote{$g$ growing at least linearly}.

Super-additivity means $g(r_1+r_2)\ge g(r_1)+ g(r_2)$ and indeed implies $g(2^{n+1}) = g(2^n+2^n)\ge 2g(2^n)$, and hence
%
%More precisely, the following is sufficient: $g(1)\ge 2$ and $\bar g$ is \emph{super-additive}, \ie\ $\bar g(r_1+r_2)\ge \bar g(r_1)+\bar g(r_2)$.
%Then $\bar g(2r)\ge 2\bar g(r)\implies f(n+1)\ge 2f(n)$, from which follows
%
$$\delta_{n+1}+1\ge \Big\lfloor\frac{g(2^{n+1})}{g(2^n)}\Big\rfloor \ge 2.$$
%
%In the following we shall therefore assume that $g$ is super-additive.
%This formalizes \enquote{$g$ should grow at least linearly}, and also yields
%This implies 
This moreover implies $c:=\sup_n g(2^n)/g(2^{n+1}) \le 1/2 <1$ and guarantees that the lower bound in \cref{res:d_i} is not vacuous.
%
%Together with $g(0)=1$, these are the only requirements on the growth of $g$ from below.
%This also captures the intuition that $g$ should grow \enquote{at least linearly}.
\end{remark}

%In the following we assume that $g$ is super-additive to ensure that $T$ exists.

\begin{remark}\label{rem:dbar}
%\Cref{constr:tree} provide a reason to put upper bounds on the growth of $g$:
%An upper bound on the growth of $g$ emerges as necessary~if~we~investigate the vertex degrees in $T$.
Recall that graphs of uniform growth are necessarily of bounded~degree.
But again, the sequence constructed in the proof of \cref{res:d_i} does not~necessarily produce such a tree unless further requirements on $g$ are met.
We elaborate how these requirements can be interpreted as \enquote{$g$ growing at most exponentially}.
%
%Making sure that \cref{constr:T} yields such a graph leads us to a more precise formulation of \enquote{$g$ should grow at most exponentially}.
% by the fact that graphs of uniform growth are necessarily of finite maximum degree.

The tree $T_{n-1}$ has exactly $\delta_1\cdots\delta_{n-1}$ apocentric vertices. That is, each apocentric vertex of the central copy $\tau_0\prec_{n-1}T_n$ is adjacent, on average,\nlspace to
%
\begin{equation}\label{eq:Delta}
\Delta(n):= \frac{\delta_n}{\delta_1\cdots\delta_{n-1}}
\end{equation}
%
apocentric copies $\prec_{n-1} T_n$.
By the maximal uniform distribution of adjacencies (\cf\ \cref{rem:max_uniform}) the maximum degree among the apocentric vertices of $\tau_0$ is exactly $\lceil \Delta(n) \rceil + 1$.
Thus, since $T$ contains $T_n$ for each $n\ge 0$, $T$ is of bounded degree~only if $\bar \Delta:=\sup_n \lceil\Delta(n)\rceil + 1<\infty$.
We can use this to put an upper bound on the growth of the sequence $\delta_1,\delta_2,\delta_3,...$: for $n\ge 2$ holds
%Expanding \eqref{eq:Delta} under the constraint $\Delta(n)\le\bar \Delta-1$ yields
%One can expand \eqref{eq:Delta} under this bound  to obtain % that this bound together with \eqref{eq:Delta} yields
%
$$
\frac{\delta_n}{\delta_1\cdots\delta_{n-1}}\le\bar\Delta - 1
\;\implies \;
\delta_n\le \big((\bar \Delta-1)\delta_1\big)^{2^{n-2}}.
$$
%
Comparing with \cref{ex:exponential} suggests that $g$ grows at most exponentially. 

%Besides bounding the growth of $g$, putting an upper bound on $\Delta(n)$ has further more subtle effects, such as preventing strong oscillations in the growth of $g$ (see~\eg\ \cref{res:conditions_in_g}).

% More precisely, the maximum degree among apocentric vertices of $T_{n-1}$ (when viewed as vertices in $T$) is $\lceil\Delta(n)\rceil+1$.
% Since a graph of uniform volume growth must be locally finite, we found that $\Delta$ must be bounded.
% This imposes a first necessary upper bound on the growth of $g$: roughly, this corresponds to $g$ growing at most exponentially; but it is more subtle in that it also prevents strong oscillations in the growth of $g$.

% However, $\Delta$ being bounded is not quite sufficient for uniform volume growth.
% In the following main theorem we show that a comparatively simple sufficient criterion can be nicely stated in terms of $\Delta$ as well.
\end{remark}

It remains to prove the main result of this section: establishing the exact growth rate of $T=T(\delta_1,\delta_2,...)$ in terms of $g$.
As we shall see, bounded degree (as discussed in \cref{rem:dbar}) is not sufficient to prove uniform volume growth. Instead we require an additional criterion that can also be concisely expressed in terms of the function $\Delta$.
In terms of $g$ this can be interpreted as preventing too strong oscillations in the growth of $g$ (\cf\ \cref{res:conditions_in_g}).

In order to state the main result we recollect that $g\:\NN_0 \to\NN$ is a strictly~increas\-ing super-additive function.
The sequence $\delta_1$,\nlspace $\delta_2$, $\delta_3,...$ $\in\NN$ is chosen to satisfy
%
$$
(1-c)\cdot g(2^n)  \;<\; (\delta_1+1)\cdots(\delta_n+1) \;<\; (1+c)\cdot g(2^n),
$$
for some $c\le 1/2$ (according to \cref{res:d_i}) and satisfies $\delta_n\ge 1$ by \cref{rem:c}. In particular, $T=T(\delta_1,\delta_2,...)$ exists.
Finally, $\Delta(n)$ is defined as in \eqref{eq:Delta}. The~main~result then reads as follows:


\iffalse 

% The choice of the sequence allows us to model a wide variety of trees. An~erratically looking example is shown in \cref{fig:construction} using the sequence $\delta_n=n+2$.
% This tree turns out to be of uniform intermediate volume growth.
% With $\delta_1=d+1$ and $\delta_n=d^{2^{n-1}},n\ge 2$ we obtain the $d$-regular tree which is clearly of uniform exponential volume growth.
% For constant sequence $\delta:=2^\alpha$ we find a sub-tree of the $(\alpha$-th power of the) $\alpha$-dimensional lattice graph, and we shall see that it is of uniform polynomial volume grwoth.

\noindent\hrulefill

We demonstrate the general idea of the construction with the following example aiming for intermediate growth in the vicinity of $r^{\log\log(r)}$.

% \begin{example}\label{ex:loglogr}
% Let $T_0$ be the 3-star, that is, the tree consisting of a vertex $x^*$~(which we call the \emph{root} of $T_0$) adjacent to three leaves (that we call the \emph{apocentric~vertices} of $T_0$).
% We then define trees $T_n,n\ge 1$ recursively as follows (\cf\ \cref{fig:construction}):
% %
% \begin{itemize}
%     \item let $T_1$ consist of \emph{four} copies of $T_0$ attached to another central copy of~$T_0$~(in a way that we make precise below).
%     \item let $T_2$ consist of \emph{five} copies of $T_1$ attached to another central copy of $T_1$.
%     \item let $T_3$ consist of \emph{six} copies of $T_2$ attached to another central copy of $T_2$.
%     \item ...
% \end{itemize}
% %
% In each step we have $n+3$ non-central copies of $T_{n-1}$ that we will call the \emph{\mbox{apocentric} co\-pies}. The root of the central copy of $T_{n-1}$ will continue to be called the root~of~$T_n$, and the apocentric vertices of the apocentric copies of $T_{n-1}$ will be called apocentric vertices of $T_n$. % (all of which are leaves, but not all leaves are apocentric; see also \cref{fig:construction}).

% %
% % \begin{itemize}
% %     \item let $T_1$ be a copy of $T_0$ (the \emph{central copy}) and \emph{four} further copies of $T_0$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy (it is permitted to identify more than one root to an apocentric vertex).
% %     \item let $T_2$ be a copy of $T_1$ (the \emph{central copy}) and \emph{five} further copies of $T_1$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy.
% %     \item let $T_3$ be a copy of $T_2$ (the \emph{central copy}) and \emph{six} further copies of $T_2$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy.
% %     \item ...
% %     \item let $T_n$ be a copy of $T_{n-1}$ (the \emph{central copy}) and $n-3$ further copies of $T_{n-1}$ (the \emph{apocentric copies}) whose roots are identified with some of the apocentric vertices of the central copy (it is permitted to identify more than one root to an apocentric vertex, though in this example this is only necessary to define $T_1$).
% % \end{itemize}

% It remains to give a precise meaning to the \enquote{attachment of the apocentric copies}:
% in each step, each apocentric copy of $T_{n-1}$ is \enquote{attached to the central copy of $T_{n-1}$} by identifying its root with some apocentric vertex of the central copy. 
% The choice of the apocentric vertex is more or less free (we can even attach more than one copy to the same vertex).
% However, it will be important for the analysis of the growth behavior that we do this in a maximally uniform manner, attaching approximately the same number of copies to each apocentric vertex.

% If we now identify $T_{n-1}$ with its central copy in $T_n$ we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $T:=\bigcup_{n\ge 0} T_n$ is well-defined.
% We claim that $T$ is a tree of intermediate volume growth.

% To see that this is plausible, make the following two observations:
% %We want to make this at least plausible. Observe the following:
% %
% \begin{itemize}
%     \item the distance from the root of $T_n$ to any apocentric vertex is exactly $2^n$. In fact, $T_n\subset T$ is the ball of radius $2^n$ centered at the \emph{global root} $x^*$ in $T$.
%     \item it holds $|T_n|=4\cdot5\cdots (n+4)=\frac16(n+4)!$. %\,\sim\, n^4n!\,\sim\, n^4 \cdot n^n \sqrt n \,e^{-n}$ 
%     %\sim n^4n! $.
% \end{itemize}
% %
% Thus, for $r=2^n$ we can estimate
% %
% \begin{align*}
% |\ball T{x^*}r| = |T_n| = \tfrac16 (n+4)! 
% \,&\sim\,
% n! \, n^4  
% \,\sim\,
% % n^n \cdot n^{9/2}e^{-n}
%  n^n e^{-n} \sqrt n \, n^4 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \, (\log r)^{9/2}  .
% %\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
% \end{align*}
% %
% Recall that we are using $\log r := \log_2 r$.

% While this suggests intermediate growth for balls around the global root $x^*$, we still need to establish
% %
% \begin{itemize}
%     \item a similar volume growth around other vertices of $T$, in particular, we need~to establish that the growth is \emph{uniform}, and
%     \item that a similar estimation is valid for balls of radii that are not of the form~$2^n$.
% \end{itemize}
% %
% Both points will be addressed in the discussion of the general construction.
% \end{example}

\begin{example}\label{ex:loglogr}
Let $T_0:=\{x^*\}$ be the tree consisting of a single vertex (called \emph{global root}).
We proceed by recursively defining trees $T_n,n\ge 1$ as follows (\cf\ \cref{fig:construction}): 
%
\begin{itemize}
    \item let $T_1$ consist of \emph{three} copies of $T_0$ connected to another central copy of~$T_0$.
    \item let $T_2$ consist of \emph{four} copies of $T_1$ connected to another central copy of $T_1$.
    \item let $T_3$ consist of \emph{five} copies of $T_2$ connected to another central copy of $T_2$.
    \item ...
\end{itemize}
%
In each step we add $n+2$ \enquote{non-central} copies of $T_{n-1}$ that we shall call the~\emph{apocentric co\-pies} of $T_{n-1}$. 
In order to describe the connection between the central and the apocentric copies we need to introduce the notion of \emph{root} and \emph{apocentric vertex} of $T_n$:
%
\begin{itemize}
    \item the unique vertex $x^*$ of $T_0$ is both the root and an apocentric vertex of $T_0$.
    \item the root of $T_n$ is the root of its central copy of $T_{n-1}$.
    \item an apocentric vertex of $T_n$ is an apocentric vertex in an apocentric copy of $T_{n-1}$ (all of them are leave of $T_n$, but not all leaves are apocentric).
\end{itemize}
%
% \begin{figure}[!h]
%     \centering
%   % \includegraphics[width=0.7\textwidth]{img/construction.pdf}
%   % \includegraphics[width=0.65\textwidth]{img/construction_2.pdf}
%     \includegraphics[width=0.83\textwidth]{img/construction_3.pdf}
%     \caption{Illustration of the first four steps in the  construction~of~\cref{ex:loglogr}. The ringed vertex is the root and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy of $T_{n-1}$ in $T_n$.}
%     \label{fig:construction}
% \end{figure}
%
We can now finalize the definition of $T_n$: each apocentric copy of $T_{n-1}$ is connected to the central copy of $T_{n-1}$ by adding an edge between the root of the apocentric copy and some apocentric vertex of the central copy.
The choice of the apocentric vertex in the central copy is more or less free (we can even connect more than one apocentric copy to the same vertex).
However, it will be important for the analysis of the growth behavior that we do this in a maximally uniform manner, attaching approximately the same number of copies to each apocentric vertex.

If we now identify $T_{n-1}$ with its central copy in $T_n$ we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ and the union $T:=\bigcup_{n\ge 0} T_n$ is well-defined.
We claim that $T$ is a tree of intermediate volume growth.

To see that this is plausible, make the following two observations:
%We want to make this at least plausible. Observe the following:
%
\begin{itemize}
    \item the distance from the root of $T_n$ to any apocentric vertex is exactly $2^n-1$. In fact, $T_n\subset T$ is the ball of radius $2^n-1$ centered at the global root~$x^*$.
    \item for $n\ge 1$ holds $|T_n|=4\cdot5\cdots (n+3)=\frac16(n+3)!$. %\,\sim\, n^4n!\,\sim\, n^4 \cdot n^n \sqrt n \,e^{-n}$ 
    %\sim n^4n! $.
\end{itemize}
%
Thus, for $r=2^n$ we can estimate
%
\begin{align*}
|\ball T{x^*}{r-1}| = |T_n|= \tfrac16 (n+3)! 
\, &\sim\,
n! \, n^3  
\,\sim\,
% n^n \cdot n^{9/2}e^{-n}
 n^n e^{-n} \sqrt n \, n^3 
\\ &= \,
r^{\log\log r}\cdot
r^{-1/\ln 2} \cdot (\log r)^{7/2}  .
%\cdot q\big(\!\sqrt{\log r}\kern0.75pt\big)
\end{align*}
%
Recall the convention $\log r := \log_2 r$.

While this suggests intermediate growth for balls around the global root $x^*$, we still need to establish
%
\begin{itemize}
    \item a similar volume growth around other vertices of $T$, in particular, we need~to establish that the growth is \emph{uniform}, and
    \item that a similar estimation is valid for balls of radii other than $2^n-1$.
\end{itemize}
%
Both points will be addressed in the discussion of the general construction.



% We make two simple observations:
% %
% \begin{itemize}
%     \item the distance from the central vertex of $T_n$ to an apocentric vertex of $T_n$ is exactly $2^n-1$, and
%     \item for $n\ge 1$ holds $|T_n|=4\cdot5\,\cdots\, (n+3)=\frac16 (n+3)!$\,.
% \end{itemize}
% %
% If we identify $T_{n-1}$ with its central copy in $T_{n}$, we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset \cdots$ and the limit tree $T:=\bigcup_n T_n$ is well-defined. Technically, we can interpret $(T,x^*)$ as the distributional limit of the sequence $(T_n,o_n)$ of biased random rooted trees, where $o_n$ is the global center of $T_n$ with probability $1$. 

% Setting $r=2^n-1$, a straight-forward estimation shows
% %
% \begin{align*}
% |\ball T{x^*}r| = |T_n| = \tfrac16 (n+4)! 
% \,&\sim\,
% n! \, n^4  
% \,\sim\,
%  n^n e^{-n} \sqrt n \, n^4 
% \\ &= \,
% r^{\log\log r}\cdot
% r^{-1/\ln 2} \, (\log r)^{9/2}.
% \end{align*}

% %Thus, we expect intermediate volume growth around the global center~$x^*$ and it remains to establish suitable behavior for the other vertices.

% Thus, we found intermediate volume growth, at least around the global root~$x^*$ for radii of the form $r=2^n,n\in\NN$.
% It would then remain to establish that
% %
% \begin{myenumerate}
%     \item a similar estimation holds for balls centered at other vertices, and
%     \item the estimation does not deviate too much from the intended growth for radii that are not of the form $2^n$.
% \end{myenumerate}
% %
% We postpone the discussion of these details until the discussion of the general case in \cref{res:g_growth_trees}.
\end{example}

The strength of the construction in \cref{ex:loglogr} lies in the many free parameters that we can use to model a wide range of growth behaviors.
More precisely,\nlspace after choosing a sequence $\delta_0,\delta_1,\delta_2,...\in\NN$ we can consider the following analogous~construction for the $T_n$:
%
\begin{itemize}
    \item let $T_0$ be the $\delta_0$-star, that is, the tree consisting of a vertex $x^*$ adjacent to $\delta_0$ further vertices.
    \item let $T_n,n\ge 1$ consist of $\delta_n$ copies of $T_{n-1}$ attached to a further central copy.
\end{itemize}
%
In \cref{ex:loglogr} we used $\delta_n:=n+3$.

If we set $T:=\bigcup_{n\ge 0} T_n$ as before, then we again find that $T_n\subset T$ is~the~ball~in $T$ of radius $2^n$ centered at the global root $x^*$.
But now these balls have volume~$|T_n|=(\delta_0+1)\cdots(\delta_n+1)$, and so to achieve a specific volume growth $g\:\NN_0\to\RR$~it is plausible to choose integers $\delta_0,\delta_1,\delta_2,...\in\NN$ for which $(\delta_1+1)\cdots(\delta_n+1)$ approximates the growth of $f(n):=g(2^n)$.

% This construction has many free parameters (the number of copies of $T_{n-1}$ that make up $T_n$) that allow us to model a wide range of growth behaviors. 
% If the~total number of copies in step $n$ (central and apocentric) is $\delta_n$, then $|T_n|=\delta_1\cdots \delta_n$, and so a first step towards the general construction is to choose the $\delta_i$ so that $\delta_1\cdots\delta_n$ approximates the desired growth, more precisely, $f(n):=g(2^n)$.


% \textcolor{lightgray}{
% As we shall see, we can most often not guarantee $|\ball Gvr|=\theta(g(r))$. For that reason, the function $g$ shall be called \emph{target growth} of our construction, in the sense that we aim for achieving this growth, but the actually provable lower and upper bounds on $|\ball Gvr|$ will be not quite $g$, but slight modifications thereof (see \cref{res:g_growth_trees}).
% }

% In order to construct this tree, we need to approximate the desired growth function $g(r)$, or more precisely $f(n):=g(2^n-1)$, by a product of integers~$\delta_1,\delta_2,\delta_3,...\in\NN$, that is, we want
% %
% $$\delta_1\cdots\delta_n\in \theta(f(n)).$$
% %
% %We call this sequence of $\delta_i$ the \emph{decomposition sequence} of $f$ (\resp\ $g$).

\begin{lemma}\label{res:d_i}
Given an increasing function $f\:\NN_0\to\RR$, there is a sequence of integers $\delta_1,\delta_2,\delta_3,...\in\NN$ so that
%
\begin{equation}\label{eq:d_bounds}
(1-c)\cdot f(n)  \;<\; \delta_1\cdots\delta_n \;<\; (1+c)\cdot f(n),\qquad\text{for all $n\ge 0$}
\end{equation}
%
%
where $c:=\sup_n (f(n)/f(n+1)) \le 1$.
%
\begin{proof}
Set $\delta_1 := f(1)$.
Then define iteratively
%
$$\delta_{n+1}:=\begin{cases}
\lceil f(n+1)/f(n)\rceil & \text{if $\delta_1\cdots\delta_{n}\le f(n)$}\\
\lfloor f(n+1)/f(n)\rfloor & \text{if $\delta_1\cdots\delta_{n}> f(n)$}
\end{cases}.
$$

That this definition satisfies \eqref{eq:d_bounds} is shown by induction. It is clearly satisfied for $n=1$. If it is satisfied for $n$ and $\delta_1\cdots\delta_{n}\le f(n)$, then
%
\begin{align*}
\delta_1\cdots \delta_n \cdot\delta_{n+1} &\le f(n) \cdot\Big\lceil \frac{f(n+1)}{f(n)} \Big\rceil 
< f(n)\cdot \Big( \frac{f(n+1)}{f(n)} + 1\Big)
\\&= \Big( 1+ \frac{f(n)}{f(n+1)} \Big) \cdot f(n+1) \le ( 1+ c )\cdot  f(n+1), \\[1ex]
\delta_1\cdots \delta_n \cdot\delta_{n+1} 
&> (1-c)\cdot f(n)\cdot \Big\lceil \frac{f(n+1)}{f(n)} \Big\rceil 
\ge (1-c)\cdot f(n)\cdot \frac{f(n+1)}{f(n)}
\\&=(1-c)\cdot f(n+1).
\end{align*}
%
Equivalently for the case $\delta_1\cdots\delta_{n}> f(n)$.
\end{proof}
\end{lemma}

Note that the lower bound is useful only for $c<1$, which requires $f(n)=g(2^n-1)$ to grow at least exponentially, or equivalently, $g(r)=\Omega(r)$.

Most properties of the constructed tree can be concisely expressed in terms of the sequence $\delta_n$.
Ultimately we are interested in expressing these properties in~terms of $g$, and so we shall spend some time understanding the relation between $g$ and its sequence.
The following list contains some first examples of this:
%
\begin{itemize}
    \item 
    A polynomial function $g(r)=r^\alpha$ will have a constant sequence $\delta_n=2^\alpha$.\nlspace If $\delta_n$ is not a power of two then this models polynomial growth with non-integer exponent $\log_2\alpha$.
    
    \item As soon as the target growth is super-polynomial, that is $g(r)=r^{\omega(1)}$, the sequence $\delta_n$ is unbounded and $\delta_n/s_n\to 1$.
    
    \item 
    If $g$ is exponential, say $g(r)=b^r$, we obtain a sequence $\delta_n=b^{2^n}$.

    \item A special role will be played by target growth $g$ with sequence $\delta_n\sim n^\alpha$ for a fixed $\alpha>0$. Roughly, those correspond to growth behaviors of the order $r^{\alpha \log\log r}$. \cref{ex:loglogr} demonstrates this for $\alpha=1$.
    Later we shall find that for $\alpha>1$ our construction exhibits additional nice properties.
\end{itemize}

A necessary criterion for uniform volume growth is a finite maximum degree, and we need to check this for $T$.
Note that in each step of the construction, we add $\delta_n-1$ new apocentric copies of $T_{n-1}$ that need to be connected to the $(\delta_1-1)\cdots(\delta_{n-1}-1)$ apocentric vertices of the central copy of $T_{n-1}$ (all of which are leaves). If for each $n\ge 1$ we distribute the connections maximally uniformly, we can achieve maximum degree
%
$$\Delta:= \Big\lceil \sup_n \frac{\delta_{n}-1}{(\delta_1-1)\cdots(\delta_{n-1}-1)} \Big\rceil +1.$$
%
In particular, this value must be finite. So, when is this the case? Roughly speaking, when $g(r)=e^{\mathcal O(r)}$ and when $g$ changes its growth behavior not~too suddenly.\nlspace We~believe that $g$ being log-concave is sufficient.


% The maximum degree of the tree that we are going to construct can be expressed in terms of the $\delta_i$ as follows
% %
% $$\Delta:= \Big\lceil \sup_n \frac{\delta_{n}-1}{(\delta_1-1)\cdots(\delta_{n-1}-1)} \Big\rceil +1.$$
% % As long as $g$ is at most exponential, this yields a finite maximum degree $\Delta=\Delta(T)$.
% We require this expression to yield a finite value. 
% This happens, roughly speaking, if $g$ grows at most exponentially.
% But this condition also captures the more technical aspect that the growth behavior of $g$ should not change too rapidly.

% \begin{lemma}\label{res:Delta_def}
% If $g=e^{\mathcal O(r)}$ with decomposition sequence $\delta_1,\delta_2,\delta_3,...\in\NN$, then
% %
% $$\Delta:=\Big\lceil \sup_n\frac{\delta_n-1}{(\delta_1-1)\cdots(\delta_{n-1}-1)}\Big\rceil+1$$
% %
% is finite.
% \end{lemma}
% %
% \begin{proof}
% We have $f(n):=g(2^n)=e^{h(n)}$ with $h\in\mathcal O(2^n)$ strictly increasing, that is, $h(n)\le C2^n$ for all $n\ge N$. Following the construction of $\delta_n$ in the proof of \cref{res:d_i} this yields
% %
% $$\delta_n\le \Big\lceil\frac{f(n)}{f(n-1)}\Big\rceil \le \frac{f(n)}{f(n-1)} + 1 
% = e^{h(n)-h(n-1)}+1 \le e^{C2^n}+1.
% $$
% $$\delta_n\ge \Big\lfloor\frac{f(n)}{f(n-1)}\Big\rfloor \le \frac{f(n)}{f(n-1)} - 1 
% = e^{h(n)-h(n-1)}-1 \ge ...
% $$
% \end{proof}

% \begin{theorem}
% Given a strictly increasing function $g\in \mathcal O(e^r)$ with $g(r)\ge r$, there is a tree $T$ all whose vertices $v\in V(T)$ satisfy
% %
% $$A \cdot g(r/4) \le |B_v^T(r)|\le B \cdot g(2r)^2,\quad\text{for all $r\ge 0$},$$
% %
% with $A>0$ and $B<8\Delta$, where $\Delta:= \lceil \sup_n g(2^{n+1})/g(2^n) \rceil + 1$ is the maximum~degree of $T$.
% \end{theorem}

We can now prove that $T$ has the desired volume growth around \emph{every} vertex.

% \begin{theorem}
% Let $\delta_1,\delta_2,\delta_3,...\in\NN$ be a sequence of integers with
% %
% $$\delta_{n+1}\le(\Delta-1)\delta_1\cdots\delta_n$$
% %
% for some $\Delta\in\NN$. Set $f(n):=\delta_1\cdots\delta_n$.

% Then there exists a tree $T$ of maximum degree $\Delta$, all whose vertices $v\in V(T)$~satisfy
% %
% $$f(n-1) \;\le\; |B_v^T(2^n)| \;\le\; 2\Delta f(n)^2,\quad\text{for all $n\ge 0$},$$
% \end{theorem}

% \hrulefill

% \begin{theorem}
% Let $g\:\NN_0\to\NN$ be strictly increasing and let $\delta_1,\delta_2,\delta_3,...\in \NN$ be its decomposition sequence, so that (by \cref{res:d_i})
% %
% $$(1-c)\cdot g(2^n) \;\le\; \delta_1\cdots\delta_n \;\le\; (1+c)\cdot  g(2^n),\quad\text{for all $n\ge 1$}.$$
% %
% with $c<1$. If the $\delta_i$ satisfy
% $$\Delta:=\Big\lceil\sup_n\frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_n-1)}\Big\rceil + 1<\infty,$$
% %
% then there exists a tree $T$ of maximum degree $\Delta$, all whose vertices $v\in V(T)$~satisfy
% %
% $$(1-c) \cdot g(r/4) \;\le\; |B_v^T(r)| \;\le\; 2\Delta(1+c) \cdot g(2r)^2,\quad\text{for all $r\ge 0$},$$
% \end{theorem}

% \hrulefill

% \begin{theorem}\label{res:g_growth_trees}
% Given an increasing function $g\:\NN_0\to\NN$ and a sequence $\delta_1,\delta_2,\delta_3,...\in\NN$ of integers satisfying (see \cref{res:d_i})
% %
% $$ %\begin{equation}\label{eq:d_bounds}
% (1-c)\cdot g(2^n-1)  \;<\; \delta_1\cdots\delta_n \;<\; (1+c)\cdot g(2^n-1),\quad\text{for all $n\ge 0$}
% $$ %\end{equation}
% %
% Suppose that $\delta_i\ge 2$ (which implies $c\le 1/2$) and
% %
% \begin{equation}\label{eq:conditions_g}
% \Delta:= \Big\lceil \sup_n \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_n-1)} \Big\rceil +1 < \infty.
% \end{equation}
% %
% Then the tree $T$ is of maximum degree $\Delta$ and all its vertices \mbox{$v\in V(T)$} satisfy
% %
% $$\textstyle\frac12 \cdot g(\frac14r-\frac34) \;\le\; |B_v^T\!(r)| \;\le\; {\textstyle\frac92\Delta} \cdot g(2r+1)^2,\quad\text{for all $r\ge 0$}.$$
% % $$(1-c) \cdot g(r/4) \;\le\; |B_v^T(r)| \;\le\; 2\Delta(1+c)^2 \cdot g(2r)^2,\quad\text{for all $r\ge 0$}.$$
% \end{theorem}

% % \begin{theorem}\label{res:g_growth_trees}
% % Let $g\:\NN_0\to\NN$ be strictly increasing so that
% % %
% % \begin{equation}\label{eq:conditions_g}
% % c:=\sup_n \frac{g(r)}{g(2r)} < 1
% % \quad\text{and}\quad
% % \Delta:= \Big\lceil\frac{c+1}{(c-1)^2}\cdot \sup_r \frac{r\cdot g(2r)}{g(r)^2} \,\Big\rceil + 1 < \infty.
% % \end{equation}
% % %
% % Then there exists a tree $T$ of maximum degree at most $\Delta$, all whose vertices \mbox{$v\in V(T)$} satisfy
% % %
% % $$(1-c) \cdot g(r/4) \;\le\; |B_v^T(r)| \;\le\; 2\Delta(1+c)^2 \cdot g(2r + 1)^2,\quad\text{for all $r\ge 0$}.$$
% % \end{theorem}

% % Conditions \eqref{eq:conditions_g} is satisfied, roughly speaking, for all functions $g$ between (and~including) linear and exponential growth, but it also ensures that $g$ does not vary too strongly in its growth behaviour.
% % In particular, \cref{res:g_growth_trees} can be used to construct trees of \emph{uniform intermediate growth}.

% \begin{proof}
% % % By \cref{res:d_i} we can choose a sequence of integers $\delta_1,\delta_2,\delta_3,...\ge 1$ so that
% % % %
% % % $$(1-c)\cdot g(2^n) \;\le\; \delta_1\cdots\delta_n \;\le\; (1+c)\cdot  g(2^n),\quad\text{for all $n\ge 1$}.$$
% % % %
% % % where $c<1$ by the first condition in \eqref{eq:conditions_g}. 
% % % %A consequence from the other part of \eqref{eq:conditions_g} for later use is

% % We recursively define trees $T_n,n\in\NN_0$ as follows: let $T_0=\{\bullet\}$ be the tree~on a single vertex called the \emph{global center}.
% % For $n\ge 1$, let $T_n$ consist of $\delta_n$ disjoint copies of $T_{n-1}$; $\delta_n - 1$ so-called \emph{apocentric} copies, and one \emph{central} copy.
% % In order to~describe how to connect these sub-trees to form the tree $T_n$, we still need to define \emph{central} and \emph{apocentric} vertices:
% % %
% % \begin{myenumerate}
% %     \item the single vertex of the tree $T_0$ is both central and apocentric.
% %     \item a vertex of a tree $T_n$ is central (\resp\ apocentric) if it is contained in~a~cen\-tral (\resp\ apocentric) copy of $T_{n-1}$, and is central (\resp\ apocentric) in this copy.
% % \end{myenumerate}
% % %
% % Each tree $T_n$ has a unique central vertex and $(\delta_1-1)\cdots(\delta_n-1)$ apocentric vertices.

% % To finalize the definition of $T_n$ we add edges as follows: for each apocentric copy of $T_{n-1}$ add an edge between the central vertex of this copy and some apocentric vertex of the central copy of $T_{n-1}$. Do this in a way to keep the maximum degree of $T_n$ at or below $\Delta$, which is possible by condition \eqref{eq:conditions_g}:
% % %
% % % \begin{align*}
% % %     \frac{\#\{\text{new apocentric copies of $T_{n-1}$}\}}{\#\{\text{apocentric vertices in the central $T_{n-1}$}\}}
% % %     &=\frac{\delta_{n}-1}{(\delta_1-1)\cdots (\delta_{n-1}-1)}
% % %     \\&\le 2^{n-1}\cdot\frac{\delta_{n}}{\delta_1\cdots \delta_{n-1}}
% % %     \\&= 2^{n-1}\cdot\frac{\delta_1\cdots \delta_{n}}{(\delta_1\cdots \delta_{n-1})^2}
% % %     \\&\le \frac{c+1}{(c-1)^2} \cdot \frac{2^{n-1}\cdot g(2^{n})}{g(2^{n-1})^2} \le \Delta - 1.
% % % \end{align*}
% % \begin{align*}
% %     \frac{\#\{\text{new apocentric copies of $T_{n-1}$}\}}{\#\{\text{apocentric vertices in the central $T_{n-1}$}\}}
% %     &=\frac{\delta_{n}-1}{(\delta_1-1)\cdots (\delta_{n-1}-1)}
% %      \le \Delta - 1.
% % \end{align*}
% % %
% % We can now see that the the distance from the central vertex of $T_n$ to every apocentric vertex of $T_n$ is exactly $2^n - 1$. We also have $|T_n|=\delta_1\cdots \delta_n$, hence
% % %
% % $$(c-1)\cdot g(2^n - 1) \;\le\; |T_n| \;\le\; (1+c)\cdot g(2^n - 1).$$
% % %

% % % Note that this ensures that all apocentric vertices of $T_n$ are leaves, and that since $\delta_i\le (\Delta-1)\kern0.7pt\delta_1\cdots\delta_{i-1}=\text{\#apocentric vertices of $T_{i-1}$}$, the edges can be chosen to keep the maximal degree of $T_i$ at at most $\Delta$.

% % By identifying $T_{n-1}$ with its central copy in $T_n$, we can write down a chain~of graphs $T_0\subset T_1\subset T_2\subset \cdots$ with limit graph $T:=\bigcup_i T_i$. Clearly, $T$ is a tree. %We show that $T$ has the appropriate growth behavior.

% % % To show this, let $x^*$ be the \emph{global center}, \ie\ the central vertex of each of the canonical subgraphs $T_i\subset T$.
% % % Next, note the following properties of $T_i$:
% % % %
% % % \begin{myenumerate}
% % %     \item The vertices farthest away from the central vertex in $T_i$ are exactly the apocentric vertices at distance $2^i$. In particular, $B_{2^i}^T(x^*)=T_i$.
% % %     \item for $i\ge 1$ we have $|T_i| = (\delta_1+1)\cdots(\delta_i+1)=g(2^i)$.
% % % \end{myenumerate}

% %It remains to prove the lower and upper bounds on the size of balls in $T$. In the following, f
% Fix a vertex $v\in V(T)$ and a number $r\ge 0$. Let $T_n(v)$ denote the copy~of~$T_n$ (from the recursive construction of $T$) that contains $v$.

% To prove the lower bound, choose $n\in\NN$ so that $2^{n+1}-1\le r\le 2^{n+2}-1$. Let~$x$ be the central vertex of $T_n(v)$. Each vertex of $T_n(v)$ can be reached from $v$ in at most $2(2^n-1)\le r$ steps: at most $2^n-1$ steps from $v$ to $x$, and at most $2^n-1$ steps from $x$ to any other vertex of $T_n(v)$. Thus
% %
% $$|B_v^T\!(r)|\ge |B_v^T\!(2(2^n-1))|\ge |T_n| \ge (1-c)\cdot g(2^n-1) \ge {\textstyle\frac12}\cdot g(\textstyle\frac14r-\frac34).$$

% To establish the upper bound, choose $n\in\NN$ so that $2^{n-1} - 1\le r\le 2^n - 1$. Let $T_n(v)$ be the copy of $T_n$ that contains $v$. Let $m\in\NN$ be the largest integers so that the apocentric vertices of $T_n(v)$ are also apocentric in $T_m\subset T$. Necessarily $m\ge n$.

% We estimate the number of copies of $T_n$ that are connected to apocentric vertices of $T_n(v)$.
% Note that there are $\delta_1\cdots\delta_m$ apocentric vertices in $T_m\subset T$ and $\delta_1\cdots\delta_n$ apocentric vertices in $T_n(v)$. Assuming that the $\delta_{m+1}$ copies of $T_m$ that are attached to the apocentric vertices of $T_m\subset T$ are distributed maximally uniformly, we can expect that there are no more than
% %
% $$
% \Big\lceil \delta_{m+1} \cdot \frac{\delta_1\cdots\delta_n}{\delta_1\cdots\delta_m}\Big\rceil
% =
% \Big\lceil \frac{\delta_{m+1}}{\delta_1\cdots\delta_m} \cdot \Big( \frac{\delta_{n+1}}{\delta_1\cdots\delta_n}\Big)^{-1} \cdot \delta_{n+1} \Big\rceil
% $$
% %
% copies of $T_m$ attached to the apocentric vertices of $T_n(v)\subseteq T_m\subset $T$.

% \noindent\hrulefill

% To establish the upper bound, choose $n\in\NN$ so that $2^{n-1} - 1\le r\le 2^n - 1$ and enumerate the copies of $T_n$ that can be reached from $v$ in at most $2^n-1$ steps.
% Note that the only way \enquote{out of $T_n(v)$} is either through one of its apocentric vertices, or through its central vertex $x$:
% %
% \begin{itemize}
%     \item through an apocentric vertex: having reached an apocentric vertex of $T_n(v)$, up to $\Delta-1$ central vertices of other copies of $T_n$ can be reached. From these no further copies can be reached, as in the remaining $<2^n-1$ steps we cannot reach any apocentric vertex in the same copy. How many apocentric vertices of $T_n(v)$ can be reached in $\le 2^n-1$ steps? Hard to say, but at most $|T_n|$ many.
%     \item through the central vertex $x$: having reached $x$ (and assuming that $x$~is not the global center), we can reach an apocentric vertex $w$ of some \enquote{earlier} copy of $T_n$. Starting in $w$ we can reach other apocentric vertices of $T_n(w)$, certainly less than $|T_n|$ many. As before, from each apocentric vertex of $T_n(w)$ we can reach up to $\Delta-1$ central vertices of other copies of $T_n$, from which no further copies can be reached. Like-wise, in the remaining $<2^n-1$ steps we cannot reach from $w$ to the central vertex of $T_n(w)$, and so we enumerated all reachable copies of $T_n$.
% \end{itemize}
% %
% To summarize, we can reach at most $2\Delta\cdot|T_n|$ copies of $T_n$ (that is, $T_n(v)$, $T_n(w)$, and from each at most $(\Delta-1)|T_n|$ other copies via apocentric vertices). In each of those we can reach at most $|T_n|$ vertices. This yields
% %
% $$|B_v^T\!(r)| \le |B_v^T\!(2^n-1)| \le 2\Delta\cdot|T_n|^2 \le 2\Delta(1+c)^2\cdot g(2^n-1)^2 \le {\textstyle\frac92}\Delta\cdot g(2r+1)^2.$$
% \end{proof}


Let $\bar g\:\NN\to\RR^d$ be super-additive, \ie\ $\bar g(a+b)\ge \bar g(a)+\bar g(b)$.

\fi

%\newpage

%The following theorem proves the essential result, that under some mild technical conditions the tree $T$ is of uniform volume growth $g$.

%\msays{We need to emphasize more that $g$ is increasing.}

\begin{theorem}\label{thm:main}
Fix $v\in V(T)$ and $r\ge 0$. Then holds
%
\begin{myenumerate}
\setlength\itemsep{1ex}
\item \, \\ \,
\vspace{-2.325\baselineskip}
\begin{align*}
\mathrlap{
    |\ball Tvr| \,\ge\, (1-c) \cdot g(r/4) 
                \,\ge\, \tfrac12\, g(r/4),
} \hspace{16em}
\end{align*}
%
where $r/4$ in the argument of $g$ is rounded down to the largest integer.
 
\item If $\bar\Delta:=\smash{\displaystyle\sup_n}\lceil\Delta(n)\rceil +1<\infty$, then $T$ is of maximum degree $\bar\Delta$ and
%
\begin{align*}
\mathrlap{
    |\ball Tvr| \,\le\,  2\bar\Delta \cdot (1+c)^2 \cdot g(2r)^2 
                \,\le\, \tfrac92\bar\Delta\cdot g(2r)^2.
} \hspace{16em}
\end{align*}

\item
If $\Gamma:= \smash{\displaystyle\sup_{m\ge n}}  \lceil\Delta(m)/\Delta(n) \rceil < \infty$, then $\bar\Delta<\infty$ and
%
\begin{align*}
\mathrlap{
     |\ball Tvr| \,\le\, 2(1+c) \cdot \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
} \hspace{16em}
\\ 
\mathrlap{
 \phantom{|\ball Tvr| } 
 \,\le\, 3 \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
} \hspace{16em}
\\ 
\mathrlap{
 \phantom{|\ball Tvr| } 
 %\,\le\, 3\max\{1,\Gamma\} \cdot g(4r).
 \,\le\, 3\Gamma \cdot g(4r).
} \hspace{16em}
\end{align*}
\end{myenumerate}
   % 
In particular, if $\Gamma<\infty$ then $T$ is of uniform volume growth $g$.
\end{theorem}

% \begin{theorem}\label{thm:main}
% For each $v\in V(T)$ and $r\ge 0$ holds
% %

% \begin{align*}
% \mathrlap{
%     |\ball Tvr| \,\ge\, (1-c) \cdot g(r/4) 
%                 \,\ge\, \tfrac12\, g(r/4)
% } \hspace{16em}
% \end{align*}
% %
% where $r/4$ in the argument of $g$ is rounded down to the largest integer.
 
% If $\bar\Delta:=\smash{\displaystyle\sup_n}\lceil\Delta(n)\rceil +1<\infty$, then $T$ is of maximum degree $\bar\Delta$ and
% %
% \begin{align*}
% \mathrlap{
%     |\ball Tvr| \,\le\,  2\bar\Delta \cdot (1+c)^2 \cdot g(2r)^2 
%                 \,\le\, \tfrac92\bar\Delta\cdot g(2r)^2.
% } \hspace{16em}
% \end{align*}

% If $\Gamma:= \smash{\displaystyle\sup_{m\ge n}}  \lceil\Delta(m)/\Delta(n) \rceil < \infty$, then $\bar\Delta<\infty$ and
% %
% \begin{align*}
% \mathrlap{
%      |\ball Tvr| \,\le\, 2(1+c) \cdot \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
% } \hspace{16em}
% \\ 
% \mathrlap{
%  \phantom{|\ball Tvr| } 
%  \,\le\, 3 \big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big)
% } \hspace{16em}
% \\ 
% \mathrlap{
%  \phantom{|\ball Tvr| } 
%  \,\le\, 3\min\{1,\Gamma\} \cdot g(4r).
% } \hspace{16em}
% \end{align*}
%   % 
% In particular, if $\Gamma<\infty$ then $T$ is of uniform volume growth $g$.
% \end{theorem}

Note that the lower bound holds unconditionally. % (only subject to $\bar g$ being super-additive to ensure that $T$ exists, \cf\ \cref{rem:c}). %(only assuming $g$ is super-additive as discussed in \cref{rem:c}.
The conditions $\bar\Delta<\infty$~and~$\Gamma<\infty$ for the upper bounds are technical, but there are natural~criteria in terms of $g$ that imply both, such as being \emph{log-concave} (see \cref{res:conditions_in_g} below).

% \begin{theorem}\label{thm:main}
% Let $g\:\NN_0\to\RR$ be an increasing function and set $f(n):=g(2^n-1)$. 
% Let $\delta_1,\delta_2,\delta_3,...\in\NN$ be a sequence of integers with
% %
% $$ %\begin{equation}\label{eq:d_bounds}
% (1-c)\cdot f(n)  \;<\; (\delta_1+1)\cdots(\delta_n+1) \;<\; (1+c)\cdot f(n)
% $$ %\end{equation}
% for all $n\ge 0$, where $c:=\sup_n f(n)/f(n+1)\le 1$. 
% Set $T:=T(\delta_1,\delta_2,...)$ and
% %
% $$\Delta(n):=\frac{\delta_n}{\delta_1\cdots\delta_{n-1}}\;\;\text{where}\;\;\Delta(1):=\delta_1.$$
% %
% For each $v\in V(T)$ and $r\ge 0$ then holds
% \begin{myenumerate}
%     \item \quad
%     \vspace{-1\baselineskip}
%     $$|\ball Tvr| \,\ge\, (1-c) \cdot g(r/4).$$
%     \item 
%     if $\bar\Delta:=\smash{\displaystyle\sup_n}\lceil\Delta(n)\rceil +1<\infty$ then $T$ is of maximum degree $\bar\Delta$ and
%     %
%     $$|\ball Tvr| \,\le\,  2\bar\Delta \cdot (1+c)^2 \cdot g(2r + 1)^2.$$
%     \item 
%     if $\Gamma:= \smash{\displaystyle\sup_{m\ge n}}  \lceil\Delta(m)/\Delta(n) \rceil < \infty$ \nf(which implies $\bar\Delta<\infty$\nf) then
%     %
%     $$|\ball Tvr| \,\le\,  (\Gamma+1)\cdot (1+c) \cdot g(2r + 1).$$
% \end{myenumerate}
% %
% In particular, if $c<1$ and \itm3 applies, then $T$ is of uniform volume growth $g$.
% \end{theorem}

% The preconditions of \itm2 and \itm3 in \cref{thm:main} are technical in nature but are usually easy to check and are also satisfied for most naturally defined functions in the feasible growth range. %; and it~is usually easy to check this for any particular function.
% In \cref{res:conditions_in_d} we give some very accessible criteria in terms of the sequence of $\delta_n$.
% Investing more effort, one can show that it suffices to have $g$ being log-concave (as we show in \cref{res:conditions_in_g}).
% %A concrete criterion is given in \cref{res:conditions_in_g}, where it is shown that any log-concave function $g$ is natural in this sense.

% We remark that for most naturally defined functions $g$ of an appropriate growth holds $c<1$ as well as that the conditions of \itm2 and \itm3 are satisfied, and thus that $T$ is of uniform volume growth $g$. See \cref{res:...} for a more precise statement about which functions satisfy these conditions.
% Roughly, if $g$ is sub-exponential, then \itm2 applies; if $g$ is even log-concave, then also \itm3 applies.

\begin{proof}[Proof of \cref{thm:main}]
%Fix $v\in V(T)$ and $r\ge 4$.
For a vertex $w\in V(T)$ we use the notation $\tau_n(w)$ to denote the unique copy $\prec_n T$ that contains $w$.
%
%Moreover, let us agree that whenever we write $T_n\subset T$, we refer to the canonical sub-graph $T_n$ in $T$ from the defining inclusion chain $T_0\subset T_1\subset T_2\subset\cdots$ in \cref{constr:tree}.

To prove \itm1 choose $n\in\NN_0$ with $2^{n+1}\le r\le 2^{n+2}$. 
%Let $x$ be the root of $T_n(v)$. 
Each vertex of $\tau_n(v)$ can be reached from $v$ in at most $2(2^n-1)$ steps: 
at most $2^n-1$ steps from $v$ to the~center of $\tau_n(v)$, and at most $2^n-1$ steps from the center to any other vertex of $\tau_n(v)$.\nlspace 
This yields
%
\begin{align*}
|\ball Tvr|
%|B_v^T\!(r)|
\ge |\ball Tv{2^{n+1}}|
%|B_v^T\!(2^{n+1})|
> |\ball Tv{2(2^n-1)}|
%|B_v^T\!(2(2^n-1))|
\ge |T_n| 
&
\ge (1-c)\cdot g(2^n) 
\\ &
\ge (1-c)\cdot g(r/4).
\end{align*}
%
Here and in the following the final form of the bound is obtained by using $c\le 1/2$.

% For \itm2 observe first that $T_{n-1}$ has $\delta_1\cdots\delta_{n-1}$ apocentric vertices, each of which is a leaf. 
% Hence, when forming $T_n$ by attaching $\delta_n$ new copies of $T_{n-1}$ to these,\nlspace and assuming a maximally uniform distribution of the attachment among them, we find that none of the formerly apocentric vertices will attain a degree above $\lceil\Delta(n)\rceil+1$ (but some will in fact attain this degree).
% Thus, if $\lceil\Delta(n)\rceil+1$ is bounded, then this gives the maximum degree of $T$.

To prove \itm2 choose $n\in\NN$ with $2^{n-1}\le r\le 2^n$.
Let $x$ be the center of $\tau_n(v)$, and, if it exists,
%(if $x$ is not the global root)
let $w$ be the unique neighbor of $x$ outside of $\tau_n(v)$.
%the parent of $x$ (\ie\ the unique neighbor of $x$ that lies closer to the global root).
%be the apocentric vertex of the central copy of $T_n$ in $T_{n+1}(v)$ to which $x$ is adjacent.
Which other copies $\prec_n T$ are reachable from $v$ within $2^n$ steps? The following list is exhaustive:
%The following list contains all copies $\tau\prec_n T$ that might be reached from $v$ in at most $2^n$ steps (some of them might actually not be reachable, but we are not missing any):
%
\begin{itemize}
    \item $\tau_n(v)$ and $\tau_n(w)$, % itself,
    \item a copy $\tau \prec_n T$ adjacent to an apocentric vertex of $\tau_n(v)$ \resp\ $\tau_n(w)$.
    %There are less than $|T_n|$ apocentric vertices and each one is attached to at most $\bar\Delta-1$ further copies of $T_n$.
    %\item $\tau_n(w)$,
    %\item a copy $\tau\prec_n T$ adjacent to an apocentric vertex of $\tau_n(w)$.
\end{itemize}
%
Both $\tau_n(v)$ and $\tau_n(w)$ have not more than $|T_n|$ apocentric vertices, each of which~is adjacent to at most $\smash{\bar\Delta-1}$ copies $\tau\prec_n T$.
In conclusion, 
%Thus, including $\tau_n(v)$ and~$\tau_n(w)$, we count that 
at most $2\bar\Delta\cdot|T_n|$ copies of $T_n$ are reachable from $v$ in $2^n$ steps, containing a total of at most $2\bar\Delta\cdot |T_n|^2$ vertices.
We therefore find
%
% To prove the upper bound, choose $n\in\NN$ so that $2^{n-1} - 1\le r\le 2^n - 1$ and enumerate the copies of $T_n$ that can be reached from $v$ in at most $2^n-1$ steps.
% Note that the only way \enquote{out of $T_n(v)$} is either through one of its apocentric vertices, or through its root $x\in T_n(v)$:
% %
% \begin{itemize}
%     \item 
%     through an apocentric vertex: having reached an apocentric vertex of $T_n(v)$, up to $\bar\Delta-1$ roots of other copies of $T_n$ can be reached. From these, no~further copies can be reached, as the remaining $<2^n-1$ steps are insufficient to reach an apocentric vertex in the same copy. How many apocentric vertices of $T_n(v)$ can be reached from $v$ in $\le 2^n-1$ steps? This is hard to say; but at most $|T_n|$ many.
%     \item 
%     through the root $x$: having reached $x$ (and assuming that $x$~is not the global root), we can step into some \enquote{earlier} copy of $T_n$ via one of its apocentric vertices, say $w$. Starting in $w$ we can reach other apocentric vertices of $T_n(w)$, certainly less than $|T_n|$ many. As before, from each apocentric vertex of $T_n(w)$ we can reach up to $\Delta-1$ central vertices of other copies of $T_n$, from which no further copies can be reached. Like-wise, in the remaining $<2^n-1$ steps we cannot reach from $w$ to the central vertex of $T_n(w)$, and so we enumerated all reachable copies of $T_n$.
% \end{itemize}
% %
% To summarize, we can reach at most $2\bar\Delta\cdot|T_n|$ copies of $T_n$ (that is, $T_n(v)$, $T_n(w)$, and from each at most $(\bar\Delta-1)|T_n|$ other copies via apocentric vertices). In each of those we can reach at most $|T_n|$ vertices. This yields
%
\begin{align*}
%|B_v^T\!(r)| 
|\ball Tvr|
\le |\ball Tv{2^n}|
%|B_v^T\!(2^n)| 
\le 2\bar\Delta\cdot|T_n|^2 
&\le 2\bar\Delta\cdot(1+c)^2\cdot g(2^n)^2 
\\&\le 2\bar\Delta \cdot (1+c)^2 \cdot g(2r)^2.    
\end{align*}

One might suggest a much better estimation for the number of copies $\tau\prec_n T$ reachable through apocentric vertices of $\tau_n(v)$ \resp\ $\tau_n(w)$: namely $\delta_{n+1}$.
However, this is only true if $\tau_n(v)$ is a central copy in $\tau_{n+1}(v)$.
In general, $\tau_n(v)$ can as well be apocentric in $\tau_{n+1}(v)$, or can even be apocentric in $\tau_m(v)$ for some very large $m > n$.
If so, then the number of copies $\prec_n T$ reachable through apocentric vertices of $\tau_n(v)$ is more plausibly related to $\delta_{m+1}$ than $\delta_{n+1}$, which is the reason for the very crude estimation above. %We make this precise below.
With a more~careful analysis we can prove the second upper bound.

To show \itm3 let $m \ge n$ be maximal so that $\tau_n(v)$ is apocentric in $\tau_m(v)$.
Such an $m$ might not exist (\eg\ when $T$ is an apocentric limit), in which case the apocentric vertices of $\tau_n(v)$ are leaves in $T$ and no other copies $\prec_n T$ are reachable through them.
If $m$ exists however, then $\tau_m(v)$~is necessarily central in $\tau_{m+1}(v)$. 
In particular, the $\delta_1\cdots \delta_m$ apocentric vertices of $\tau_m(v)$ are adja\-cent to $\delta_{m+1}$ apocentric copies $\prec_{m} \tau_{m+1}(v)$.
By the maximally uniformly distribution of adjacencies we can estimate how many of these copies are reachable through the $\delta_1\cdots\delta_n$ apocentric vertices of $\tau_n(v)$.
Following \cref{rem:max_uniform} this number is at most
%
%
%is apocentric in $T_m(v)$ 
% Note~that such an $m$ exists and satisfies $m\ge n$. 
% Note further that $\tau_m(v)$ is then a central copy in $\tau_{m+1}(v)$: otherwise $\tau_n(v)$ and $\tau_{m+1}(v)$ share apocentric vertices, contradicting the choice of $m$.
% The $\delta_1\cdots \delta_m$ apocentric vertices of $\tau_m(v)$ are therefore adjacent to $\delta_{m+1}$ apocentric copies $\tau \prec_{m} \tau_{m+1}(v)$.
% Recall that these adjacencies are distributed maximally uniformly, so that we can estimate how many of them involve the $\delta_1\cdots\delta_n$ apocentric vertices of $\tau_n(v)\prec_n\tau_m(v)$.
% Following \cref{rem:max_uniform} this number is at most
%
%
%
% The careful reader may have realized that there is a much tighter (and somewhat obvious) estimation for the number of copies of $T_n$ attached to apocentric vertices of $T_n(a)$, namely, $\delta_{n+1}$.
% Unfortunately, this estimation does not necessarily apply to the number of copies of $T_n$ attached to $T_n(v)$.
%
%Recall now that $T_m(v)$ has $\delta_1\cdots\delta_m$ apocentric vertices and $T_n(v)$ has  $\delta_1\cdots\delta_n$ apocentric vertices. 
%Recall also that the adjacencies between the $\delta_1\cdots\delta_m$ apocentric vertices of $T_m(v)$ and the $\delta_{m+1}$ apocentric copies of $T_m$ in $T_{m+1}(v)$ distributed maximally uniformly among the apocentric vertices.
%There are then no more than 
%\msays{Why does such an $m$ exist?} \gsays{$m$ obviously exists, since everything is only a finite distance from $x^*$...} \msays{There are copies of $T_n$ that are not apocentric in any $T_m$.} \gsays{Oh, you don't mean that the set of m's may be unbounded, you mean that it may be empty. Yeah, that's fair. But doesn't the same upper bound apply then as well? In which case, we can simply distinguish cases.} \msays{I think I fixed it; we don't want a maximally large $T_m\subset T$ but a maximally large $T_m(v)$, such one always exists so that $T_n(v)$ is apocentric in it ($m=n$ works), and $m$ is, as you say, obviously bounded.}
%
\begin{align*}
\Big\lceil \frac{\delta_1\cdots\delta_n}{\delta_1\cdots\delta_m} \cdot \delta_{m+1}  \Big\rceil
&=
\Big\lceil \frac{\delta_{m+1}}{\delta_1\cdots\delta_m} \cdot \Big( \frac{\delta_{n+1}}{\delta_1\cdots\delta_n}\Big)^{-1} \cdot \delta_{n+1} \Big\rceil
\\&=\Big\lceil\frac{\Delta(m+1)}{\Delta(n+1)}\cdot\delta_{n+1}\Big\rceil
\le  \Gamma \cdot\delta_{n+1}.
\end{align*}
%
%copies of $T_n$ (inside of copies of $T_m$) adjacent to the apocentric vertices of $T_n(v)$.
This yields an improved upper bound on the number of copies $\tau\prec_n T$ adjacent to apo\-centric vertices of $\tau_n(v)$.
The same argument applies to $\tau_n(w)$.
Including $\tau_n(v)$ and $\tau_n(w)$ there are then at most $2\Gamma \cdot\delta_{n+1} + 2$ copies $\prec_n T$ reachable from $v$ in $2^n$ steps, and thus:
%
\begin{align*}
|\ball Tvr|
%|B_v^T\!(r)| 
\le |\ball Tv{2^n}|
%|B_v^T\!(2^n)| 
&\le (2\Gamma\cdot\delta_{n+1}+2)|T_n|
%\\ &\le 2\Gamma\cdot\delta_{n+1}\cdot|T_n| + 2|T_n|
\\ &\le 2\big(\Gamma\cdot (\delta_{n+1}+1)|T_n| - (\Gamma-1)\cdot|T_n|\big)
\\ &\le 2\big(\Gamma\cdot |T_{n+1}| - (\Gamma-1)\cdot|T_n|\big)
\\ &\le 2(c+1)\cdot\big(\Gamma\cdot g(2^{n+1}) - (\Gamma-1)\cdot g(2^n)\big).
\\ &\le 2(c+1)\cdot\big(\Gamma\cdot g(4r) - (\Gamma-1)\cdot g(2r)\big).
\end{align*}
%
%This establishes the improved upper bound.
\end{proof}

%One might wonder for which $g$ the technical condition $\Gamma<\infty$ in \cref{thm:main}~is satisfied.
%For the remainder of this section we make an effort to derive various~sufficient conditions.

It appears non-trivial to actually provide a target growth rate $g$ for which $\Gamma$~diverges, and so it seems we can feel confident that \cref{thm:main} applies quite generally.
Yet, for the remainder of this section we discuss criteria that are sufficient to imply  $\Gamma<\infty$.

\begin{proposition}\label{res:conditions_in_d}
$\Gamma<\infty$ holds in any of the following cases:
%
\begin{myenumerate}
    \item
    $\delta_{n+1}\le \delta_n^2$ eventually.
    % \item
    % $\delta_{n+1}\ge \delta_n^2$ and $\delta_{n+1}\le C\delta_n^2$ for some $C>1$ eventually.
    \item 
    the sequence of $\delta_n$ is bounded.
\end{myenumerate}
%
\begin{proof}
Note that $\Delta(n+1)=\delta_{n+1}/\delta_n^2 \cdot\Delta(n)$.
Assuming \itm1, $\Delta(n)$ will eventually~be non-increasing and so either $\Gamma\le1$ or the value $\Gamma$ is attained only on a finite initial segment, thus, is finite.

For part \itm2 observe $\Delta(m)/\Delta(n)=\delta_m / (\delta_n^2\cdot\delta_{n+1}\cdots\delta_{m-1})\le \displaystyle\smash{\max_i \delta_i}$.
\end{proof}
\end{proposition}

Condition \itm2 of \cref{res:conditions_in_d} holds, for example, when $g$ is a polynomial as discussed in \cref{ex:polynomial}.
%Note that this is not quite the same as being of polynomial growth $g(r)\in\theta(r^\alpha)$, which is not sufficient.

% Part \itm1 of \cref{res:conditions_in_d} holds for all $g$ that are not growing to fast.
% Part \itm2 includes in particular all $g$ of polynomial growth (\cf\ \cref{ex:lattice_tight_upper_bound}.

% One natural condition that \emph{almost} makes the preconditions of \itm2 and \itm3~satisfied is requiring $g$ to be \emph{log-concave}.
% The relevant instance of this is
% %
% $$
% \tfrac13 \log g(2r) + \tfrac23 \log g(r/2) \le \log 
% g(r)
% %g\big(\overbrace{\tfrac13 (2r) + \tfrac23 (r/2)}^{=\, r}\big).
% $$
% %
% (note that indeed $\frac13(2r)+\frac23(r/2)=r$).
% Unfortunately, this is not quite sufficient, and we instead need an $\eps>1$ for which the following stronger equation holds
% %
% $$
% \tfrac13 \log g(2r) + \tfrac23 \log g(r/2) \le \eps \log 
% g(r),
% $$
% %
% at least eventually.

% \begin{proposition}
% If for some $\eps>1$ holds
% %
% $$
% \tfrac13 \log g(2r) + \tfrac23 \log g(r/2) \le \eps \log 
% $$
% %
% eventually (\ie\ for all sufficiently large $r\ge1$), then the conditions of \itm2 and \itm3 in \cref{thm:main} are satisfied.
% %
% \begin{proof}
% \TODO
% \end{proof}
% \end{proposition}

% In general, $g$ being log-concave is already a pretty good indicator that the bounds of \cref{thm:main} apply. Constructing counterexamples in a reasonable growth range is possible but needs some work.

% \begin{example}
% \TODO
% \end{example}

It remains to provide a criterion for $\Gamma<\infty$ in terms of $g$.
Below we show that~$g$ being \emph{log-concave} is sufficient, where log-concave means
%
$$\alpha\log g(x) + \beta \log g(y) \le \log g(\alpha x + \beta y)$$
%
for all $\alpha,\beta\in[0,1]$ with $\alpha+\beta=1$.
Intuitively, being log-concave works because~it prevents both super-exponential growth and strong oscillations in the growth rate. 

\begin{theorem}\label{res:conditions_in_g}
If $g$ is log-concave, then $\Gamma<\infty$.
%
\begin{proof}
%The presented proof consists of a rather intuitive, and a more technical~part.
We start from a well-chosen instance of log-concavity:
%
$$\alpha=1/3,\quad \beta=2/3, \quad x=2^{n+1},\quad y=2^{n-1}.$$
%
One can verify $\alpha x+\beta y = 2^n$.
Since $g$ is log-concave, we have
%
$$\tfrac13\log g(2^{n+1}) + \tfrac23 \log g(2^{n-1}) \le \log g(2^n).$$
%
This further rearranges to
%
$$\log g(2^{n+1}) + 2\log g(2^{n-1}) \le 3\log g(2^n) \;\implies\; \frac{g(2^{n+1})}{g(2^n)} \le \Big(\frac{g(2^n)}{g(2^{n-1})}\Big)^2\!.$$
%
Recall that roughly $\delta_n\approx g(2^n)/g(2^{n-1})$, and so the right-most inequality resembles $\delta_{n+1}\le \delta_n^2$.
If this were exact then $\Gamma<\infty$ would already follow from \cref{res:conditions_in_d} \itm1.
%
However, the actual definition of $\delta_n$ from the proof of \cref{res:d_i} only yields
%The reality however is less nice: from the actual definition of the $\delta_n$
%\cref{res:d_i}
%follows %, and using the actual definition of $\delta_n$ from \cref{res:d_i} yields:
%
\begin{equation}\label{eq:d_d_2}
\delta_{n+1}
\le \Big\lfloor\frac{g(2^{n+1})}{g(2^n)}\Big\rfloor
\le \frac{g(2^{n+1})}{g(2^n)}
\le \Big(\frac{g(2^n)}{g(2^{n-1})}\Big)^2
\le \Big\lceil\frac{g(2^n)}{g(2^{n-1})}\Big\rceil^2
\le (\delta_n+2)^2.
\end{equation}
%
% which we can rearrange to
% %
% \begin{equation}\label{eq:nu}
% \nu(n)
% :=\frac{\delta_{n+1}}{\delta_n^2}
% \le \Big(1+\frac2{\delta_n}\Big)^2
% %\le 1+\frac4{\delta_n}+\frac4{\delta_n^2}
% . %\le 1 + \frac{2}{\delta_n-2}.
% \end{equation}
% %
% Recall that $\Delta(n+1)=\nu(n)\Delta(n)$.
% By \eqref{eq:nu} it is possible that $\Delta$ is increasing and so we can not put a bound on $\Delta(m)/\Delta(n)$ right away.

This turns out to be sufficient for proving $\Gamma<\infty$, though the argument becomes more technical.
Define $\gamma\:\NN\to\RR$ with
%
$$
\gamma(1):=25,\qquad \gamma(\delta):=\prod_{k=0}^{\infty} %\Big(1+\frac4{\delta^{2^k}}+\frac4{\delta^{2^{k+1}}}\Big)
\Big(1+\frac2{\delta^{2^k}}\Big)^{\!2}\!
,\;\;\,\text{whenever $\delta\ge 2$.}
$$
%
To keep this proof focused, most technicalities surrounding this function have been moved to \cref{sec:gamma_properties}.
This includes a proof of convergence of the infinite product (\cref{res:estimate_gamma}) as well as a proof of the following crucial property $(*)$ of $\gamma$: for~any two integers $\delta_1,\delta_2\ge 1$ with $\delta_1\le(\delta_2+2)^2$ holds $\delta_1\gamma(\delta_1)\le\delta_2^2\gamma(\delta_2)$ (\cref{res:gamma_property_d_d2}).

Lastly, we define $\pot(n):=\gamma(\delta_n)\Delta(n)$, intended to represent the \emph{potential} for $\Delta$ to increase, as we shall see that it is an upper bound on $\Delta(m)$ for \emph{all} $m\ge n$.
This follows from two observations.
First, $\Delta(m)< \pot(m)$ since $\gamma(\delta)>1$. Second, $\pot(n)$ is decreasing in $n$: since $\delta_{n+1}\le(\delta_n+2)^2$ by \eqref{eq:d_d_2}, we can apply property $(*)$ to find
%
$$\pot(n+1) = \gamma(\delta_{n+1})\Delta(n+1) = \gamma(\delta_{n+1})\frac{\delta_{n+1}}{\delta_n^2}\Delta(n) \overset{\smash{(*)}}\le \gamma(\delta_n)\Delta(n)=\pot(n).$$
%
To summarize, for all $m\ge n$ holds
%
\begin{equation*}\label{eq:goal}
\Delta(m)<\pot(m)
%\overset{\mathclap{(*)}}
\le\pot(n)=\Delta(n)\gamma(\delta_n) \,\implies\, \frac{\Delta(m)}{\Delta(n)}\le\gamma(\delta_n)\le 25,
\end{equation*}
%
where we used that $\gamma(\delta)$ is decreasing in $\delta$ (\cref{res:gamma_decreasing}) and so attains its maximum at $\gamma(1)=25$. This proves $\Gamma\le25$.
\end{proof}
\end{theorem}

As a corollary of \cref{thm:main} and \cref{res:conditions_in_g} we have proven

\begin{theoremX}{\ref{main}}
   If $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ is (eventually) super-additive and log-concave, then there exists a tree $T$ of uniform growth $g$. 
\end{theoremX}



\iftrue % remark for non-central inclusion chains

%\begin{remark}\label{rem:general_limit_growth}
%Let $T'$ be the limit tree obtained from a different inclusion chain compared to \cref{constr:T} (\eg\ always identifying $T_{n-1}$ with an apocentric copy in $T_n$). 
%For each $v\in V(T')$ and $r\ge 0$ the ball~$\ball {T'}vr$ appears as a subgraph of $T$. Additionally, $\ball {T'}vr$ contains a subtree isomorphic to a ball of radius $r/2$ in $T$. \msays{how so?}
%Therefore, using the growth estimations for $T$ proven in \cref{thm:main}, we see that $T'$ has uniform volume growth $g$ as well. In particular, for any arbitrary tree $T'$ obtained from our construction with appropriate identifications, we have
%\[\tfrac12 g(r/8)\leq \ball {T'}vr\leq 3\max\{1,\Gamma\}\cdot g(4r).\]
%\[\tfrac12 g(r/8)\leq \ball {T'}vr\leq 3\Gamma\cdot g(4r).\]

%Finally, note that every ball of radius $\leq 2^n-1$ in $T_n$ is isomorphic to a ball of such a limit tree $T'$, and therefore admits the same bounds. This observation will be of use in the next section.
%\msays{Not entirely true, \eg\ if $T'$ is completely apocentric and $v$ is completely apocentric the ball cannot necessarily be found in $T$.} \gsays{Of course it can, it just won't be a ball.}
%\end{remark}

% \sepline

% This infinite product converges, and the function $\gamma$ has the following essential properties (see \cref{sec:gamma_properties} for proofs of these facts):
% %
% \begin{myenumerate}
%     \item $\gamma(\delta)$ is decreasing in $\delta$, \ie\ if $\delta_1 < \delta_2$ then $\gamma(\delta_1) > \gamma(\delta_2)$. This is clear from the definition if $\delta_1,\delta_2\ge 2$, but it requires estimating $\gamma(2)$ when $\delta_1=1$ (see \cref{res:gamma_bounds}).
%     \item if $\delta_1\le \delta_2$ then $\delta_1\gamma(\delta_1)\le\delta_2^2\gamma(\delta_2)$ (see \cref{res:gamma_property_d_d2}).
% \end{myenumerate}

% The second function is the \emph{potential} $\pot(n):=\gamma(\delta_n)\Delta(n)$.
% Intuitively, it measures how much $\Delta$ can still increase for $m\ge n$, or formally, it is an upper bound on $\Delta(m)$ for any $m\ge n$; a fact that we are going to prove.
% This suffices to prove $\Gamma<\infty$:
% %
% \begin{equation}\label{eq:goal}
% \Delta(m)<\pot(m)
% %\overset{\mathclap{(*)}}
% \le\pot(n)=\Delta(n)\gamma(\delta_n) \,\implies\, \frac{\Delta(m)}{\Delta(n)}\le\gamma(\delta_n)\le 25,
% \end{equation}
% %
% hence $\Gamma\le 25$.
% In the remaining proof we show that $\pot(n)$ is non-increasing.

% Fix a pair $m > n$ for which we aim to show $\Delta(m)/\Delta(n)\le 25$ (the case $m=n$ being trivial). 
% We can assume that $n$ is a local minimum, \ie\ $\Delta(n) < \Delta(n+1)$, and that $m$ is a local maximum, \ie\ $\Delta(m) > \Delta(m-1)$; as otherwise we can move $n$ and $m$ closer together, making the quotient $\Delta(m)/\Delta(n)$ at most bigger.
% %W.l.o.g.\ assume $\Delta(n)<\Delta(n+1)$ and $\Delta(m)>\Delta(m-1)$, as otherwise the pair $m-1\ge n$ or $m\ge n+1$ yields an even bigger quotient.

% Let then $[n_1,m_1],...,[n_s,m_s]\subset[n,m]$ be an enumeration of maximal intervals on which $\Delta$ is strictly increasing, where the indexing is chosen to satisfy $n=n_1<m_1<n_2<m_2<\cdots<n_s<m_s=m$ (see \cref{fig:Delta_n}). 
% %In particular, $\Delta(n_i)<\Delta(n_i+1)$ for all $i\in\{1,...,s\}$. 
% %\msays{Why do we emphasize this?} \gsays{So that the reader understands where the decreasing interval ends and the increasing interval begins when we have many consecutive numbers with the same $\Delta$}
% %
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.65\textwidth]{img/Delta_n_2.pdf}
%     \caption{Visualization of $\Delta(n)$ and the parition of $[n,m]$ into increasing and non-increasing intervals.}
%     \label{fig:Delta_n}
% \end{figure}

% Our plan is to show $\pot(m)\le \pot(n)$ and to invoke the reasoning of \eqref{eq:goal}.
% More precisely, we show $\pot(n_1)\ge \pot(n_2)\ge \cdots\ge\pot(n_s)\ge\pot(m_s)$.
% This is achieved in two separate steps: showing $\pot(n_i)\ge\pot(n_{i+1})$ and $\pot(n_i)\ge \pot(m_i)$.

% \emph{Step 1}: we show $\pot(n_i)\ge \pot(m_i)$.
% By the definition of the intervals, for any $k\in[n_i,m_i-1]$ holds $\Delta(k)<\Delta(k+1)=\nu(k)\Delta(k)\implies\nu(k)>1\implies\delta_{k+1}>\delta_k^2\implies\gamma(\delta_{k+1})<\gamma(\delta_k^2)$, and therefore
% %
% \begin{align*}
% \pot(k+1)
% &=\Delta(k+1) \gamma(\delta_{k+1})
% <\Delta(k+1) \gamma(\delta_k^2)
% =\Delta(k) \nu(k)\cdot \gamma(\delta_k^2)
% \\&\le \Delta(k) \cdot \Big(1+\frac2{\delta_k}\Big)^2  \cdot  \prod_{k = 0}^\infty \Big(1+\frac2{(\delta_k^2)^{2^k}}\Big)^2  
% = \Delta(k) \cdot \prod_{k = 0}^\infty \Big(1+\frac2{\delta_k^{2^k}}\Big)^2  
% \\&= \Delta(k) \gamma(\delta_k) = \pot(k).
% \end{align*}
% %
% We conclude that $\pot(\free)$ is increasing on $[n_i,m_i]$, from which the claim of step 1 follows.
% Note also $\Delta(m_i)\le \pot(m_i)\le\pot(n_i)$.

% Next we show that $\pot(\free)$ is non-increasing on the intervals $[m_i,n_{i+1}]$. 
% As before, we pick a $k\in[m_i,n_{i+1}-1]$ and show $\pot(k+1)\le\pot(k)$. 
% Note that $\Delta(k+1)\le\Delta(k)$. 
% If $\delta_{k+1}\ge\delta_k$ then immediately follows
% %
% \begin{align*}
% \pot(k+1) 
% &= \Delta(k+1)\gamma(\delta_{k+1})
% \le \Delta(k)\gamma(\delta_k)
% =\pot(k).
% \end{align*}
% %
% If however $\delta_{k+1}<\delta_k$, then we proceed via
% %
% $$\pot(k+1)=\Delta(k+1)\gamma(\delta_{k+1}) = \nu(k)\Delta(k)\gamma(\delta_{k+1}) \overset{\smash{(*)}}\le \Delta(k)\gamma(\delta_k)=\pot(k),$$
% %
% where in $(*)$ we used $\delta_{k+1}\gamma(\delta_{k+1})\le\delta_k^2\gamma(\delta_k)$ (property \itm3 of $\gamma$, \cf\ \cref{res:estimate_gamma}).





% If however $\delta_{k+1}<\delta_k$, then we have to distinguish several cases:
% %
% \begin{enumerate}[label=(\arabic*),topsep=1em,itemsep=1em]
%     \item if $\delta_k\ge5$, then we show
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1})
%     = \nu(k) \Delta(k) \gamma(\delta_{k+1}) \overset{\smash{(*)}}\le \Delta(k)\le\pot(k).
%     \end{align*}
%     %
%     where in $(*)$ we use $\nu(k)\gamma(\delta_{k+1})\le \gamma(\delta_k)$.
    
%     \item if $\delta_{k+1}<\delta_k\le 4$, we are left with the finitely many cases
%     %
%     $$(\delta_{k+1},\delta_k)\in\{\;(2,1),(3,1),(3,2),(4,1),(4,2),(4,3) \;\}$$
%     %
%     and one can verify (see \cref{res:estimate_gamma} for the approximate value of $\gamma(\delta)$ for small $\delta$) that $\nu(k)\gamma(\delta_{k+1})\le\gamma(\delta_k)$ for all of them.
%     It follows
%     %
%     $$\pot(k+1)=\gamma(\delta_{k+1})\Delta(k+1) = \gamma(\delta_{k+1})\nu(k)\Delta(k) \le \gamma(\delta_k)\Delta(k)=\pot(k).$$
% \end{enumerate}
% \hrulefill
% %
% \begin{enumerate}[label=(\arabic*),topsep=1em,itemsep=1em]
%     \item 
%     if $\delta_{k}\geq 5$ and $\delta_{k+1}\geq 3$, then \mbox{$\Delta(k+1)/\Delta(k)\le \delta_{k+1}/\delta_{k}^2< \frac{1}{5}$} and it follows 
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1}) <  \tfrac15 \Delta(k)\gamma(\delta_{k+1}) 
%     %\\&
%     \overset{\smash{(*)}}< \Delta(k)\le\pot(k),
%     \end{align*}
%     %
%     where in $(*)$ we used $\gamma(\delta_{k+1})\le\gamma(3)<4$.
    
%     \item if $\delta_{k}\geq 5$ and $\delta_{k+1}=2$, then \mbox{$\Delta(k+1)/\Delta(k)\le\delta_{k+1}/\delta_{k}^2 \le \frac{2}{25}$} and it follows
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1}) \le  \tfrac2{25} \Delta(k)\gamma(2) 
%     %\\& 
%     \overset{\smash{(**)}}< \Delta(k)\le\pot(k),
%     \end{align*}
%     %
%     where in $(**)$ we used $\gamma(2)<12.5$.
    
%     \item if $\delta_{k}\geq 5$ and $\delta_{k+1}=1$, then analogously \mbox{$\Delta(k+1)/\Delta(k) \le \frac{1}{25}$} and 
%     %
%     \begin{align*}
%     \pot(k+1) &= \Delta(k+1)\gamma(\delta_{k+1}) \le  \tfrac1{25} \Delta(k)\gamma(1) 
%     %\\& 
%     \overset{\smash{(***)}}= \Delta(k)\le\pot(k),
%     \end{align*}
%     %
%     where in $(*\!*\!*)$ we used $\gamma(1)=25$.
    
%   % \TODO
    
%     \item it remains $\delta_{m_i}\le 4$. 
%     Recall $\delta_k^2 < \delta_{k+1}$ for all $k\in[n_i,m_i-1]$.
%     \mbox{In particular}, $\delta_{m_i-1}^2<\delta_{m_i}\le 4$ and therefore $\delta_{m_i-1}=1$.
%     It furthermore follows~$(\x)\;\nu(m_i-1)$ $=$ $\delta_{m_i}/\delta_{m_i-1}^2 = \delta_{m_i}$.
%     Moreover, $n_i=m_i-1$, because if $n_i<m_i-1$ then $1\le \delta_{n_i}^2<\delta_{m_i-1}=1$.
%     Taken together we obtain
%     %
%     \begin{align*}
%     \Delta(n_{i+1}) 
%       &= \nu(m_i+1)\cdots\nu(n_{i+1}) \cdot \Delta(m_i)
%       =\frac{\delta_{n_i+1}}{\delta_{m_i}} \cdots \frac{1}{\delta_{m_i}\cdots\delta_{n_{i+1}-1}}\cdot \Delta(m_i)
%     \\&\le \frac{\Delta(m_i)}{\delta_{m_i}}
%       = \frac{\nu(m_i-1)\Delta(m_i-1)}{\delta_{m_i}} 
%       %= \frac{\Delta(n_i)}{\delta_{m_i-1}^2} 
%       \overset{(\x\x)}= \Delta(m_i-1) \overset{(\x)}=\Delta(n_i).
%     \end{align*}
%     %
%     %From this and $\delta_{n_i}=1\le\delta_{n_i+1}$ follows
%     From this and $\gamma(\delta_{n_{i+1}})\le \gamma(1) = \gamma(\delta_{n_i})$ follows
%     %
%     $$\pot(n_{i+1})=\gamma(\delta_{n_{i+1}}) \Delta(n_{i+1}) \le \gamma(\delta_{n_i})\Delta(n_i) \le \pot(n_i).$$
    
% \end{enumerate}
% %
% This concludes the proof.


% \hrulefill

% \emph{Step 2}: we show $\pot(n_{i+1})\le\pot(n_i)$ via case analysis.
% Note that~$\Delta$ is non-increasing on $[m_i,n_{i+1}]$, in particular, $\Delta(n_{i+1})\le \Delta(m_i)$.
% %
% \begin{enumerate}[label=(\arabic*)]
%     \item if $\delta_{m_i}\le\delta_{n_{i+1}}$ then
%     %
%     \begin{align*}
%     \pot(n_{i+1}) 
%     &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}})
%     < \Delta(m_i)\gamma(\delta_{m_i})
%     \\&=\pot(m_i)\le\pot(n_i).
%     \end{align*}
    
%     \item otherwise $\delta_{m_i}>\delta_{n_{i+1}}$and we distinguish the following sub-cases:
%     % In the following we repeatedly use
%     % %
%     % $$m\ge n \implies \frac{\Delta(m)}{\Delta(n)} = \frac{\delta_{m}/\delta_n}{\delta_n\cdots\delta_{m-1}}.$$
%     % %
%     % for various estimations of the quotient.
    
%     \vspace{1ex}
%     \begin{enumerate}[label=(\alph*)]
%         \item 
%         if $\delta_{m_i}\geq 5$ and $\delta_{n_{i+1}}\geq 3$, then \mbox{$\Delta(n_{i+1})/\Delta(m_i)\le \delta_{n_{i+1}}/\delta_{m_i}^2< \frac{1}{5}$} and 
%         %
%         \begin{align*}
%         \pot(n_{i+1}) &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}}) <  \tfrac15 \Delta(m_i)\gamma(\delta_{n_{i+1}}) \\
%         & \overset{\smash{\mathclap{(*)}}}< \Delta(m_i)\le\pot(n_i),
%         \end{align*}
%         %
%         where in $(*)$ we used $\gamma(\delta_{n_{i+1}})\le\gamma(3)<4$.
        
%         \item if $\delta_{m_i}\geq 5$ and $\delta_{n_{i+1}}=2$, then \mbox{$\Delta(n_{i+1})/\Delta(m_i)\le\delta_{n_{i+1}}/\delta_{m_i}^2 \le \frac{2}{25}$} and 
%         %
%         \begin{align*}
%         \pot(n_{i+1}) &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}}) \le  \tfrac2{25} \Delta(m_i)\gamma(2) \\
%         & \overset{\smash{\mathclap{(**)}}}< \Delta(m_i)\le\pot(n_i),
%         \end{align*}
%         %
%         where in $(**)$ we used $\gamma(2)<12.5$.
        
%         \item if $\delta_{m_i}\geq 5$ and $\delta_{n_{i+1}}=1$, then analogously \mbox{$\Delta(n_{i+1})/\Delta(m_i) \le \frac{1}{25}$} and 
%         %
%         \begin{align*}
%         \pot(n_{i+1}) &= \Delta(n_{i+1})\gamma(\delta_{n_{i+1}}) \le  \tfrac1{25} \Delta(m_i)\gamma(1) \\
%         & \overset{\smash{\mathclap{(***)}}}= \Delta(m_i)\le\pot(n_i),
%         \end{align*}
%         %
%         where in $(*\!*\!*)$ we used $\gamma(1)=25$.
        
%       % \TODO
        
%         \item it remains to discuss $\delta_{m_i}\le 4$. 
%         Recall from step 1 that $\delta_k^2 < \delta_{k+1}$ for all $k\in[n_i,m_i-1]$.
%         So we can conclude $\delta_{m_i-1}^2<\delta_{m_i}\le 4\implies \delta_{m_i-1}=1$.
%         Moreover, $n_i<m_i-1$ yields the contradiction $1\le \delta_{n_i}^2<\delta_{m_i-1}=1$, thus $n_i = m_i-1$.
%         Note that $\nu(m_i-1) = \delta_{m_i}/\delta_{m_i-1}^2 = \delta_{m_i}$. Then
%         %
%         \begin{align*}
%         \Delta(n_{i+1}) 
%           &= \nu(n_{i+1}-1)\cdots\nu(m_i) \cdot \Delta(m_i)
%         \\&=\frac{\delta_{n_i+1}}{\delta_{m_i}} \cdots \frac{1}{\delta_{m_i}\cdots\delta_{n_{i+1}-1}}\cdot \Delta(m_i)
%         \\&\le \frac{\Delta(m_i)}{\delta_{m_i}}
%           = \frac{\nu(m_i-1)\Delta(m_i-1)}{\delta_{m_i}} 
%           %= \frac{\Delta(n_i)}{\delta_{m_i-1}^2} 
%           = \Delta(n_i).
%         \end{align*}
%         %
%         and finally
%         %
%         $$\pot(n_{i+1})=\gamma(\delta_{n_{i+1}}) \Delta(n_{i+1}) \le \gamma(\delta_{n_i})\Delta(n_i) \le \pot(n_i).$$
        
%     \end{enumerate}
% \end{enumerate}
% %
% This finishes the proof.




% \sepline

% If $\delta_{n+1} \ge \delta_n^2$ then
% %
% $$\delta_{n+1}\gamma(\delta_{n+1}) \le \delta_{n+1}\gamma(\delta_n^2) = \frac{\delta_{n+1}}{\delta_n^2} \delta_n^2 \gamma(\delta_n^2) \le \Big(1+\frac2{\delta_n}\Big)^2 \delta_n^2 \gamma(\delta_n^2) = \delta_n^2 \gamma(\delta_n).$$

% If $\delta_n\le\delta_{n+1}\le\delta_n^2$ then
% %
% $$\delta_{n+1}\gamma(\delta_{n+1}) \le \delta_n^2 \gamma(\delta_n).$$

% If $\delta_{n+1}\le\delta_n$ then by \cref{res:gamma_property_d_d2}
% %
% $$\delta_{n+1}\gamma(\delta_{n+1})\le\delta_n^2\gamma(\delta_n).$$

% \begin{lemma}
% If $a\le (b+2)^2$, then $a\gamma(a)\le b^2\gamma(b)$.
% \end{lemma}

% $$\gamma(\delta_{n+1})\Delta(n+1) = \frac{\delta_{n+1}\gamma(\delta_{n+1})}{\delta_n^2}\Delta(n) \le \gamma(\delta_n)\Delta(n).$$





\iffalse

\newpage

\msays{I believe we have a working proof of \cref{res:conditions_in_g} now, but it is quite a bit different than anticipated. I was able to shorten the proof significantly by outsourcing the case analysis to a discussion of properties of $\gamma$ in the Appendix (I like to have it in an Appendix because these technicalities distract from our main message). The key insight was that the previous case analysis came down to repeatedly using one special property of $\gamma$. It is even a bit stronger now, as it proves that $\pot(\free)$ is always decreasing, not only on the $\Delta$-increasing segments}

\msays{For cleanup, I removed (that is, made into a comment) most of the previous proof attempts, but I left what you wrote in case we need to rewind. }

We aim to show that $\frac{\Delta(m)}{\Delta(n)}$, $m\geq n$ is bounded. It is sufficient to prove this if $\Delta$ assumes a local minimum in $n$ (we may also assume that $\Delta(n)<\Delta(n+1)$, without loss of generality). To achieve this, we will prove that $pot(n')<pot(n)$ for every $n'>n$ at which $\Delta$ assumes a local minimum, where $pot(i):=\Delta(i)\gamma(\delta_i)$ if $\delta_i\geq 2$ and $pot(i):=24.66\Delta(i)$ otherwise. From this the desired result immediately follows. Indeed, observe that $[n,m]$ is partitioned in $\Delta$-monotone intervals $[n_0:=n,m_0]$, $[m_0,n_1]$, $[n_1,m_1]$,...$[n_l,m_l:=m]$. Then $\Delta(m)\leq pot(n_l)\leq pot(n)<24.66\Delta(n)$.

The proof will be by induction over the number of maximal monotone intervals partitioning $[n,n']$. The inductive basis is trivial.

For the inductive step, let $[n_j,m_j]$, $[m_j,n']$ be the last two maximal $\Delta$-monotone intervals of $[n,n']$, the former increasing and the latter decreasing, and suppose that we know that $pot(n_j)\leq pot(n)$. We shall show that $pot(n')\leq pot(n)$. 

We distinguish cases:

\begin{enumerate}
    \item If $\delta_{m_j}\leq ...\leq \delta_{n'}$, then we have $\gamma(\delta_{n'})\leq \gamma(\delta_{m_j})\Rightarrow pot(n')<pot(m_j)\leq pot(n_j)\leq pot(n)$.
    \item If there exists some index $i$ in $[m_j+1,n']$ with $\delta_i<\delta_{i-1}$, then:
    \begin{enumerate}
        \item If $\delta_{m_j}\geq 5$ and $\delta_{n'}\geq 3$, we observe that $\frac{\Delta(n')}{\Delta(m_j)}\leq \frac{1}{5}$. Therefore, \[pot(n')\leq \frac{\Delta(m_j)}{5}\gamma(\delta_{n'})<\Delta(m_j)\leq pot(n_j)\leq pot(n).\]
        \item If $\delta_{m_j}\geq 5$ and $\delta_{n'}=2$, we observe that $\frac{\Delta(n')}{\Delta(m_j)}\leq \frac{2}{25}$. Therefore, \[pot(n')\leq \frac{2\Delta(m_j)}{25}\gamma(2)<\Delta(m_j)\leq pot(n_j)\leq pot(n).\] 
        \item If $\delta_{m_j}\geq 5$ and $\delta_{n'}=1$, we observe that $\frac{\Delta(n')}{\Delta(m_j)}\leq \frac{1}{25}$. Therefore, \[pot(n')<\Delta(m_j)\leq pot(n_j)\leq pot(n).\] 
        \item If $\delta_{m_j}<5$, then $\delta_{n_j}=1$ and 
        \begin{enumerate}
            \item either $n_j=m_j-1$ and $\delta_{m_j}\in\{2,3,4\}$, in which case $\Delta(m_j)=\delta_{m_j}\Delta(n_j)$ and $\Delta(n')\leq \frac{\Delta(m_j)}{\delta_{m_j}}=\Delta(n_j)$;
            \item or $n_j=m_j-2$, $\delta_{m_j-1}=2$ and $\delta_{m_j}=4$, in which case $\Delta(m_j)=2\Delta(n_j)$ and $\Delta(n')\leq \frac{\Delta(m_j)}{\delta_{m_j}}=\frac{\Delta(n_j)}{2}$.
        \end{enumerate}
        In either case $\Delta(n')\leq \Delta(n_j)$, so \[pot(n')\leq pot(n_j)\leq pot(n).\]
    \end{enumerate}
\end{enumerate}

The proof is complete.




\noindent\hrulefill

To put an upper bound on $\Delta(m)/\Delta(n)$ note that it suffices to consider $m,n\in\NN$ so that for all $k\in[n,m]$ holds $\Delta(n)<\Delta(k)<\Delta(m)$, as otherwise the quotient can be further increased.
For such $m$ and $n$ we are going to prove $\Delta(m)/\Delta(n)\le \gamma(\delta_n)$, where
%
$$
\gamma(\delta):=\prod_{k=0}^{\infty} %\Big(1+\frac4{\delta^{2^k}}+\frac4{\delta^{2^{k+1}}}\Big)
\Big(1+\frac2{\delta^{2^k}}\Big)^2
,\quad\text{if $\delta\ge 2$, \quad and $\gamma(1):=24$.}
$$
%
%and $\gamma(1) := 24$ otherwise.
This will be sufficient as the infinite product converges whenever $\delta\ge 2$ (see Appendix A), and in fact, $\gamma(\delta)\le 100$ for all $\delta$. Note also that~$\gamma$ is decreasing in its argument.

Proving this upper bound will proceed differently depending on whether we consider a decreasing or increasing segment of $\Delta$.
For that reason let $[n_1,m_1],...,[n_s,m_s]$ $\subseteq[n,m]$ be an enumeration of the maximal intervals on which $\Delta$ is non-decreasing.
Then $n=n_1<m_1<n_2<\cdots<n_s<m_s=m$.
We then are going to show that $\Delta(m_i)/\Delta(n)\ge\gamma(\delta_n)$ for all $i\in\{1,...,s\}$ by induction on $i$. 

In the next step we prove $\Delta(m_i)/\Delta(n_i)\ge\gamma(\delta_{n_i})$ which contains the induction base as the special case for $i=1$.
Since $\Delta$ is non-decreasing on $[n_i,m_i]$, we have $\delta_{n_i+k+1}\ge\delta_{n_i+k}^2$ for all $k\in\{0,...,m_i-n_i-1\}$, which expands to $\delta_{n_i+k}\ge \smash{\delta_{n_i}^{2^k}}$.
For $\delta_{n_i}\ge 2$ follows
%
\begin{align*}
\frac{\Delta(m_i)}{\Delta(n_i)}
\;&=\; \prod_{k=0}^{\mathclap{m_i-n_i-1}} \nu(n_i+k) 
\;\le\; \prod_{k=0}^{\mathclap{m_i-n_i-1}}\; \Big(1+\frac2{\delta_{n_i+k}}+\frac4{\delta_{n_i+k}^2}\Big)
\\\;&\le\; \prod_{k=0}^{\mathclap{m_i-n_i-1}}\; \Big(1+\frac2{\delta_{n_i}^{2^k}}+\frac4{\delta_{n_i}^{2^{k+1}}}\Big)
< \gamma(\delta_{n_i}).
\end{align*}
%
If $\delta_{n_i}=1$, by \eqref{eq:nu} holds $\delta_{n_i+1}\le 7$.

\fi

% $$
% \Delta(m_{i+1})\gamma(\delta_{m_{i+1}}) 
% \,\overset{\mathclap{(*)}}\le\, \Delta(n_{i+1})\gamma(\delta_{n_{i+1}})
% \,\overset{\mathclap{(**)}}\le\, \Delta(m_i)\gamma(\delta_{m_i})
% \,\overset{\mathclap{(***)}}\le\, \Delta(n)\gamma(\delta_{n})
% $$

% \newpage

% Define the \emph{potential} $\pot(k):=\Delta(k)\gamma(\delta_k)$ at index $k$.
% We are going to show
% %
% \begin{equation}
%     \tag{$*$} \pot(n_1)\ge\pot(m_1)\ge\pot(n_2)\ge\cdots\ge\pot(n_s)\ge\pot(m_s).
% \end{equation}
% %
% This would suffice to conclude the proof as $\Delta(m)\le \pot(m)\le\pot(n)=\Delta(n)\gamma(n)\le 36\Delta(n)$.
% The chain $(*)$ is composed of two types of inequalities: $\pot(n_i)\ge\pot(m_i)$ and $\pot(m_i)\ge\pot(n_{i+1})$.

% For the first inequality, recall that $\Delta$ is non-decreasing on $[n_i,m_i]$, and so $\delta_{k+1}\ge\delta_k^2$ for all $k\in[n_i,m_i-1]$. The first inequality then follows from
% %
% \begin{align*}
% \pot(k+1)
% &=\Delta(k+1) \cdot \gamma(\delta_{k+1})
% \le\Delta(k+1) \cdot \gamma(\delta_k^2)
% \\&=\Delta(k) \cdot \nu(k+1)\cdot \gamma(\delta_k^2)
% \\&\le \Delta(k) \cdot \Big(1+\frac4{\delta_k}+\frac4{\delta_k^2}\Big)  \cdot  \prod_{k = 0}^\infty \Big(1+\frac4{(\delta_k^2)^{2^{k}}}+\frac4{(\delta_k^2)^{2^{k+1}}}\Big) 
% \\&= \Delta(k) \cdot \prod_{k = 0}^\infty \Big(1+\frac4{\delta_k^{2^k}}+\frac4{\delta_k^{2^{k+1}}}\Big) 
% \\&= \Delta(k) \cdot \gamma(\delta_k) = \pot(k).
% \end{align*}

% For the second inequality we first show $\delta_{n_{i+1}}\ge \delta_{m_i}$. Otherwise there would be a $k\in[m_i,n_{i+1}-1]$ for which $\delta_{k+1}<\delta_k\implies \nu(k+1)<1/\delta_k$, and therefore
% %
% $$
% \Delta(k+1)
% =\nu(k+1)\Delta(k)
% <\frac1{\delta_k}\Delta(k)
% \le \frac1{\delta_k}\Delta(m_i)
% \le\frac{\gamma(\delta_{n_i})}{\delta_k}\Delta(n_i)
% \le\Delta(n_i).
% $$
% %
% This is a contradiction to the choice of the interval $[n,m]$.
% The second~inequality is now a simple consequence of combining $\Delta(m_i)>\Delta(n_{i+1})$ and $\delta_{n_{i+1}}\ge \delta_{m_i}$:
% %
% $$
% \pot(n_{i+1}) 
%   = \Delta(n_{i+1})\gamma(\delta_{n_{i+1}})
%   < \Delta(m_i) \gamma(\delta_{m_i})
%   = \pot(m_i).
% $$

% \noindent
% \hrulefill

% %We now decompose the interval $[n,m]$ into segments of increasing and decreasing $\Delta$.
% Let $[n_i,m_i]\subseteq[n,m],i\in\{1,...,s\}$ be an enumeration of the maximal intervals on which $\Delta$ is non-decreasing.
% Then $n=n_1<m_1<n_2<\cdots<n_s<m_s=m$.

% For that purpose, let $n=n_1<n_2<\cdots<n_s$ be an enumeration of the start indices of increasing segments of $\Delta$, and likewise, let $m_1<m_2<\cdots<m_s=m$ be an enumeration of the end indices of increasing segments of $\Delta$. In particular, $n_1<m_1<n_2<\cdots<n_s<m_s$ (see \cref{fig:Delta_n}).


% %

% Fix $m,n\in\NN$ with $m\ge n$.
% Our goal is to derive an upper bound for $\Delta(m)/\Delta(n)$. 
% Our argument is strongest when the fraction is largest, and so w.l.o.g.\ we can assume that for all $k\in[n,m]$ holds $\Delta(n)\le\Delta(k)\le\Delta(m)$.

% % \noindent
% % \hrulefill

% % From log-concave follows
% % %
% % $$
% % \delta_{n+1}-1
% % \le\Big\lfloor\frac{f(n+1)}{f(n)}\Big\rfloor 
% % \le \frac{f(n+1)}{f(n)} 
% % \le \Big(\frac{f(n)}{f(n-1)}\Big)^2
% % \le \Big\lceil\frac{f(n)}{f(n-1)}\Big\rceil^2
% % \le (\delta_n+1)^2.
% % $$
% % %
% % which rearranges to
% % %
% % $$
% % \nu(n+1):=\frac{\delta_{n+1}}{\delta_n^2}\le 1+\frac2{\delta_n}+\frac2{\delta_n^2} 
% % %\le 1+\frac1{\sqrt{\delta_n}}+\frac1{\delta_n}.
% % %\le 1+\frac1{\delta_n-1}.
% % \le 1+ \frac1{\delta_n^{1/2}},
% % $$
% % %
% % where the last inequality holds at least for $\delta_n\ge 6$.

% % Suppose that $\nu(n+k)\ge 1$ for all $k\in\{1,...,m-n\}$.
% % First, it follows $\delta_{n+k}\ge \delta_n^{2^k}$ which yields
% % %
% % \begin{align*}
% % \frac{\Delta(m)}{\Delta(n)} = \prod_{k=1}^{\mathclap{m-n}} \nu(n+k) 
% % &\le \prod_{k=1}^\infty \Big(1+\frac{1}{(\delta_n^{2^k})^{1/2}}\Big) =: G(\delta_n). \\ 
% % G(\delta_n)&\le \prod_{k=0}^\infty \Big(1+\frac{1}{\delta_n^{2^k}}\Big) = \sum_{s=0}^\infty \delta_n^{-s} = \frac{1}{1-1/\delta_n} = \frac{\delta_n}{\delta_n-1}\le \delta_n.
% % \end{align*}
% % %
% % Note that $G(\delta)$ is decreasing in $\delta$.
% % Thus, in order for $\Delta(\free)$ to grow beyond $G(\delta_n)\cdot\Delta(n
% % )$.

% % \hrulefill

% % Choose $m,n\in\NN$ with $m\ge n$.
% % Since our goal is to derive an upper bound for $\Delta(m)/\Delta(n)$ we can assume w.l.o.g.\ that for all $k\in(n,m)$ holds $\Delta(n)<\Delta(k)<\Delta(m)$.

% Let $n=n_1<n_2<\cdots<n_s$ be an enumeration of the start indices of increasing segments of $\Delta$, and likewise, let $m_1<m_2<\cdots<m_s=m$ be an enumeration of the end indices of increasing segments of $\Delta$. In particular, $n_1<m_1<n_2<\cdots<n_s<m_s$ (see \cref{fig:Delta_n}).

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.65\textwidth]{img/Delta_n.pdf}
%     \caption{...}
%     \label{fig:Delta_n}
% \end{figure}

% Consider the infinite product
% %
% $$G(\delta):=\prod_{k = 1}^\infty \Big(1+\frac2{\delta^{2^k}}+\frac4{\delta^{2^{k+1}}}\Big).$$
% %
% One can show (see Appendix 1.1) that $G(\delta)<36$ for all $\delta\ge 2$ and that $G$ is decreasing in $\delta$.
% Our goal is now to show that $\Delta(m)/\Delta(n)\le G(\delta_n)$.
% More precisely, we show that $\Delta(m_i)/\Delta(n)\le G(\delta_n)$ for all $i\in\{1,...,s\}$. We show this by induction.

% For the induction base, note that since $\Delta$ is increasing on $[n_i,m_i]$, it holds $\nu(n_i+k)=\Delta(n_i+k)/\Delta(n_i+k-1)\ge 1$ for all $k\in[1,...,m_i-n_i]$, which rearranges to $\delta_{n_i+k}\ge \delta_{n_i+k-1}^2$. Expanding this recursive inequality yields $\delta_{n_i+k}\ge \delta_{n_i}^{2^k}$.
% Thus
% %
% \begin{align*}
% \frac{\Delta(m_i)}{\Delta(n_i)}
% &= \prod_{k=1}^{\mathclap{m_i-n_i}} \nu(n_i+k) 
% \le \prod_{k=1}^{\mathclap{m_i-n_i}} \Big(1+\frac2{\delta_{n_i+k}}+\frac2{\delta_{n_i+k}^2}\Big)
% \\&\le \prod_{k=1}^{\mathclap{m_i-n_i}} \Big(1+\frac2{\delta_{n_i}^{2^k}}+\frac2{\delta_{n_i}^{2^{k+1}}}\Big)
% < G(\delta_{n_i}).
% \end{align*}
% %
% With $i=1$ this gives the induction base $\Delta(m_1)/\Delta(n)<G(\delta_n)$.
% In fact, this can be strengthened: for $k\in[n_i,m_i-1]$ holds
% %
% \begin{align*}
% \Delta(k+1) \cdot G(\delta_{k+1})
% &\le\Delta(k+1)\cdot G(\delta_k^2)
% =\Delta(k) \cdot \nu(k+1)\cdot G(\delta_k^2)
% \\&\le \Delta(k) \cdot \Big(1+\frac2{\delta_k}+\frac2{\delta_k^2}\Big)  \cdot  \prod_{k = 0}^\infty \Big(1+\frac2{(\delta_k^2)^{2^{k}}}+\frac2{(\delta_k^2)^{2^{k+1}}}\Big) 
% \\&= \Delta(k) \cdot \prod_{k = 0}^\infty \Big(1+\frac2{\delta_k^{2^k}}+\frac2{\delta_k^{2^{k+1}}}\Big) 
% = \Delta(k)\cdot G(\delta_k).
% \end{align*}
% %
% Applied iteratively, this yields $\Delta(m_i)G(\delta_{m_i})\le\Delta(n_i)G(\delta_{n_i})$.

% For the induction step we first need to prove that $\delta_{n_{i+1}}\ge \delta_{m_i}$. If this were not the case, then there would be a $k\in[m_i,n_{i+1}-1]$ so that $\delta_{k+1}<\delta_k$ which implies $\nu(k+1)=\delta_{k+1}/\delta_k^2 <1/\delta_k$ and further
% %
% $$
% \Delta(k+1)
% =\nu(k+1)\Delta(k)
% <\frac1{\delta_k}\Delta(k)
% \le \frac1{\delta_k}\Delta(m_i)
% \le\frac1{\delta_n}G(\delta_n)\Delta(n)
% \le\Delta(n).
% $$
% %
% This would be a contradiction to the choice of $n$.

% With this in place, we can finish the induction step by
% %
% $$
% \Delta(m_{i+1})
% \le G(\delta_{n_{i+1}})\Delta(n_{i+1})
% \le G(\delta_{m_i})\Delta(m_i) 
% \le G(\delta_n)\Delta(n).
% $$



% \noindent\hrulefill


% Note that the upper bound in \cref{res:g_growth_trees} is quadratic in $g$, hence does capture the desired growth behavior even worse than, say, an upper bound of $g(2r+1)$. This is not a problem for establishing the existence of trees of intermediate growth.
% But it prevents us from concluding that there are trees of any particular polynomial growth.

% In the next section we show that for a target growth rate of at least $g(r)\sim r^{\alpha\log\log r}$ for $\alpha>1$, together with some further natural condition, the upper bound can be improved to be linear in $g(2r+1)$.

% This still fails to rescue the case for polynomial growth.
% However, if $\bar g(r)=r^\alpha$ has integer exponents and $\delta_n=2^\alpha-1$, then we can embed $T$ into the $\alpha$-th power of the $\alpha$-dimensional integer lattice as shown in \cref{fig:2_lattice_construction} (recall that the $\alpha$-th power $G^\alpha$ of a graph $G$ is obtained by adding edges to $G$ between any pair of vertices at distance at most $\alpha$).
% This established a $r^\alpha$ upper bound on the volume growth of $T$.

%\begin{example}\label{ex:lattice_tight_upper_bound}

% Consider the following slightly modified construction of the tree $T_n$: instead of identifying the root of each apocentric copy of $T_{n-1}$ with an apocentric vertex of the central copy of $T_{n-1}$, we now let the central and apocentric copies of $T_{n-1}$ be disjoint, and we add edges between their apocentric vertices (see \cref{fig:compare_constructions}).

% \begin{figure}[h!]
%     \centering
%     %\includegraphics[width=0.5\textwidth]{img/compare_constructions.pdf}
%     \includegraphics[width=0.55\textwidth]{img/compare_constructions_2.pdf}
%     \caption{Comparison of $T_1$ from \cref{ex:loglogr} for the old construction (left) and the new construction (right). The dashed lines on the~right~indicate the new edges added to $T_1$ that connect the disjoint copies of $T_0$.}
%     \label{fig:compare_constructions}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     %\includegraphics[width=0.95\textwidth]{img/2_lattice_subgraph_2.pdf}
%     \includegraphics[width=0.95\textwidth]{img/2_lattice_subgraph_3.pdf}
%     %\caption{Illustration of the first four steps in the  construction~of~\cref{ex:lattice_tight_upper_bound}. %The ringed vertex is the root, and the white vertices are the apocentric vertices in the respective tree. The highlighted subgraph is the central copy of $T_{n-1}$ in $T_n$.
%     %}
%     \caption{
%         Embedding of the tree $T$ with constant sequence $\delta_n=3$ into the square of the 2-dimensional lattice graph.
%     }
%     \label{fig:2_lattice_construction}
% \end{figure}

% There are two things to note about this modified construction: first, the proof of \cref{res:g_growth_trees} applies with only minor modifications (one of which is that the distance from the central vertex to an apocentric vertex in $T_n$ is no longer $2^n$, but $(3^n-1)/2$).
% Second, if we use a constant sequence $\delta_n=3^\alpha-1$ for $\alpha\ge 1$we find that the resulting tree is a spanning tree of $L^2$, where $L$ is the $\alpha$-dimensional lattice graph, and $L^2$ means that we add additional edges between vertices that are at distance two in $L$.
% In particular, since the volume growth of $L^2$ is still of on the order of $r^\alpha$, this provides an equivalent upper bound on the volume growth of the resulting limit tree $T$.

%\end{example}




% \section{A linear upper bound}
% \label{sec:linear_bound}

% In this section we assume that $g$ has the following three properties:
% %
% \begin{enumerate}
%     \item $g$ is log-concave.
%     \item $f(n):=g(2^n)$ is log-convex.
%     \item $g\in\Omega(r^{\alpha\log\log r})$ for some $\alpha>1$.
% \end{enumerate}
% %
% The first two conditions just make sure that $g$ grows nicely enough, that is, does not change its growth behavior too rapidly. Most naturally occurring functions satisfy these conditions anyway.
% The last condition turns out to be a \enquote{magic} barrier to our techniques analysing this specific construction.

% \begin{proposition} \label{res:d_i_loglog_r}
% If $g(r)=r^{\omega(1)}$ grows super-polynomially then $s_n:=f(n)/f(n-1)$ is increasing, and $(\delta_n-1)/s_n\to 1$. 

% If we furthermore have $g\in\Omega(r^{\alpha\log\log r})$ for some $\alpha>1$, then there are $0<A_n \le B_n<1$ with
% %
% $$A_n s_n \le \delta_n-1 \le B_n s_n,\quad\text{for all $n\ge 1$},$$
% %
% and so that $A_n,B_n\to 1$, and
% %
% $$\prod_{i=1}^\infty \frac{B_i}{A_i^2}<\infty$$
% %
% converges \emph{(\emph{note that the terms $B_i/A_i^2\ge 1$, so the partial products never decrease})}.
% \end{proposition}

% \begin{proof}
% For brevity, define $s_n:=g(2^n)/g(2^{n-1})$. By definition of the $\delta_n$, we have
% %
% $$\frac{\delta_n-1}{s_n} \ge \frac{\lfloor s_n\rfloor -1}{s_n} =: A_n, \qquad \frac{\delta_n-1}{s_n} \le \frac{\lceil s_n\rceil -1}{s_n} =: B_n.$$
% % 
% Since $s_n\ge 2$ we indeed have $0<A_n\le B_n<1$.
% Since $g$ is super-polynomial, the $s_n$ are unbounded, and so $A_n,B_n\to1$.
% If $s_n=2$, then $B_n/A_n^2=1$. If $s_n>2$ we have the following estimation:
% %
% $$1<\frac{B_n}{A_n^2} = \frac{s_n(\lceil s_n\rceil-1)}{(\lfloor s_n\rfloor-1)^2} \ge \frac{s_n^2}{(s_n-2)^2} = \Big(1-\frac2{s_n}\Big)^{-2}<\infty$$
% %
% As established previously, the conditions on $g$ guarantee that the infinite product~of these terms converges.
% \end{proof}

% \begin{proposition}\label{res:average_degree_estimation}
% There exists a constant $C>1$ so that for all $m\ge n$ holds
% %
% $$\frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)} \le C\cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)}.$$
% %
% In particular, the maximum degree 
% %
% \begin{equation*}%\label{eq:conditions_g}
% \Delta:= \Big\lceil \sup_m \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_m-1)} \Big\rceil +1 \;\le\; \lceil C(\delta_1-1)\rceil + 1.
% \end{equation*}
% %
% is finite.
% \end{proposition}
% %
% \begin{proof}
% Since $g$ is log-concave, we have
% %
% \begin{align*}
%     \textstyle \frac13\log g(2^{m+1}) + \frac23 \log g(2^{m-1}) &\le \log g\big(\overbrace{\textstyle\frac23(2^{m-1})+\overset{\phantom .}{\frac13}(2^{m+1})}^{2^m}\big)
%     \\
%     g(2^{m+1})[g(2^{m-1})]^2 &\le [g(2^m)]^3
%     \\
%     \frac1{B_n}(\delta_{m+1} - 1)\le \frac{g(2^{m+1})}{g(2^m)} &\le \Big[\frac{g(2^{m})}{g(2^{m-1})}\Big]^2 \le \frac1{A_m^2}(\delta_m-1)^2
%     \\
%     \delta_{m+1}-1 &\le \frac{B_m}{A_m^2} \cdot (\delta_m-1)^2
%     \\
%     \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)} &\le \frac{B_m}{A_m^2} \cdot \frac{\delta_{m}-1}{(\delta_1-1)\cdots(\delta_{m-1}-1)}
%     \\
%     &\le \cdots \le 
%     \Big(\prod_{i=n+1}^{m}\frac{B_i}{A_i^2}\Big) \cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)}
%     \\
%     &\le C \cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)},
% \end{align*}
% %
% where we set $C:=\prod_{i=1}^\infty B_i/A_i^2$, which exists by \cref{res:d_i_loglog_r}.
% \end{proof}

% \begin{theorem}
% There is a constant $D>1$ so that
% %
% $$|B_v^T\!(r)|\le D\cdot g(2r-1).$$
% %
% %In particular, $|B_v^T\!(r)| = \theta(g)$.
% \end{theorem}
% %
% \begin{proof}
% Fix a vertex $v\in V(T)$ and $r\ge 0$. Choose $n$ so that $2^{n-1}-1 \le r \le 2^n-1$ and let $T_n(v)$ be the copy of $T_n$ that contains $v$. Let $m$ be the biggest number so that $T_n(v)$ is an apocentric copy of $T_n$ in $T_m\subset T$, or $n$ if $T_n(v)=T_n\subset T$. Then $m\ge n$ and by  \cref{res:average_degree_estimation} holds
% %
% $$
% \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)} 
% \le C \cdot \frac{\delta_{n+1}-1}{(\delta_1-1)\cdots(\delta_{n}-1)}
% $$
% %
% for some $C>1$ that only depends on $g$.
% This rearranges to
% %
% \begin{align*}
% \delta_{n+1}-1 
% &\ge \frac1C \cdot (\delta_1-1)\cdots(\delta_{n}-1) \cdot \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)}.
% % \\
% % &\le \frac1C \cdot \Big\lceil(\delta_1-1)\cdots(\delta_{n}-1) \cdot \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)}\Big\rceil.
% \end{align*}
% %
% Since $\delta_{n+1}-1$ is an integer, we actually have
% %
% \begin{align*}
% \delta_{n+1}-1 
% &\ge \frac1C \cdot \Big\lceil(\delta_1-1)\cdots(\delta_{n}-1) \cdot \frac{\delta_{m+1}-1}{(\delta_1-1)\cdots(\delta_{m}-1)}\Big\rceil.
% \end{align*}
% %
% The left side of this inequality is the number of edges leaving $T_n\subset T$ via apocentric vertices, while the right side is $1/C$ times an upper bound for the number of edges leaving $T_m(v)$ via apocentric vertices.

% % As in the proof of the upper bound in \cref{res:g_growth_trees}, $T_n(v)$ can be left in only two ways, via an apocentric vertex of $T_n(v)$, or via the center of $T_n(v)$.
% % %
% % \begin{itemize}
% %     \item How many copies ...
% % \end{itemize}
% \end{proof}

\section{Unimodular random trees}
\label{sec:unimodular}

%\begin{mnote}
%Notes:
%\begin{enumerate}
    %\item We need to define a ton of terminology surrounding (unimodular) random graphs/trees, and in my opinion the right place for this would be over the course of this section. Note that this does not mean that everything has to be define in the first paragraph: random graph should be define at the start, but \eg\ transport functions, BS-convergence and unimodularity can be defined only when we explain how to obtain unimodular graphs later on (before Theorem 4.1).
    %\item What are \enquote{nice functions}?
    %\item In Theorem 4.1, better use the sequence $(T_n,x^*)$, and maybe subsequence $(T_{n_i},x^*)$? \gsays{I would advise against it; even if these graphs are conceptualised as an inclusion chain, I still need their roots to be chosen \emph{independently} u.r., so I cannot use the same variable for all of their roots. That said, we can still discuss changes in style.}
    %\item I would say for defining \enquote{generalized canopy tree} we can combine intuition and formal definition: start from the modified inclusion chain $T_1\subset T_2\subset \dots$ where we identify $T_{n-1}$ with an \emph{apocentric} copy in $T_{n}$ instead of the central copy. Then all $T_n$ can still be chosen rooted at $o_n=x^*$, because this \enquote{global root} (a bad name now) stays apocentric forever. \gsays{I think we've already written this.}
    %\item Perhaps we should explain what the usual canopy tree is in a footnote.
    %\item We need a new graphics for the generalized canopy tree (I am working on that).
    %\item I am not a fan of abbreviations, I would write \enquote{almost surely} instead of a.s. (or at least mention once what it stands for). \gsays{But this is very standard!}
    %\item Is the sequence $(T_n,o_n)$ in the definition of  \enquote{complete central/apocentric} and \enquote{eventually apocentric} \emph{the} sequence from Construction 2.1? If yes, say so.
    %\item You define \enquote{undecided} for a sequence of vertices instead of rooted trees. \gsays{I mean, those vertices are the roots of rooted trees. Yes I would rather say that the root of a tree is undecided rather than that a rooted tree is undecided. Does it make a difference? I mean, apart from the fact that using these words for roots is more intuitive.}
    %\item On that note, maybe we can/should define these notions (completely central/apocentric and undecided) also for random trees. For example, a random tree $(T,x)$ is completely apocentric if $x$ is apocentric in every $T_n(x)$ with probability one (see my note on Proposition 4.2 below for why I think so).\gsays{...but we have done this. This is exactly what I mean when I write "these adjectives also apply to...". The only difference between what you are proposing and what is written is that you say that a rooted tree is, say, completely apocentric, and I say that its root is completely apocentric. And might I add, we already have a word for what you would call an "eventually apocentric tree": it is the generalised canopy tree.} \gsays{Hm, all right, we never explained that if the root of a limit tree is eventually central or eventually apocentric or undecided, then so is every vertex of the tree, and therefore that these are properties of both the tree and the root. I should say that.}
    %\item I consider proofs black boxes. If you use something outside of a proof, then it should be defined outside of a proof. I am specifically referring to $\mathcal T$. \gsays{But this is the underlying graph of the limit of a subsequence of $(T_n,o_n)$ that is only important in the context of the proof!}
    %\item You need to explain what Kolmogorov's law is, or avoid using it (we don't necessarily need to invoke big theorems if it can be done elementary :D).
    %\item Proposition 4.2 is supposed to be a general structure theorem on the limit tree. Maybe it is better to formulate it as follows: if the $\delta_n$ grow like this, then the limit is completely apocentric, if it grows like that, then it is completely central, otherwise undecided.
    %\item Proposition 4.3 is not used anywhere, is it? It should also be proven properly. \gsays{Apart from one minor thing that I fixed, it looks correct.}
    %\item We should use consistent terminology: always Benjamini-Schramm limit, or always distributional limit (idea: let's stick to BS limit). \gsays{Hm, but there is a slight difference here...}
    %\item Should we make Example 4.4 more rigorous? (especially the last two sentences).
    %\item Should we say a word about why the limit trees that result from inclusion chains $T_0\subset T_1\subset T_2\subset\cdots$ other than the standard one (where $T_{n-1}$ is central in $T_n$) still satisfy the conclusion of Theorem 3.4 (that is, the uniform volume growth)?
    %\item Meta thought: there are clearly two styles of writing and two styles of formatting in this paper. I wonder whether we should make this more uniform. And how?
%\end{enumerate}
%\end{mnote}

%\begin{mnote}
%Notes (08/07/2022):
%\begin{enumerate}
 %   \item can we show that $T_1,T_2,T_3,...$ actually BS-converge, not just that it has a convergent sub-sequence?
    %\item Is a generalized canopy tree the same as a 1-ended tree?
%\end{enumerate}
%\end{mnote}

\emph{Rooted graphs} are pairs of the form $(G,o)$, $o\in V(G)$. For the purpose of this section it is useful to define the notion of a \emph{random rooted graph} as introduced in \cite{benjamini2011recurrence}. For this, we must firstly note that there is a natural topology over the set of rooted graphs, the \emph{local topology}, induced by the metric 
%
\begin{align*}
\dist\!\big((G,o),(G',o')\big):=2^{-R} \quad &\text{if } \ball Gor\cong \ball{G'}{o'}r \text{ for all } 0\leq r\leq R
\\
&\text{and } \ball Go{R+1}\ncong \ball{G'}{o'}{R+1}.
\end{align*}
%
% \[d((G,o),(G',o'))=2^{-k} \hspace{1mm}\text{if}\hspace{1mm} \ball Gor\cong \bal{G'}{o'}r \hspace{1mm} \text{for}\hspace{1mm} 0\leq r\leq k\]
% %
% \[\text{and}\hspace{1mm} \ball Go{k+1}\ncong \ball{G'}{o'}{k+1}.\]

A random rooted graph $(G,o)$ is a Borel probability measure (for the local topology) over the set of locally finite, connected rooted graphs. We call $(G,o)$ \emph{finite} if the set of infinite rooted graphs has $(G,o)$-measure $0$. If the conditional distribution of the root of a finite random rooted graph $(G,o)$ over each of the underlying graphs in its support is uniform, then $(G,o)$ is called \emph{unbiased}. 

Given a sequence $(G_n,o_n)$ of unbiased random rooted graphs together with a random rooted graph $(G,o)$, we say that $(G,o)$ is the \emph{Benjamini-Schramm limit} of $(G_n,o_n)$ if for every finite rooted graph $H$ and natural number $r$ we have 
%
\[\lim_{\mathclap{n\to \infty}}P\big(\ball{G_n\!}{o_n}r\cong H\big)=P\big(\ball{G}{o}r\cong H\big).\] 
%
If a random rooted graph $(G,o)$ is the Benjamini-Schramm limit of some sequence, we say that it is \emph{sofic}. By a standard result \cite{benjamini2011recurrence}, any set of graphs of uniformly bounded degree is compact in the local topology, from which it follows that a sequence $(G_n,o_n)$ of uniformly bounded degree graphs always has a convergent subsequence.

The notion of uniform growth is well-defined in random rooted graphs. We say that a random rooted graph $(G,o)$ has uniform growth $g(r)$ if there exists a function $g:\RR_{\ge 0}\rightarrow \RR_{\ge 0}$ and positive constants $c_1, C_1, c_2, C_2$ such that for every $r\ge 0$ \as\ $C_1\cdot g(c_1r)\leq |B_G(o,r)|\leq C_2\cdot g(c_2r)$, \ie\ if almost all the vertices (measured by the distribution of $o$) exhibit a common uniform growth. 

The precise statement of Benjamini's question requests a \emph{unimodular} tree of intermediate growth. A random rooted graph $(G,o)$ is unimodular if it obeys the mass transport principle, \ie
%
\[\mathbb E\Big[\sum_{\mathclap{x\in V(G)}}f(G,o,x)\Big]=\mathbb E\Big[\sum_{\mathclap{x\in V(G)}}f(G,x,o)\Big]\]
%
for every transport function $f$. For an exact definition of transport functions we direct the reader to \cite{aldouslyons}. For the purpose of this paper, it suffices to say that transport functions are Borel functions over doubly-pointed graphs that output non-negative values and simulate mass transport between vertices. The mass transport principle simply states that the root $o$ on average sends as much mass to other vertices as it receives from them. Unimodular graphs are quite significant in the theory of random graphs and encompass some interesting classes. The most basic non-trivial example is that all sofic graphs are unimodular. The famous Aldous-Lyons conjecture asks for the converse \cite{aldouslyons}. 

In the preceding sections, given a super-additive, log-concave growth function $g\:\RR_{\ge 0}\to\RR_{\ge 0}$, we constructed a deterministic rooted tree $(T,x^*)$ ($x^*$ being the original copy of $T_0$)  which exhibits uniform growth $g(r)$. However, $(T,x^*)$ is not necessarily unimodular. Indeed, suppose that we construct $(T,x^*)$ as a centric limit, and that $|\frac{\delta_n}{\delta_1...\delta_{n-1}}-(\delta_1-1)|\geq 1$ for every $n\geq 2$. Then $x^*$ is the only vertex with degree $\delta_1$. Consider the transport function $f(G,x,y)$ which equals $1$ if $G=T$, $x\sim y$ and $d_T(x,x^*)<d_T(y,x^*)$, and $0$ otherwise. Then $\mathbb{E}[\Sigma_{x\in V(T)}f(T,x^*,x)]=\delta_1\neq 0=\mathbb{E}[\Sigma_{x\in V(T)}f(T,x,x^*)]$.

That said, a unimodular tree with uniform growth $g(r)$ necessarily exists: 

\begin{proposition}\label{converge?}
    Let $g\:\RR_{\ge 0}\to\RR_{\ge 0}$ be super-additive and log-concave. Then the sequence $T_n$ has a subsequence that converges in the Benjamini-Schramm sense to a unimodular random rooted tree with uniform growth $g(r)$. %In particular, there exists a unimodular tree with intermediate uniform growth.
\end{proposition}

\begin{proof}
Consider a sequence $(T_n,o_n)$ of unbiased random rooted trees, where each $T_n$ is \as\ as in \cref{constr:T_n}. Since by \cref{res:conditions_in_g} and \cref{thm:main} $(T_n,o_n)$ has uniformly bounded degrees and is therefore compact in the local topology, there exists a subsequence of $(T_n,o_n)$, say $(T_{k_n},o_{k_n})$, converging to a random rooted tree $(\mathcal{T},\mathcal{o})$. By the definition of the Benjamini-Schramm limit, every ball of $(\mathcal{T},\mathcal{o})$ centered at $\mathcal{o}$ is \as\ isomorphic to a ball of $\mathcal{T}_{k_n}$ for $n$ large enough. However, every ball of radius $\leq 2^{k_n}-1$ in $T_{k_n}$ is isomorphic to a ball of a limit tree $T$ as in \cref{constr:T}, and therefore admits the respective bounds. %Every ball of $(\mathcal{T},\mathcal{o})$ is contained in a ball rooted at  $\mathcal{o}$, and is thus \as\ a ball of $\mathcal{T}_n$. 
Hence, $\mathcal{T}$ exhibits uniform growth of order $g(r)$. Additionally, since $(\mathcal{T},\mathcal{o})$ is sofic, it is also unimodular.
\end{proof}

In fact, we may even eschew focusing on a subsequence:

\begin{proposition}\label{converge}
    The sequence $T_n,n\ge 0$ is Benjamini-Schramm convergent.
\end{proposition}

\begin{proof}
    Fix $r\ge 1$ and a graph $H$.
    Call a vertex $v\in V(T_n)$ \emph{good} if $\ball{T_n} v r\cong H$.
    Let $P_n$ be the probability that a uniformly chosen vertex of $T_n$ is good.
    %We show $|P_{n+k}-P_n|\le C_r 2^{-n}$ for all $k\ge 0$ and a constant $C_r\ge 1$ that only depends on $r$.
    %In other words, $P_n$ is a Cauchy sequence, hence convergent, and $T_n$ is BS-convergent.
    We show that $P_n$ is a Cauchy sequence, hence convergent.

    Let $s_n$ be the number of good vertices in $T_n$.
    Since $T_n$ consists of $\delta_n+1$ copies of $T_{n-1}$, one might expect $s_n\approx (\delta_n+1)s_{n-1}$.
    However, besides the copies, $T_n$ also contains $\delta_n$ new edges, and so for $\tau\prec_{n-1} T_n$ and $v\in V(\tau)$, the $r$-ball around $v$ in $\tau\cong T_{n-1}$ might look different from the $r$-ball around $v$ in $T_n$.
    Still, this can only happen if $v$ is $r$-close to one of the $2\delta_n$ ends of the new edges.
    Let $C_r$ be an upper bound on the size of an $r$-ball in $T$ (which exists since $T$ is of bounded degree). We can then conclude
    %
    $$|s_n-(\delta_n+1)s_{n-1}|\le 2C_r\delta_n.$$
    %
    Since $P_n=s_n/|T_n|$, division by $|T_n|=(\delta_n+1)|T_{n-1}|$ yields
    %
    \begin{align*}
        &|P_n-P_{n-1}|\le \frac{\delta_n}{\delta_n+1}\frac{2C_r}{|T_{n-1}|}\le \frac{2C_r}{|T_{n-1}|}.
    \end{align*}
    %
    It follows for all $k\ge 1$
    %    
    \begin{align*}
    |P_{n+k}-P_n| 
    &\le |P_{n+k}-P_{n+k-1}|+\cdots+|P_{n+1}-P_n|
    \\ &\le 2C_r\Big(\frac1{|T_{n+k-1}|}+\cdots+\frac1{|T_{n}|}\Big)
    \le 2C_r\sum_{i=n}^{\infty} \frac1{|T_i|}.
    \end{align*}
    %
    Since $\delta_n\ge 1$ and $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ we have $|T_n|\ge 2^n$. It therefore follows
    %
    \begin{align*}
    |P_{n+k}-P_n| \le \frac{4C_r}{2^n},
    \end{align*}
    %
    and $P_n$ is indeed a Cauchy sequence.
\end{proof}


 \cref{unimain} is a corollary of \cref{converge?}. However, since \cref{converge?} does not offer a constructive proof of \cref{unimain}, one might still wonder about the exact structure of $\mathcal{T}$. To answer this question, we require certain definitions and observations. We allow the notations $(T_n,o_n)$, and $(\mathcal{T},\mathcal{o})$ to retain their meaning for the rest of this section.  

Let $p_n:=\frac{\delta_n}{\delta_n+1}$, and note that $p_n$ is precisely the probability that for a vertex $v$ of $T_k$, $k\geq n$, chosen uniformly at random we have $v\in \tau\prec_{n-1} \tau'\prec_n T_k$ and $\tau$ is apocentric in $\tau'$. We say that the sequence $(T_n,o_n)$ is \emph{apocentric} if $\prod_{n=1}^{\infty}p_n>0$. Otherwise, we say that it is \emph{balanced}. Note that a sequence is apocentric if and only if the same is true for each of its subsequences. %For brevity, these adjectives will be called the \emph{type} of the subsequence.  

A \emph{generalized canopy tree}\footnote{Recall that the \emph{canopy tree} is the Benjamini-Schramm limit of a sequence of full binary trees of increasing depths. The canopy tree is the single most famous example of a generalized canopy tree.} is the Benjamini-Schramm limit of an apocentric sequence. On the other hand, a \emph{balanced tree} is the Benjamini-Schramm limit of a balanced sequence.

Let us continue our analysis by establishing conditions on $\delta_n$ (and, by extension, $g$) under which $(\mathcal{T}, \mathcal{o})$ is a generalized canopy tree or a balanced tree.

\begin{proposition}\label{res:types_of_limits}
If $\delta_n>n^{\alpha}$ for some $\alpha>1$ and all sufficiently large $n$, then $(\mathcal{T}, \mathcal{o})$ is \as\ a generalized canopy tree. 
If $\delta_n$ grows at most linearly, then $(\mathcal{T},\mathcal{o}$) is \as\ a balanced tree.
\end{proposition}

\begin{proof}
The limit tree $(\mathcal{T},\mathcal{o})$ is \as\ a generalized canopy tree if and only if $(T_n,o_n)$ is an apocentric sequence, equivalently if $\Sigma_{n=1}^{\infty}\ln\frac{\delta_n+1}{\delta_n}<\infty$, which is true for $\delta_n>n^{\alpha}$. Indeed,
%
%\begin{align*}
%\ln\frac{\delta_n+1}{\delta_n}&<\frac{1}{n^{\alpha}}\Leftrightarrow
%\\
%\frac{\delta_n+1}{\delta_n}&<e^{\frac{1}{n^{\alpha}}}\Leftrightarrow
%\\
%1-\frac{1}{\delta_n+1}&>e^{-\frac{1}{n^{\alpha}}}\Leftrightarrow
%\\
%\delta_n>\frac{1}{1-e^{-\frac{1}{n^{\alpha}}}}-1&=\frac{e^{-\frac{1}{n^{\alpha}}}}{1-e^{-\frac{1}{n^{\alpha}}}}=\frac{1}{e^{\frac{1}{n^{\alpha}}}-1}\Leftarrow
%\\
%\delta_n&>n^{\alpha}.
%\end{align*}
%
\begin{align*}
\delta_n>n^\alpha \ge \frac{1}{\exp(1/n^\alpha)-1}
%=\frac1{1-\exp(-1/n^\alpha)}-1 
\;\implies\; \ln\Big(\frac{\delta_n+1}{\delta_n}\Big)<\frac1{n^\alpha}
\;\implies\; \sum_{n=0}^\infty \ln\Big(\frac{\delta_n+1}{\delta_n}\Big) <\infty.
\end{align*}

Therefore, if we eventually have $\delta_n>n^{\alpha}$, $\alpha>1$, $(\mathcal{T},\mathcal{o})$ is \as\ a generalized canopy tree with an apocentric vertex for a root. 

%Subsequently, we may ask for the probability that  $(\mathcal{T}_n,\mathcal{o}_n)$ is eventually apocentric. But this event contains the event that $\mathcal{o}_n$ is a sequence of apocentric vertices, and for $\delta_n>n^{\alpha}$ the latter has positive probability. By Kolmogorov's Law, every tail event has probability either $0$ or $1$. Therefore, for $\delta_n>n^{\alpha}$, $(\mathcal{T},\mathcal{o})$ is a.s. a generalized canopy tree. 

On the other hand, if $\delta_n<kn$, and since $kn(e^{\frac{1}{kn}}-1)\rightarrow 1$, we obtain
%
%\[\delta_n+1<\frac{1}{1-e^{-\frac{1}{kn}}}\Leftrightarrow\]\[1-\frac{1}{\delta_n+1}<e^{-\frac{1}{kn}}\Leftrightarrow\]\[\ln \frac{\delta_n+1}{\delta_n}>\frac{1}{kn},\] 
%
%\msays{My attempt:}
\begin{align*}
\delta_n<kn \le \frac{1}{\exp(1/kn)-1}
%=\frac1{1-\exp(-1/n^\alpha)}-1 
\;\implies\; \ln\Big(\frac{\delta_n+1}{\delta_n}\Big)>\frac1{kn}
\;\implies\; \sum_{n=0}^\infty \ln\Big(\frac{\delta_n+1}{\delta_n}\Big) =\infty,
\end{align*}
%
implying that $(T_n,o_n)$ is balanced. %As mentioned previously, the probability that $(\mathcal{T}_n,\mathcal{o}_n)$ is eventually central is also 0. 
So, for linear or sublinear $\delta_n$, $(\mathcal{T},\mathcal{o})$ is \as\ balanced.
\end{proof}

\begin{proposition}
If $g\in\Omega(r^{\alpha\log\log r})$ for some $\alpha >0$ and $f(n):=g(2^n-1)$ is log-con\-vex, then $\delta_n=\Omega(n^\alpha)$. For $\alpha>1$ it follows that $(\mathcal{T},\mathcal{o})$ is \as\ a generalized canopy tree. As a consequence, every nice growth ($g$ super-additive, log-concave; $g(2^n-1)$ log-convex) is exhibited by a generalized canopy tree.
%
$$
%\lim_{n\to\infty} \frac{(\delta_1)\cdots (\delta_n)}{(\delta_1-1)\cdots(\delta_n-1)} = \prod_{n=1}^\infty \Big(1-\frac1{\delta_n+1}\Big) > 0.
$$
\end{proposition}
\begin{proof}
Let $C>0$ so that $g(r)\ge C r^{\alpha\log\log r}$ for all sufficiently large $r$. 
In terms of $\log f(n)$ this reads
%
$$(*)\quad \log f(n)
\ge \log(C) + \alpha \log(2^n-1) \log\log(2^n-1) 
\geq \log(C) + \alpha n \log(n).
$$
%
for all sufficiently large $n$.

We show that $s_n:=f(n)/f(n-1)\ge n^\alpha$ for all sufficiently large $n$. The statement for $\delta_n$ then follows from $\delta_n/s_n \to 1$ for super-polynomial $g$.

Assume the contrary, that $s_n< n^\alpha$ for infinitely many $n$, or equivalently, that $(**)\;\log f(n) - \log f(n-1) < \alpha \log(n)$. By log-convexity $(\times)$ of $f$ follows
%
\begin{align*}
    \frac{1}{n-1} \log f(1) + \Big(1-\frac{1}{n-1}\Big)\log f(n) \,& \overset{\mathclap{(\times)}}\ge\, \log f(n-1)
    %\\&
    \,\overset{\mathclap{(**)}}>\,  \log f(n) - \alpha\log(n)
    \\
    \implies\quad \log f(1)  &> \log f(n) - \alpha(n-1)\log(n)
    \\[-1ex]
    & \overset{\mathclap{(*)}}\ge \log(C) + \alpha n \log(n) - \alpha(n-1)\log(n)
    \\[0.7ex]
    &= \alpha\log(n) + \log(C),
\end{align*}
%
which cannot be true for arbitrary large $n$.
\end{proof}

Having established some fundamentals about balanced and apocentric sequences and their limits, we are now equipped to prove our structure theorem:

\begin{main}[Structure Theorem]\label{structure}\quad
\begin{myenumerate}
    \item
    If $(\mathcal{T},\mathcal{o})$ is a generalized canopy tree, then it is \as\ an apocentric limit. In particular, it is 1-ended.
    \item
    If $(\mathcal{T},\mathcal{o})$ is a balanced tree, then it is \as\ a balanced limit and it is \as\ 1-ended or 2-ended. In particular, if $\delta_n\neq 1$ eventually, then $(\mathcal{T},\mathcal{o})$ is a.s. 1-ended and the probability that any specific tree is its underlying tree is 0.    
\end{myenumerate}
\end{main}
\begin{proof}\quad 
\begin{myenumerate}
    \item For an apocentric sequence, any tail product $p^{(k)}:=\prod_{n=k+1}^{\infty}p_n$ is positive. Additionally, $p^{(k)}$ is the limit of the probability that $o_n$ lies in an apocentric $\tau\prec_k T_n$ as $n\to\infty$. So, consider the event $A_{k,r}$ that the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball centered at a vertex of an apocentric $\tau\prec_k T_n$ (for $n$ large enough that the center of $T_n$ is not contained in the ball of radius $r$ centered at the center of $\tau$) and note that, for every $r\geq 0$, $P(A_{k,r})\geq p^{(k)}$. Let $A_k:=\bigcap_{r\geq 0}A_{k,r}$. That is, $A_k$ is the event that for every $r\geq 0$ the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball centered at an apocentric $\tau\prec_k T_n$ for $n$ large enough. Since $A_{k,r}$ is decreasing in $r$, we have $$P(A_k)=\lim_{r\rightarrow \infty}P(A_{k,r})\geq p^{(k)}.$$ Since $A_k$ is increasing in $k$, $$P(\bigcup_{i=1}^{\infty}A_k)=\lim_{k\rightarrow \infty}P(A_k)\geq \lim_{k\rightarrow \infty}p^{(k)}=1.$$ Therefore, there exists \as\ $k\in \NN_0$ such that the event $A_k$ occurs, implying that $(\mathcal{T},\mathcal{o})$ is an apocentric limit. 

    Let $v\in V(\mathcal{T})$ and let $m\geq k$ be such that a copy $\tau\prec_m\mathcal{T}$ contains both $\mathcal{o}$ and $v$. Take $r$ large enough so that $N(\tau)\subset B_{\mathcal{T}}(\mathcal{o},r)$ and recall that (since $A_k$ is increasing and $m\geq k$) $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball of a tree $T_n$ centered at a vertex of an apocentric $\tau'\prec_m T_n$. Since the apocentric vertices of $\tau'$ are leaves in $T_n$, the apocentric vertices of $\tau$ are leaves in $\mathcal{T}$, so the only vertex of $\tau$ that has a neighbor outside of $\tau$ is its center. Only one of the connected components of $\mathcal{T}\setminus v$ contains the center of $\tau$, so the rest are subtrees of $\tau$, therefore finite. Hence, $\mathcal{T}$ is 1-ended.

    \item For a balanced sequence, let $p_{(k)}:=\prod_{n=1}^kp_n$ and note that $p_{(k)}$ is the probability that a uniformly chosen vertex of a tree $T_n$, $n\geq k$ is apocentric in a copy $\tau\prec_k T_n$. Such a vertex will be called a $k$\emph{-boundary vertex}, and any ball centered at it will be called a $k$-boundary ball. Let $B_{k,r}$ be the event that the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a $k$-\emph{boundary ball} of $T_n$ for $n$ large enough. Note that, for $r\geq 2^{k+1}-1$, the only vertices that are the centers of balls isomorphic to $k$-boundary balls are indeed $k$-boundary vertices, hence $P(B_{k,r})\leq p_{(k)}$. Also, observe that $B_{k,r}$ is a decreasing sequence in $r$. Let $B_k:=\bigcap_{r\geq 0}B_{k,r}$. That is, $B_k$ is the event that for every $r\geq 0$ the ball $B_{\mathcal{T}}(\mathcal{o},r)$ is isomorphic to a ball centered at an apocentric vertex of a copy $\tau\prec_k T_n$ that is a leaf of $T_n$. We deduce that 
    %
    $$P(B_k)=\lim_{r\rightarrow \infty}P(B_{k,r})\leq \lim_{r\rightarrow \infty}p_{(k)}=p_{(k)}.$$ 
    %
    Since $B_k$ is also a decreasing sequence in $k$, 
    %
    $$P(\liminf_{k\rightarrow \infty B_k})=P(\bigcap_{k\geq 0}B_k)=\lim_{k\rightarrow \infty}P(B_k)\leq \lim_{k\rightarrow \infty}p_{(k)}=0.$$ 
    %
    Therefore $\mathcal{o}$ lies \as\ in a sequence of copies $\tau\prec_{k_n}\tau'\prec_{k_n+1}\mathcal{T}$ with $\tau$ central in $\tau'$. The proof that $\mathcal{o}$ lies \as\ in a sequence of copies $\tau\prec_{l_n}\tau'\prec_{l_n+1}\mathcal{T}$ with $\tau$ apocentric in $\tau'$ is completely analogous. We have shown that $(\mathcal{T},\mathcal{o})$ is \as\ a balanced limit. 

    We now proceed to deduce the number of ends of a balanced random rooted tree. It is well-known result that every unimodular random rooted tree with average root degree 2 has \as\ either one or two ends. However, this set happens to include all the Benjamini-Schramm limits of sequences of finite trees, and in particular $\mathcal{T}$. Indeed, the average degree of a tree on $n$ vertices is $2-\frac1{n}$, and, since $\lim_{n\to \infty}P\big(\ball{T_n\!}{o_n}1\cong S\big)=P\big(\ball{\mathcal{T}}{\mathcal{o}}1\cong S\big)$ for every star $S$, we obtain 
    %
    $$E(\deg(\mathcal{o}))=\lim_{n\rightarrow \infty}\sum_{m=1}^{\Delta}mP\big(\ball{T_n\!}{o_n}1\cong S_m\big)=\lim_{n\rightarrow \infty}2-\frac1{n}=2.$$

\begin{comment}
    \msays{use short version}

    Let us direct our attention to the neighbourhood of the root $\mathcal{o}$ and calculate its mean degree. 

With probability $1-p_1=\frac{1}{\delta_1+1}$, $\mathcal{o}$ is the centre of a copy of $T_1$, which has degree $\delta_1+1$, yielding a summant of 1. 

With probability $p_1=\frac{\delta_1}{\delta_1+1}$, $\mathcal{o}$ is a leaf of a copy of $T_1$. Therefore, its average degree depends on the minimum $k\in\NN$ such that $v\in \tau\prec_k\tau'\prec_{k+1} \mathcal{T}$ with $\tau$ being apocentric in $\tau'$. Specifically, it equals $\frac{\delta_{k+1}}{\prod_{n=1}^k\delta_n}+1$. The probability that a specific number $k$ has this property if $\mathcal{o}$ is a leaf of a copy of $T_1$ is $(1-p_{k+1})\prod_{n=1}^kp_k=\frac{\prod_{n=1}^k\delta_k}{\prod_{n=1}^{k+1}(\delta_n+1)}$. Thus, the second summant is $\sum_{k=1}^{\infty}\frac{\delta_{k+1}}{\prod_{n=1}^{k+1}(\delta_n+1)}+p_1=(1-p_1)+p_1=1$ and we have $\mathbf{E}(deg(\mathcal{o}))=1+1=2$.
\end{comment}

We have shown that balanced trees have \as\ one or two ends. If $(\mathcal{T},\mathcal{o})$ has two ends, then there exists a vertex in $\mathcal{T}$ that belongs to a double ray, so by \cite{...} $\mathcal{o}$ belongs to a double ray with positive probability. One ray $R_1$ is obtained by starting at $\mathcal{o}$ and moving to the center of $\tau'$ for each instance of $\mathcal{o}\in\tau\prec_n\tau'\prec_{n+1}\mathcal{T}$ where $\tau$ is apocentric in $\tau'$.  Let $k_n$ be the sequence for the terms of which we have $\mathcal{o}\in \tau\prec_{k_n}\tau'\prec_{k_n+1} \mathcal{T}$ and $\tau$ is central in $\tau'$. Say that $\tau\prec_{k_n}\mathcal{T}$ is \emph{reachable} if either $n=0$ and $\tau=\mathcal{o}$ or the center of $\tau$ is adjacent to an apocentic vertex of a reachable $\tau'\prec_{k_{n-1}} \mathcal{T}$. Then $\mathcal{o}$ emits another ray $R_2$ disjoint from $R_1$ if and only if for each $k_n$ there exists a reachable $\tau\prec_{k_n}\mathcal{T}$. 
By calculating the average number of reachable copies $\tau\prec_{k_n}\mathcal{T}$ and taking the limit as $n\rightarrow \infty$ we find that the average number of rays disjoint from $R_1$ that start from $\mathcal{o}$ is 
%
$$\mathcal{R}:=\prod_{n=1}^{\infty}\frac{\delta_{k_n}}{\prod_{m=k_{n-1}}^{k_n-1}\delta_m}.$$
%
Suppose that $\delta_n>1$ for every $n>~c$. 
Using \cref{res:types_of_limits}, we have $\delta_n=o(n^2)$ and we observe that $\frac{k_n^2}{2^{k_n-n-c}}$ is eventually an upper bound for the partial products of $\mathcal{R}$. For $\mathcal{o}\in \tau\prec_n\tau'\prec_{n+1} \mathcal{T}$, let $X_n$ be the random variable that equals 1 if $\tau$ is central in $\tau'$ and 0 otherwise. Define $X(k)=\sum_{n=1}^kX_n$ and note that the $X_i$ are independent, and that $X(k_n)=n$. By Hoeffding's inequality, 
%
$$\hspace{10mm}P\big(n-(1-p_{k_n})k_n>p_{k_n}k_n-3\log k_n-c\big)\leq e^{-\frac{2(p_{k_n}k_n-3\log k_n-c)^2}{k_n}}\leq e^{-\frac{k_n}{8}}.$$
%
Since $\sum_{n=1}^{\infty}e^{-\frac{k_n}{8}}<\infty$, by the Borel-Cantelli Lemma it \as\ eventually holds that $n\leq k_n-3\log k_n-c$ for every $n$, implying that $\mathcal{R}\leq\lim_{n\rightarrow \infty}\frac1{k_n}=0$. Therefore, \as\ no such rays exist, and we have that $\mathcal{T}$ is 1-ended. 

Finally, note that, if $\delta_n>1$ eventually, then each identification chain yields a different sequence of balls $|B_{\mathcal{T}}(\mathcal{o},r)|$, i.e. a different rooted limit tree. Also, for a balanced sequence in particular, $\prod_{n=1}^{\infty}\mathcal{P}_n=0$, where each $\mathcal{P}_n$ can be equal to either $p_n$ or $1-p_n$. That is to say, each particular identification chain, and therefore from the previous observation each rooted limit tree of \cref{constr:T}, is sampled from our balanced tree $(\mathcal{T},\mathcal{o})$ with probability 0. Since each such tree has only countable vertices, any particular tree has probability 0 to be the underlying tree of $(\mathcal{T},\mathcal{o})$. 

\end{myenumerate}

\end{proof}

%This observation reveals the structure of $\mathcal{T}$: it is a tree that we obtain by modifying \cref{constr:T_n} so that, for each $n\in \NN$, $T_n$ is identified with an apocentric copy of $T_{n+1}$. For instance, the generalised canopy tree for \cref{ex:loglogr} would look as follows: 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.43\textwidth]{img/canopy_3.pdf}
    %\includegraphics[width=0.8\textwidth]{img/canopy_2.pdf}
    %\includegraphics[width=0.6\textwidth]{img/canopy.pdf}
    \caption{The balanced tree corresponding to the sequence $\delta_n=n$. It is locally indistinguishable from a generalised canopy tree.}
\end{figure}

%Types can also apply to the vertices of the limit $(\mathcal{T}, \mathcal{o})$ of a converging subsequence $(T_{n_k},o_{n_k})$ in the obvious manner. It is an easy exercise to prove that the root $\mathcal{o}$ will be of the same type as $o_{n_k}$. Since every vertex of $\mathcal{T}$ lies at a finite distance from $\mathcal{o}$, all of $V(\mathcal{T})$ agrees in type with $\mathcal{o}$. Therefore, the type of the underlying tree $\mathcal{T}$ is well-defined. 

%Note that the tree of \cref{constr:T_n} is completely central, whereas the eventually apocentric trees are exactly the generalized canopy trees.    

%Finally, on the antipode from generalised canopy trees sits the limit tree of \cref{constr:T_n}, which can be similarly obtained as the limit of an eventually central sequence. However, due to the fact that any ball of fixed radius around the centre of a tree $T_n$ must be finite, whereas the trees $T_n$ grow arbitrarily large, we deduce that almost no unbiased sequences $(\mathcal{T}_n, \mathcal{o}_n)$ are eventually central.   

%We are now sufficiently equipped to explore the structure of the limit tree $(\mathcal{T},\mathcal{o})$. The following structure theorem describes the structure of $(\mathcal{T},\mathcal{o})$ depending on the sequence $\delta_1,\delta_2,\delta_3...\in\NN$ that generates it.

%We have demonstrated that every fast-growing nice function is the growth function of a random rooted generalized canopy tree, given as a limit of a subsequence of $(T_n,o_n)$. In fact, even the following is true:

%\begin{theorem}
    %If $\delta_{n+1}\geq e^{\frac{\alpha}{n}}\delta_n-1$ eventually for some $\alpha>1$ (which again implies a minimum growth of at least around $r^{\alpha \log\log r}$), then the very sequence $T_n$ converges to $\mathcal{T}$ (rather than merely a subsequence). 
%\end{theorem}

%\begin{proof}
 %Indeed, for $\mathcal{B}$ an isomorphism class of rooted balls of radius $r$, take $m\gg\log r$ and let $c$ be the density of $\mathcal{B}$ in $T_m$. Then in $T_{m+1}$, only the vertices that are $r$-close to the apocentric leaves of the central copy of $T_m$ may see changes in their respective $r$-balls. Suppose that there exist $\kappa$ such vertices and let $\lambda:=\frac{\kappa}{\prod_{k=1}^{m+1}(\delta_k+1)}$. Then the density of $\mathcal{B}$ in $T_{m+1}$ lies between $c-\lambda$ and $c+\lambda$. In general, the density of $\mathcal{B}$ in $T_n$, $n>m$ is between $c-\lambda(\sum_{k=m+1}^{n-1}\prod_{j=m+1}^k\frac{\delta_j}{\delta_{j+1}+1})$ and $c-\lambda(\sum_{k=m+1}^{n-1}\prod_{j=m+1}^k\frac{\delta_j}{\delta_{j+1}+1})$. Under the assumption, it is straightforward to show that the sequence $\sum_{k=m+1}^{n-1}\prod_{j=m+1}^k\frac{\delta_j}{\delta_{j+1}+1}$ converges, so that the density of $\mathcal{B}$ converges absolutely.  
%\end{proof}

 Depending on the circumstances, our knowledge about the structure of $(\mathcal{T},\mathcal{o})$ can be even more precise; in fact, as seen in the following example, there exists a particular choice of the sequence $\delta_n$ for which the Benjamini-Schramm limit of $(\mathcal{T}_n,\mathcal{o}_n)$ is has a single deterministic underlying tree. Note that, once again, this felicitous situation requires fast growth, since the probability that a single tree is the underlying tree of a balanced tree is $0\neq 1$.  

%\msays{I tried to make the example below rigorous, and while I succeeded in proving that the $T_n$ are very symmetric, as you can see, the argument exploded. I am experimenting with the proof in the sandbox \cref{res:symmetric_tree}.}

%\msays{To show that the symmetry of the $T_n$ leads to a deterministic unimodular tree it would be better to first finish the definition parts of this section, so that we know what we are working with.}

%\begin{example}\label{ex:deterministic}
%Define the sequence $\delta_0,\delta_1,\delta_2,...$ with initial terms $\delta_0\ge 1,\delta_1\geq 2$ and recurrence $\delta_{n+1}:=\delta_n\delta_{n-1}$.
%In explicit form this yields
%
%$$\delta_n=\delta_0^{\smash{F_{n-1}}}\delta_1^{\smash{F_{n}}},\quad\text{for $n\ge 2$},$$
%
%where $F_n$ is the $n$-th Fibonacci number starting with $F_0=F_1=1$. 

%Let $T_n, n\in \NN_0$ be the trees constructed from this sequence as in \cref{constr:tree}.
%Since $\delta_{n+1} =\delta_n\delta_{n-1}\le \delta_n^2$ for $n\ge 2$, the sequence satisfies \cref{res:conditions_in_d} \itm1 and \cref{thm:main} yields uniform volume growth for the limit tree $T:=\bigcup_n T_n$.

%For $\bar g(2^n)=(\delta_0+1)\cdots(\delta_n+1)$, one can verify that 
%
%\msays{I don't remember how I came to these estimates. Should be checked.}
%
%\[b^{r^\alpha-\frac{\log r}{2}} \leq \bar g(r)\leq (\delta_0+1)rb^{(r^\alpha+\frac{1}{2})\log r}\!\!,\] \[\quad\text{with $b=(\delta_0^{1/\varphi}\delta_1)^{1/\sqrt{5}}\gtrsim 1.363$ and $\alpha=\log\varphi \approx 0.694$},\]
%
%where $\varphi\approx 1.618$ is the golden ratio. In particular, $T$ is of intermediate growth.

%It remains to verify that the Benjamini-Schramm limit of the sequence of $T_n$ is supported on a single tree.
%The key  observation is that the $T_n$ are very symmetric, in that they are transitive on their apocentric copies of $T_k$, for any $k\le n$. 
%More precisely, for any two apocentric copies $\tau_1,\tau_2\subset T_n$ of $T_k$, there is an automorphism $\phi\in\Aut(T_n)$ that fixes the root of $T_n$ and sends $\phi(\tau_1)=\tau_2$.
%This is clear for $T_0$ and $T_1$.
%Suppose that it is proven for $T_0,...,T_n$, then we can prove it for $T_{n+1}$:
%observe first that $\delta_{n+1}=\delta_n\delta_{n-1}$ is exactly the number of apocentric copies of $T_{n-2}$ in $T_n$.
%That is, by maximal uniform distribution of adjacencies, each apocentric copy of $T_{n-2}$ in the central $T_n\subset T_{n+1}$ is adjacent to \emph{exactly one} apocentric copy of $T_n$ in $T_{n+1}$. The unique vertex of each $T_{n-2}$ participating in this \enquote{outwards adjacency} will be called the \emph{outwards vertex}.
%Let now $\tau_1,\tau_2\subset T_{n+1}$ be two apocentric copies of $T_k,k\le n+1$ in $T_{n+1}$.
%The existence of an appropriate symmetry is clear when $k=n+1$, so let us assume $k<n+1$.
%Let $T_n(\tau_i)$ be the apocentric copy of $T_n$ that contains $\tau_i$, let $v_i$ be the outwards vertex in the central copy $T_n\subset T_{n+1}$ adjacent to $T_n(\tau_i)$, and let $T_{n-2}(v_i)$ be its containing copy of $T_{n-2}$, which is apocentric in the central $T_n\subset T_{n+1}$.
%By induction assumption there exists a symmetry $\phi_1\in\Aut(T_n)$ of the central $T_n\subset T_{n+1}$ that sends $T_{n-2}(v_1)$ onto $T_{n-2}(v_2)$. 
%Also by induction assumption, any apocentric copy of $T_{n-2}$ in $T_n$ is transitive on its apocentric vertices, and so we can modify $\phi_1$ into a symmetry $\phi_2\in\Aut(T_n)$ that sends outwards vertices to outwards vertices. 
%This then allows us to extend $\phi_2$ to a symmetry $\phi_3\in\Aut(T_{n+1})$.
%This symmetry necessarily sends $T_n(\tau_1)$ to $T_n(\tau_2)$. By induction assumption $T_n(\tau_2)$ is transitive on its apocentric copies of $T_k$, and so we can modify $\phi_3$ into a symmetry $\phi_4\in\Aut(T_{n+1})$ that sends $\tau_1$ onto $\tau_2$. All involved symmetries clearly fix the root of $T_{n+1}$.

%The upshot of this is: up to isomorphism of rooted graphs there exists a unique rooted tree $(T_n,r)$ with root $r$ at an apocentric vertex.

%If we identify $T_n$ with an apocentric copy of $T_n$ in $T_{n+1}$ we obtain an inclusion chain $T_0\subset T_1\subset T_2\subset \cdots$ whose limit tree $T:=\bigcup_n T_n$ is a generalized canopy tree. Note that because of symmetry, the identification of $T_n$ with a sub-tree of $T_{n+1}$ involved no choice, and so $T$ is the unique limit tree obtainable by this procedure.

\begin{comment}
From this construct trees $T_n$ according to \cref{constr:T_n}, but as before, identify $T_{n-1}$ with an \emph{apocentric copy} in $T_n$. The sequence $(T_n,x^*)$ is then completely apocentric and the limit tree $T:=\bigcup_n T_n$ is a generalized canopy tree.

To see this for $T_{n+1}$, note that $\delta_{n+1}=\delta_n\delta_{n-1}$ is exactly the number of apocentric copies of $T_{n-2}$ in $T_n$. By maximal uniform distribution of adjacencies, we find that each apocentric copy of $T_{n-2}$ in the central copy $T_n$ in $T_{n+1}$ is adjacent to exactly one apocentric copy of $T_n$ in $T_{n+1}$.
That is, up to isomorphism of rooted graphs, there is a unique rooted tree $(T_n,x^*)$, where $x^*$ is apocentric.

Note that the sequence $\delta_0,\delta_1,\delta_2,...$ satisfies \cref{res:conditions_in_d} \itm1 and $T$ is thus of uniform growth (by \cref{thm:main}).
According to \cref{res:types_of_limits} the Benjamini-Schramm limit of (some sub-sequence of) the sequence $(T_n,x^*)$ is a generalized canopy tree, and we claim that this is exactly $T$.

Let $(T_n,x^*)$ be the completely apocentric sequence, where the trees $T_n$ are constructed from the sequence $\delta_0,\delta_1,\delta_2,...$ according to \cref{constr:tree}.


Construct trees $T_n$ according to \cref{constr:tree}, but as before, consider $T_{n-1}$ as an apocentric copy in $T_n$. The limit $T:=\bigcup_n T_n$ is then a generalize canopy tree.
We show that also the Benjamini-Schramm limit of $(T_n,x^*)$ (where $x^*$ is 

By \cref{res:conditions_in_d} and \cref{thm:main}, the tree $T$ constructed according to the sequence $\delta_n$ has uniform growth. In particular, for the growth $g(r)$ of $T$ we have $g(r)\sim A^{r^\alpha}$ with~$A=(\delta_0^{1/\phi}\delta_1)^{1/\sqrt{5}}\ge 1.6513...$ and $\alpha=\log\phi = 0.6942...$\,, therefore the growth of $T$ is intermediate. 

In particular, $g(r)=\Omega(r^{a\log \log r})$, so that the Benjamini-Schramm limit of the sequence $T_i$ is a random rooted generalised canopy tree with an a.s. eventually apocentric root. Since \cref{constr:tree} dictates that at step $n$ we distribute the apocentric copies of $T_{n-1}$ over the apocentric vertices of the central copy as uniformly as possible, and the function $\delta_n$ has been chosen so that exactly one apocentric copy of $T_{n-1}$ can be glued to each apocentric copy of $T_{n-2}$ in the central copy of $T_{n-1}$, all of the apocentric vertices in each step have identical neighbourhoods of each order. Thus, the Benjamini-Schramm limit of the $T_i$ is indeed supported on a single tree.   
\end{comment}
%\end{example}

\begin{example}\label{ex:deterministic}
Define recursively $\delta_1:=1,\delta_2:=2$ and $\delta_{n+1}:=\delta_n\delta_{n-1}$.
In explicit form this reads
%
$$\delta_n=2^{F_n}, \quad\text{for all $n\ge 0$},$$
%
where $F_n$ denotes the $n$-th Fibonacci number starting with $F_1=0, F_2=1$. 

%Let $T=T(\delta_1,\delta_2,\delta_3,...)$ be the tree according to \cref{constr:T}.
Let $T_n$ for $n\ge 0$ be the trees according to \cref{constr:T_n}.
%The sequence~is~BS-convergent to a unimodular tree $\mathcal T$.
%Since $\delta_{n+1} =\delta_n\delta_{n-1}\le \delta_n^2$ for $n\ge 2$, the sequence satisfies \cref{res:conditions_in_d}~\itm1, and 
\Cref{converge} yields that $(T_n,o_n)$ converges in the Benjamini-Schramm sense to a random rooted tree $(\mathcal T,\mathcal{o})$ that is \as\ of uni\-form volume growth. 
%
%Since $\delta_n$ is unbounded, the volume of $T$ grows super-polynomially.
%One can~furthermore verify that $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ approximates $g(2^n)$ where
From $|T_n|=(\delta_1+1)\cdots(\delta_n+1)$ one can estimate
%
$$\tfrac12 D^{r^\alpha}\!\! \le |T_n|\le \tfrac 12r\cdot D^{r^\alpha}\!\!\!,\;\;\text{with $D:=2^{\varphi^2/\sqrt 5}\approx 2.251$ and $\alpha:=\log\varphi\approx 0.6942$}.$$
%
Here $\varphi\approx 1.618$ denotes the golden ratio.
The growth is therefore \emph{intermediate}.
\end{example}

We claim that $(\mathcal T, \mathcal{o})$ has a single underlying tree: by \cref{res:types_of_limits} $(\mathcal T,\mathcal{o})$ is a generalized canopy tree, \ie\ its underlying tree is \as\ an apocentric limit.
But as we show below (\cref{res:highly_symmetric}), the $T_n$ are highly symmetric in~that any two apocentric copies $\tau,\tau'\prec_{n-1} T_n$ are in fact indistinguishable by symmetry. 
In consequence, there exists (up to symmetry) only one apocentric inclusion chain, and $\mathcal T$ is the unique tree obtained as its limit.

In the following we establish the symmetry of $T_n$ in an even stronger form:

%As we shall see, this is because the $T_n$ are~highly symmetric, and the BS-limit therefore \enquote{has no choice} but to converge to one single tree.
%We characterize the symmetry of $T_n$:

\begin{lemma}\label{res:highly_symmetric}
%If $\delta_{n+1}=\delta_{n-1}\delta_n$ for $n\ge 1$, then 
With the sequence of \cref{ex:deterministic} the trees $T_n$ are transitive on~apocentric copies $\tau\prec_m T_n$ for each $m\le n$, \ie\ for any two apocentric copies $\tau_1,\tau_2\prec_m T_n$ there is a symmetry $\phi\in\Aut(T_n)$ sending $\phi(\tau_1)=\tau_2$.
\end{lemma}

\begin{proof}
The proof is by induction on $n$. The cases $n\in\{0,1\}$ are trivially verified~and form the induction basis. Suppose that the statement is proven up to some $n\ge 1$; we prove the statement for $T_{n+1}$.

Let $\tau_0\prec_n T_{n+1}$ denote the central copy, and let $\tau_1,...,\tau_{\delta_{n+1}} \prec_n T_{n+1}$ denote the apocentric copies.
%
From our specific choice of sequence follows that the apocentric copies $\prec_n T_{n+1}$ are in one-to-one relation with the apocentric copies $\prec_{n-2} \tau_0$: by the \enquote{maximally uniform distribution of adjacencies} (\cf\ \cref{rem:max_uniform}, especially~equation \eqref{eq:max_uniform}) the expected number of \enquote{outwards adjacencies} of an apocentric copy $\hat\tau\prec_{n-2}\tau_0$ is exactly
$$
\frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
= \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
$$
%
In other words, there are exactly $\delta_{n+1}$ apocentric copies $\hat\tau_1,...,\hat\tau_{\delta_{n+1}}\prec_{n-2} \tau_0$ and they are in one-to-one relation with the $\tau_i$.
We can assume an enumeration so that $\hat\tau_i$ and $\tau_i$ are connected by an edge, its end in $\hat\tau_i$ we call $x_i$. %and that $x_i\in\hat\tau_i$ is the \enquote{outwards vertex} adjacent to $\tau_i$.

Fix two apocentric copies $\rho_1,\rho_2\prec_m T_{n+1}$ for some $m\le n+1$.
The goal is to construct a symmetry of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$. 

Let $i_k\in\NN$ be indices so that $\rho_k\prec_m \tau_{i_k}$.
%
By induction hypothesis there is a symmetry $\phi_0\in\Aut(\tau_0)$ that maps $\hat\tau_{i_1}$ onto $\hat\tau_{i_2}$. More generally, $\phi_0$ permutes the trees $\hat\tau_1,...,\hat\tau_n$, that is, $\phi_0$ sends $\hat\tau_i$ onto $\hat\tau_{\sigma(i)}$ for some permutation $\sigma\in\Sym(n)$.
It holds $\sigma(i_1)=i_2$.
Note however that $\phi_0$~does not necessarily map $x_i$ onto $x_{\sigma(i)}$. %\enquote{outwards vertices} onto \enquote{outwards vertices}.
We can fix this: invoking the induction hypothesis again, for each $i\in\{1,...,n\}$ exists a symmetry $\phi_1^i\in\Aut(\hat\tau_i)$ that sends $\phi_0(x_i)$ onto $x_{\sigma(i)}$. The map
%
$$
\phi_2(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
is then a symmetry of $\tau_0$ that sends the pair $(\hat\tau_i,x_i)$ onto $(\hat\tau_{\sigma(i)},x_{\sigma(i)})$.
Having this, $\phi_2$ extends to a symmetry $\phi_3\in\Aut(T_{n+1})$ that necessarily sends $\tau_i$ onto $\tau_{\sigma(i)}$.
In particular, it sends $\tau_{i_1}$ (which contains $\rho_1$) onto $\tau_{i_2}$ (which contains $\rho_2$).
As before, $\phi_3$ does not necessarily send $\rho_1$ onto $\rho_2$ right away; but also as before, this can be fixed: by induction hypothesis there is a symmetry $\phi_4\in\Aut(\tau_{i_2})$ that sends $\phi_3(\rho_1)$ onto $\rho_2$. The map
%
$$
\phi_5(x):=\begin{cases}
(\phi_4\circ\phi_3)(x) & \text{if $x\in \tau_{i_1}$} \\
\phi_3(x) & \text{otherwise}
\end{cases}.
$$
is a symmetry of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$.
\end{proof}

% \begin{theorem}
%     $\mathcal T$ is deterministic.
% \end{theorem}

% \begin{proof}
%     Since $\delta_n=\Omega(n)$, $\mathcal T$ is a generalized canopy tree, \ie\ $\mathcal T$ is supported exactly on the limits of completely apocentric inclusion chains (\cf\ \cref{rem:general_limit_growth}).
%     Note however that up to symmetry there is only one such chain: since $T_{n+1}$ is transitive on its apocentric copies $\prec_{n} T_{n+1}$, there is (up to symmetry) no choice for the apocentric identification $T_n\subset T_{n+1}$. 
%     Since there is no choice involved, $\mathcal T$ is supported on a single tree.
% \end{proof}

Unimodular random rooted trees with a unique underlying tree of even smaller uniform growth can be construct\-ed by choosing $\delta_{n+1}:=\delta_n\delta_{n-1}$ only for some $n$, and $\delta_{n+1}:=\delta_n$ otherwise.
However, since Benjamini-Schramm limits of balanced sequences have probability zero for any particular underlying tree, this technique cannot yield unimodular random trees with a unique underlying tree for growth too slow.

% \begin{question}
%     Can a deterministic tree of uniform growth, say, $g\in O(r^{\log\log r})$ be unimodular?
% \end{question}

\begin{question}
Is there a random rooted tree $(\mathcal T,\mathcal o)$ that satisfies simultaneously~all of the following three properties?:
\begin{myenumerate}
    \item $(\mathcal T,\mathcal o)$ is unimodular.
    \item $(\mathcal T,\mathcal o)$ is supported on a unique deterministic tree.
    \item $(\mathcal T,\mathcal o)$ is of uniform volume growth, say, $g\in O(r^{\log\log r})$.
\end{myenumerate}
\end{question}

%A slight modification of the above example in which we define $\delta_{n+1}:=\delta_n\delta_{n-1}$ for some $n$, and $\delta_{n+1}:=\delta_n$ for others, yields deterministic unimodular random trees of a wide range of uniform volume growth above $r^{\log\log r}$.

\section{Conclusions and open questions}
\label{sec:last}

\subsection{Planar triangulations}

Planar triangulations of an unexpected uniform volume growth $\sim r^4$ have previously been observed in physical context \cite{angel2003growth,ambj1997quantum}.
This was generalized to $\sim r^\alpha$ for any $\alpha\ge 1$ in \cite{benjamini2011recurrence} by observing that any tree $T$ of maximum degree $\bar \Delta$ can be turned into a planar triangulation with the same grwoth behavior: fix a triangulated sphere with at least $\bar\Delta$ pairwise disjoint triangles. Take a copy of this sphere for each vertex of $T$ and glue two spheres along a triangle when the associated vertices are adjacent. 

Having established the existence of trees for a variety of growth rates, we can likewise conclude the existence of planar triangulations with the same wide range of growth behaviors.

But we can say even more: previously known triangulations of polynomial growth are planar, but not necessarily triangulations of the plane, \ie\ they are not necessarily homeomorphic to $\RR^2$. For this to be true, one needs the tree $T$ to be \emph{one-ended}.
Going back to \cref{constr:T} and instead associating $T_n$ with some \emph{apocentric copy} $\prec T_{n+1}$ instead of the central copy, we obtain a one-ended limit tree $T'$. 
From this we obtain triangulations of the plane for a wider range of growth behaviors.
%The same analysis \cref{thm:main} of the growth behavior applies to this tree and so we obtain triangulations of the plane with arbitrary uniform growth.

\subsection{Future research}

Having shown that trees of intermediate growth exist and that their growth can be determined at high granularity, the next natural step is to identify such trees in other objects. As discussed in Section 2, the trees of \cref{constr:T} occasionally span graphs which are ``typical'' for their growth. It would be interesting to determine whether this is by necessity:

\begin{question} \label{quest1}
Let $G$ be a graph of uniform growth $g(r)$. Is there a tree embedded in $G$ with the same uniform growth? In particular, is there a spanning tree of $G$ with the same uniform growth? 
\end{question}

This is more general than requesting a tree quasi-isometric to $G$. Indeed, although quasi-isometry implies agreement of growth (up to a multiplicative constant), one can construct a counterexample to the converse by taking a set of cycles of unbounded length and connecting them serially with edges. Then $G$ is a homeomorphic image of the double ray with fibers of size at most $2$ and therefore has linear growth, but $G$ has infinite perimeter, hence no quasi-isometric spanning trees. 

\begin{center}
    \includegraphics[width=0.65\textwidth]{img/chain_of_cycles}
\end{center}

%\msays{The subsequent paragraph is not true. An affirmative answer to Question 6.1 shows the existence of intermediate growth trees, but does not prove Theorem 3.4.}

Observe that \cref{quest1}, if proven true, would immediately imply the existence of trees of intermediate volume growth by considering, for instance, an appropriate spanning tree of the Grigorchuck Cayley graph.

Weaker versions of \cref{quest1} may also be interesting:

\begin{question}
Let $G$ be a graph of uniform growth $g(r)$. Does every graph $G$ have a planar subgraph with the same uniform growth? What about subgraphs from other minor-closed families?
\end{question}

Or even:

\begin{question}
Let $G$ be a graph with uniform growth $g(r)$. Is there some $k\in\mathbb{N}$, perhaps dependent on $g(r)$, such that $G$ has a subgraph which is not $k$-connected and has the same uniform growth?  
\end{question}

%\msays{Potential open question: is there a unimodular deterministic tree of intermediate volume growth below, say, $\exp(\sqrt n)$ or even $\exp(n^{o(1)})$?}

%\msays{We can probably find all kind of feasible growth behaviors: just define the sequence of $\delta_i$ to sometimes satisfy $\delta_{n+1}=\delta_n\delta_{n-1}$, and sometimes just $\delta_{n+1}=\delta_n$, see also \cref{res:symmetric_tree}.}





\begin{comment}
\msays{This section is just a bunch of experiments. Can be ignored}

%\section{Some interesting properties of $T(\delta_0,\delta_1,...)$}
\section{Some experiments}

The following function will play a central role in our investigation of $T$:

$$\Delta(n):=\frac{\delta_{n}}{\delta_0\cdots\delta_{n-1}}.$$

\begin{proposition}
Among the apocentric vertices of $T_n\subset T$, the average \resp\ maximum degree is $\Delta(n+1)+1$ \resp $\lceil\Delta(n+1)\rceil + 1$.

In particular, the maximum degree of $T$ is $\displaystyle\sup_n\lceil\Delta(n)\rceil + 1$.
\begin{proof}
\TODO
\end{proof}
\end{proposition}

\begin{proposition}
If $\delta_{n+1}\le \delta_0\cdots\delta_{n}$, then all vertices of $T$ have degree $1$, $2$, $\delta_0$ or $\delta_0+1$, where if $\delta_0\not=1$, then the only vertex with degree $\delta_0$ s the global root. %If we smooth vertices of degree $2$, then the resulting tree has only two possible vertex degrees, while the growth behavior changes at most by a factor of 2.
%
\begin{proof}
\TODO
\end{proof}
\end{proposition}

The next theorem shows that the rule of maximally uniform distribution~of~ad\-ja\-cen\-cies can lead to highly symmetric trees if the sequence of $\delta_i$ is chosen appropriately. 

% \begin{theorem}
% Fix $N\ge 0$. If $\delta_0\ge1$, $\delta_1 = \kappa\delta_0$ $($for some $\kappa\ge 1)$ and for all $n\in\{1,...,N\}$ holds either
% %
% $$\delta_{n+1}=\delta_n\delta_{n-1}\cdots\delta_{s(n)},$$
% %
% then $T_N$ is transitive on apocentric copies of $T_k$ for each $k\le N$. That means that for any two apocentric copies $\tau_1,\tau_2\subset T_N$ of $T_k$ exists a symmetry $\phi\in\Aut(T_N)$ that sends $\phi(\tau_1)=\tau_2$.
% \end{theorem}

\begin{theorem}\label{res:symmetric_tree}
Fix $N\ge 0$. If for each $n\in\{0,...,N-1\}$ holds either
\begin{myenumerate}
    \item $\delta_{n+1}=\delta_n\delta_{n-1}\cdots\delta_{s(n)}$ for some $s(n)\ge 0$, or
    %for some $K(n)\ge 1$ and $s(n)\le n$, or
    \item $\delta_{n+1}=K(n)\cdot \delta_n\delta_{n-1}\cdots\delta_0$ for some $K(n)\ge 1$,
    %
    %for some $K(n)\ge 1$, 
\end{myenumerate}
%
then $T_N$ is transitive on apocentric copies of $T_k\subset T_N$ for each $k\le N$.
That means that for any two apocentric copies $\tau_1,\tau_2\subset T_N$ of $T_k$ there is an automorphism~$\phi\in\Aut(T_N)$ that sends $\phi(\tau_1)=\tau_2$.
\end{theorem}

Some of the previously discussed examples are instances of \cref{res:symmetric_tree}. This includes constant sequences $\delta_n=c$, which lead to polynomial growth; and $\delta_0:=2$, $\delta_{n+1}:=\delta_0\cdots\delta_n=2^{2^n}$\!, which leads to exponential growth. 
The simplest instance resulting in intermediate growth is perhaps $\delta_0:=1, \delta_1:=2$, $\delta_{n+1}:=\delta_n\delta_{n-1}$, which expands to
%
$$\delta_n=2^{F_n},$$
%
where $F_n$ is the $n$-th Fibonacci number, starting with $F_0=0, F_1=1$.

\begin{proof}[Proof of \cref{res:symmetric_tree}]
We prove the statement by induction in $N$. The statement is clearly true for $N=0$.

Assume that the statement is proven up to some $N-1$ and that \itm1 \resp\ \itm2 holds for each $n\in\{1,...,N\}$.
Fix some $k\le N-1$ (the statement is trivial for $k=N$) and choose apocentric copies $\tau_1,\tau_2\subset T_N$ of $T_k$.
We construct the symmetry $\phi\in\Aut(T_N)$ that sends $\phi(\tau_1)=\tau_2$.
We consider two cases depending on whether $\delta_N$ falls in case \itm1 or \itm2.

\emph{Case \itm1}:
note that $\delta_n\cdots\delta_{s(n)}$ is exactly the number of apocentric copies of $T_{s(n)-1}$ in $T_N$. 
By the maximal uniform distribution of the adjacencies we find that in case \itm1 each of these copies of $T_{s(n)-1}$ in the central $T_N\subset T_{N+1}$ has therefore \emph{exactly one} \enquote{outwards adjacencies} to an apocentric $T_N\subset T_{N+1}$.

\TODO
\end{proof}


\newpage

Consider the recursively defined sequence of integers $\delta_0:=1$, $\delta_1:=2$ and~$\delta_{n+1}:=\delta_{n-1}\delta_n$.
Let $T_n,n\ge 0$ be the corresponding sequence of trees from \cref{constr:T_n}. 

\begin{lemma}
%If $\delta_{n+1}=\delta_{n-1}\delta_n$ for $n\ge 1$, then 
Each $T_n$ is transitive on apocentric copies $\tau\prec_m T_n$ for each $m\le n$, \ie\ for any two apocentric copies $\tau_1,\tau_2\prec_m T_n$ there is a symmetry $\phi\in\Aut(T_n)$ sending $\phi(\tau_1)=\tau_2$.
%
\begin{proof}
The proof is by induction on $n$. The cases $n\in\{0,1\}$ are trivially verified~and form the induction basis. Suppose that the statement is proven up to some $n\ge 1$; we prove the statement for $T_{n+1}$.

Let $\tau_0\prec_n T_{n+1}$ denote the central copy, and let $\tau_1,...,\tau_{\delta_{n+1}} \prec_n T_{n+1}$ denote the apocentric copies.
%
By our specific choice of sequence we find that the apocentric copies $\prec_n T_{n+1}$ are in one-to-one relation with the apocentric copies $\prec_{n-2} \tau_0$.\nlspace
In fact, by the \enquote{maximally uniform distribution of adjacencies} (see \cref{rem:max_uniform}, especially equation \eqref{eq:max_uniform}) we find that the expected number of \enquote{outwards adjacencies} of an apocentric copy $\hat\tau\prec_{n-2}\tau_0$ is exactly
$$
\frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
= \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
$$
%
Thus, there are exactly $\delta_{n+1}$ apocentric copies $\hat\tau_1,...,\hat\tau_{\delta_{n+1}}\prec_{n-2} \tau_0$ with $\hat\tau_i$ being adjacent to $\tau_i$. Let $x_i\in\hat\tau_i$ be the \enquote{outwards vertex} adjacent to $\tau_i$.

Fix two apocentric copies $\rho_1,\rho_2\prec_m T_{n+1}$ for some $m\le n+1$.
The goal is to find a sequence of symmetries of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$. Let $i_k\in\NN$ be so that $\tau_{i_k}$ contains $\rho_k$.

By induction hypothesis there is a symmetry $\phi_0\in\Aut(\tau_0)$ that maps $\hat\tau_{i_1}$ onto $\hat\tau_{i_2}$. More generally, $\phi_0$ permutes the trees $\hat\tau_1,...,\hat\tau_n$, that is, $\phi_0$ sends $\hat\tau_i$ onto $\hat\tau_{\sigma(i)}$ for some permutation $\sigma\in\Sym(n)$.
It holds $\sigma(i_1)=i_2$.
Note however that $\phi_0$~does not necessarily map \enquote{outwards vertices} onto \enquote{outwards vertices}.
We can fix this: invoking the induction hypothesis again, for each $i\in\{1,...,n\}$ exists a symmetry $\phi_1^i\in\Aut(\hat\tau_i)$ that sends $\phi_0(x_i)$ onto $x_{\sigma(i)}$. The map
%
$$
\phi_2(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
is then a symmetry of $\tau_0$ that sends the pair $(\hat\tau_i,x_i)$ onto $(\hat\tau_{\sigma(i)},x_{\sigma(i)})$.
Because of this, $\phi_2$ actually extends to a symmetry $\phi_3\in\Aut(T_{n+1})$ that necessarily sends $\tau_i$ onto $\tau_{\sigma(i)}$.
In particular, it sends $\tau_{i_1}$ (which contains $\rho_1$) onto $\tau_{i_2}$ (which contains $\rho_2$).
As before, $\phi_3$ does not necessarily send $\rho_1$ onto $\rho_2$ right away; but also as before, this can be fixed: by induction hypothesis there is a symmetry $\phi_4\in\Aut(\tau_{i_2})$ that sends $\phi_3(\rho_1)$ onto $\rho_2$. The map
%
$$
\phi_5(x):=\begin{cases}
(\phi_4\circ\phi_3)(x) & \text{if $x\in \tau_{i_1}$} \\
\phi_3(x) & \text{otherwise}
\end{cases}.
$$
is a symmetry of $T_{n+1}$ that sends $\rho_1$ onto $\rho_2$.
%
%
% Given an apocentric copy $\hat\tau\prec_{n-2}\tau_0$, how many edges emanate from $\hat \tau$ \enquote{outwards} to the apocentric copies $\tau_1,...,\tau_{\delta_{n+1}}$?
% %
% As it turns out, by our specific choice of sequence and by \enquote{maximally uniform distribution of adjacencies} there is always \emph{exactly one} such edge (\cf\ \cref{rem:max_uniform}, especially \eqref{eq:max_uniform}):
% %
% $$
% \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
% = \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
% $$
% %
% Each apocentric copy of $T_{n-1}$ in $\tau_0$ can therefore be denoted by $\hat\tau_i$, where the subscript 
%
% The apocentric copies $\hat\tau\prec_{n-2}\tau_0$ are therefore in one-to-one correspondence with the apocentric copies $\tau_i\prec_n T_{n+1}$.
% Let then $\hat\tau_i\prec_{n-2}\tau_0$ be the unique apocentric copy adjacent to $\tau_i$, and let $x_i\in\hat\tau_i$ be its \enquote{outwards vertex}.
%
%
% Let us fix an enumeration $\tau_1,...,\tau_{\delta_{n+1}}\prec_n T_{n+1}$ of the apocentric copies. We furthermore define
% %
% \begin{itemize}
%     \item $x_i\in\tau_0$, the \enquote{outwards vertex} adjacent to $\tau_i$, and
%     \item $\hat\tau_i\prec_{n-2} \tau_0$, the apocentric copy containing $x_i$.
% \end{itemize}
%
% For some $m \le n$ choose $\tau_i^m \prec_m \tau_i$.
% \Wlog\ the goal is to find a symmetry $\phi\in\Aut(T_{n+1})$ mapping $\phi(\tau_1^m)=\tau_2^m$.
%
%
%
%
% Note that $\delta_{n-1}\delta_n$ is exactly the number of apocentric copies of $T_{n-2}$ in $\tau_0$. By $\delta_{n+1}=\delta_{n-1}\delta_n$, this matches the number of apocentric copies of $T_n$ in $T_{n+1}$, and by maximally uniform distribution of adjacencies (\cf\ \cref{rem:max_uniform}) every apocentric copy $\tau\prec_{n-2}\tau_0$ contains a unique \enquote{outwards vertex}, that is, a vertex adjacent to an apocentric copy $\tau'\prec_n T_{n+1}$.
%
\iffalse

Fix two apocentric copies $\tau_1,\tau_2\prec_m T_{n+1}$ for some $m\le n+1$.
The goal is to find a sequence of symmetries of $T_{n+1}$ that send $\tau_1$ onto $\tau_2$.
%
We need to give names to some sub-structures of $T_{n+1}$:
%
\begin{itemize}
    \item let $\tau_0\prec_n T_{n+1}$ be the central copy of $T_n$
    in $T_{n+1}$.
    \item let $\tau_i^n \prec_n T_{n+1}$ be the unique apocentric copy of $T_n$ that contains $\tau_i$.
    \item let $x_i\in\tau_0$ be the apocentric vertex of $\tau_0$ that is adjacent to $\tau_i^n$.
    \item let $\hat \tau_i \!\prec_{n-2} \tau_0$ be the unique apocentric copy of $T_{n-2}$ in $\tau_0$ that contains $x_i$.
\end{itemize}

By induction hypothesis there is a symmetry $\phi_0\in\Aut(\tau_0)$ that maps $\hat\tau_1$ onto $\hat\tau_2$.
Note that $\phi_0$ not necessarily sends $x_1$ onto $x_2$.
We can fix this: by induction hypothesis there is also a symmetry $\phi_1\in\Aut(\hat\tau_2)$ that maps $\phi_0(x_1)$ onto $x_2$.
Then
%
$$
\phi_2(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
is a symmetry of $\tau_0$ and sends the pair $(\hat\tau_1,x_1)$ onto $(\hat\tau_2,x_2)$.


\par\medskip
Let $\tau_0\prec_n T_{n+1}$ denote the central copy.
We first note that each apocentric copy $\prec_{n-2}\tau_0$ has \emph{exactly one} \enquote{outwards adjacency} to an apocentric copy $\prec_n T_{n+1}$.
This follows from our special choice of sequence $\delta_{n+1}=\delta_{n-1}\delta_n$ and \enquote{maximally uniform distribution of adjacencies} (\cf\ \cref{rem:max_uniform} \eqref{eq:max_uniform}):
$$
\frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n+1} 
= \frac{\delta_1\cdots\delta_{n-2}}{\delta_1\cdots\delta_n} \cdot \delta_{n-1}\delta_n = 1.
$$

\sepline

Fix two apocentric copies $\tau_1,\tau_2\prec_m T_{n+1}$ for some $m\le n+1$, the goal is to find a symmetry $\phi\in\Aut(T_{n+1})$ sending $\phi(\tau_1)=\tau_2$. The statement is clear for $m=n+1$; so we assume $m\le n$. 
We give names to the following substructures:
%
\begin{itemize}
    %\item let $\tau_0\prec_n T_{n+1}$ be the central copy of $T_n$.
    \item let $\tau_i^n \prec_n T_{n+1}$ be the unique apocentric copy of $T_n$ that contains $\tau_i$.
    \item let $\hat x_i\in\tau_0$ be the apocentric vertex of $\tau_0$ that is adjacent to $\tau_i^n$.
    \item let $\hat \tau_i \!\prec_{n-2} \tau_0$ the unique apocentric copy of $T_{n-2}$ in $\tau_0$ that contains $\hat x_i$.
\end{itemize}

W.l.o.g.\ fix apocentric copies $\tau_1^m,\tau_2^m\prec_m T_{n+1}$, where 

The symmetry $\phi$ is build in multiple steps.
%
\begin{enumerate}
    \item 
By induction hypothesis there exists a symmetry $\phi_0\in\Aut(\tau_0)$ sending $\phi_0(\hat\tau_1)=\hat\tau_2$.
More generally, there is a permutation $\sigma\in\Sym(n)$ with $\phi_0(\hat \tau_i)=\hat \tau_{\sigma(i)}$. Note that $\phi_0$ not necessarily sends $x_i$ onto $x_{\sigma(i)}$, but onto $y_i:=\phi_0(x_i)\in\hat \tau_{\sigma(i)}$. 

    \item 
Invoking the induction hypothesis again, for each $i\in\{1,...,\delta_n\}$ there is a symmetry $\phi_1^i\in\Aut(\hat\tau_{\sigma(i)})$ sending $y_i$ onto $x_{\sigma(i)}$. From this we can build a symmetry $\phi_1\in\Aut(\tau_0)$:
%
$$
\phi_1(x):=\begin{cases}
(\phi_1^i\circ\phi_0)(x) & \text{if $x\in \hat\tau_i$} \\
\phi_0(x) & \text{otherwise}
\end{cases}.
$$
%
This symmetry now maps $\phi_1(x_i)=x_{\sigma(i)}$.
In particular, this symmetry now extends to a symmetry $\phi_2\in\Aut(T_{n+1})$ that maps $\phi_2(\tau_1)=\tau_2$.
However, it not necessarily sends $\tau_1^m$ to $\tau_2^m$, but only to $\tau_2^m':=\phi_2(\tau_2^m)$. Again, this can be fixed.

    \item
As before, we invoke the induction hypothesis to obtain a symmetry $\phi_3\in\Aut(\tau_2)$ that maps $\phi_3(\tau_2^m')=\tau_2^m$. 
This can be combined in the final symmetry $\phi\in\Aut(T_{n+1})$:
%
$$\phi(x):=\begin{cases}
(\phi_3\circ\phi_2)(x) & \text{if $x\in\tau_1$} \\
\phi_2(x) & \text{otherwise}
\end{cases}.$$
%
This symmetry maps $\phi(\tau_1^m)=\tau_2^m$.   

\end{enumerate}
%
This concludes the proof.
%
\fi
\iffalse
\sepline

% Let furthermore $\tau_0\prec_n T_{n+1}$ be the central copy.
% Let now $\tau_i^n \prec_n T_{n+1}$ be the unique apocentric copy that contains $\tau_i$, $x_i\in\tau_0$ the apocentric vertex of $\tau_0$ adjacent to $\tau_i^n$, and $\tau_i^m \prec_m \tau_0$ the unique apocentric copy that contains $x_i$.

By induction hypothesis we know that the following symmetries exist:
%
\begin{itemize}
    \item a symmetry $\phi_0\in\Aut(\tau_0)$ sending $\phi_0(\tau_1^{n-2}) = \tau_2^{n-2}$. Then $x_1':=\phi_0(x_1)$ is an apocentric vertex of $\tau_2^{n-2}$.
    \item a symmetry $\phi_1\in\Aut(\tau_2^{n-2})$ sending $\phi_1(x_1')=x_2$.
\end{itemize}
%
The following is then also a symmetry of $\tau_0$:
%
$$\phi_2(x):=\begin{cases}
\phi_0(x) & \text{if $x\not\in\tau_1^{n-2}$} \\
\phi_1\circ \phi_0(x) & \text{if $x\in\tau_1^{n-2}$}
\end{cases}.
$$
%
This symmetry sends the pair $(\tau_1^{n-2}\!,x_1)$ onto $(\tau_2^{n-2}\!, x_2)$.
%$\phi_2(\tau_1^m)=\tau_2^m$ and $\phi_2(x_1)=x_2$.

We now use that $\delta_{n+1}=\delta_{n-1}\delta_n$ is exactly the number of apocentric copies of $T_{n-2}$ in $\tau_0$. By the maximally uniform distribution of adjacencies, every apocentric copy $\tau\prec_{n-2} \tau_0$ therefore contains a unique \enquote{outwards vertex}, that is, a vertex adjacent to an apocentric copy of $T_n$ in $T_{n+1}$. Since $\phi_2$ sends an outwards


This now guarantees that $\phi_2$ extends to a symmetry $\phi_3\in\Aut(T_{n+1})$ sending $\phi_3(\tau_1^n)=\tau_2^n$. Then $\tau_1':=\phi_3(\tau_1)\prec_m \tau_2^n$ is an apocentric copy of $T_m$. Again, by induction hypothesis there exists 
%
\begin{itemize}
    \item a symmetry $\phi_4\in\Aut(\tau_2^n)$ sending $\phi_4(\tau_1')=\tau_2$.
\end{itemize}
%
As before, the following is then also a symmetry of $T_{n+1}$:
%
$$\phi(x):=\begin{cases}
\phi_3(x) & \text{if $x\not\in\tau_1$} \\
\phi_4\circ \phi_3(x) & \text{if $x\in\tau_1$}
\end{cases}.
$$
%
The symmetry $\phi\in\Aut(T_{n+1})$ sends $\tau_1$ onto $\tau_2$, which concludes the proof.
\fi
\end{proof}
\end{lemma}

\begin{theorem}
The distributional limit of the sequence $T_n$ is supported on a single tree.
%
\begin{proof}
\TODO
\end{proof}
\end{theorem}



\newpage







\newpage

\subsection{Unimodular trees supported on a single tree}

%A random rooted graph $\mathcal G$ is \emph{deterministic} if it is supported on a single tree.
%In other words, it is a usual (non-random) graph with merely a random choice of root.
%One might wonder whether a determi\-nistic tree of intermediate growth can be unimodular.
%The answer is affirmative as we demonstrated below.








\newpage

We say that a sequence $\delta_n$ is \emph{growing fast} if
%
$$\sum_{n=0}^\infty \frac1{\delta_n}<\infty,$$
%$$\prod_{n=0}^\infty \frac{\delta_n}{\delta_n+1}>0,$$
%$$\prod_{n=0}^\infty \frac{1}{1+1/\delta_n}>0,$$
%
otherwise we say it is \emph{growing slow}.
It turns out that this distinction is a crucial~deciding factor for the structure of the limit $$T_n\xrightarrow{\mathrm{BS}} \mathcal T.$$

\begin{remark}
    \msays{$\delta_n>n^\alpha$ with $\alpha>1$ grows fast, $\delta_n\in O(n)$ grows slow}
\end{remark}

\begin{remark}
    \msays{What does this mean in terms of $g$?}
\end{remark}

\newpage 
\end{comment}
